A New Framework for Quantum Oblivious Transfer

We present a new template for building oblivious transfer from quantum information that we call the "fixed basis" framework. Our framework departs from prior work (eg., Crepeau and Kilian, FOCS '88) by fixing the correct choice of measurement basis used by each player, except for some hidden trap qubits that are intentionally measured in a conjugate basis. We instantiate this template in the quantum random oracle model (QROM) to obtain simple protocols that implement, with security against malicious adversaries: 1. Non-interactive random-input bit OT in a model where parties share EPR pairs a priori. 2. Two-round random-input bit OT without setup, obtained by showing that the protocol above remains secure even if the (potentially malicious) OT receiver sets up the EPR pairs. 3. Three-round chosen-input string OT from BB84 states without entanglement or setup. This improves upon natural variations of the CK88 template that require at least five rounds. Along the way, we develop technical tools that may be of independent interest. We prove that natural functions like XOR enable seedless randomness extraction from certain quantum sources of entropy. We also use idealized (i.e. extractable and equivocal) bit commitments, which we obtain by proving security of simple and efficient constructions in the QROM.

==> BCKM21-BF10-quantum-sampling.tex <==
\subsection{Statistical Hiding}
\label{subsec:stat-hiding}

In this subsection, we prove that our extractable commitment scheme described in~\cref{fig:ext-com} is statistically hiding, assuming that $\eqcommit$ is a statistically binding (equivocal) commitment scheme.

Our proof closely follows techniques of~\cite{C:BouFeh10}, who developed techniques for analyzing~\cite{FOCS:CreKil88}-style oblivious transfer protocols based on quantum sampling techniques. We import a lemma from~\cite{C:BouFeh10}.

\paragraph{\cite{C:BouFeh10} Quantum Sampling.} 

Consider the following interaction between a player $P$ and a challenger $C$.
\begin{enumerate}
    \item $P$ prepares an arbitrary quantum state $\ket{\psi}_{\gray{X}\gray{Y}}$ where $\gray{X}$ is a $2n$-qubit register and $\gray{Y}$ is an arbitrary-size register of $P$'s choice. 
    
    $P$ sends the contents of $\gray{X}$ to $C$ along with two length-$2n$ classical strings $\hat{x} \in \{0,1\}^{2n}$ and $\hat{\theta} \in \{+,\times\}^{2n}$.
    
    \item\label[step]{step:check-T} $C$ samples a uniformly random set of $n$ indices $T \subset [2n]$ as well as a uniformly random $\theta \in \{+,\times\}^{2n}$.
    
    For each $i \in T$ it measures the $i$th qubit of $\gray{X}$ in basis $\hat{\theta}_i$. If there exists $i \in T$ where $\theta_i = \hat{\theta}_i$ and the measurement outcome does not match $\hat{x}_i$, then $C$ aborts the experiment and outputs $\bot$. Otherwise, $C$ sends $\overline{T} \coloneqq [2n] \setminus T$ to $P$.
    
    \item $P$ responds with a subset $S \subseteq \overline{T}$. 
    
    \item\label[step]{step:measure} $C$ measures the indices of $\gray{X}$ specified by $S$, obtaining a length-$|S|$ bitstring $X_S$ of measurement outcomes; let $s$ denote the number of indices $i \in S$ where $\theta_i \neq \hat{\theta}_i$. 
\end{enumerate}

\begin{lemma}[\cite{C:BouFeh10} Quantum Sampling Lemma]
\label{lemma:sampling}
For any computationally unbounded player $P$ and $0 < \varepsilon < 1$, the probability the sampling experiment does not abort and
\[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\bar{S}}, \gray{Y}) > s- \varepsilon \cdot |S|. \]
is at most $\negl(|S|^2/n)$.
\end{lemma}


\begin{proof}(Sketch.)
This lemma follows readily from techniques developed in~\cite{C:BouFeh10} to relate quantum sampling to classical sampling. Following~\cite{C:BouFeh10}, it suffices to analyze the case where $\hat{x} = 0^{2n}$ and $\hat{\theta} = +^{2n}$, since all other settings of $\hat{x}$ and $\hat{\theta}$ follow from an identical argument under a change of basis. 

In \cref{step:check-T} of the quantum sampling experiment, $C$ verifies that for every index in a random choice of $n$ indices $T \subset [2n]$, measuring the corresponding qubit in the computational basis yields $0$. As observed in~\cite{C:BouFeh10}, this is a natural quantum analogue of the following classical sampling experiment (\cite[Example 4]{C:BouFeh10}) on a length-$2n$ bitstring $X$:
\begin{enumerate}
    \item randomly select a size-$n$ subset $T \subset [2n]$,
    \item randomly select a string $\theta \in \{0,1\}^{2n}$,
    \item verify that $X_i = 0$ on each index $i \in T$ where $\theta_i = 1$, and abort otherwise.
\end{enumerate}
Let $X_{\overline{T}}$ denote the string $X$ restricted to the $n$ indices $\overline{T} = [2n] \setminus T$. For any initial bitstring $X$, the ``classical error probability'' is the probability that the sampling experiment succeeds and $X_{\overline{T}}$ has relative Hamming weight $\geq \delta$ is at most $6e^{-n \delta^2/50}$ (bound derived in \cite[Appendix B.4]{C:BouFeh10}).

\cite[Theorem 3]{C:BouFeh10} demonstrates that the ``quantum error probability'' is at most the square root of the classical error probability. That is, if the verification in \cref{step:check-T} passes, then the residual state on $\gray{X}$ restricted to $\overline{T}$ is within trace distance $\sqrt{6e^{-n \delta^2/50}}$ of a superposition of states with relative Hamming weight at most $\delta$.

Suppose for a moment that the state were \emph{exactly} a superposition of states with relative Hamming weight at most $\delta$. Now consider the restriction of $\gray{X}$ to a subset of indices $S \subset \overline{T}$ where exactly $s$ positions have $\hat{\theta}_i \neq \theta_i$. The relative Hamming weight of the state when restricted to $S$ is at most $\delta n/ |S|$. As long as $\delta n/ |S| < 1/2$, by~\cite[Corollary 1]{C:BouFeh10}, we have
\[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\overline{S}}, \gray{Y}) > s - h(\delta n/|S|)\cdot |S|\]
where $h: [0,1] \rightarrow [0,1]$ is the binary entropy function defined as $h(p) = p \log (p) + (1-p) \log (1-p)$ for $0 < p < 1$ and as $0$ for $p = 0$ or $1$. For any desired $\varepsilon \in (0,1)$, there exists an $\epsilon' \in (0,1/2)$ such that $h(\varepsilon') = \varepsilon$, so we can plug in $\delta = \varepsilon' |S|/n$ to achieve the stated min-entropy lower bound of $s - \varepsilon \cdot |S|$.
\end{proof}

% Before we apply this lemma to prove statistical hiding of our extractable commitments, we provide some brief intuition behind the~\cite{C:BouFeh10} techniques used to prove this lemma. At a very high level, the main result of~\cite{C:BouFeh10} is that up to polynomial factors, ``quantum sampling'' behaves like classical sampling.

\paragraph{Proof of Statistical Hiding.} We now prove statistical hiding of our extractable commitment scheme in~\cref{fig:ext-com}. The core proof idea is due to~\cite{C:BouFeh10}.

Consider a \emph{purification} of the committer's strategy from~\cref{fig:ext-com}, where instead of sampling random $x \gets \{0,1\}^{2\secp^3}, \theta \gets \{+,\times\}^{2\secp^3}$ and sending $\ket{x}_\theta$ to $\mathcal{R}$ in~\cref{step:sample}, the committer $\mathcal{C}$ generates $2\secp^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$, and sends $\mathcal{R}$ one half of each pair. This change has no effect on the receiver's view. In this modification of~\cref{step:sample}, the committer will still sample random $\theta \gets \{+,\times\}^{2\secp^3}$ but does not use it to perform any measurements (and hence $x$ is not yet determined). We now recast~\cref{step:sample,step:open,step:commit,step:challenge,step:verify} of~\cref{fig:ext-com}, i.e., the ``measurement-check subprotocol'' to correspond with this undetectable modification of the committer's behavior:

% \begin{enumerate}
% \item The committer (inefficiently) opens the commitments to recover the receiver's choice of $(\hat{\theta},\hat{x})$.
% \item Rather than checking that 
% \end{enumerate}

\begin{enumerate}
\item $\cC$ chooses $2\lambda^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$ and sends $\mathcal{R}$ one half of each pair. The committer samples random $\theta \gets \{+,\times\}^{2\lambda^3}$ but does not perform any measurements (and hence $x$ is not yet determined).
\item $\cR$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{2\lambda^3}$
and obtains $\widehat{x} \in \{0, 1\}^{2\lambda^3}$ by measuring its $2\lambda^3$ EPR pair halves in bases specified by $\widehat{\theta}$.

$\cR$ commits to $\widehat{\theta}$ and $\widehat{x}$ using \emph{statistically binding commitments}.

\item $\cC$ sends a random test subset $T \subset [{2\lambda^3}]$ of size ${\lambda^3}$ to $\cR$. 

\item For every $i \in T$, $\cR$ decommits to $(\widehat{\theta}_i,\widehat{x}_i)$, and $\cC$ aborts if any decommitment is invalid.

\item $\cC$ checks that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $\cC$ proceeds with the protocol,
otherwise, $\cC$ aborts. 
\end{enumerate}

Notice that $\cC$'s messages are completely independent of its bit $b$ up to this point. If $\cR$ passes the check above, then $\cC$ will obtain a $\secp^3$-bit string $x$ by measuring its qubits (i.e., EPR pair halves) in positions $\overline{T} \coloneqq [2\secp] \setminus T$ in the bases specified in $\theta$. $\cC$ then partitions $x$ into $\secp$ different $\secp^2$-bit strings strings $x^{(1)},\dots,x^{(\secp)}$ and sends the receiver
\[ (s_1,b \oplus h(s_1,x^{(1)})),\dots,(s_\secp,b \oplus h(s_\secp,x^{(\secp)})), \]
where each $s_1,\dots,s_\secp$ is a random seed for the universal hash function $h$. By the leftover hash lemma (\cref{thm:privacy-amplification}), $b$ will be statistically hidden if each $x^{(\ell)}$ has sufficient independent min-entropy.

To that end, observe (following~\cite[Section 5]{C:BouFeh10}) that the committer decides to accept the receiver's commitment openings $(\hat{\theta}_i,\hat{x}_i)_{i \in [T]}$ \emph{only if} a certain ``quantum sampling experiment'' succeeds. Since the commitments are statistically binding, the values of $\hat{x},\hat{\theta}$ that $\mathcal{C}$ would accept are statistically determined after $\mathcal{R}$ commits. Let $\ket{\psi}_{\gray{X}\gray{Y}}$ be the joint state of the committer and receiver where $\gray{X}$ corresponds to the committer's $2\secp^3$ registers, and $\gray{Y}$ corresponds to the receiver's state. Then the committer's check can only pass if the sampling strategy of~\cref{lemma:sampling} succeeds for the committed values of $\hat{x},\hat{\theta}$. We remark that while no efficient $\mathcal{C}$ can actually \emph{perform} this sampling strategy (as it involves breaking the computational hiding of the underlying equivocal commitments), its behavior is statistically indistinguishable from $\mathcal{C}$ that does perform this sampling. 

By applying~\cref{lemma:sampling}, we conclude that each $x^{(\ell)}$ must therefore have min-entropy $\Omega(\lambda^2)$ conditioned on $\mathcal{R}$'s view and on all $x^{(j)}$ for $j \neq \ell$, since by Hoeffding's inequality, $\theta$ and $\hat{\theta}$ differ in at least $\Omega(\lambda^2)$ places within the $\lambda^2$ indices corresponding to $x^{(\ell)}$ with $1-\negl(\lambda)$ probability. Applying~\cref{thm:privacy-amplification} (leftover hash lemma) one by one to each $x^{(\ell)}$, this implies that each $(s_\ell,h(s_\ell,x^{(\ell)}))$ is statistically indistinguishable from uniform even given the receiver's view, and thus $b$ is statistically hidden.

==> abstract-old.tex <==
% \begin{abstract}
% We prove that quantum-hard one-way functions imply \emph{simulation-secure} oblivious transfer in a quantum world, and therefore suffice for secure computation of arbitrary quantum (or classical) functionalities.
% \end{abstract}

\begin{abstract}
We initiate the explicit study of quantum oblivious transfer (OT) in the quantum random oracle model (QROM). As the feasibility of unconditionally-secure quantum OT in the QROM has been implicitly established in prior work, we focus on the following questions: how many rounds of interaction and how many (quantum) resources are required for quantum OT?
%e propose new general frameworks for constructing round-efficient and concretely-efficient quantum OT in the QROM. 

We obtain the following unconditionally-secure protocols in the QROM, satisfying simulation-based security against malicious adversaries.

\begin{itemize}

    
    \item One-message bit OT between two parties that initially share a set of EPR pairs, realizing an ideal functionality that obtains two chosen bits $(m_0, m_1)$ from the sender and outputs $(b, m_b)$ to the receiver for uniformly random $b$. Such a \emph{non-interactive} protocol is impossible with a classical common reference string setup, and thus our protocol crucially relies on the unique properties of entanglement.

    \item Two-message bit OT without pre-shared entanglement, realizing the same functionality as above. This is obtained by showing that the above protocol remains secure even if the (potentially malicious) receiver sets up the entanglement, and constitutes the first two-message solution for (some flavor of) OT that does not rely on public-key encryption.

    \item Three-message chosen-input string OT. Natural QROM implementations of prior templates for quantum OT require at least five messages.

    
\end{itemize}
Our conceptual contribution is a new template for quantum OT that we call the ``fixed basis framework''. In this framework, which departs from previous ``random basis frameworks'' initiated by Crepeau and Kilian (FOCS '88), the {\em correct} choice of basis used by one player to polarize qubits is largely fixed and public at the time of measurement, except for some hidden {\em trap} qubits that are intentionally polarized in a conjugate basis. To analyze some of our protocols, we develop techniques of independent interest that enable \emph{seedless} extraction from quantum sources of entropy. 

%We also construct three-message random-input and four-message chosen-input OT assuming non-interactive idealized (i.e. extractable and equivocal) bit commitments. In fact, all our protocols use such commitments, for which we provide simple and efficient constructions in the QROM. These may be of independent interest.

Finally, we optimize for and estimate the number of BB84 states or EPR pairs required by each of our protocols, and by natural QROM implementations of prior protocols. Our work positions the QROM as both a practically and theoretically interesting model in which to study unconditionally-secure quantum oblivious transfer.
\end{abstract}

\iffalse{
    Oblivious transfer is a fundamental cryptographic primitive, known to suffice for the secure computation of arbitrary classical and quantum functionalities. 
    %All known constructions of oblivious transfer with classical communication crucially rely on the use of public-key style assumptions. In 1988, 
    Crepeau and Kilian (FOCS, 1988) first presented a template for achieving oblivious transfer using photons polarized in conjugate bases and bit commitments. The provable security of this template has been studied for decades and recently culminated in a line of work proving the feasibility of basing oblivious transfer entirely on symmetric-key cryptography.
    
    
    In this work, we present new templates for {\em round efficient} and {\em concretely efficient} oblivious transfer based on symmetric cryptography and quantum communication. We present our results in the idealized (quantum) random oracle model (QROM), which is 
    %an idealization of symmetric-key cryptography, and is 
    often leveraged to argue the security of concretely efficient protocols.
    Like prior work, our protocols build on Wiesner's observation that a photon polarized with respect to one basis but measured in another ends up deleting information. 
    Unlike all prior work, the exact choice of basis in used to polarize photons in our protocols is largely fixed and public at the time of measurement, except for a few hidden ``trap'' photons that are intentionally polarized in a different basis.
    
    This new perspective allows us to obtain simple protocols for two-round random input bit OT and three-round chosen input string OT in the QROM.
    This also implies {\em non-interactive random OT} in a model where parties share EPR pairs {\em a priori}.
    All our protocols use idealized (i.e. extractable and equivocal) bit commitments, for which we provide simple and efficient constructions in the QROM. These may be of independent interest.
}\fi
%Finally, we also optimize round complexity in the 
%We use different methods to enforce measurement, resulting in protocols that fall under two broad frameworks.
%The random oracle model has historically been used to model an “ideal” symmetric-key primitive, and has been leveraged throughout cryptography to argue the security of highly efficient protocols. 
\iffalse{
    Our protocols build on Wiesner's observation that a photon polarized with respect to one basis but measured in another ends up deleting information. We split our protocols into two categories depending on how deletion is enforced.
}\fi
%We observe that prior work 
%can be broadly classified into the following frameworks.
%by {\em departing} from the Crepeau-Kilian template.
%depart from the Creaeau
%In this work, we propose {\em new protocol templates} that use quantum communication to obtain {\em round efficient} and {\em concretely efficient} bit oblivious transfer in the quantum random oracle model (QROM). 
\iffalse{
    \begin{itemize}
        \item {\bf Hidden Basis Framework.} 
        In this framework, the choice of bases used to polarize photons remains hidden until after photons have been measured.
        %Given two conjugate bases $\{\mathsf{B}_0, \mathsf{B}_1\}$, one player samples $\theta = \theta_1 \theta_2 \ldots \theta_n \leftarrow \{\mathsf{B}_0, \mathsf{B}_1\}^n$, encodes a classical string $x = x_1 x_2 \ldots x_n$ into a quantum state $\psi = \{\ket{x_i}_{\theta_i}\}_{i \in [n]}$ that they send to the other player. 
        %Crucially, the choice of basis $\theta$ is revealed {\em only after} the other player has been forced to perform measurements.
        The Crepeau-Kilian template falls into this framework, and we observe that a modification of their template yields three round random input string OT in the QROM.
        
        %One player samples a string 
        
        \item {\bf Public Basis Framework.}
        In this framework, the choice of bases used to polarize photons is largely public at the time of measurement, except for a few hidden ``trap'' photons that are intentionally polarized in a different basis.
        %one player encodes their classical string $x = x_1 x_2 \ldots x_n$ into a {\em fixed public basis} $\mathsf{B}_0$ but embeds a few {\em trap} qubits polarized in basis $\mathsf{B}_1$ at hidden positions. The trap qubits serve to ensure that the other player deletes information by performing measurements in basis $\mathsf{B}_1$.
        %The other player is forced to perform measurements to delete information 
        This framework allows us to obtain two-round random input bit OT and three-round chosen input string OT in the QROM.
        In particular, this implies {\em non-interactive random OT} in a model where parties share EPR pairs {\em a priori}.
    \end{itemize}
}\fi
\iffalse{
    %This allowed 
    %In particular, 
    This opened up the possibility that the use of quantum communication may allow oblivious transfer to be based solely on symmetric-key style assumptions. Indeed, it was recently shown that quantum oblivious transfer (QOT) can be based on the (black-box use of) one-way functions (Grilo et al., EUROCRYPT 2021, Bartusek et al., CRYPTO 2021).
    
    The random oracle model has historically been used to model an “ideal” symmetric-key primitive, and has been leveraged throughout cryptography to argue the security of highly efficient protocols. In this work, we initiate the formal study of unconditionally secure quantum oblivious transfer protocols in the (quantum) random oracle model (QROM).
    
    In particular, we make use of the QROM in order to obtain \emph{concretely efficient} and \emph{round efficient} protocols. We first observe that 
    %the well-known Crepeau-Kilian template can be instantiated to give a five-round protocol in QROM. Next, we somewhat 
    a departure from the standard Crepeau-Kilian template yields a (maliciously-secure) four-round protocol in the QROM, where the quantum communication still only consists of BB84 states, and no quantum memory is required by either party. Finally, we present a qualitatively different template for quantum oblivious transfer that makes use of \emph{entangled} two-qubit states. We instantiate this template to give a two-round protocol for random bit OT in the QROM.
    %(with security aginst malicious receivers and \emph{specious} senders). 
}\fi

==> abstract-sub.tex <==
We propose new general frameworks for constructing round efficient and concretely efficient quantum oblivious transfer (OT) in the quantum random oracle model (QROM). We obtain the following unconditionally secure protocols in the QROM, satisfying simulation-based security against malicious adversaries.
\begin{itemize}
    \item \emph{Non-interactive} (i.e., one-message) bit OT between two parties that initially share a set of EPR pairs. This realizes an ideal functionality that obtains two chosen bits $(m_0, m_1)$ from a sender and outputs $(b, m_b)$ to a receiver, for uniformly random $b$.
    
    \item Two-message bit OT without setup, realizing the same functionality as above. 
    This is obtained by showing that the EPR pair based protocol above remains secure even if the receiver is the one that sets up the entanglement.

    \item Three-message chosen-input string OT without entanglement or setup.
\end{itemize}

Our conceptual contribution is a new template for quantum OT, that we call the ``fixed basis framework''. In this framework, the {\em correct} choice of basis used by one player to polarize qubits is largely fixed and public at the time of measurement, except for some hidden {\em trap} qubits that are intentionally polarized in a conjugate basis. To analyze some of our protocols, we develop new techniques that enable seedless extraction from quantum sources of entropy. Finally, we also construct three-message random-input and four-message chosen-input OT assuming non-interactive idealized (i.e. extractable and equivocal) bit commitments.
In fact, all our protocols use such commitments, for which we provide simple and efficient constructions in the QROM. These may be of independent interest.

==> app-sampling-lemma.tex <==
% \paragraph{\cite{C:BouFeh10} Quantum Sampling~\cite{BCKM2021}} 

% Consider the following interaction between a player $P$ and a challenger $C$.
% \begin{enumerate}
%     \item $P$ prepares an arbitrary quantum state $\ket{\psi}_{\gray{X}\gray{Y}}$ where $\gray{X}$ is a $2n$-qubit register and $\gray{Y}$ is an arbitrary-sized register of $P$'s choice. It sends the contents of $\gray{X}$ to $C$ along with two length-$2n$ classical strings ${x} \in \{0,1\}^{2n}$ and ${\theta} \in \{+,\times\}^{2n}$.
    
%     \amit{The following point needs to rephrased: i) There is no need to explicitly prepare the state $\ket{\psi_i}$ in order to measure a qubit in $\{\dyad{\psi_i}{\psi_i}, \bbI- \dyad{\psi_i}{\psi_i}\}$. We can just mention that the measurement happens using projectors $\{\dyad{\psi_i}{\psi_i}, \bbI- \dyad{\psi_i}{\psi_i}\}$ where $\ket{\psi_i} = \ket{x_i}_{\theta_i}$, ii) The measurement output will be either 0 or 1, not $\dyad{\psi_i}{\psi_i}$ or $\bbI - \dyad{\psi_i}{\psi_i}$}
    
%     \item\label[step]{step:check-T} $C$ samples a uniformly random set of $n$ indices $T \subset [2n]$ as well as a uniformly random $\widehat{\theta} \in \{+,\times\}^{2n}$.
%     For each $i \in T$, it prepares the state $\ket{\psi_i} = \ket{x_i}_{\theta_i}$, and measures the $i$th qubit of $\gray{X}$ in $\{\dyad{\psi_i}{\psi_i}, \bbI- \dyad{\psi_i}{\psi_i}\}$.  If there exists $i \in T$ where the measument doesn't result in $\dyad{\psi_i}{\psi_i}$, then $C$ aborts the experiment and outputs $\bot$. Otherwise, it sends $T, \{\widehat{\theta}_i\}_{i \in \overline{T}}$, where $\overline{T} \coloneqq [2n] \setminus T$, to $P$.
    
%     \item $P$ responds with a subset $S \subseteq \overline{T}$. 
    
%     \item\label[step]{step:measure} $C$ measures the indices of $\gray{X}$ specified by $S$, obtaining a length-$|S|$ bitstring $X_S$ of measurement outcomes; let $s$ denote the number of indices $i \in S$ where $\theta_i \neq \widehat{\theta}_i$.
% \end{enumerate}

% \begin{lemma}[\cite{C:BouFeh10} Quantum Sampling Lemma]
% \label{lemma:sampling}
% For any computationally unbounded player $P$ and a constant $0 < \varepsilon < 1$, the probability the sampling experiment does not abort and
% \[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\bar{S}}, \gray{Y}) \leq s- \varepsilon \cdot |S|. \]
% is at most $\negl(|S|^2/n)$.
% \end{lemma}


% \begin{proof}(Sketch.)
% This lemma follows from the techniques developed in~\cite{C:BouFeh10} to relate quantum sampling to classical sampling. Following~\cite{C:BouFeh10}, it suffices to analyze the case where ${x} = 0^{2n}$ and ${\theta} = +^{2n}$, since all other settings of ${x}$ and ${\theta}$ follow from an identical argument under a change of basis. 

% In \cref{step:check-T} of the quantum sampling experiment, $C$ then verifies that for every index in a random choice of $n$ indices $T \subset [2n]$, measuring the corresponding qubit in $\{\dyad{0}{0}, \bbI - \dyad{0}{0} = \dyad{1}{1}\}$ yields 0. This is a natural quantum analogue of the following classical sampling experiment (\cite[Example 4]{C:BouFeh10}) on a length-$2n$ bitstring $X$:
% \begin{enumerate}
%     \item randomly select a size-$n$ subset $T \subset [2n]$,
%     \item verify that $X_i = 0$ on each index $i \in T$, and abort otherwise.
% \end{enumerate}

% Let $X_{\overline{T}}$ denote the string $X$ restricted to the $n$ indices $\overline{T} = [2n] \setminus T$. For any initial bitstring $X$, the ``classical error probability'' is the probability that the sampling experiment succeeds and $X_{\overline{T}}$ has relative Hamming weight $\geq \delta$ is at most $2e^{-n\delta^2/4}$ (bound derived in \cite[Appendix B.1]{C:BouFeh10}).

% \cite[Theorem 3]{C:BouFeh10} demonstrates that the ``quantum error probability'' is at most the square root of the classical error probability. That is, if the verification in \cref{step:check-T} passes, then the residual state on $\gray{X}$ restricted to $\overline{T}$ is within trace distance $\sqrt{2e^{-n \delta^2/4}}$ of a superposition of states with relative Hamming weight at most $\delta$.

% Suppose for a moment that the state were \emph{exactly} a superposition of states with relative Hamming weight at most $\delta$. Now consider the restriction of $\gray{X}$ to a subset of indices $S \subset \overline{T}$ where exactly $s$ positions have $\widehat{\theta}_i \neq \theta_i$. The relative Hamming weight of the state when restricted to $S$ is at most $\delta n/ |S|$. As long as $\delta n/ |S| < 1/2$, by~\cite[Corollary 1]{C:BouFeh10}, we have

% \[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\overline{S}}, \gray{Y}) > s - h(\delta n/|S|)\cdot |S|\]
% where $h: [0,1] \rightarrow [0,1]$ is the binary entropy function defined as $h(p) = p \log (p) + (1-p) \log (1-p)$ for $0 < p < 1$ and as $0$ for $p = 0$ or $1$.

%  For any desired $\varepsilon \in (0,1)$, there exists an $\epsilon' \in (0,1/2)$ such that $h(\varepsilon') = \varepsilon$, so we can plug in $\delta = \varepsilon' |S|/n$ to achieve the stated min-entropy lower bound of $s - \varepsilon \cdot |S|$. The error probability as already noted is $\sqrt{2e^{-n \delta^2/4}} = \sqrt{2e^{-n \varepsilon'^2|S|^2/{4n^2}}} = \sqrt{2e^{- \varepsilon'^2|S|^2/{4n}}} = negl(|S|^2/n)$.

% \end{proof}

% \section{Proof of Lemma~\ref{thm:quantumsampling}}
% \label{app:quantumsamplingproof}




==> app-tracedistance.tex <==
\section{Trace Distance between $\brho_{0,s_0,s_1}$, $\brho_{1,s_0,s_1}$}
\label{app:tracedistance}

In this section, we provide a proof of the following lemma:
\begin{lemma}
For any fixed $s_0,s_1 \in \zo^{\secp/2}$, consider the following quantum states:
\begin{align*}
    &\brho_{0,s_0,s_1} = \left\{\frac{1}{2^\secp},\frac{\ket{0,s_0,r_0} + \ket{1,s_1,r_1}}{\sqrt{2}}\right\}_{r_0,r_1 \in \{0,1\}^{\secp/2}},\\
    &\brho_{1,s_0,s_1} = \left\{\frac{1}{2^\secp},\frac{1}{2}\dyad{0,s_0,r_0}{0,s_0,r_0} + \frac{1}{2}\dyad{1,s_1,r_1}{1,s_1,r_1}\right\}_{r_0,r_1 \in \{0,1\}^{\secp/2}}.
\end{align*}
We then have that $\TD(\brho_{0,s_0,s_1},\brho_{1,s_0,s_1}) = \frac{1}{2^{\frac{\secp}{2}+1}}$
\end{lemma}
\begin{proof}
     \begin{align*}
        \brho_{0,s_0,s_1} &= \sum_{i,j \in \zo^{\secp/2}} \frac{1}{2^\secp} \left(\frac{\ket{0,s_0,i} + \ket{1,s_1,j}}{\sqrt{2}} \times \frac{\bra{0,s_0,i} + \bra{1,s_1,j}}{\sqrt{2}}  \right)\\
        &= \frac{1}{2^{\secp+1}} \sum_{i,j \in \zo^{\secp/2}}  \dyad{0,s_0,i}{0,s_0,i} + \dyad{1,s_1,j}{1,s_1,j} + \dyad{0,s_0,i}{1,s_1,j} + \dyad{1,s_1,j}{0,s_0,i} \\
        \brho_{1,s_0,s_1} &= \sum_{i,j \in \zo^{\secp/2}}  \frac{1}{2^\secp} \left( \frac{1}{2}\dyad{0,s_0,i}{0,s_0,i} + \frac{1}{2}\dyad{1,s_1,j}{1,s_1,j} \right)\\
        &= \frac{1}{2^{\secp+1}} \sum_{i,j \in \zo^{\secp/2}}  \dyad{0,s_0,i}{0,s_0,i} + \dyad{1,s_1,j}{1,s_1,j}
     \end{align*}
Hence,
    \begin{align*}
        \brho_{0,s_0,s_1} - \brho_{1,s_0,s_1} &= \frac{1}{2^{\secp+1}} \sum_{i,j \in \zo^{\secp/2}} \dyad{0,s_0,i}{1,s_1,j} + \dyad{1,s_1,j}{0,s_0,i}\\
        &= \frac{1}{2^{\secp+1}} \sum_{i,j \in \zo^{\secp/2}} \dyad{0,s_0}{1,s_1} \otimes \dyad{i}{j} + \dyad{1,s_1}{0,s_0} \otimes \dyad{j}{i}\\
        &= \frac{1}{2^{\secp+1}} \left( \dyad{0,s_0}{1,s_1} \otimes \sum_{i,j} \dyad{i}{j} + \dyad{1,s_1}{0,s_0} \otimes \sum_{i,j} \dyad{j}{i} \right)\\
        &= \frac{1}{2^{\frac{\secp}{2}+1}} \left( \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} \right)  \otimes {O}
     \end{align*}
where $O = \frac{1}{2^{\secp/2}} \sum_{i,j \in \zo^{\secp/2}}  \dyad{i}{j} = \dyad{\psi_P}{\psi_P}$, with $\ket{\psi_P} = \ket{++ \ldots +}$ being a quantum state on $\secp/2$ qubits.
Therefore, 
\begin{align*}
    \brho_{0,s_0,s_1} - \brho_{1,s_0,s_1} &= \frac{1}{2^{\frac{\secp}{2}+1}} \left( \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} \right)  \otimes \dyad{\psi_P}{\psi_P}\\
    % &= \frac{1}{2^{\frac{\secp}{2}}} \left( \frac{1}{2}\dyad{0,s_0}{1,s_1} + \frac{1}{2} \dyad{1,s_1}{0,s_0} \right)  \otimes \dyad{\psi_P}{\psi_P}
\end{align*}
We prove the following claim:
\begin{claim}
    For any fixed $s_0,s_1 \in \zo^{\secp/2}$, define the following states.
    \[
        \ket{\phi_{s_0,s_1}} = \frac{\ket{0, s_0} + \ket{1, s_1}}{\sqrt{2}} , \quad \ket{\phi'_{s_0,s_1}} = \frac{\ket{0, s_0} - \ket{1, s_1}}{\sqrt{2}}
    \]
    Then, the eigenvalue/spectral decomposition \nishant{should we discuss this somewhere?} of the hermitian matrix $\dyad{0,s_0}{1,s_1} +  \dyad{1,s_1}{0,s_0}$ is given by:
    \[ 
        \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} = \dyad{\phi_{s_0,s_1}}{\phi_{s_0,s_1}} - \dyad{\phi'_{s_0,s_1}}{\phi'_{s_0,s_1}}
    \]
\end{claim}
\begin{proof}
    We first show that both $\ket{\phi_{s_0,s_1}},\ket{\phi'_{s_0,s_1}}$ are orthonormal eigen vectors of the matrix under consideration. 
    \begin{align*}
        \left( \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} \right) \ket{\phi_{s_0,s_1}} &= \dyad{0,s_0}{1,s_1}\ket{\phi_{s_0,s_1}} + \dyad{1,s_1}{0,s_0}\ket{\phi_{s_0,s_1}}\\
        &= \frac{1}{\sqrt{2}} \ket{0,s_0} +  \frac{1}{\sqrt{2}} \ket{1,s_1} \\
        &= \ket{\phi_{s_0,s_1}}\\
        \left( \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} \right) \ket{\phi'_{s_0,s_1}} &= \dyad{0,s_0}{1,s_1}\ket{\phi'_{s_0,s_1}} + \dyad{1,s_1}{0,s_0}\ket{\phi'_{s_0,s_1}}\\
        &= \frac{-1}{\sqrt{2}} \ket{0,s_0} +  \frac{1}{\sqrt{2}} \ket{1,s_1} \\
        &= -\ket{\phi'_{s_0,s_1}}
    \end{align*}
    Also,
    \begin{align*}
        \bracket{\phi_{s_0,s_1}}{\phi'_{s_0,s_1}} &= \frac{\bra{0,s_0}+\bra{1,s_1}}{\sqrt{2}} \times \frac{\ket{0,s_0}-\ket{1,s_1}}{\sqrt{2}} \\
        &= 0
    \end{align*}
    Hence, both $\ket{\phi_{s_0,s_1}},\ket{\phi'_{s_0,s_1}}$ are orthonormal eigen-vectors of $\dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0}$ with eigen-values $1,-1$ respectively. Next, we show that they also form a complete eigenbasis.
    \begin{align*}
        \dyad{\phi_{s_0,s_1}}{\phi_{s_0,s_1}} &= \frac{1}{2} \left( \ket{0,s_0} + \ket{1,s_1} \right) \left( \bra{0,s_0} + \bra{1,s_1} \right)\\
        &= \frac{1}{2} \left( \dyad{0,s_0}{0,s_0} + \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0} + \dyad{1,s_1}{1,s_1}  \right)
    \end{align*}
    Similarly,
    \begin{align*}
    \dyad{\phi'_{s_0,s_1}}{\phi'_{s_0,s_1}} &= \frac{1}{2} \left( \dyad{0,s_0}{0,s_0} - \dyad{0,s_0}{1,s_1} - \dyad{1,s_1}{0,s_0} + \dyad{1,s_1}{1,s_1}  \right) \\
    \therefore \dyad{\phi_{s_0,s_1}}{\phi_{s_0,s_1}} - \dyad{\phi'_{s_0,s_1}}{\phi'_{s_0,s_1}} &= \frac{1}{2} \left( 2\dyad{0,s_0}{1,s_1} + 2\dyad{1,s_1}{0,s_0} \right) \\
    &= \dyad{0,s_0}{1,s_1} + \dyad{1,s_1}{0,s_0}
    \end{align*}
\end{proof}
Hence, 
\begin{align}
    \brho_{0,s_0,s_1} - \brho_{1,s_0,s_1} &= \frac{1}{2^{\frac{\secp}{2}+1}} \left( \dyad{\phi_{s_0,s_1}}{\phi_{s_0,s_1}} - \dyad{\phi'_{s_0,s_1}}{\phi'_{s_0,s_1}}\right) \otimes \dyad{\psi_P}{\psi_P} \nonumber \\
    &= \frac{1}{2^{\frac{\secp}{2}+1}} \dyad{\phi_{s_0,s_1},\psi_P}{\phi_{s_0,s_1},\psi_P} - \dyad{\phi'_{s_0,s_1},\psi_P}{\phi'_{s_0,s_1},\psi_P} \nonumber \\
    \implies \TD(\brho_{0,s_0,s_1}, \brho_{1,s_0,s_1}) &= \frac{1}{2} \Tr\left( \sqrt{\left(\brho_{0,s_0,s_1}- \brho_{1,s_0,s_1}\right)^2} \right) \nonumber \\
    &= \frac{1}{2} \Tr \left( \sqrt{ \dyad{\phi_{s_0,s_1},\psi_P}{\phi_{s_0,s_1},\psi_P} + \dyad{\phi'_{s_0,s_1},\psi_P}{\phi'_{s_0,s_1},\psi_P}}\right) \nonumber \\
    &= \frac{1}{2} \Tr \left( { \dyad{\phi_{s_0,s_1},\psi_P}{\phi_{s_0,s_1},\psi_P} + \dyad{\phi'_{s_0,s_1},\psi_P}{\phi'_{s_0,s_1},\psi_P}}\right) \label{eq:trdrootstep} \\
    &= \frac{1}{2} \times \frac{2}{2^{\frac{\secp}{2}+1}} \nonumber \\
    &= \frac{1}{2^{\frac{\secp}{2}+1}} \nonumber
    \end{align}
Where Equation~\ref{eq:trdrootstep} follows because $\{\ket{\phi_{s_0,s_1},\psi_P},\ket{\phi'_{s_0,s_1},\psi_P}\} $ forms a complete eigenbasis of the $\dyad{\phi_{s_0,s_1},\psi_P}{\phi_{s_0,s_1},\psi_P} + \dyad{\phi'_{s_0,s_1},\psi_P}{\phi'_{s_0,s_1},\psi_P}$.
% \begin{align*}
%     \TD(\brho_{0,s_0,s_1}, \brho_{1,s_0,s_1}) &= \frac{1}{2} || \brho_{0,s_0,s_1} - \brho_{1,s_0,s_1} ||_{\mathsf{Tr}}\\
%     &= \frac{1}{2^{\frac{\secp}{2}+1}} \bigg|\bigg|\left( \frac{1}{2}\dyad{0,s_0}{1,s_1} + \frac{1}{2} \dyad{1,s_1}{0,s_0} \right)  \otimes \dyad{\psi_P}{\psi_P}\bigg|\bigg|_{\mathsf{Tr}}
% \end{align*}

% We prove the following claim:
% \begin{subclaim}
%     For any $s_0,s_1 \in \zo^{\secp/2}$ and any state $\psi_P$, the eigen decomposition of the 
%     \[\bigg|\bigg|\left( \frac{1}{2}\dyad{0,s_0}{1,s_1} + \frac{1}{2} \dyad{1,s_1}{0,s_0} \right)  \otimes \dyad{\psi_P}{\psi_P}\bigg|\bigg|_{\mathsf{Tr}} = 2\]
% \end{subclaim}
% \begin{proof}
    
% \end{proof}
% By properties of trace distance, we know for every $s_0,s_1$, we have \nishant{todo:expand + define trace norm, trace dist in prelims?}
% \[\bigg|\bigg|\left( \frac{1}{2}\dyad{0,s_0}{1,s_1} + \frac{1}{2} \dyad{1,s_1}{0,s_0} \right)  \otimes \dyad{\psi_P}{\psi_P}\bigg|\bigg|_{\mathsf{Tr}} = 2\] 
% And hence, 
% \begin{align*}
%     \TD(\brho_{0,s_0,s_1}, \brho_{1,s_0,s_1}) &= \frac{1}{2^{\secp/2}}
% \end{align*}
\end{proof}

==> composition.tex <==
\section{Quantum stand-alone composition in the QROM}

In this section, we present a quantum stand-alone composition theorem for protocols that are defined in the quantum random oracle model (QROM). We take inspiration from the quantum stand-alone composition theorem from \cite{C:HalSmiSon11} (in the plain model), but make adjustments to handle composition in the QROM. 

%There are two major differences in our setting. First, we strengthen the notion of quantum stand-alone (QSA) emulation from \cite{C:HalSmiSon11} to quantum \emph{oracle} stand-alone emulation (QOSA), where emulation must hold with respect to any external oracle $O$ that may be accessed by the honest party, adversary, and environment \nishant{i think it would be nice to define what the environment is informally as well? found this para hard to follow without knowing what environment was referring to?}. This enables us to use the security of an ``inner'' protocol even when the inner protocol adversary can access the random oracle used in an ``outer'' protocol. \amit{The following statement is unclear. Specifically, what exactly does ``simulator interacting in the actual protocol'' mean ?}Next, we weaken the notion of simulation to allow for simulators that can answer random oracle queries made by the environment (and share state with the simulator interacting in the actual protocol). We also further weaken this notion to consider simulators that only work for environments that make some bounded number of $q$ queries to the random oracle.


\paragraph{Quantum interactive machines.} A quantum interactive machine (QIM) is a family of machines $\{M_\secp\}_{\secp \in \bbN}$, where each $M_{\secp}$ consists of a sequence of quantum operations $M_{\secp,1},\dots,M_{\secp,\ell(\secp)}$, where $\ell(\secp)$ is the number of rounds in which $M_\secp$ operates. Usually, we drop the indexing by $\secp$ and refer to $M = M_1,\dots,M_\ell$. 

%$M$ operates on an input register $\gray{M_0}$, memory registers $\gray{M_1},\dots,\gray{M_\ell}$, and communication registers $\gray{C_1},\dots,\gray{C_\ell}$.

When two QIMs $A$ and $B$ interact in a $(2\ell-1)$-round protocol, they share communication registers $\gray{C_1},\dots,\gray{C_{2\ell}}$. $A$ additionally operates on an input register $\gray{A_\inp}$, memory registers $\gray{A_1,\dots,\gray{A_{\ell}}}$, and output register $\gray{A_\out}$, where 

\begin{itemize}
    \item $A_1: \gray{A_\inp} \otimes \gray{A_1} \to \gray{A_2} \otimes \gray{C_1}$,
    \item for each $i \in [\ell-1]$, $A_i : \gray{A_i} \otimes \gray{C_{2i-2}} \to \gray{A_{i+1}} \otimes \gray{C_{2i-1}}$,
    \item and $A_\ell: \gray{A_\ell} \otimes \gray{C_{2\ell-2}} \to \gray{A_\out} \otimes \gray{C_{2\ell-1}}$.
\end{itemize}

$B$ additionally operates on an input register $\gray{B_\inp}$, memory registers $\gray{B_1},\dots,\gray{B_{\ell-1}}$, and output register $\gray{B_\out}$, where 

\begin{itemize}
    \item $B_1: \gray{B_\inp} \otimes \gray{B_1} \otimes \gray{C_1} \to \gray{B_2} \otimes \gray{C_2}$,
    \item for each $i \in [\ell-1]$, $B_i: \gray{B_i} \otimes \gray{C_{2i-1}} \to \gray{B_{i+1}} \otimes \gray{C_{2i}}$,
    \item and $B_\ell : \gray{B_\ell} \otimes \gray{C_{2\ell-1}} \to \gray{B_\out}$.
\end{itemize}

We can also consider more than two QIMs interacting, and set up communication registers between each pair of machines.
 

\paragraph{Functionalities, protocols, and emulation.} Let $\cF$ denote a \emph{functionality}, which is a classical interactive machine specifying the instructions to realize a cryptographic task. A two-party protocol\footnote{One can also consider multi-party protocols, but we restrict to the two-party setting in this work.} $\Pi$ for $\cF$ consists of two QIMs $(A,B)$.\footnote{Technically, each of $A$ and $B$ is an infinite family of interactive machines, parameterized by the security parameter $\secp$.} An adversary $\cA$ is another quantum interactive machine that intends to attack the protocol. In this work, we only consider \emph{static} adversaries, that operate in the presence of an \emph{environment} $\cZ = (\cZ_0,\cZ_1)$ that consists of two quantum operations. The execution of the protocol $\Pi$ in the presence of environment $\cZ$ and adversary $\cA$ defines a quantum operation that outputs a single bit, which we denote by $M[\Pi,\cZ,\cA](1^\secp)$. This quantum operation is defined as follows.

\begin{itemize}
    \item $\cA$ is defined to either corrupt party $A$ or $B$, $P \in \{A,B\}$ is defined to be the uncorrupted party, and $\secp \in \bbN^+$ is the security parameter. 
    \item $\cZ_0(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$,
    where $\brho_\secp$ is $\cA$'s input, $x$ is $P$'s (classical) input, and $\bsigma_\secp$ is an auxiliary quantum state.
    \item $\cA(\brho_\secp)$ interacts with $P(x)$ during the execution of $\Pi$, and outputs a quantum state $\btau_\secp$.
    \item $\cZ_1(\btau_\secp,\bsigma_\secp)$ outputs a bit $b$.
\end{itemize}

Let $\Pi$ and $\Gamma$ be two protocols. We say that $\Pi$ statistically \emph{quantum stand-alone emulates}\footnote{One can also consider the notion of \emph{computational} stand-alone emulation, in which $\Pi,\Gamma,\cA,\cS,$ and $\cZ_1$ are all restricted to be polynomial-time (though $\cZ_0$ may be unbounded).} (QSA emulates) $\Gamma$ if for all $\cA$ there exists a $\cS$ (sometimes called a \emph{simulator}) such that for all $\cZ$, \[\left|\Pr[M[\Pi,\cZ,\cA](1^\secp)] - \Pr[M[\Gamma,\cZ,\cS](1^\secp)]\right| = \negl(\secp).\]  

An \emph{ideal-world} protocol $\widetilde{\Pi}_\cF$ for functionality $\cF$ consists of two ``dummy'' parties $\widetilde{A},\widetilde{B}$ that have access to an additional ``trusted'' party that implements $\cF$. That is, $\widetilde{A},\widetilde{B}$ each hand their inputs to $\cF$, which runs and then returns outputs to $\widetilde{A},\widetilde{B}$. An execution of $\widetilde{\Pi}_\cF$ in the presence of an adversary $\cS$ and environment $\cZ$ is defined as before except that $\cS$ may not corrupt $\cF$. We say that a protocol $\Pi$ (statistically) \emph{quantum stand-alone realizes} (QSA realizes) $\cF$ if $\Pi$ statistically QSA emulates $\widetilde{\Pi}_\cF$.

\paragraph{\cite{C:HalSmiSon11} composition.} Let $\Pi$ be a protocol that uses another protocol $\Gamma$ as a subroutine, and let $\Gamma'$ be a protocol that QSA emulates $\Gamma$. Define the \emph{composed} protocol $\Pi^{\Gamma/\Gamma'}$ to be the protocol $\Pi$ with every execution of $\Gamma$ replaced by $\Gamma'$. In this work, we consider protocols $\Pi$ that can invoke $\Gamma$ (and potentially other subprotocols) multiple times, but where only a \emph{single invocation} of any subprotocol is invoked at any given time. In a \emph{hybrid} model, parties can make calls to an ideal-world protocol $\widetilde{\Pi}_\cG$ for some functionality $\cG$. We call such a protocol a $\cG$-hybrid protocol and denote it $\Pi^\cG$.

\begin{theorem}[\cite{C:HalSmiSon11}]
Let $\cF$ and $\cG$ be functionalities, let $\Pi_\cG$ be a $\cG$-hybrid protocol that statistically (resp. computationally) QSA realizes $\cF$ and let $\Gamma$ be a protocol that statistically (resp. computationally) QSA realizes $\cG$. Then $\Pi^{\cG/\Gamma}$ statistically (resp. computationally) QSA realizes $\cF$.
\end{theorem}

\paragraph{Quantum oracle algorithms.} Let $\cX,\cY$ be finite sets and let $O : \cX \to \cY$ be an arbitrary function. We say that $A^{O}$ is a $q$-query \emph{quantum oracle algorithm} if it can be written as $A_{q+1}U_OA_{q}U_O\dots U_OA_2U_O\cA_1$, where $A_1,\dots,A_{q+1}$ are arbitrary quantum operations, and $U_O$ is the unitary defined by \[U_O: \ket{x}\ket{y} \to \ket{x}\ket{y \oplus O(x)},\] operating on the appropriate registers of $A$'s state. Sometimes, it will be convenient to consider algorithms $A^{O_1,O_2}$ with access to \emph{multiple} oracles $O_1: \cX_1 \to \cY_1, O_2: \cX_2 \to \cY_2$, written as $A_{q+1}U_{O_2}A_{q}U_{O_1}\dots U_{O_2}A_2U_{O_1}A_1$. Defining $O(b,x) = O_b(x)$ for $(b,x) \in (1,\cX_1) \union (2,\cX_2)$, it is easy to see that any $A^{O_1,O_2}$ can be written as an oracle algorithm ${A'}^O$ and that any $A^O$ can be written as an oracle algorithm ${A'}^{O_1,O_2}$, with an appropriate increase in number of queries.

We say that $A$ is a \emph{quantum interactive oracle machine} if $A = A_1^O,\dots,A_\ell^O$ is such that each $A_i^O$ is a quantum oracle algorithm.

\paragraph{The quantum random oracle model.} We will consider protocols $\Pi_\RO$ that operate in the \emph{quantum random-oracle model} (QROM). In such a protocol, a random function $H \gets \cH_{\cX,\cY}$ is first sampled, where $\cH_{\cX,\cY}$ is the uniform distribution over functions $H: \cX \to \cY$. Then, oracle algorithms $A^H$ and $B^H$ interact in the protocol. Note that this model also captures protocols that are defined with respect to \emph{multiple} random oracles $H_1 \gets \cH_{\cX_1,\cY_1}, H_2 \gets \cH_{\cX_2,\cY_2}$, where honest parties are oracle algorithms $A^{H_1,H_2}$ and $B^{H_1,H_2}$. This follows by letting $\cX \coloneqq (1,\cX_1) \cup (2,\cX_2)$, letting $\cY$ be such that $|\cY| \geq \max\{|\cY_1|,|\cY_2|\}$ \nishant{Shouldn't this be $|\cY_1|+|\cY_2|$? for example if $\cY_1,\cY_2$ are $\zo$, then $\cY$ needs to be 2 bits long?}\james{in this case the output should still be one bit long for each input}, and defining appropriate embedding operations from $\cY$ to $\cY_1$ and to $\cY_2$.

\paragraph{QSA emulation in the QROM.} Quantum stand-alone security of a protocol $\Pi_\RO$ in the quantum random oracle model is formalized slightly differently than stand-alone security in the standard model (as described above). First, we split the random oracle into an ``internal'' random oracle $H_\internal$ and an external random oralce $H_\ext$, where $H_\internal$ is the oracle used in $\Pi_\RO$, and $H_\ext$ is an oracle that may be accessed in the case that $\Pi_\RO$ is run within a larger context. Next, we give slightly more power to the ideal-world adversary $\cS$. In particular, $\cS$ may answer random oracle queries to $H_\internal$ made by the environtment. That is, when $\cZ$ issues a query to $H_\internal$, the unitary $U_{H_\internal}$ is replaced with a quantum operation specified by $\cS$, that itself may make calls to $H_\internal$.


%We now formally define what it means for a protocol $\Pi_\RO$ to statistically quantum oracle stand-alone (QOSA) realize a functionality $\cF$ in the QROM.




%In this work, we will consider protocol execution in the presence of adversaries and environments that have access to some external oracle $O$. That is, adversaries $\cA^O$ and environments $\cZ^O = (\cZ_0^O,\cZ_1^O)$ may be \emph{quantum oracle algorithms} that query $O$ throughout their execution. The following definition can be seen as a strict generalization of the notions of QSA emulation / realization.

%\begin{definition}

%\amit{Why are we quantifying over \textbf{all} oracles in the security definition ? Seems that it would be too strong of a definition ? (e.g. consider an oracle for halting problem, no protocol would be secure in the presence of this oracle) }


%Let $\Pi$ and $\Gamma$ be two protocols. We say that $\Pi$ statistically \emph{quantum oracle stand-alone emulates} (QOSA emulates) $\Gamma$ if for all quantum oracle adversaries $\cA$, there exists a quantum oracle algorithm $\cS$ such that for all finite sets $\cX,\cY$, oracles $O: \cX \to \cY$, and environments $\cZ^O = (\cZ_0^O,\cZ_1^O)$,

%\[\left|\Pr[M[\Pi,\cZ^O,\cA^O](1^\secp) = 1] - \Pr[M[\Gamma,\cZ^O,\cS^O](1^\secp) = 1]\right| = \negl(\secp).\]

%Let $\cF$ be a functionality. We say that a protocol statistically \emph{quantum oracle stand-alone realizes} (QOSA realizes) $\cF$ if $\Pi$ statistically QOSA emulates $\widetilde{\Pi}_\cF$.

%\end{definition}






%\footnote{It is also meaningful to consider protocols $\Pi_\RO$ that just QSA realize a functionality $\cF$ in the QROM, but here we explicitly describe the more general notion of QOSA realization.} 

%\amit{Again, I think quantifying over all oracles $O$ is quite strong. Also, shouldn't $H$ be simulated at some point i.e. in one of the experiments, $H$ shouldn't appear as an oracle at all ?}

\begin{definition}\label{def:QSA-in-QROM}
Let $\Pi_\RO$ be a protocol in the QROM and let $\cF$ be a functionality. We say that $\Pi_\RO$, which operates with respect to a random oracle sampled from $\cH_{\cX_\internal,\cY_\internal}$, statistically quantum oracle realizes $\cF$ in the QROM if for any quantum oracle adversary $\cA$, there exists a quantum oracle algorithm $\cS$ such that for all finite sets $\cX_\ext,\cY_\ext$ and environments $\cZ = \left(\cZ_0,\cZ_1\right)$,

\begin{align*}
&\bigg|\Pr_{\substack{H_\internal \gets \cH_{\cX_\internal,\cY_\internal},\\ H_\ext \gets \cH_{\cX_\ext,\cY_\ext}}}\left[M\left[\Pi_\RO,\cZ^{H_\internal,H_\ext},\cA^{H_\internal,H_\ext}\right](1^\secp) = 1\right]\\ &- \Pr_{\substack{H_\internal \gets \cH_{\cX_\internal,\cY_\internal},\\ H_\ext \gets \cH_{\cX_\ext,\cY_\ext}}}\left[M\left[\widetilde{\Pi}_\cF,\cZ^{\cS^{H_\internal},H_\ext},\cS^{H_\internal,H_\ext}\right](1^\secp) = 1\right]\bigg| = \negl(\secp).
\end{align*}


%where $M\left[\widetilde{\Pi}_\cF,\cZ^{\cS^{H_\internal},H_\ext},\cS^{H_\internal,H_\ext}\right](1^\secp)$ consists of the following steps:

%\begin{itemize}
    %\item $\cZ_0^{O,\cS_0^H}(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$. $\cZ_0$'s queries to $H$ are answered by the (stateful) oracle machine $\cS_0^H$.  \nishant{$\cS_0^H$ state also passed to $\cS_1^{O,H}$ right? if so, we should state it explicitly otherwise it is not clear if that is happening}
    %\item $\cS_1^{O,H}(\brho_\secp)$ interacts with the honest party $P(x)$ and the trusted party implementing $\cF$, and outputs a quantum state $\btau_\secp$, along with an additional quantum state that is passed back to $\cS_0$. \amit{Should we be more explcit about this state transfer from $\cS_1 \rightarrow \cS_0$ ? i.e. what exactly is the consequence of allowing such transfer versus not allowing ?}
    %\item $\cZ_1^{O,\cS_0^H}(\btau_\secp,\bsigma_\secp)$ outputs a bit $b$. $\cZ_1$'s queries to $H$ are answered by the (stateful) oracle machine $\cS_0^H$. 
%\end{itemize}

%\amit{Should we also be defining $M\left[\Pi_\RO,\cZ^{O,H},\cA^{O,H}\right](1^\secp)$ ?}

\end{definition}

Next, we define a weakening of QSA realization of functionalities in the QROM that allows the simulator $\cS$ to have some dependence on the environment $\cZ$. In particular, we will consider simulators that may depend on the number of queries that $\cZ$ makes to the random oracle $H$, and we call this \emph{$q$-dependent simulation}.

\begin{definition}
Let $\Pi_\RO$ be a protocol in the QROM and let $\cF$ be a functionality. We say that $\Pi_\RO$ statistically quantum stand-alone realizes $\cF$ in the QROM with \emph{query-dependent simulation} if for any $q \in \bbN$, \cref{def:QSA-in-QROM} holds with respect to any environment $\cZ$ that makes at most $q$ total queries to $H_\internal$. We refer to the simulator guaranteed by the definition as $(\cS[\cA,q])$.
\end{definition}


\paragraph{Oracle composition theorem.} Finally, we give a quantum stand-alone composition theorem that may be utilized for the composition of protocols operating in the QROM.

\begin{theorem}
\label{thm:malc-qrom-composition}
Let $\cF$ and $\cG$ be functionalities, let $\Pi_\RO^\cG$ be a $\cG$-hybrid protocol in the QROM that QSA realizes $\cF$ with query-dependent simulation (resp. without query-dependent simulation) and let $\Gamma_\RO$ be a protocol in the QROM that QSA realizes $\cG$ with query-dependent simulation (resp. without query-dependent simulation). Then $\Pi_\RO^{\cG/\Gamma_\RO}$ is a protocol in the QROM that QSA realizes $\cF$ with query-dependent simulation (resp. without query-dependent simulation).
\end{theorem}

\begin{proof}
We prove the theorem for the case of query-dependent simulation, since it is the harder case to prove. We also assume without loss of generality that $\Pi$ calls $\Gamma$ exactly once, since we anyway only allow at most one session of $\Gamma$ to be called at a time. Let $H_\Pi$ be the random oracle used in $\Pi_\RO^\cG$ and let $H_\Gamma$ be the random oracle used in $\Gamma_\RO$. Then the random oracle used in $\Pi_\RO^{\cG/\Gamma_\RO}$ consists of the pair of oracles $(H_\Pi,H_\Gamma)$. Now, we want to show that for any $q \in \bbN$ and any adversary $\cA$ interacting in $\Pi_\RO^{\cG/\Gamma_\RO}$, there exists a simulator $\cS[\cA,q]$ such that for any finite sets $\cX_\ext,\cY_\ext$, and any environment $\cZ$ that makes at most a total of $q$ combined queries to $H_\Pi$ and $H_\Gamma$, it holds that 

\begin{align*}
&\bigg|\Pr_{H_\Pi,H_\Gamma,H_\ext}\left[M\left[\Pi_\RO,\cZ^{H_\Pi,H_\Gamma,H_\ext},\cA^{H_\Pi,H_\Gamma,H_\ext}\right](1^\secp) = 1\right]\\ &- \Pr_{H_\Pi,H_\Gamma,H_\ext}\left[M\left[\widetilde{\Pi}_\cF,\cZ^{\cS[\cA,q]^{H_\Pi,H_\Gamma},H_\ext},\cS[\cA,q]^{H_\Pi,H_\Gamma,H_\ext}\right](1^\secp) = 1\right]\bigg| = \negl(\secp).
\end{align*}

We will show this in the two steps.

\begin{enumerate}
    \item First, we split $\cA$ into three parts $(\cA_0,\cA_\Gamma,\cA_1)$, \nishant{since $\Gamma$ can be an interactive machine, $\cA_0,\cA_1$ are not necessarily the part before/after $\Gamma$ right? i think $\cA_0$ is part of $\cA$ before any call to $\Gamma$, in the remaining adversary $\cA_\Gamma$ is the part which interacts with $\Gamma$ and $\cA_1$ is the remaining adversary. Is this how you are also thinking about it?}\james{good point, I think we will actually have to use a more UC-style definition. Our setting differs from that considered by HSS, since we want to combine the invocation of the inner protocol with messages exchanged for the outer protocol, and we could have interleaved inner and outer protocol messages.} where $\cA_\Gamma$ is the part of $\cA$ that interacts in $\Gamma_\RO$. Let $q_\Gamma$ be the total number of queries that $(\cA_0,\cA_1)$ make to $H_\Gamma$. Let $O_\Gamma = (O,H_\Pi)$ \nishant{this is not used in this step right?}. Then since $\Gamma_\RO$ QOSA realizes $\cG$ with $q$-dependent simulation, there exist algorithms $(\cS[\cA_\Gamma,q+q_\Gamma]_0,\cS[\cA_\Gamma,q+q_\Gamma]_1)$ such that, for any $\cZ$ that makes at most $q$ total queries to $H_\Pi$ or $H_\Gamma$, the output of $M
    \left[\Pi_\RO,\cZ^{O,H_\Pi,H_\Gamma},\cA^{O,H_\Pi,H_\Gamma}\right](1^\secp)$ is negligibly close to the output of the following experiment.
    \begin{itemize}
        \item $\cZ_0^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$.
        \item $\cA_0^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\brho_\secp)$ interacts with the honest party $P(x)$ and outputs a quantum state $\brho'_\secp$.
        \item $\cS[\cA_\Gamma,q+q_\Gamma]_1^{O,H_\Pi,H_\Gamma}(\brho'_\secp)$ interacts with the honest party $P(x)$ and the trusted party implementing $\cG$, and outputs a quantum state $\brho''_\secp$.
        \item $\cA_1^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\brho''_\secp)$ interacts with the honest party $P(x)$ and outputs a quantum state $\btau_\secp$.
        \item $\cZ_1^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\btau_\secp,\bsigma_\secp)$ outputs a bit b.
    \end{itemize}
    \item Next, define \nishant{should the $q_\Gamma$ be $q+q_\Gamma$ all over below?}
    \begin{align*}
    &\cZ_{0,\Pi}^{O,H_\Pi,H_\Gamma} \coloneqq \cZ_0^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}\\
    &\cA_\Pi^{O,H_\Pi,H_\Gamma} \coloneqq \left(\cA_0^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}},\cS[\cA_\Gamma,q_\Gamma]_1^{O,H_\Pi,H_\Gamma},\cA_1^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}\right)\\
    &\cZ_{1,\Pi}^{O,H_\Pi,H_\Gamma} \coloneqq \cZ_1^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}.
    \end{align*}
    Define $O_\Pi = (O,H_\Gamma)$ and note that $\cA_\Pi^{O,H_\Pi,H_\Gamma}$ is an adversary for $\Pi_\RO$ in the $\cG$-hybrid model, with access to external oracle $O_\Pi$. Since $\Pi_\RO^\cG$ QOSA realizes $\cF$ with $q$-dependent simulation, there exist algorithms $(\cS[\cA_\Pi,q]_0,\cS[\cA_\Pi,q]_1)$  such that the output of the above experiment is negligibly close to the output of $M\left[\widetilde{\Pi}_\cF,\cZ^{O,\cS[\cA_\Pi,q]_0^{H_\Pi},\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}},\cS[\cA_\Pi,q]_1^{O,H_\Pi,H_\Gamma}\right](1^\secp)$,
    since the environment $(\cZ_{0,\Pi},\cZ_{1,\Pi})$ makes at most $q$ queries the random oracle $H_\Pi$. Thus, define $\cS[\cA,q]_0$ to run $\cS[\cA_\Pi,q]_0^{H_\Pi}$ on $H_\Pi$ queries and $\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}$ on $H_\Gamma$ queries, and define $\cS[\cA,q]_1 \coloneqq \cS[\cA_\Pi,q]_1$. This completes the proof. 
    
  
    
\end{enumerate}


%Let $\cX_\Pi,\cY_\Pi$ be the domain and range for the random oracle used in $\Pi_\RO^\cG$, and let $\cX_\Gamma,\cY_\Gamma$ be the domain and range for the random oracle used in $\Gamma_\RO$. Then define $\cX_{\Pi/\Gamma} \coloneqq (0,\cX_\Pi) \union (1,\cX_\Gamma)$ and $\cY_{\Pi/\Gamma}$ of appropriate size. We consider $\Pi_\RO^{\cG/\Gamma_\RO}$ to be a protocol in the QROM  
\end{proof}


==> intro.tex <==
\section{Introduction}
%\james{maybe add an initial paragraph about the power of quantum information in cryptography? QKD, quantum money, uncloneable primitives etc., then identifying OT without structured hardness assumptions as another example, leading into the definitional next paragraph... }

Quantum information has proven to have several remarkable applications in the field of cryptography, from unconditionally secure key agreement~\cite{BenBra84}, to cryptographically uncloneable currency~\cite{Wiesner1983ConjugateC}, to certifiable randomness~\cite{8555116}, and many others. In fact, Wiesner’s original paper introducing the concept of quantum money~\cite{Wiesner1983ConjugateC} also paved the way for applications of quantum information to the cryptographic task of \emph{oblivious transfer}~\cite{Rabin81,EGL}. It has since been shown that quantum information can be leveraged to obtain oblivious transfer from symmetric-key cryptography~\cite{FOCS:CreKil88,C:DFLSS09,C:BouFeh10,BCKM2021,GLSV}, which is widely believed to be impossible in a classical world~\cite{C:ImpRud88}.

In this paper, we further explore the application of quantum information to constructing oblivious transfer. In particular, we investigate the possibility of using the (quantum) random oracle model to obtain \emph{efficient} (in terms of round complexity and communication complexity) and \emph{unconditionally secure} quantum oblivious transfer, contributing conceptually new protocols and analyses. First, we introduce the reader to various cryptographic notions that we employ.





\paragraph{Oblivious Transfer.} Oblivious Transfer (OT) allows a sender to obliviously transmit one out of two strings to a receiver, while keeping the other string hidden. OT is simple yet powerful, and forms the basis for \emph{secure computation} of arbitrary classical and quantum functionalities.
%primitive. known to be complete for secure computation, which %forms . 
Secure computation, which is a fundamental notion in the field of modern cryptography, allows a set of mutually distrusting parties to compute arbitrary functions on their private inputs, without revealing these inputs to each other. 
%That is, 
Protocols for secure computation of any classical (or quantum) functionality can be obtained from just a protocol for oblivious transfer, and one-way functions. 

%This work considers (quantum) OT in the (quantum) random oracle model, which we discuss next.
%That is, one can construct a protocol for secure computation of any classical (or quantum) functionality, starting with just a protocol for oblivious transfer.


%\paragraph{The Random Oracle Model.}
\paragraph{The (Quantum) Random Oracle Model.} The random oracle (RO) model~\cite{C:BelRog93} is the most common heuristic in cryptography. It has been widely used to argue the security of efficient and minimally interactive constructions of oblivious transfer and secure computation protocols. In this model, the adversary is given oracle access to a truly random hash function $H : \{0, 1\}^* \rightarrow \{0, 1\}^*$, and it can only learn $H(x)$ by explicitly querying the oracle $H$ on input $x$. In actual implementations, $H$ is replaced by a concrete hash function that is heuristically assumed to behave like a random oracle. 

A quantum attacker, however, can always evaluate this hash function on a superposition of inputs, and this is modeled by allowing the adversary {\em superposition access} to the random oracle. This model is called the Quantum Random Oracle Model (QROM)~\cite{AC:BDFLSZ11}, and allows the adversary to submit quantum states $\ket{\psi} = \Sigma_x \alpha_x \ket{x}$ to an oracle $H$ and receive the evaluated state $\Sigma_x \alpha_x \ket{x}\ket{H(x)}$.


%\paragraph{Oblivious Transfer and Random Oracles.}
When participants have access to classical resources, it was shown in the seminal work of~\cite{C:ImpRud88} that any construction of OT must rely on cryptographic hardness {\em beyond} the use of a random oracle. 
Nevertheless, the random oracle model allows for {\em efficient} constructions of classical OT while additionally relying on other structured asymmetric hardness assumptions~\cite{C:BelMic89,LC:ChoOrl15,HauLos17,BDDMN17,CCS:MasRin19,PKC:CanSarWan20}.
%\dakshita{say something about classical OT constructions here}

\paragraph{Quantum OT in the QROM.}
With access to quantum resources, it was recently shown by~\cite{BCKM2021,GLSV} building on~\cite{FOCS:CreKil88,C:BBCS91,C:DFLSS09,C:BouFeh10} that no cryptographic hardness besides the existence of a natural type of (classically statistically binding) commitment is required to obtain OT. Such commitments are known to exist from one-way functions\footnote{In fact, even more recent work~\cite{cryptoeprint:2021:1691,cryptoeprint:2021:1663} has shown that such commitments can be based on assumptions potentially weaker than the existence of one-way functions, namely pseudorandom quantum states~\cite{JiL18}. While this is a very exciting and actively developing line of research, our goal in this work is to develop new frameworks for \emph{efficient} quantum OT using classical building blocks such as hash functions.}, and exist unconditionally in the Quantum Random Oracle model (QROM) (we refer the reader to~\cite{DFMS21} and references therein). 
%Thus, quantum oblivious transfer (QOT) exists {\em unconditionally} in the QROM. 

%However, the only known realizations of pseudorandom quantum states rely on the existence of one-way functions.


Besides being conceptually exciting, realizations of OT that rely only on simple quantum capabilities and hash functions may be of significant practical interest in the coming decades. 
In fact, unconditional realizations of OT from polarized photons in incomparable models such as the bounded storage and noisy storage models have already been studied (eg., in~\cite{Wehner2010,Erven2014,Ito2017,Furrer2018}). Unconditional realizations in the QROM may offer some benefits over these realizations, as we discuss in Section \ref{subsec:related work}. 

All prior constructions of OT that rely on quantum communication and bit commitments build on the Crepeau-Kilian OT template~\cite{FOCS:CreKil88}, which we discuss next.



\paragraph{The Crepeau and Kilian Template.} 
%\paragraph{Quantum OT in the QROM.} 
%Recent works~\cite{GLSV,BCKM2021} built on a template of 
Crepeau and Kilian~\cite{FOCS:CreKil88} first proposed a template for achieving quantum oblivious transfer based on Wiesner's conjugate encoding scheme~\cite{Wiesner1983ConjugateC}. 
The scheme begins with the sender transmitting single qubit states encoding either $0$ or $1$ in either the computational or Hadamard basis (so-called BB84 states~\cite{BenBra84}). 
Crucially, measuring in the wrong basis completely destroys information about the encoded bit. 
This allows a sender and receiver to establish two channels, where the capacity of one is larger than that of the other. 
The sender can then transmit one message over each channel, encoded at a rate that is intermediate to the capacity of both channels. To enforce that the receiver measure transmitted states (and hence delete some information by measuring in the wrong bases), the protocol requires the sender and receiver to run a {\em measurement-check subprotocol}.
This is essentially a game where the receiver {\em commits} to their measurement outcomes and the sender checks a subset of these commitments. 
The security of this protocol was subsequently proved assuming different properties of the commitment scheme~\cite{MayersSalvail94,STOC:Yao95,Mayers97,LoChau97,EC:Unruh10,C:DFLSS09,GLSV,BCKM2021}, which we discuss in Section \ref{subsec:related work}.



%The focus of this work is to study qualitatively new and quantitatively efficient constructions of quantum oblivious transfer by leveraging the quantum random oracle model. We discuss our results next.
%Importantly, all prior constructions of OT from quantum communication and bit commitments follow essentially the same template, due to CK88. 

\subsection{Our Results} 
The starting point for this work is the idea that the quantum random oracle model (QROM) is a natural and practically relevant model in which to study unconditionally secure quantum oblivious transfer. Then, we seek to design quantum oblivious transfer protocols from the \emph{ground up} by leveraging properties of the QROM. We attempt to minimize both \emph{interaction} and \emph{communication complexity}, and derive concrete security bounds along with exact specifications for the amount of quantum resources required by all of our protocols. Along the way, we (i) develop a \emph{new framework} for quantum OT which we refer to as the ``fixed basis'' framework, showing that it can be used to obtain resource-efficient and minimally-interactive protocols in the QROM, and (ii) provide new optimizations, concrete security bounds, and quantum resource estimates for quantum OT protocols that have appeared before in the literature, following what we refer to as the ``random basis'' framework.
At a technical level, we also develop techniques to extract from quantum sources of entropy without relying on uniformly sampled ``seeds''. 
Before describing our results, we develop notation for variants of oblivious transfer that we realize in this work.

\paragraph{Notation.} 
We consider the following types of OT protocols.
\begin{itemize}
    \item $\cF_{\OT[k]}$: the \emph{chosen-input string} OT functionality takes as input a bit $b$ from the receiver and two strings $m_0,m_1 \in \{0,1\}^k$ from the sender. It delivers $m_b$ to the receiver.
    \item $\cF_{\RROT[1]}$: the \emph{random-receiver-input bit} OT functionality takes as input $\top$ from the receiver and two bits $m_0,m_1 \in \{0,1\}$ from the sender. It samples $b \gets \{0,1\}$ and delivers $(b,m_b)$ to the receiver.
    \item $\cF_{\SROT[k]}$: the \emph{random-sender-input string} OT functionality takes as input $\top$ from the sender and $(b,m)$ from the receiver for $b \in \{0,1\}, m \in \{0,1\}^k$. It set $m_b = m$, samples $m_{1-b} \gets \{0,1\}^k$ and delivers  $(m_0,m_1)$ to the sender.
    %\iffalse{
    %\item $\cF_{\SROT[1]}$: the \emph{random-receiver-input bit} OT functionality takes as input $(b,\top)$ or $(b,m_b)$ from the receiver and $\top$ from the sender.
    %\begin{itemize}
        %\item In the case of $(b,\top)$ from the receiver and $\top$ from the sender, it samples $m_0,m_1 \gets \{0,1\}$ and delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
        %\item In the case of $(b,m_b)$ from the receiver and $\top$ from the sender, it samples $m_{1-b} \gets \{0,1\}$ and delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
    %\end{itemize}
    %\item $\cF_{\EndSROT}$: the \emph{random-sender-input} with \emph{endemic security} OT functionality takes as input $(b,\top)$ or $(b,m_b)$ from the receiver and $\top$ or $(m_0,m_1 \in \{0,1\}^k)$ from the sender. 
    %\nishant{Should this also say if both sender and receiver are corrupt, and both give corrupt inputs, then what happens?}\james{should it abort? I'm not sure its necesary to write since this case is never considered when proving that a protocol realizes a functionality}
    %\dakshita{I think we can remove $\abort$ from the description of the functionality and add it to the security definition. Just did this.}
    %\begin{itemize}
        %\item In the case of an $\abort$, it delivers $\bot$ to the both parties.
        %\item In the case of $(b,\top)$ from the receiver and $\top$ from the sender, it samples $m_0,m_1 \gets \{0,1\}^k$ and delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender. 
        %\item In the case of $(b,m_b)$ from the receiver and $\top$ from the sender, it samples $m_{1-b} \gets \{0,1\}^k$ and delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
        %\item In the case of $(b,\top)$ from the receiver and $(m_0,m_1)$ from the sender, it delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
    %\end{itemize}    
    %}\fi
    
    %\item $\cF_{\EndRROT}$: the \emph{random-receiver-input bit} OT with %\emph{endemic security}~\cite{CCS:MasRin19} OT functionality takes as input $\top$ or $b$ from the receiver and two bits $m_0,m_1 \in \{0,1\}$ from the sender. 
    %\begin{itemize}
        %\item \underline{Correctness.} Obtain $\top$ from an honest receiver and $(m_0,m_1)$ from the sender, sample $b \gets \{0,1\}$ and deliver $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender. 
        %{\em This corresponds to honest behavior.}
        %\item \underline{Endemic Security against a Malicious Receiver.} Obtain $b$ from a malicious receiver and $(m_0,m_1)$ from the sender, deliver $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
    %\end{itemize}
   
    %\item $\cF_{\RROT[k]}(\cdot,\cdot)$: the \emph{random-receiver-input} OT functionality takes as input $\top$, $b \in \{0,1\}$, or $\abort$  from the receiver and $m_0,m_1 \in \{0,1\}^k$ or $\abort$ from the sender. 
    %\begin{itemize}
        %\item In the case of an $\abort$, it delivers $\bot$ to both parties.
        %\item In the case of $\top$ from the receiver and $(m_0,m_1)$ from the sender, it samples $b \in \{0,1\}$ and delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender
    %\end{itemize}
     %. In the case of $b \in \{0,1\}$ from the receiver, it delivers $(b,m_b)$ to the receiver and $(m_0,m_1)$ to the sender.
\end{itemize}

We also note that all of the protocols constructed in this work satisfy (standard) simulation-based security with abort, where a corrupted player may choose to abort the protocol at any time, potentially before an honest party has obtained their output.

\paragraph{Our Protocols.}
%\dakshita{add somewhat concrete params to theorem statements once they are finalized}
First, we ask if back-and-forth interaction is even required in order to set up oblivious transfer correlations using quantum resources. Towards answering this question, we consider a shared EPR pair setup, where a trusted setup algorithm generates sufficiently many (polynomial in the security parameter $\lambda$) EPR pairs, and sends each party one half of every pair. Assuming such ideal EPR pair setup, we obtain the following protocol in the QROM. 
\begin{informaltheorem}
\label{infthm:one}
There exists a non-interactive\footnote{Following common convention, we use {\em non-interactive} to denote one-message or one-shot protocols that involve a single message from one party to the other.} protocol that securely realizes  $\cF_{\RROT[1]}$ with shared EPR pair setup in the QROM.
That is, assuming such setup, a sender with input bits $(m_0, m_1)$, can send a single (classical) message to a receiver that allows the receiver to only recover $(b, m_b)$ for a uniformly random bit $b$.
\end{informaltheorem}

%And yet, this model appears to be a-priori weaker than general correlated randomness setup, where both parties have access to OT-like correlations.
%\dakshita{talk about obliviously deleting one out of two messages, can be a building block etc.}

%\james{could we remark that, beyond the fact that we only use symmetric key crypto, this protocol is also conceptually interesting regardless of assumptions, as in the classical setting we can't obtain non-interactive OT with such ``unstructured'' setup - not sure how to formalize this but would be nice to find a way to say something to this effect. We could even just say something like, non-interactive OT is impossible in the classical setting, and it is interesting that the resource of entanglement gives rise to this possibility in the quantum setting}




We find this protocol to be conceptually interesting, even beyond the fact that its only source of cryptographic hardness is a hash function. Indeed, non-interactive (one-message) oblivious transfer is impossible classically, under any computational assumption, even in the common reference string and/or random oracle model. The classical impossibility stems from the fact that after the sender sends its message, the sender knows the receiver's view and can therefore run the receiver's algorithm -- so either the sender can determine which $m_b$ the receiver obtained (and therefore also determine $b$), or the receiver knows both $m_0,m_1$. In a shared EPR setup model, this impossibility no longer holds because the sender and receiver cannot access each other's halves of EPR pairs. 


Our theorem establishes that a simple EPR pair setup (which is often considered the quantum analogue of a CRS, and may be a common shared setup in a quantum network) is indeed enough not just to break the impossibility but actually to obtain full-fledged non-interactive oblivious transfer (with random receiver input). We also note that the restriction to randomized receiver input is necessary: in a non-interactive protocol, only the party that speaks can generate messages as a function of its chosen input.


Next, we show that the same protocol remains secure even if the receiver were the one performing the setup phase (as opposed to a trusted third party). That is, we consider a two-message protocol where the receiver first sets up EPR pairs and sends one half of every pair to the sender, following which the sender sends a message to the receiver as before. We show that this protocol also realizes the random-receiver-input bit OT functionality. 


%with a variant of malicious security that has previously been referred to as {\em endemic security} in the literature. 
%This is like random-receiver input bit OT, except that a malicious receiver is allowed to {\em choose} and input $b$ to the functionality, obtaining $m_b$ in return. 
%We emphasize that this is not identical to chosen-input bit OT because an honest receiver cannot choose the input $b$ (i.e. correctness holds only for uniform $b$).
\begin{informaltheorem}
\label{infthm:two}
There exists a two-message protocol that securely realizes  $\cF_{\RROT[1]}$ in the QROM. 
%That is, an input-less receiver sends a first quantum message that comprises only of halves of EPR pairs, after which a sender with input bits $(m_0, m_1)$, can send a single (classical) message to a receiver. This message allows an honest receiver to recover $(b, m_b)$ for a uniformly random bit $b$. The protocol satisfies standard simulation-based security against malicious senders and endemic security against malicious receivers. The latter is like standard simulation-based security except that a malicious receiver in the ideal world is allowed to choose a bit $b$ and obtain $m_b$ from the ideal functionality.
\end{informaltheorem}

In order to obtain the protocols discussed above, we first develop protocols achieveing the {\em random-sender-input} chosen-receiver-input bit OT functionality described above. We reverse this protocol to obtain the {\em random-receiver-input} chosen-sender-input bit OT protocols in Informal Theorems \ref{infthm:one} and \ref{infthm:two} without any additional interaction, by relying on OT reversal techniques from the literature~\cite{C:IKNP03,EC:WolWul06}.


Furthermore, the protocols in Informal Theorems \ref{infthm:one} and \ref{infthm:two} be converted into protocols realizing the chosen-input string OT ($\cF_{\OT[k]}$) functionality by adding just one reorientation message at the end. This can be based on existing compilers in the literature and standard OT reorientation techniques~\cite{C:IKNP03,EC:WolWul06}.

In fact, we show that it is possible to eliminate the need for entanglement with three messages of communication.  The resulting protocol uses no entanglement, and only requires one quantum message containing BB84 states followed by two classical messages.

%, and achieves concretely efficient parameters.
%\dakshita{bit worried about raising the reader's hopes that they will see amazingly efficient protocols}

\begin{informaltheorem}
\label{infthm:three}
For every $k = \poly(\lambda)$, there exists a three-message protocol that securely realizes $\cF_{\OT[k]}$ in the QROM.
\end{informaltheorem}

Finally, in light of prior works~\cite{C:DFLSS09,GLSV,BCKM2021} that establish commitments as the only necessary cryptographic building block for quantum OT, we consider a model where we \emph{only} assume access to idealized classical (quantum-secure) bit commitments (in lieu of a random oracle). Informally, these are commitments that allow for the existence of an extractor which extracts the message committed to by a malicious committer, and a simulator that is able to equivocate a committed string to provide openings to multiple messages in the opening phase. We observe that the original~\cite{FOCS:CreKil88} protocol, as analyzed in the many followups including~\cite{C:DFLSS09,C:BouFeh10}, can naturally be written as a five-message protocol in the ideal non-interactive commitment model. Then, we show how to optimize the protocol in order to obtain the following new results. 

\begin{informaltheorem}
\label{infthm:four}
There exists a three-message protocol that securely realizes $\cF_{\RROT[1]}$ in the ideal non-interactive commitment model. For every $k = \poly(\lambda)$, there exists a four-message protocol that securely realizes $\cF_{\OT[k]}$ in the ideal non-interactive commitment model.
\end{informaltheorem}

%We note that one difference between the protocols in Informal Theorem \ref{infthm:four} and our other protocols is that the ones in Informal Theorem \ref{infthm:four} do not explicitly rely on the random oracle, but only on idealized commitments, whereas previous ones also require the use of the random oracle for the Fiat-Shamir transform.

\paragraph{Additional remarks.} We note that all of our protocols rely on ideal (extractable and equivocal) bit commitments, which we realize unconditionally in the QROM by adapting techniques from prior work. 
We conjecture that one may be able to plug in other secure $k$-round realizations of ideal commitments (eg., in the CRS model or the plain model) to the protocol in Informal Theorem \ref{infthm:four} to obtain realizations of $k+3$-round OT,  without a random oracle.

We also compute concrete parameter estimates for our protocols. In particular, we estimate the number of EPR pairs/BB84 states required for each of our protocols, and derive concrete security losses incurred by our protocols. This is discussed further in \cref{subsec:concrete-parameters}, where we also provide a table of our estimates. 

%We perform a more optimal analysis of quantum cut-and-choose strategies than prior work, allowing us to obtain tighter bounds than those that would follow by a more direct application of prior techniques to our frameworks.
%\james{we shuold have a note about quantum resource estimates in our results section}
%\dakshita{added something}

%the protocol in Informal Theorem \ref{infthm:four} is presented in the ideal commitment model, so that 


%These are commitments satisfying {\em extractability}, which intuitively requires the existence of a simulator that extracts committed bits.

%In this work, we first put a new twist on the CK88 template in order to obtain a {\em round efficient} unconditional quantum OT protocol in the ideal (extractable and equivocal) commitment model.
    
    %We also suggest a qualitatively different but natural unconditional OT protocol, and prove its security against specious adversaries. In particular, we obtain the following round-efficient constructions. %This protocol relies on entanglement but has lower round complexity. 
%\end{itemize}

%Furthermore, constructions that rely on cheaper symmetric-key assumptions 
%-- in fact, also been experimentally realized --




%This template, described in detail in Section \ref{sec:overview} (Figure \ref{fig:template}) has five steps that fundamentally correspond to (at least) five messages communicated between the sender and receiver, even in the Quantum Random Oracle Model. But can we do better?

%In this work, we {\em depart} from this template, and obtain a 















%\paragraph{Round Efficient Oblivious Transfer.}
%\subsection{Our Results}
%\dakshita{
%-- wiesner encodings
%-- send measurement
%-- only then safe to reveal
%-- then set up two channels
%-- then reorient sender inputs}
%\dakshita{
%reverse the direction of erasures.
%qualitatively different, uses entanglement.
%}
%In particular, we obtain the following round efficient constructions.

%\begin{informaltheorem}
%There exists a four-round oblivious transfer protocol with query-bounded simulation security against malicious adversaries in the quantum random oracle model.
%\end{informaltheorem}

%We then suggest a qualitatively different but natural unconditional OT protocol with even fewer rounds, but where one side is only proven secure against \emph{specious} adversaries, a quantum analogue of classical semi-honest adversaries.
%\begin{informaltheorem}
%There exists a three-round oblivious transfer protocol with query-bounded simulation security against specious senders and against malicious receivers in the quantum random oracle model.
%\end{informaltheorem}
%In fact, this protocol achieves security against specious senders and arbitrarily malicious receivers.

\subsection{Related Work}
\label{subsec:related work}
\paragraph{Provable Security of the CK88 Protocol.}
The work of~\cite{C:BBCS91} suggested a transmission-error resistant version of the CK88 protocol. Subsequently, Mayers and Salvail~\cite{MayersSalvail94} proved that the CK88 protocol is secure against a restricted class of attackers that only perform single-qubit measurements, assuming the existence of information-theoretically secure quantum bit commitments. This was later improved by Yao~\cite{STOC:Yao95}, who extended the~\cite{MayersSalvail94} result to handle general quantum adversaries, assuming the existence of ideal bit commitments.
However, Mayers~\cite{Mayers97} and Lo and Chau~\cite{LoChau97} independently proved that information-theoretic quantum bit commitments were impossible.


Years later,~\cite{C:DFLSS09} proved that bit commitments satisfying additional properties, namely extractability and equivocation, suffice to achieve provable security of the CK88 protocol. Around the same time, Unruh~\cite{EC:Unruh10} showed how to obtain quantum
oblivious transfer from UC-secure commitments in the common reference string (CRS) model.
%, and as a consequence, the precise security of~\cite{FOCS:CreKil88} QOT was once again unclear. 
%However, more than a decade later, Damgard, Fehr, Lunemann, Salvail, and Schaffner \cite{C:DFLSS09} proved that bit commitment schemes satisfying certain additional properties, namely \emph{extraction and equivocation}, suffice to instantiate~\cite{FOCS:CreKil88} QOT.~\cite{C:DFLSS09} called their commitments {\em dual-mode} commitments, and provided a construction based on the quantum hardness of the learning with errors (QLWE) assumption. However, assumptions about the hardness of specific problems like QLWE are qualitatively worse than general assumptions like post-quantum one-way functions and quantum OT. 
In recent work,~\cite{GLSV,BCKM2021} obtained the required extractable and equivocal commitments based on (the black-box use of) any statistically binding, quantum computationally hiding commitment, which can in turn be based on the black-box use of one-way functions. This demonstrated that quantum oblivious transfer can be solely based on (the black-box use of) post-quantum secure one-way functions. 
%A similar result was achieved independently and concurrently by~\cite{GLSV}.
%\textcolor{red}{be nicer to GLSV}

\paragraph{Other Models.}
Unconditional realizations of (quantum) oblivious transfer are also known in the bounded storage~\cite{DFSS} and more generally the noisy storage \cite{noisy-storage} models, and these protocols have in fact even be experimentally demonstrated (we refer the reader to~\cite{Erven2014,Ito2017,Furrer2018} and references therein). 
The bounded quantum storage model~\cite{DFSS} assumes an upper bound on the amount of quantum storage that an adversary can maintain, and requires the honest party to transmit {\em more} qubits than this bound. The noisy storage model~\cite{noisy-storage} is a generalization of this model which does not assume an upper bound on quantum memory, but instead assumes that any qubit placed into quantum memory undergoes a certain amount of noise, and relies on sending sufficiently many qubits to hide information from an adversary. Because these protocols inherently rely on the inability of devices to store quantum information, advances in quantum storage and computing technology will increase the quantum communication required to securely realize these protocols.

On the other hand, the (quantum) random oracle model, which is the focus of our work, is a qualitatively different model that corresponds to the most common heuristic used in applied cryptography.
Unlike the noisy/bounded storage models, this model is likely to yield more concretely efficient protocols where the quantum communication complexity depends only on a (statistical) security parameter, in the QROM. 
However, to the best of our knowledge, it was only recently~\cite{BCKM2021,GLSV} that the feasibility of (simulation-secure) unconditional OT in the quantum random oracle model was demonstrated. 
Unfortunately, their protocols have round complexity that grows linearly with the security parameter.
On the other hand, our work lays down the theoretical foundations for round-efficient, concrete realizations of QOT in the QROM.
%practical realizations of quantum oblivious transfer in the QROM.
%the amount of quantum communication required by our protocols depends only on a (statistical) security parameter, in the QROM.

%It was only recently~\cite{BCKM2021,GLSV} that the feasibility of unconditional OT in the quantum random oracle model was demonstrated: 

%\james{motivate the QROM as another model where QOT can be acheived unconditionally - like bounded storage \cite{FOCS:DFSS05}, or more generally noisy storage \cite{noisy-storage}, compare potential practicality of protocols \cite{QOT-implementation} and tradeoffs with how reasonable each model is to assume, highlight that our QROM study has lead to QOT protocols with qualitatively different structure (departing from the basic CK88 template)}

==> mpcdef.tex <==
\section{Secure Multiparty Computation}
\label{app:mpcdefn}
Here, we provide a formal definition of secure multiparty computation.
Parts of this section have been taken verbatim from \cite{Goldbook}.

A multi-party protocol is cast by specifying a random process that maps pairs of inputs to pairs of outputs (one for each party). We refer to such a process as a functionality. The security of a protocol is defined with respect to a functionality $f$. In particular, let $n$ denote the number of parties. A non-reactive $n$-party functionality $f$ is a (possibly randomized) mapping of $n$ inputs to $n$ outputs. A multiparty protocol with security parameter $\lambda$ for computing a non-reactive functionality $f$ is a protocol running in time $\poly(\lambda)$ and satisfying the following correctness requirement: if parties $P_1, \ldots, P_n$ with inputs $(x_1,\ldots,x_n)$ respectively, all run an honest execution of the protocol, then the joint distribution of the outputs  $y_1, \ldots, y_n$ of the parties is statistically close to $f(x_1,\ldots,x_n)$.
A reactive functionality $f$ is a sequence of non-reactive functionalities $f = (f_1,\ldots, f_\ell)$ computed in a stateful fashion in a series of phases. Let $x^j_i$ denote the input of $P_i$ in phase $j$, and let $s^j$ denote the state of the computation after phase $j$. Computation of $f$ proceeds by setting $s^0$ equal to the empty string and then computing $(y_1^j,\ldots,y_n^j,s^j) \leftarrow f_j(s^{j-1},x^j_1,\ldots,x^j_n)$ for $j \in [\ell]$, where $y_i^j$ denotes the output of $P_i$ at the end of phase $j$. A multi-party protocol computing $f$ also runs in $\ell$ phases, at the beginning of which each party holds an input and at the end of which each party obtains an output. (Note that parties may wait to decide on their phase-$j$ input until the beginning of that phase.) Parties maintain state throughout the entire execution. The correctness requirement is that, in an honest execution of the protocol, the joint distribution of all the outputs $\{y_1^j,\ldots,y_n^j\}^\ell_{j=1}$ of all the phases is statistically close to the joint distribution of all the outputs of all the phases in a computation of $f$ on the same inputs used by the parties.
\subsection{Defining Security.}
We assume that readers are familiar with standard simulation-based definitions of secure multi-party computation in the standalone setting. We provide a self-contained definition for completeness and refer to \cite{Goldbook} for a more complete description.
The security of a protocol (with respect to a functionality $f$) is defined by comparing the real-world execution of the protocol with an ideal-world evaluation of $f$ by a trusted party. More concretely, it is required that for every adversary $\cA$, which attacks the real execution of the protocol, there exist an adversary $\Sim$, also referred to as a simulator, which can \emph{achieve the same effect} in the ideal-world. Let's denote $\vec{x} = (x_1,\ldots,x_n)$.
\paragraph{The real execution} In the real execution of the n-party protocol $\pi$ for computing $f$ is executed in the presence of an adversary $\Adv$. The honest parties follow the instructions of $\pi$. The adversary $\Adv$ takes as input the security parameter $k$, the set $I \subset [n]$ of corrupted parties, the inputs of the corrupted parties, and an auxiliary input $z$. $\Adv$ sends all messages in place of corrupted parties and may follow an arbitrary polynomial-time strategy.
 
 
 The interaction of $\Adv$ with a protocol $\pi$ defines a random variable $\REAL_{\pi,\Adv(z),I}(\secpar, \vec{x})$ whose value is determined by the coin tosses of the adversary and the honest players. This random variable contains the output of the adversary (which may be an arbitrary function of its view) as well as the outputs of the uncorrupted parties. We let $\REAL_{\pi,\Adv(z),I}$ denote the distribution ensemble $\{\REAL_{\Pi,\Adv(z),I}(\secpar, \vec{x})\}_{k\in\mathsf{N},\langle \vec{x},z
\rangle\in\{0,1\}^*}$.
\paragraph{The ideal execution -- security with abort.} In this second variant of the ideal model, fairness and output delivery are no longer guaranteed. This is the standard relaxation used when a strict majority of honest parties is not assumed.  In this case, an ideal execution for a function $f$ proceeds as follows:
\begin{itemize}
\item{ \bf Send inputs to the trusted party:} As before, the parties send their inputs to the trusted party, and we let $x'_i$ denote the value sent by $P_i$. Once again, for a semi-honest adversary we require $x'_i = x_i$ for all $i \in I$.
\item{ \bf Trusted party sends output to the adversary:} The trusted party computes $f(x'_1,\ldots,x'_n) = (y_1,\ldots,y_n)$ and sends $\{y_i\}_{i\in I}$ to the adversary.
\item{ \bf Adversary instructs trusted party to abort or continue:} This is formalized by having the adversary send either a continue or abort message to the trusted party. (A semi-honest adversary never aborts.) In the latter case, the trusted party sends to each uncorrupted party $P_i$ its output value $y_i$. In the former case, the trusted party sends the special symbol $\bot$ to each uncorrupted party.
\item{\bf Outputs:} 
$\Sim$ outputs an arbitrary function of its view, and the honest parties output the values obtained from the trusted party.
\end{itemize}
The interaction of $\Sim$ with the trusted party defines a random variable $\IDEAL_{f,\Adv(z)}(\secpar, \vec{x})$ as above,and we let $\{\IDEAL_{f,\Adv(z),I}(\secpar, \vec{x})\}_{k\in\mathsf{N},\langle \vec{x},z
\rangle\in\{0,1\}^*}$.
%where the subscript ``$\bot$'' indicates that the adversary can abort computation of $f$.
Having defined the real and the ideal worlds, we now proceed to define our notion of security.
\begin{definition}
\label{def:mpcdefn}
Let $k$ be the security parameter. Let $f$ be an $n$-party randomized functionality, and $\Pi$ be an $n$-party protocol for $n\in \mathsf{N}$.
%\begin{enumerate}
%\item 
We say that $\Pi$ $t$-securely computes $f$ in the presence of malicious (resp., semi-honest) adversaries if for every PPT adversary (resp., semi-honest adversary) $\Adv$ there exists a PPT adversary (resp., semi-honest adversary) $\Sim$ such that for any $I \subset [n]$ with $|I| \leq t$ the following quantity is negligible:
$$|Pr[\REAL_{\Pi,\Adv(z),I}(\secpar, \vec{x}) = 1] - Pr[\IDEAL_{f,\Adv(z),I}(\secpar, \vec{x}) = 1]|$$
where $\vec{x}=\{ x_i\}_{i\in[n]} \in \{0,1\}^{*}$ and $z\in \{0,1\}^*$.
%\item Similarly, $\pi$ $t$-securely computes $f$ \emph{with abort} in the presence of malicious adversaries if for every PPT adversary $\Adv$ there exists a super-polynomial time adversary $\Sim$ such that for any $I \subset [n]$ with $|I| \leq t$ the following quantity is negligible:
%$$|Pr[\REAL_{\pi,\Adv(z),I}(\secpar, \vec{x}) = 1] - Pr[\IDEAL_{f_{\bot},\Adv(z),I}(\secpar, \vec{x}) = 1]|.$$
%\end{enumerate}
\end{definition}

\begin{remark}[Security with Selective Abort]
We can consider a slightly weaker definition of security where the ideal world adversary can instruct the trusted party to send aborts to a subset of the uncorrupted parties. For the rest of the uncorrupted parties, it instructs the trusted functionality to deliver their output. This weakened definition is called as security with selective abort.

\begin{remark}[Privacy with Knowledge of Outputs]
\label{rem:pko}
Ishai et al.~\cite{C:IshKusPas10} considered a further weakening of the security definition where the trusted party first delivers the output to the ideal world adversary which then provides an output to be delivered to all the honest parties. They called this security notion as privacy with knowledge of outputs and showed a transformation from this notion to security with selective abort using unconditional MACs.
\end{remark}

\end{remark}
\subsection{Security Against Semi-Malicious Adversaries}
\label{app:semi-mal-defn}
We take this definition almost verbatim from \cite{AJL+12}.
We consider a notion of a semi-malicious adversary that is stronger than the standard notion of semi-honest adversary and formalize security against semi-malicious adversaries. A semi-malicious adversary is modeled as an interactive Turing machine (ITM) which, in addition to the standard tapes, has a special witness tape. In each round of the protocol, whenever the adversary produces a new protocol message $\msg$ on behalf of some party $\PP_k$, it must also write to its special witness tape some pair $(x,r)$ of input $x$ and randomness $r$ that explains its behavior. More specifically, all of the protocol messages sent by the adversary on behalf of $\PP_k$ up to that point, including the new message $m$, must exactly match the honest protocol specification for $\PP_k$ when executed with input $x$ and randomness $r$. Note that the witnesses given in different rounds need not be consistent. Also, we assume that the attacker is rushing and hence may choose the message $m$ and the witness $(x, r)$ in each round adaptively, after seeing the protocol messages of the honest parties in that round (and all prior rounds). Lastly, the adversary may also choose to abort the execution on behalf of $\PP_k$ in any step of the interaction.
\begin{definition}
 We say that a protocol $\Pi$ securely realizes $f$ for semi-malicious adversaries if it satisfies \defref{mpcdefn} when we only quantify over all semi-malicious adversaries A.	
\end{definition}





==> new-intro.tex <==
\section{New Introduction}

In 1984, Bennett and Brassard~\cite{BenBra84}, building on the work of Wiesner~\cite{Wiesner1983ConjugateC}, demonstrated that properties of quantum information can be leveraged to obtain secure key distribution, without the use of cryptographic assumptions~\cite{1055638,10.1145/359340.359342}. This result led to widespread interest in using quantum information as the basis for secure communication, which continues to this day. 

A fascinating followup question soon emerged: can quantum information be used as the basis for any cryptographic task \emph{beyond} secure communication? A natural candidate for such a task is secure \emph{computation}, which allows mutually distrusting parties to securely compute a public functionality over their private inputs. As shown by Kilian~\cite{STOC:Kilian88}, the primitive of \emph{oblivious transfer}~\cite{Rabin81,EGL}, which allows a sender to transmit one of two strings $m_0,m_1$ to a receiver without learning which was transferred, can serve as the foundation for secure computation. This motivates the question of whether oblivious transfer can be obtained by only relying on properties of quantum information.

Initially, there was progress towards a positive resolution to this question. Indeed, the ideas from Wiesner's paper that were eventually used to construct secure key distribution were originally motivated by their application to oblivious transfer: "A means for transmitting two messages either but not both of which may be received"~\cite{Wiesner1983ConjugateC}. Though Wiesner's paper did not contain a security proof (and even discussed some potential attacks), the work of Crepeau and Kilian~\cite{FOCS:CreKil88} made progress by demonstrating an approach for basing oblivious transfer on properties of quantum information \emph{plus} a secure "bit commitment" scheme. This led to interest in building bit commitment from quantum information. Unfortunately, it was eventually shown by Mayers, Lo, and Chau~\cite{Mayers97,LoChau97} that bit commitment (and thus oblivious transfer) is \emph{impossible} to build by relying solely on the properties of quantum information. 

This is indeed a strong negative result, and rules out the possibility of basing secure computation on quantum information alone. However, it was still apparent to researchers that quantum information must offer \emph{some} advantage in building secure computation systems. One could interpret the Mayers, Lo, Chau impossibility result as indicating that in order to hone in and understand this advantage, it will be necessary to make \emph{additional} physical, computational, or modeling assumptions \emph{beyond} the correctness of quantum mechanics. Indeed, much research has been performed in order to tease out the answer to this question, with three lines of work being particularly prominent and relevant to this work.\footnote{Another line of work studies (unconditional) oblivious transfer with \emph{imperfect} security \cite{10.5555/2481591.2481600,Chailloux2016OptimalBF,Kundu2020ADP}, which we view as largely orthogonal to our work.}

\begin{itemize}
    \item \textbf{Quantum OT from bit commitment.} Although unconditionally-secure bit commitment cannot be constructed using quantum information, \cite{FOCS:CreKil88}'s protocol is still meaningful and points to a fundamental difference between the quantum and classical setting, where bit commitment is not known to imply OT. A long line of work has been devoted to understanding the security of \cite{FOCS:CreKil88}'s proposal: e.g. \cite{C:BBCS91,MayersSalvail94,STOC:Yao95,C:DFLSS09,EC:Unruh10,C:BouFeh10}.
    \item \textbf{Quantum OT in the bounded storage model.} One can also impose physical assumptions in order to recover quantum OT with unconditional security. \cite{DFSS} introduced the \emph{quantum bounded-storage model}, and \cite{noisy-storage} introduced the more general \emph{quantum noisy-storage model}, and showed how to construct unconditionally-secure quantum OT in these idealized models. There has also been much followup work focused on implementation and efficiency \cite{Wehner2010,Erven2014,Ito2017,Furrer2018}.
    \item \textbf{Quantum OT from "minicrypt" assumptions.} While \cite{FOCS:CreKil88}'s proposal for obtaining OT from bit commitment scheme suggests that public-key cryptography is not required for building OT in a quantum world, a recent line of work has been interested in identifying the \emph{weakest} concrete assumptions required for quantum OT, with \cite{BCKM2021,GLSV} showing that the existence of one-way functions suffices and \cite{cryptoeprint:2021:1691,cryptoeprint:2021:1663} showing that the existence of pseudo-random quantum states suffices.
\end{itemize}


%introducing the physical assumption of bounded (or noisy) quantum storage~\cite{DFSS,noisy-storage,Wehner2010,Erven2014,Ito2017,Furrer2018}, studying a model that grants parties access to (some flavor of) a bit commitment resource~\cite{FOCS:CreKil88,C:BBCS91,MayersSalvail94,STOC:Yao95,C:DFLSS09,EC:Unruh10,C:BouFeh10}, or understanding the concrete difference in computational assumptions required in the classical vs. quantum world~\cite{C:ImpRud88,BCKM2021,GLSV,cryptoeprint:2021:1691,cryptoeprint:2021:1663}.

\subsection{Quantum OT in the quantum random oracle model} In this work, we take a new approach towards understanding and analyzing quantum OT, and initiate the explicit study of quantum OT in the \emph{quantum random oracle model} (QROM)~\cite{C:BelRog93,AC:BDFLSZ11}. The (classical) random oracle model \cite{C:BelRog93} is an idealized model in which every party is granted oracle access to a uniformly random function $H: \{0,1\}^* \to \{0,1\}^*$, and adversaries are traditionally limited by the number of \emph{queries} they can make to the oracle. A natural extension of this model to the quantum setting was described by \cite{AC:BDFLSZ11}, who allow the parties (and adversaries) to query the $H$ oracle in \emph{superposition}. We believe that there are several compelling reasons to study quantum OT in the QROM, which we list below, in particular drawing contrasts with the previously studied idealized model of bounded/noisy storage.

%The traditional random oracle model is the most widely used heuristic in cryptography, and the quantum random oracle model has been extensively used to reason about the post-quantum security of cryptographic protocols over the past decade.

\begin{itemize}
    \item \textbf{Replacing public-key assumptions.} First, we observe that previous works already implicitly establish the feasibility of \emph{unconditionally-secure} quantum OT in the QROM. In particular, \cite{C:BouFeh10} establish this for indistinguishability-based OT, and \cite{BCKM2021,GLSV} establish this for simulation-secure OT. On the other hand, in the classical setting, OT cannot be constructed unconditionally in the random oracle model \cite{C:ImpRud88}, and appears to still require public-key cryptographic assumptions. Thus, OT in the random oracle model provides a setting in which public-key cryptographic assumptions can be completely replaced by quantum information, which mirrors the situation for key exchange (in the plain model). The previously studied bounded (or noisy) storage model, which places an idealized assuption on the \emph{memory} of the adversary rather than the number of \emph{queries} (to an oracle) does not offer the same flavor of advantage. Indeed, unconditionally-secure \emph{classical} OT can be built from bounded storage assumptions, though quantum communication does provide a significant improvement in the adversary's storage bound. 
    \item \textbf{Real-world instantiations.} Any protocol proven secure in the idealized random oracle model immediately gives rise to a natural "real-world" protocol where the oracle is replaced by a cryptographic hash function, such as SHA-256. As long as there continue to exist candidate hash functions with good security properties against quantum attackers, the protocol remains useful and practically relevant. On the other hand, the noisy storage model assumes that any qubit placed into quantum memory undergoes a certain amount of noise. Thus, advances in quantum storage and computing technology will steadily degrade the security of these protocols.
    \item \textbf{Efficiency.} The random oracle model is the most widely used heuristic in cryptography, and has been used to argue the security of concretely efficient and minimally interactive constructions of (classical) oblivious transfer and secure computation protocols. Given that the feasibility of unconditionally-secure quantum OT in the QROM has previously been established, the most pressing questions to study involve efficiency. How much interaction is required for quantum OT? How many quantum resources are required for quantum OT? These same questions have been extensively studied in the classical random oracle model, under additional public-key style assumptions~\cite{C:BelMic89,LC:ChoOrl15,HauLos17,BDDMN17,CCS:MasRin19,PKC:CanSarWan20}. Thus, studying these questions in the quantum random oracle model allows a clean comparison / trade-off with the classical setting: how much (if any) additional interaction or (quantum) resources are required to remove the need for public-key assumptions when constructing oblivious transfer?
\end{itemize}


\subsection{Our contributions}

In this work, we employ the quantum random oracle model in order to study the two central efficiency questions mentioned above: how many rounds of interaction and how many resources are required for quantum OT? Rather than take the \cite{FOCS:CreKil88} protocol as a starting point, we design unconditionally-secure quantum oblivious transfer protocols from the \emph{ground up} by leveraging properties of the QROM. Along the way, we develop techniques and obtain results that are of independent interest. We now provide a high-level overview of our main contributions.


\paragraph{A new framework for quantum OT.} When optimizing for interaction, we find that using the \cite{FOCS:CreKil88} template for OT runs into a serious obstacle. The first message in \cite{FOCS:CreKil88}'s protocol consists of a sequence of uniformly randomly BB84 states, which are then measured by the receiver using their own random choice of bases. Following this, the parties have to exchange basis information in order to establish two channels, where the capacity of one is larger than that of the other. Finally, the sender can transmit their two messages, one over each channel. 
    
In order to remove the need for this multi-stage approach, we introduce a new framework for quantum OT, where the choice of bases used to prepare the initial BB84 states are mostly \emph{fixed and public}, except for a few randomly interspersed "trap" qubits. We refer to our template as the "fixed basis framework", and draw a contrast with \cite{FOCS:CreKil88}'s "random basis framework". As an initial result, we use the fixed basis framework to obtain a three-round protocol in the QROM that implements the standard chosen-input string OT functionality.

\paragraph{One-shot bit OT via entanglement.} Next, we take the fixed basis framework to its limit, and discover that if the sender and receiver begin with shared EPR pairs, they can implement a \emph{one-shot}\footnote{We use the terms "one-shot", "one-message", and "non-interactive" interchangably in this work, all referring to a protocol between two parties Alice and Bob that consists only of a single message from Alice to Bob.} bit OT protocol, implementing an ideal functionality that takes two \emph{bits} $m_0,m_1$ from Alice and delivers $m_b$ for a uniformly random $b \gets \{0,1\}$ to Bob. EPR pairs are maximally entangled two-qubit states $\frac{\ket{00} + \ket{11}}{\sqrt{2}}$, and are a very well-studied physical resource. They have been shown to be useful for many two-party tasks, including quantum communication via teleportation, quantum key distribution, and entanglement-assisted quantum error correction, and our work adds non-interactive bit OT to this list of applications.
    
We find this non-interactive feasibility result to be a scientifically interesting contribution towards understanding the power of entanglement as a resource. Indeed, non-interactive oblivious transfer is impossible classically, under any computational assumption, even in the common reference string and/or random oracle model. The classical impossibility stems from the fact that after the sender sends its message, the sender has full information about the receiver's view, and can therefore run the receiver's algorithm. So either the sender can determine which $m_b$ the receiver obtained (and therefore also determine $b$), or the receiver must know both $m_0,m_1$. In a setup model that includes pre-shared entanglement, this impossibility no longer holds because the sender and receiver cannot access each other's registers. This highlights the fundamental property of entanglement that departs from classical physics: even given perfect information about how a two-part system is prepared, knowledge of one part of the system may be entirely lost given only the other part.
    
Our work establishes that a simple, deterministic EPR pair setup is enough not just to break the impossibility but actually to obtain full-fledged non-interactive bit OT with random receiver choice bit.\footnote{Note that the restriction to randomized receiver input is necessary: in a non-interactive protocol, only the party that speaks can generate messages as a function of its chosen input.} We note that EPR pairs may be a common shared setup in a quantum network \cite{10.1145/3387514.3405853}, and have already attracted interest as a quantum analogue of a CRS \cite{10.1007/978-3-540-24587-2_20,https://doi.org/10.48550/arxiv.2102.09149,https://doi.org/10.48550/arxiv.2204.02265}. We also remark that a classical "OT correlation" setup, which trivially implies one-message OT, is fundementally different than an EPR pair setup. Indeed, OT correlations are \emph{specific to OT} and require \emph{private} randomness to set up. One consequence of this latter point is that a semi-honest dealer setting up OT correlations can observe the sender's message and learn their inputs, while a semi-honest dealer setting up EPR pairs will not learn anything by observing the subsequent communication.  
    
\paragraph{Two-round bit OT.} The notion of two-round oblivious transfer has been extensively studied in the classical setting \cite{EC:AieIshRei01,NP01,C:PeiVaiWat08,HalKal,EC:DGHMW20} and is of particular theoretical and practical interest. We show that the above protocol remains secure even if the receiver were the one performing the EPR pair setup (as opposed to a trusted dealer / network administrator). That is, we consider a two-message protocol where the receiver first sets up EPR pairs and sends one half of every pair to the sender, following which the sender sends a message to the receiver as before. We show that this protocol also realizes the same bit OT functionality with random receiver choice bit.

This results in the \emph{first} two-round protocol that satisfies some flavor of OT functionality without the use of public-key cryptography. The only setup assumption we make is the random oracle. However, we remark that we still only obtain the random receiver input functionality in this setting, and leave the construction of two-round chosen-input string OT without public-key cryptography as an intriguing open problem.

\paragraph{Seedless extraction from quantum sources of entropy.} Randomness extraction has been a crucial component in security proofs of prior quantum OT protocols, and \emph{seeded} randomness extraction from the quantum sources of entropy that arise in such protocols has been extensively studied (see e.g. \cite{TCC:RenKon05,C:BouFeh10}). In our quest to obtain two- and one- round quantum OT protocols, we lose the ability to make use of seeded randomness extraction. Thus, we prove the security of \emph{seedless} randomness extractors in this context, which may be of independent interest. In particular, we show that either the XOR function or a random oracle (for better efficiency) can be used in place of the seeded universal hashing used in prior works. See \cref{subsec:overniot} for more details.
\paragraph{Quantum resource estimations.} As mentioned earlier, we also study the question of how many (quantum) resources are required for quantum OT. In particular, we estimate the number of EPR pairs/BB84 states required for each of our protocols, and derive concrete security losses incurred by our protocols. This is discussed further in \cref{subsec:concrete-parameters}, where we also provide a table of our estimates. At a high level, we find that, while there is a fairly significant overhead arising from the "cut-and-choose" nature of quantum OT, our protocols are not prohibitively expensive. For example, our non-interactive OT in the EPR pair model requires the parties to begin with $300\secp$ shared EPR pairs, where $\secp$ is the security parameter. We expect that future work will be able to further study and optimize the concrete efficiency of quantum OT in the QROM, and our work provides a useful starting point.
\paragraph{Additional contributions.} Along the way, we make various additional observations. We formalize the notion of (non-interactive) extractable and equivocal bit commitments in the quantum random oracle, and provide a simple construction based on prior work ~\cite{C:AmbHamUnr19,C:Zhandry19,DFMS21}. We also show how to apply recent results on the security of Fiat-Shamir in the QROM \cite{C:DFMS19} in the context of quantum OT. Finally, we see many directions for future study that arise from our initial exploration of quantum OT in the QROM, which we discuss in detail in \cref{subsec:future-work}. 


==> old-3-round-receiver.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%       Old iterations
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse{
    %% [Nishant] This one is the ECC version of the 2 round protocol, which did not work out
    \begin{figure}[h]
    \begin{framed}
    \nishant{TODO - change to 3 round without ECC}
    {\bf Notation.}
    \begin{itemize}
    \item The protocol is described in terms of an $(N, k, d)$ code $\cC$ over the binary alphabet with $N = \frac{\secp}{2}$,
    %\amit{Shouldn't $N$ equal $\secp - |T| = \frac{\secp}{2}$ ?} 
    $k = \frac{\secp}{4}$ and
    $d = 2\sqrt{\secp}$. Let $\nc_\cC$ be the corresponding decoding algorithm.
    % \dakshita{this means that there are a total of $2^\frac{\secp}{4}$ codewords}
    . %\amit{Shouldn't the total number of codewords be $|\Sigma|^\frac{\secp}{4}$ where $\Sigma$ is the alphabet.} We let $\nc_\cC(\cdot)$ denote an algorithm that given a string $w$ outputs a nearest codeword to $w$.
    \item For classical bits $(x,\theta)$, let $\ket{x}_\theta$ denote $\ket{x}$ if $\theta = 0$, and $(\ket{0} + (-1)^x\ket{1})/\sqrt{2}$ if $\theta = 1$.
    % \item For polynomials $m = m(\secp), n = n(\secp)$, let $\com(\cdot) \rightarrow \zo^{3m} \times \zo^{3n}$ denote a 3-bit commitment scheme in the QROM. 
    \item Let $\comro: \zo^{\secp+1} \rightarrow \zo^{\secp+1}$, $\fsro:\zo^{3\secp(\secp+1)} \rightarrow {{\secp}\choose{\secp/2}}$ and $\maskro:\zo^{\secp} \rightarrow \zo^\secp$ denote random oracles. For $n = n(\secp) = 3\secp$, let $(\Com^{\comro},\allowbreak\Open^{\comro},\allowbreak\Rec^{\comro})$ denote a non-interactive extractable and equivocal commitment scheme in the QROM (\cref{sec:uccomm}).
    \end{itemize}
    
    {\bf Receiver Input:} Choice bit b.
    %Let $h:\zo^{3\secp/2} \rightarrow \zo^{\secp}$ denote a pairwise independent hash function. 
    
    
    
    \begin{enumerate}
    \item {\bf Sender Message.}
    $\sendr$ samples strings $x \leftarrow \zo^{\secp},x' \leftarrow \zo^{\secp}$, and a random subset $U \subset [\secp]$ of size $\sqrt{\secp}$, and for $i \in U$, it samples $b_i \leftarrow \zo$ uniformly at random.
    It computes state $\ket{\psi} = \ket{\psi}_1, \ldots, \ket{\psi}_\secp$ as follows. 
    For $i \in U$, $\ket{\psi}_i = (\ket{x_i}_{b_i}, \ket{x'_i}_{b_i})$ and for $i \in [\secp] \setminus U$, $\ket{\psi}_i = (\ket{x_i}_{0}, \ket{x'_i}_{1})$.
    
    \item {\bf Receiver Message.} $\recv$ does the following.
    \begin{itemize}
    \item Choose $\widehat{\theta} \leftarrow \zo^{\secp}$ and measure the $i^{th}$ pair of qubits in basis $\widehat{\theta}_i$ to obtain $\widehat{x}_i, \widehat{x'_i}$.
    %\footnote{We stress that for $i \in [\secp]$, the $i^{th}$ qubits of both $\widehat{x}$ and $\widehat{x'}$ must be measured in an identical basis.}.
    
    \item {\bf Measurement Check Message.} 
        \begin{itemize}
            \item Compute $c = c_1|| \ldots ||c_\secp$ for $(\{c_i\}_{i \in [n]}, \mathsf{st}) = \Com^{\comro}(\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i\}_{i \in [\secp]})$.
            \item Set $T = \fsro(c)$, as a subset of $[\secp]$ of size $\secp/2$,
            %\item 
            %For $T' = \{\text{indices of }\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i\}_{i \in T} \text{ in }\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i\}_{i \in [\secp]}\}$, \dakshita{Why isn't $T'$ just the same as $T$? $T$ is defined to be a set of indices in $[\secp]$. Also "indices of" is not clear terminology.}
            and  $\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i,\state_i\}_{i \in T} \leftarrow \Open^{\comro}(\state,T)$.
            \item Send $c, T, \{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i,\state_i\}_{i \in T}$ to $\sendr$.
            % \{(x_i, \widehat{x}_i, \widehat{\theta}_i, \mathsf{st}_i) \}_{i \in T}$ to $\sendr$.
        \end{itemize}
    
    \item
    {\bf Reorientation Message.} Let $\overline{T} = [\secp] \setminus T$, $S_0 = \{ i \in \overline{T} \text{ s.t. } \widehat{\theta}_i = 0 \}$ and $S_1 = \{ i \in \overline{T} \text{ s.t. } \widehat{\theta}_i = 1 \}$.
    Set $I_b = S_0$ and $I_{1-b} = S_1$. Sample $z_0 \leftarrow \zo^\secp, z_{1} \leftarrow \zo^\secp$  and send $(I_0,I_1,z_0,z_1)$ to $\sendr$. 
    
    %\item {\bf Output masks} Sample  and send $(z_0,z_1)$ to $\sendr$
    
    \item {\bf Receiver Output.}
    For all $i \in S_0$, set $m_i = \widehat{x_i}$ and for all $i \in S_1$, set $m_i = \widehat{x'_i}$. Output $\maskro(\nc_{\cC}(\{{m}_i\}_{i \in \overline{T}})) \oplus z_b$.
    \end{itemize}
    
    \item {\bf Sender Output.} 
    % $\sendr$ obtains $c, T, \{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i, \mathsf{st}_i \}_{i \in T}, (I_0, I_1), (z_0,z_1)$.
    $\sendr$ obtains $c, T, \{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i,\state_i\}_{i \in T}, (I_0, I_1), (z_0,z_1)$.
    \begin{itemize}
    \item {\bf Check Receiver Message.} $\sendr$ aborts if any of these checks fail:
    \begin{itemize}
    \item Check that $T = \fsro(c)$.
    \item If  $w \leftarrow \Rec^{\comro}(c,\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i,\state_i\}_{i \in T})$, check that $w \neq \bot$. Parse $w$ as $\{\widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i\}_{i \in T}$.
    % for every $i \in T$, check that $\decom(c_i, \widehat{x}_i, \widehat{x'_i}, \widehat{\theta}_i, \mathsf{st}_i) = 1$.
    \item For every $i \in T \cap U$ such that $b_i = \widehat{\theta}_i$, check that
    $\widehat{x}_i = x_i$ and $\widehat{x'_i} = x'_i$.
    %$\widehat{x}_i = \widehat{x'_i}$.
    %\item For every $i$ , check that $\widehat{x}_i = x_i$. \nishant{this should be when $b_i = \widehat{\theta}_i$, }.
    %\dakshita{this and the previous bullet together should imply what you need?}
    %\amit{Should only check if $b_i$ equals $\widehat{\theta_i}$}
    
    \end{itemize}
    
    \item {\bf Compute Sender Output.} For all $i \in I_0$, set
    $m^0_i = x_i, m^1_i = x'_i$, and for all $i \in I_1$, set $m^0_i = x'_i, m^1_i = x_i$.
    Output 
    $y_0 = z_0 \oplus \maskro(\nc_{\cC}(\{m^0_i\}_{i \in \overline{T}}))$, $y_1 = z_1 \oplus \maskro(\nc_{\cC}(\{m^1_i\}_{i \in \overline{T}}))$.
    \end{itemize}
    \end{enumerate}
         \end{framed}
        \caption{Two Round Quantum chosen-receiver, random-sender string OT}
        \label{fig:qot-3r-bb84}
    \end{figure}







    \begin{figure}[ht!]
          \begin{framed}
    
    
    For classical bits $(x,\theta)$, let $\ket{x}_\theta$ denote $\ket{x}$ if $\theta = 0$, and $(\ket{0} + (-1)^x\ket{1})/\sqrt{2}$ if $\theta = 1$. 
    
    %\begin{tabular}{ l l }
    {\bf Sender $\sendr$ input:} Bits $m_0,m_1 \in \zo$. 
    {\bf Receiver $\recv$ input:} Choice bit $b \in \zo$. \\
    \amit{Decide the paramters for $|U|, |V|, |W|$ etc}
    % \textbf{Sender $S$ Output:} $\perp$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
    %\end{tabular}
    
    
    \begin{enumerate}
    \item {\bf Sender message.}
    $\sendr$ samples $2n$ random bits $\{ r_0^i, r_1^i \}_{i \in [n]}$ and a random subset $U \subseteq [n]$. Then it prepares $2n$ qubits $\{R_0^i, R_1^i \}_{i \in [n]}$ in the following way. For all $i \in [n]:$
    
    \begin{enumerate}
        \item For all $i \in U$, sample $b^\mathsf{plant}_i \leftarrow \{+, \times \}$. Then encode $r_0^i$ and $r_1^i$ in the basis $b^\mathsf{plant}_i$ as $R_0^i$ and $R_1^i$ respectively. Formally, if $b^\mathsf{plant}_i$ is $+$, then set $R_0^i := \ket{r_0^i}$ and $R_1^i := \ket{r_1^i}$. Otherwise, set $R_0^i := H \ket{r_0^i}$ and $R_1^i := H \ket{r_1^i}$.
        
        \item For all $i \notin U$, encode $r_0^i$ in the computational basis as $R_0^i$ and $r_1^i$ in the hadamard basis as $R_1^i$. Formally, set $R_0^i := \ket{r_0^i}$ and $R_1^i := H \ket{r_1^i}$.
        
    %    \item Encode $r_0^i$ in computational basis as $R_0^i$. Formally, set $R_0^i := \ket{r_0^i}$.
        
     %   \item If $i \in U$, encode $r_1^i$ in the computational basis as $R_1^i$, i.e. set $R_1^i := \ket{r_1^i}$. Otherwise, encode $r_1^i$ in the hadamard basis as $R_1^i$, i.e. set $R_1^i := H \ket{r_1^i}$
        
    \end{enumerate}
    
    It sends $\{R_0^i, R_1^i \}_{i \in [n]}$ to the receiver.
    
    
    \item {\bf Receiver message.} $\recv$ samples $\{b_i\}_{i \in [n]}$ where $b_i \leftarrow \{+, \times \}$. For all $i \in [n]$, it measures $R_0^i, R_1^i$ in the basis $b_i$ to obtain measurement outcome $\widetilde{r_0}^i, \widetilde{r_1}^i$. Now it creates a measurement check proof $\pi_{\mathsf{measure}}$ in the following way.
    
    \begin{enumerate}
        \item Commit: Generate $\{c_0^i, c_1^i, c_\mathsf{basis}^i\}_{i \in [n]}$, where $c_0^i \gets \Com(\widetilde{r_0}^i; s_0^i)$, $c_1^i \leftarrow \Com(\widetilde{r_1}^i; s_1^i)$ and $c_\mathsf{basis}^i \leftarrow \Com(b_i; s_\mathsf{basis}^i)$
        
        \item Challenge: Compute $T \leftarrow \fsro ( \{ c_0^i, c_1^i, c_\mathsf{basis}^i \}_{i \in [n]})$ where $T$ is implicitly parsed as a subset of $[n]$.
        
        \item Response: Set $\pi_{\mathsf{measure}} := \{c_0^i, c_1^i, c_\mathsf{basis}^i\}_{i \in [n]}, T, \{\widetilde{r_0}^i, s_0^i, \widetilde{r_1}^i, s_1^i, b_i, s_\mathsf{basis}^i \}_{i \in T}$
    \end{enumerate}
    
    $\recv$ also computes the re-orientation bits $\{ b^i_\mathsf{orient} \}_{i \in \overline{T}}$ where $b^i_\mathsf{orient} := b \oplus b_i$ and $\overline{T} := [n] \setminus T$. It then sends $\pi_{\mathsf{measure}}, \{ b^i_\mathsf{orient} \}_{i \in \overline{T}}$ to $\sendr$.
    
    \item {\bf Sender Message.} $\sendr$ performs the following two checks on the receiver message:
    
    \begin{enumerate}
        \item Opening check: For all $i \in T$, check whether $(\widetilde{r_0}^i, s_0^i), (\widetilde{r_1}^i, s_1^i), (b_i, s_\mathsf{basis}^i)$ correspond to valid openings for the commitments $c_0^i, c_1^i, c_\mathsf{basis}^i$ respectively. 
        
        \amit{Also check whether all $b_i$ are either $+$ or $\times$}
        
        \item Measurement check: Let $V := \{ i | i \in T \cap U, b_i = b_i^\mathsf{plant} \}$. Check whether the following condition is true:    $\forall i \in V, \widetilde{r_0}^i = r_0^i \wedge \widetilde{r_1}^i = r_1^i$
    \end{enumerate}
    
    If any of the above check fails, then abort. Otherwise, perform the following for all $i \in W$, where $W := [n] \setminus (T \cup U)$:
    
    \begin{enumerate}
            
        \item Re-orientation: If $b^i_\mathsf{orient} = 0$, set $(\widehat{r_0}^i, \widehat{r_1}^i) := (r_0^i, r_1^i)$. Otherwise, set $(\widehat{r_0}^i, \widehat{r_1}^i) := (r_1^i, r_0^i)$.
        
        \item Combine: Set $r_0^\mathsf{final}:= \bigoplus_{i \in W} \widehat{r_0}^i$ and $r_1^\mathsf{final} := \bigoplus_{i \in W} \widehat{r_1}^i$.
    
        
    \end{enumerate}
    
    Now, $\sendr$ encodes its message $m_0, m_1$ in the following way: 
    
    \begin{enumerate}
        \item Set $ct_0 := m_0 \oplus r_0^\mathsf{final}$
        
        \item Set $ct_1 := m_1 \oplus r_1^\mathsf{final}$
    \end{enumerate}  
    
    It sends $ct_0, ct_1, W$ to $\recv$.
    
    \item {\bf Receiver Output.} $\recv$ computes $\widetilde{r_b}^\mathsf{final} := \oplus_{i \in W} \widetilde{r_{b_i}}^i$. It then outputs $\widetilde{m_b} := m_b \oplus \widetilde{r_b}^\mathsf{final}$
    
    
    \end{enumerate}
          \end{framed}
        \caption{Three Round chosen-input Quantum OT Protocol \nishant{Is this protocol doing something new?}}
        \label{fig:3-round-ot}
    \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%       NON EPR version string OT (with error correction)
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{figure}[ht!]
          \begin{framed}
    
    
    %\begin{tabular}{ l l }
    {\bf Sender $\sendr$ input:} Messages $m_0,m_1 \in \zo^\secp$. 
    {\bf Receiver $\recv$ input:} Choice bit $b \in \zo$. \\
    
    {\bf Public input:} Parameters $n = \secp$, $|U| = \frac{\secp}{10}$, $|T| = \frac{\secp}{10}$. Code $\cC$ of block length $n - |T| = \frac{9\secp}{10}$, alphabet $\{0, 1\}$, distance $2 |U| = \frac{\secp}{5}$, efficient encoding algorithm $E$, efficient decoding algorithm $D$. We can set $k$ using the singleton bound i.e. $k$ = Code block length - Distance + 1 = $\frac{9\secp}{10} - \frac{\secp}{5} + 1 = \frac{}{}$. Reed Solomon code s
    
    \amit{Check the parameters and code}
    
    % \textbf{Sender $S$ Output:} $\perp$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
    %\end{tabular}
    
    
    \begin{enumerate}
    \item {\bf Sender message.}
    $\sendr$ samples $2n$ random bits $\{ r_0^i, r_1^i \}_{i \in [n]}$ and a random subset $U \subseteq [n]$. Then it prepares $2n$ qubits $\{R_0^i, R_1^i \}_{i \in [n]}$ in the following way. For all $i \in [n]:$
    
    \begin{enumerate}
        \item For all $i \in U$, sample $b^\mathsf{plant}_i \leftarrow \{+, \times \}$. Then encode $r_0^i$ and $r_1^i$ in the basis $b^\mathsf{plant}_i$ as $R_0^i$ and $R_1^i$ respectively. Formally, if $b^\mathsf{plant}_i$ is $+$, then set $R_0^i := \ket{r_0^i}$ and $R_1^i := \ket{r_1^i}$. Otherwise, set $R_0^i := H \ket{r_0^i}$ and $R_1^i := H \ket{r_1^i}$.
        
        \item For all $i \notin U$, encode $r_0^i$ in the computational basis as $R_0^i$ and $r_1^i$ in the hadamard basis as $R_1^i$. Formally, set $R_0^i := \ket{r_0^i}$ and $R_1^i := H \ket{r_1^i}$.
        
    %    \item Encode $r_0^i$ in computational basis as $R_0^i$. Formally, set $R_0^i := \ket{r_0^i}$.
        
     %   \item If $i \in U$, encode $r_1^i$ in the computational basis as $R_1^i$, i.e. set $R_1^i := \ket{r_1^i}$. Otherwise, encode $r_1^i$ in the hadamard basis as $R_1^i$, i.e. set $R_1^i := H \ket{r_1^i}$
        
    \end{enumerate}
    
    It sends $\{R_0^i, R_1^i \}_{i \in [n]}$ to the receiver.
    
    
    \item {\bf Receiver message.} $\recv$ samples $\{b_i\}_{i \in [n]}$ where $b_i \leftarrow \{+, \times \}$. For all $i \in [n]$, it measures $R_0^i, R_1^i$ in the basis $b_i$ to obtain measurement outcome $\widetilde{r_0}^i, \widetilde{r_1}^i$. Now it creates a measurement check proof $\pi_{\mathsf{measure}}$ in the following way.
    
    \begin{enumerate}
        \item Commit: Generate $\{c_0^i, c_1^i, c_\mathsf{basis}^i\}_{i \in [n]}$, where $c_0^i \gets \Com(\widetilde{r_0}^i; s_0^i)$, $c_1^i \leftarrow \Com(\widetilde{r_1}^i; s_1^i)$ and $c_\mathsf{basis}^i \leftarrow \Com(b_i; s_\mathsf{basis}^i)$
        
        \item Challenge: Compute $T \leftarrow \fsro ( \{ c_0^i, c_1^i, c_\mathsf{basis}^i \}_{i \in [n]})$ where $T$ is implicitly parsed as a subset of $[n]$.
        
        \item Response: Set $\pi_{\mathsf{measure}} := \{c_0^i, c_1^i, c_\mathsf{basis}^i\}_{i \in [n]}, T, \{\widetilde{r_0}^i, s_0^i, \widetilde{r_1}^i, s_1^i, b_i, s_\mathsf{basis}^i \}_{i \in T}$
    \end{enumerate}
    
    $\recv$ also computes the re-orientation bits $\{ b^i_\mathsf{orient} \}_{i \in \overline{T}}$ where $b^i_\mathsf{orient} := b \oplus b_i$ and $\overline{T} := [n] \setminus T$. It then sends $\pi_{\mathsf{measure}}, \{ b^i_\mathsf{orient} \}_{i \in \overline{T}}$ to $\sendr$.
    
    \item {\bf Sender Message.} $\sendr$ performs the following two checks on the receiver message:
    
    \begin{enumerate}
        \item Opening check: For all $i \in T$, check whether $(\widetilde{r_0}^i, s_0^i), (\widetilde{r_1}^i, s_1^i), (b_i, s_\mathsf{basis}^i)$ correspond to valid openings for the commitments $c_0^i, c_1^i, c_\mathsf{basis}^i$ respectively. 
        
        \amit{Also check whether all $b_i$ are either $+$ or $\times$}
        
        \item Measurement check: Let $V := \{ i | i \in T \cap U, b_i = b_i^\mathsf{plant} \}$. Check whether the following condition is true:    $\forall i \in V, \widetilde{r_0}^i = r_0^i \wedge \widetilde{r_1}^i = r_1^i$
    \end{enumerate}
    
    If any of the above check fails, then abort. Otherwise, perform the following for all $i \in \overline{T}$, where $\overline{T} := [n] \setminus T$:
    
    \begin{enumerate}
        
        \item Re-orientation: If $b^i_\mathsf{orient} = 0$, set $(\widehat{r_0}^i, \widehat{r_1}^i) := (r_0^i, r_1^i)$. Otherwise, set $(\widehat{r_0}^i, \widehat{r_1}^i) := (r_1^i, r_0^i)$.
    
    
        \item Combine: Set $\widehat{r_0} := ||_{i \in \overline{T}} \widehat{r_0}^i$ and $\widehat{r_1} := ||_{i \in \overline{T}} \widehat{r_1}^i$. Compute $\widehat{r_0}^\mathsf{corrected}$ and $\widehat{r_1}^\mathsf{corrected}$ by finding the nearest codewords of $\widehat{r_0}$ and $\widehat{r_1}$ respectively. Formally, $\widehat{r_0}^\mathsf{corrected} : E(D(\widehat{r_0}))$ and $\widehat{r_1}^\mathsf{corrected} := E(D(\widehat{r_1}))$. Then, set $r_0^\mathsf{final} := \maskro(\widehat{r_0}^\mathsf{corrected})$ and $r_1^\mathsf{final} := \maskro(\widehat{r_1}^\mathsf{corrected})$.
        
    \end{enumerate}
    
    Now, $\sendr$ encodes its message $m_0, m_1$ in the following way: Set $ct_0 := m_0 \oplus r_0^\mathsf{final}$ and $ct_1 := m_1 \oplus r_1^\mathsf{final}$. It sends $ct_0, ct_1$ to $\recv$.
    
    \item {\bf Receiver Output.} $\recv$ computes $\widetilde{r_b}^\mathsf{final} := \oplus_{i \in \overline{T}} \widetilde{r_{b_i}}^i$. It then outputs $\widetilde{m_b} := m_b \oplus \widetilde{r_b}^\mathsf{final}$
    
    
    \end{enumerate}
          \end{framed}
        \caption{Three Round chosen-input Quantum OT Protocol}
        \label{fig:3-round-ot}
    \end{figure}
}\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse{
        %old sampling strategy
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %
        %
        %       Sender security
        %
        %
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \noindent\underline{\textbf{Sender security}}
        
        Let $\SimExt = (\SimExt.\RO,\SimExt.\Ext)$ be the simulator for the extractable commitment scheme from \cref{sec:uccomm}. Let $+$ refer to the computational basis and $\times$ to the hadamard basis \nishant{do we need to define this?}. Below we describe the simulator $\Sim[\sR^*]$ against a malicious receiver $\sR^*$ for \proref{fig:qot-3r-bb84}\nishant{these figures don't have protocol number in them ; fix later at all places}.
        
        \underline{$\Sim[\sR^*](\brho)$}:
        \begin{itemize}
            \item Initialize the on-the-fly random oracle simulator $\simro$ from \cref{impthm:extROSim}. Run $\sR^*(\brho)$ answering its oracle queries to $\fsro$ using $\simro$ and queries to $\comro$ using $\SimExt.\RO$.
            \item Sample $2n$ EPR pairs on registers $\{(\cE_{i,b,S},\cE_{i,b,R})\}_{i \in [n], b \in \zo}$ and send registers $\{\cE_{i,b,R}\}_{i \in [n],b \in \zo}$ to $\sR^*$. 
            \item When $\sR^*$ outputs $\{c_i\}_{i \in [n]}, T, \{(\widehat{r_i}^0, \widehat{r_i}^1, \widehat{\theta}_i)\}_{i \in T}, \{d_i\}_{i \in \overline{T}}$, then run $\{(\widetilde{r_{i}}^0,\widetilde{r_{i}}^{1},\widetilde{\theta}_i)\}_{i \in [n]} \leftarrow \SimExt.\Ext(\{c_i\}_{i \in [n]})$. 
            \item Run the ``check receiver message" part of the honest sender strategy, except do the following in place of the third check:
                \begin{itemize}
                    \item Sample subset $U \subset [n]$ of size $d$ and for each $i \in [n]$, sample bit $b_i \in \zo$. 
                    \item For each $i \in [n]$, do the following: 
                        \begin{itemize}
                            \item If $i \in U$, measure registers $\cE_{i,0,S}$ and $\cE_{i,1,S}$ in basis $+$ if $b_i = 0$, or else in basis $\times$ if $b_i = 1$, to get measurement outcomes $r_i^0$ and $r_i^1$ respectively. 
                            \item If $i \notin U$, then measure $\cE_{i,0,S}$ in basis $+$ and $\cE_{i,1,S}$ in basis $\times$ to get outcomes $r_i^0,r_i^1$ respectively. 
                        \end{itemize}
                    \item For each $i \in T\cap U$ such that $\widetilde{\theta}_i = b_i$, check that $\widetilde{r_i}^0 = r_i^0$ and $\widetilde{r_i}^1 = r_i^1$.
                \end{itemize}
            \item Set $b \coloneqq \maj(\{\widetilde{\theta}_i \oplus d_i\}_{ i\in \overline{T}\setminus U})$ and send $b$ to $\cF_{\OT[\secp]}$ to receive back $m_b$.
            \item Compute the last message using the honest sender strategy except for using $m_{1-b} \coloneqq 0^\secp$. 
            \item Run $\sR^*$ on this last message, output its state and terminate.
            \item Answer queries of distinguisher to $\fsro$ and $\comro$ using $\simro$ and $\SimExt.\RO$ respectively.
        \end{itemize}
        Let $(\sD,\bsigma)$ be a distinguisher s.t.\ $\sR^*,\sD$ make a total of $q$ queries to $\fsro$ and $\comro$. Consider the following sequence of hybrids:
        \begin{itemize}
            \item $\Hyb_0$: This is the real world interaction between $\sR^*$ and $\sS$. Using the notation of \cref{def:secure-realization}, this is a distribution over $\zo$ denoted by $\Pi[\brho,\bsigma,\sR^*,\sD,(m_0,m_1)]$.
            \item $\Hyb_1$: This is the same as the previous hybrid, except the following are run instead to generate the first sender message: (1) Sample $2n$ EPR pairs on registers $\{(\cE_{i,b,S},\cE_{i,b,R})\}_{i \in [n], b \in \zo}$. (2) Run the following algorithm: 
            
                \underline{\textbf{Algorithm Measure-EPR}}:
                \begin{itemize}
                    \item Sample subset $U \subset [n]$ of size $d$ and for each $i \in [n]$, sample bit $b_i \in \zo$. 
                    \item For each $i \in [n]$, do the following: 
                        \begin{itemize}
                            \item If $i \in U$, measure registers $\cE_{i,0,S}$ and $\cE_{i,1,S}$ in basis $+$ if $b_i = 0$, or else in basis $\times$ if $b_i = 1$, to get outcomes $r_i^0$ and $r_i^1$ respectively. 
                            \item If $i \notin U$, then measure $\cE_{i,0,S}$ in basis $+$ and $\cE_{i,1,S}$ in basis $\times$ to get outcomes $r_i^0,r_i^1$ respectively. 
                        \end{itemize}
                \end{itemize}
            Thereafter, registers $\{\cE_{i,b,R}\}_{i \in [n],b \in \zo}$ are sent over to $\sR^*$ and the rest of the experiment works as the previous hybrid.
            \item $\Hyb_2$: This is the same previous hybrid, except that the sender delays running the algorithm Measure-EPR to just before executing the third check in ``check receiver message" part of the honest sender strategy.
            \item $\Hyb_3$: This is the same as the previous hybrid, except for the following changes: queries of $\sR^*$ to $\comro$ are now answered using $\SimExt.\RO$. Once $\sR^*$ outputs its second message, the following is run: $\{(\widetilde{r_{i}}^0,\widetilde{r_{i}}^1,\widetilde{\theta}_i)\}_{i \in [n]} \leftarrow \SimExt.\Ext(\{c_i\}_{i \in [n]})$. Thereafter, $\{(\widetilde{r_i}^0,\widetilde{r_i}^1,\widetilde{\theta}_i)\}_{i \in T}$ are used for the third check in the ``check receiver part" of the honest sender strategy.
            \item $\Hyb_4$: This is the result of the interaction between $\Sim[\sR^*]$, $\cF_{\OT[\secp]}$ and honest sender $\sS$. Using the notation of \cref{def:secure-realization}, this is denoted by $\widetilde{\Pi}_{\cF_{\OT[\secp]}}[\brho,\bsigma,\Sim[\sR^*],\sD,(m_0,m_1)]$.
        \end{itemize}
        We prove the indistinguishability between the hybrids using the following claims:
        \begin{claim} $\Pr[\Hyb_0=1] = \Pr[\Hyb_1=1]$
        \end{claim}
        \begin{proof}
            This follows from elementary properties of EPR pairs. In either hybrid, the distribution of the states sent from sender to receiver is a completely mixed state. \nishant{elaborate more}
        \end{proof}
        \begin{claim} $\Pr[\Hyb_1=1] = \Pr[\Hyb_2=1]$
        \end{claim}
        \begin{proof}
            This also follows using elementary properties of quantum mechanics, i.e.\ that the measurements on different sub-systems commute. \nishant{todo elaborate more}
        \end{proof}
        \begin{claim} Under the constraints that $148(q+3(A+B)\secp+1)^3+1 \leq 2^{3\secp}, 8qn \leq 2^\secp$, we have, 
        \[
            |\Pr[\Hyb_2=1] - \Pr[\Hyb_3=1]| \leq \frac{2}{2^\secp}.
        \]
        \end{claim}
        \begin{proof}
            This follows by a reduction to the \nishant{todo} with error $\frac{148(q+3n+1)^3+1}{2^{\secp_\com}} + \frac{8qn}{2^{\secp_\com/2}}$.
            Setting $\secp_\com = 4\secp$ and assuming $148(q+3(A+B)\secp+1)^3+1 \leq 2^{3\secp}, 8qn \leq 2^\secp$, we get, $\frac{2}{2^\secp}$. \nishant{perhaps not updated in the other place}
        \end{proof}
        \begin{claim}
        \label{claim:qot-3r-bb84-hyb34}
        For $A=10^6,B=8\times 10^5,C=5\times 10^4$ and $q\geq 5$,
        \begin{align*}
            % |\Pr[\Hyb_3=1] - \Pr[\Hyb_4=1]| \leq &\sqrt{2}(2q+1)\left(\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}}\right)^{1/2} \\ &+ 2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
            |\Pr[\Hyb_3=1] - \Pr[\Hyb_4=1]| \leq \frac{3\sqrt{10}q^{3/2}}{2^{\secp}}
        \end{align*}
        \end{claim}
        \begin{proof}
        The only difference between $\Hyb_3$ and $\Hyb_4$ is that $m_{1-b} = 0^\secp$, where $b = \maj(\{\widetilde{\theta}_i \oplus d_i\}_{i \in \overline{T}})$. Intuitively we show that the mask of $m_{1-b}$ is a uniformly random string from the point of view of $\sR^*$ in either hybrid, which would imply the given claim. 
        \fflater{\nishant{There }}
        \paragraph{Notation:} We setup some notation before proceeding.
        \begin{itemize}
        \item Let $\bc \coloneqq (c_1,\dots,c_n)$ be the classical commitments and $\bb \coloneqq (b_1,\dots b_n)$ be the bits sampled by the sender while executing its checks.
        \nishant{there is a small notational inconsistency here between $\bb_i$ vs $b_i$}
        \item Write the classical extracted values $\{(\widetilde{r_i}^0,\widetilde{r_i}^1,\widetilde{\theta}_i)\}_{i \in [n]}$ as matrices
        \[
            \widetilde{\bR} \coloneqq \begin{bmatrix}\widetilde{r_1}^0 \ \dots \ \widetilde{r_n}^0 \\ \widetilde{r_1}^1 \ \dots \ \widetilde{r_n}^1\end{bmatrix}, 
            \widetilde{\btheta} \coloneqq \begin{bmatrix}\widetilde{\theta}_{1} \ \dots \ \widetilde{\theta}_{n} 
            % \\ \widetilde{\theta}_{1} \ \dots \ \widetilde{\theta}_n
            \end{bmatrix}.
        \]
        \item Given any $\bR \in \{0,1\}^{2 \times n}$, $\btheta \in \zo^n$, define $\ket{\bR_{\btheta}}$ as a state on $n$ $4$-dimensional registers, where register $i$ contains the state \nishant{ch} $\ket{\bR_{i,0},\bR_{i,1}}$ prepared in the $(\btheta_{i},\btheta_{i})$-basis. \nishant{define what this means}
        \item Given $\bR,\widetilde{\bR} \in \{0,1\}^{2 \times n}$ and a subset $T \subseteq [n]$, define $\bR_T$ be the columns of $\bR$ indexed by $T$, and define $\Delta\left(\bR_T,\widetilde{\bR}_{T}\right)$ as the fraction of columns $i \in T$ such that $(\bR_{i,0},\bR_{i,1}) \neq (\widetilde{\bR}_{i,0},\widetilde{\bR}_{i,1})$.
        \item For $T \subset [n]$, let $\overline{T} \coloneqq [n] \setminus T$.
        \item Given $\widetilde{\bR} \in \{0,1\}^{2 \times n}, \widetilde{\btheta} \in \zo^n$, $T \subseteq [n]$, $U \subseteq [n]$, $\bb \in \zo^n$, and $\delta \in (0,1)$, define
        \[
            \Pi^{\widetilde{\bR},\widetilde{\btheta},T,U,\bb,\delta} \coloneqq \sum_{\substack{\bR \, : \, \bR_{S'} = \widetilde{\bR}_{S'}, \Delta\left(\bR_{\overline{T}}, \widetilde{\bR}_{\overline{T}}\right) \geq \delta\\\text{where }S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_{j}\}}}\ket{\bR_{\widetilde{\btheta}}}\bra{\bR_{\widetilde{\btheta}}}.
        \]
    \end{itemize}
    
    \noindent Now, consider the following projection, which has hard-coded the description of $\fsro$:
    
    \[
        \Pi_{\mathsf{bad}}^\delta \coloneqq \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb,\\U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \Pi^{\widetilde{\bR},\widetilde{\btheta},\fsro(\bc),U,\bb,\delta}_{\cS},
    \]
    where $\cC$ is the register holding the classical commitments, $\cZ_1$ is the register holding the output of $\SimExt.\Ext$, $\cZ_2$ is the register holding the subset $U$ and bits $\bb$ sampled by sender, and $\cS$ is the register holding the sender's halves of EPR pairs.
    
    \begin{subclaim}\label{subclaim:tau}
    Let 
    \[
        \tau \coloneqq \sum_{\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb}p^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)} \tau^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)},
    \] 
    where 
    \[
        \tau^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)} = \ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)}_{\cS,\cX}
    \] 
    is the entire state of $\Hyb_3$ right after $\rcv^*$ outputs its message (which includes $\bc$), $\SimExt.\Ext$ is run to get $\widetilde{\bR},\widetilde{\btheta}$, and sender samples the set $U \subseteq [n]$ of size $d$ and bits $\bb \in \zo^n$. Here, each $p^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)}$ is the probability that the string $\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb$ is contained in the registers $\cC,\cZ_1,\cZ_2$. Also, $\cS$ is the register holding the sender's halves of EPR pairs and $\cX$ is a register holding remaining state of the system, which includes the rest of the receiver's classical message and its private state. Then, for $A=10^6,B=8\times 10^5,C=5\times 10^4$ and for $q\geq 5$,
    \[
        % \Tr(\Pi_{\mathsf{bad}}^{\delta} \tau) \leq (2q+1)^2 \left[\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}} \right].
        \Tr(\Pi_{\mathsf{bad}}^{19/200} \tau) \leq \frac{45q^3}{2^{2\secp}}
    \]
    \end{subclaim}
    \begin{proof}
    Define $\Adv_{\rcv^*}^{\fsro}$ to be the oracle machine that runs $\Hyb_3$ until $\rcv^*$ outputs $\bc$ (and the rest of its message), then runs $\SimExt.\Ext$ to obtain $\ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}$, followed by sampling the set $U \subseteq [n]$ of size $d$, and bits $\bb \in \zo^n$ in the register $\cZ_2$, and finally outputting the remaining state $\rho_{\cS,\cX}$. Consider running the measure-and-reprogram simulator $\Sim[\Adv_{\rcv^*}]$ from \cref{thm:measure-and-reprogram}, which simulates $\fsro$ queries, measures and outputs $\bc$, then receives a uniformly random subset $T \subset [n]$ of size $k$, and then continues to run $\Adv_{\rcv^*}$ until it outputs $\ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}$. Letting 
    \[
        \Pi_{\mathsf{bad}}^{\delta}[T] \coloneqq \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb \\ U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \Pi^{\widetilde{\bR},\widetilde{\btheta},T,U,\bb,\delta}_{\cS},
    \] for $T \subset [n]$, \cref{thm:measure-and-reprogram} implies that \begin{align*}
    &\Tr\left(\Pi_\mathsf{bad}^{\delta}\tau\right) \\ &\leq (2q+1)^2 \E\left[\Tr\left(\Pi_{\mathsf{bad}}^{\delta}[T]\left(\ket{\bc}\bra{\bc}_\cC \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}\otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}\right)\right): \begin{array}{r}(\bc,\state) \gets \Sim[\Adv_{\rcv^*}] \\ T \gets S_{n,k} \\ \left(\substack{\widetilde{\bR},\widetilde{\btheta},U,\\\bb,\rho_{\cS,\cX}}\right) \gets \Sim[\Adv_{\rcv^*}](T,\state)\end{array}\right],\end{align*} 
    where $S_{n,k}$ is the set of all subsets of $[n]$ of size $k$.
    
    Now, recall that one of the last things that $\Adv_{\rcv^*}$ does in $\Hyb_3$ is run $\SimExt.\Ext$ on $\bc$ to obtain $(\widetilde{\bR},\widetilde{\btheta})$. Consider instead running $\SimExt.\Ext$ on $\bc$ immediately after $\Sim[\Adv_{\rcv^*}]$ outputs $\bc$. Note that $\SimExt.\Ext$ only operates on the register holding $\bc$ and its own private state used for simulating $\comro$, so since $\Com^{\comro}$ \nishant{$\comro$} has a $\frac{8}{2^{{\secp_\com}/2}}$-commuting simulator (\cref{def:fextractable}), we have that, 
    
    \begin{align}
    \Tr\left(\Pi_\mathsf{bad}^{\delta}\tau\right) &\leq (2q+1)^2\left(\epsilon + \frac{8q}{2^{{\secp_\com}/2}}\right) \label{eq:taueq1}
    \end{align}
    % &\leq (2q+1)^2\left(\right) \\ 
    % &\coloneqq (2q+1)^2\left(\epsilon + \frac{8q}{2^{{\secp_\com}/2}}\right), \nonumber
    % \end{align}
    where 
    \[
        \epsilon \coloneqq \E\left[\Tr\left(\Pi_{\mathsf{bad}}^{\delta}[T]\left(\ket{\bc}\bra{\bc}_\cC  \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}\otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}\right)\right): \begin{array}{r}(\bc,\state) \gets \Sim[\Adv_{\rcv^*}] \\ (\widetilde{\bR},\widetilde{\btheta}) \gets \SimExt.\Ext(\bc) \\ T \gets S_{n,k} \\ \left(\substack{\widetilde{\bR},\widetilde{\btheta},U,\\\bb,\rho_{\cS,\cX}}\right) \gets \Sim[\Adv_{\rcv^*}](T,\state)\end{array}\right].
    \]
    Now, consider the following quantum sampling game.
    
    \begin{itemize}
        \item Fix a state on register $\cS$ (and potentially other registers of arbitrary size), where $\cS$ is split into $n$ registers $\cS_1,\dots,\cS_n$ of dimension 4, and fix matrices $\widetilde{\bR}\in \{0,1\}^{2 \times n},\widetilde{\btheta} \in \zo^n$.
        \item Sample a uniformly random subset $T \subset [n]$ of size $k$.
        \item Sample a subset $S' \subseteq T$ \nishant{later at all places - $\subset$ vs $\subseteq$} as follows:    \begin{itemize}
            \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
            \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
        \end{itemize}
        \item For each $i \in S'$, measure the register $\cS_i$ in basis  $\widetilde{\btheta}_{i}$ to get $\bR_{S'} \in \zo^{2 \times |S'|}$. \nishant{sizeof} Output $\Delta(\bR_{S'},\widetilde{\bR}_{S'})$. 
        %as the estimate for the ``closeness''\footnote{The notion of closeness to a quantum state is not defined here, but is captured by the quantum error probability as defined in \cref{def:quantum-error-probability}.} of the state on registers $\cS_{\overline{T}}$ to $\ket{{\widetilde{\bR}_{\overline{T}}}_{\widetilde{\btheta}_{\overline{T}}}}$.
        
        
        %Register $\cE_S$, when written in the $\btheta^*$-basis, has non-zero amplitude on some string $\br$ such that $\br_{\widehat{T}} = \br^*_{\widehat{T}}$, but $\omega\left(\br_{\overline{\widehat{T}}} \oplus \br^*_{\overline{\widehat{T}}}\right) \geq \delta$.
    \end{itemize}
    
    \nishant{this can use some more explanation}
    The quantum error probability $\epsilon^{\delta}_{\mathsf{quantum}}$ (\cref{def:quantum-error-probability}) of the above game corresponds to the trace distance between the initial state on register $\cS$ and an ``ideal'' state (as defined in \cref{def:quantum-error-probability}). By definition of the above sampling game, for any $(T,\widetilde{\bR},\widetilde{\btheta})$, this ideal state is orthogonal to the subspace $\Pi^{\widetilde{\bR},\widetilde{\btheta},T,\delta}_\cS$ since for any vector $\ket{\bR_{\widetilde{\btheta}}}$ in the ideal state, if $\Delta(\bR_T,\widetilde{\bR}_T) = 0$, then $\Delta(\bR_{\overline{T}},\widetilde{\bR}_{\overline{T}}) < \delta$. Thus, noting that the trace inside the expectation defining $\epsilon$ would be 0 for any state orthogonal to this subspace, it follows that $\epsilon$ is bounded by $\epsilon^{\delta}_{\mathsf{quantum}}$.
    
    Thus, by \cref{impthm:error-probability}, $\epsilon$ is then bounded by $\sqrt{\epsilon^\delta_{\mathsf{classical}}}$, where $\epsilon^\delta_{\mathsf{classical}}$ is the \emph{classical} error probability (\cref{def:classical-error-probability}) in the following classical sampling game. \nishant{i think its better to say this just outputs $\widetilde{\delta}$}
    \begin{itemize}
        \item Let $\bR, \widetilde{\bR} \in \{0,1\}^{2 \times n}$ s.t.\ $\bR$ is the matrix on which we are running the sampling and $\widetilde{\bR}$ is an an arbitrary matrix.
        \item Sample a uniformly random subset $T \subset [n]$ of size $k$.
        \item Sample a subset $S' \subset T$ as follows: 
        \begin{itemize}
            \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
            \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
        \end{itemize}
        \item Output $\Delta(\bR_{S'},\widetilde{\bR}_{S'})$.
    \end{itemize}
    
    We analyze the classical error probability of the above game by looking at the same, but with sampling happening on a string $q \in \zo^n$ as follows:
    \paragraph{Analysis of the corresponding classical sampling strategy}
    For a string $\strq \in \zo^n$ and $S \subset [n]$, let $\strq_S = \{\strq_i \, | \, i \in S\}$. Consider the following classical sampling strategy to determine the relative hamming weight of a string $\strq \in \zo^n$.
    \begin{itemize}
        \item Choose a random subset $T \subset [n]$ of size $k$.
        \item Choose a subset $S' \subset T$ as follows: 
            \begin{itemize}
                \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
                \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
            \end{itemize}
        \item Output $\omega(\strq_{S'})$ as the estimate of the hamming weight of $\strq$.
    \end{itemize}
    This defines the corresponding classical sampling strategy, with $P_T$ as the distribution induced by sampling subset $T \subset [n]$ of size $k$ without replacement. $P_S$ is the distribution induced by sampling $S' \subset T$ as above, and $f(T,\strq_T,S') = \omega(\strq_{S'})$. We then prove the following for this classical sampling strategy:
    \begin{lemma}
        $\epsilon^\delta_{\mathsf{classical}} \leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) $ for $0 < \delta < 1$.
        % $\epsilon^\delta_{\mathsf{classical}} \leq
        % 9 \exp\left(-\frac{3\delta^2dk}{288n}\right)$ for $0 < \delta < 1$.
    \end{lemma}
    \begin{proof}
        Let $S = T \cap U$ in the above sampling strategy. We have,
        \begin{align*}
            \epsilon^\delta_{\mathsf{classical}} &= \max_\strq \Pr_{T \leftarrow P_T, S' \leftarrow P_S}\left[\strq \notin B_{T,S'}^\delta\right]\\
            &= \max_\strq \Pr_{T \leftarrow P_T, S' \leftarrow P_S}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right]\\
            &\leq \max_\strq \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{T})| + |\omega(\strq_{{T}}) - \omega(\strq_{S'})| \geq \delta\right]
        \end{align*}
        Considering the sampling of $T$ as a separate sampling strategy, we know from the analysis in \cite[Appendix B.1]{C:BouFeh10}, for $0 < \delta < 1$,
        \begin{align}
            \max_\strq \Pr_{T \leftarrow P_T, |T|=k} \left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{T})| \geq \delta \right] \leq 2\exp\left( - \frac{k\delta^2}{2} \right)
            \label{eq:classampTTbar}
        \end{align}
        We prove the following sub-claim:
        \begin{subclaim}
            For any given string $\strq$,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right] \leq 6\exp\left( -\frac{2\delta^2 s}{81} \right)
            \]
        \end{subclaim}
        \begin{proof}
            Note that $|\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \implies |\omega(\strq_T) - \omega(\strq_{S})| + |\omega(\strq_S) - \omega(\strq_{S'})| \geq |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta$ (using triangle inequality). Therefore,
            \begin{align}
                \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right] \leq \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S})| + |\omega(\strq_S) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right]
                \label{eq:classampeq1}
            \end{align}
            Given $|S| = |T \cap U| = s$, sampling $S'$ in the sampling game above is equivalent to first sampling a set $S \subset T$ of size $s$, then sampling $\theta \leftarrow \zo^{|S|}$ to define $S'$. Using Heoffding's inequality \nishant{add it - its tighter than chernoff}, for sampling $S \subset T$ of size $s$ at random without replacement, we have, for $\epsilon_1 > 0$,
            \begin{align*}
                \Pr_{S}\left[ |\omega(\strq_{T}) - \omega(\strq_S)| \geq \epsilon_1 \, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right)
            \end{align*}
            Also, since sampling of $S'$ from $S$ is equivalent to sampling a random subset of $S$, using \cite[Appendix B.2]{C:BouFeh10}, for $0 < \epsilon_2 < 1$, \nishant{this is not tight + if we get time, we should give a tighter analysis of even B.4} \nishant{todo - $S \setminus S'$}
            \begin{align*}
                &\Pr_{S'}\left[ |\omega(\strq_{S}) - \omega(\strq_{S'})| \geq \epsilon_2 \, \Big| \, |S|=s \right] \leq 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)\\
            % Noting that $|\omega(\strq_{S \setminus S'}) - \omega(\strq_{S'})| \geq \epsilon_2 \implies |\omega(\strq_{S}) - \omega(\strq_{S'})| =  \geq \epsilon_2$
                \implies &\Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_S)| \geq \epsilon_1 \wedge |\omega(\strq_{S}) - \omega(\strq_{S'})| \geq \epsilon_2 \, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)\\
                \implies &\Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq (\epsilon_1 + \epsilon_2)\, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right) \quad \text{(using \cref{eq:classampeq1})}
            \end{align*}
            Setting $\delta = \epsilon_1 + \epsilon_2$, we get,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \leq 2\exp\left(-2(\delta - \epsilon_2)^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)
            \]
            Setting $\epsilon_2 = \frac{8\delta}{9}$, we get the two exponents as equal to get,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \leq 6\exp\left(- \frac{2\delta^2 s}{81}\right)
            \]
        \end{proof}
        \begin{subclaim}
            \label{subclaim:classampTS}
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \right] \leq 7\exp\left(- \frac{0.019 \delta^2  d  k}{n}\right)
            \]
        \end{subclaim}
        \begin{proof}
            We do this by noting the distribution of $S = T \cap U$. We use a Chernoff Bound for sampling with replacement. Let $U$ be drawn with replacement after $T$ is sampled, and let for all $i \in [d], X_i = 1$ iff the $i^{th}$ draw lands in $T$. Then, $\Pr[X_i=1] = \frac{k}{n}$. Let $X = \sum_{i=0}^d X_i$. $\E[X] = \frac{kd}{n}$. Since $X_i$ are independently drawn binary random variables, we get using Chernoff bound, for $0 < \epsilon_3 < 1$,
            \begin{align*}
                \Pr[X \leq (1-\epsilon_3)\frac{dk}{n}] &\leq \exp\left( -\frac{\epsilon_3^2 dk}{2n} \right)\\
                \implies \Pr_{S}\left[ \, |S| \leq (1-\epsilon_3)\frac{dk}{n}\right] &\leq \exp\left( -\frac{\epsilon_3^2 dk}{2n} \right)
            \end{align*}
            Therefore, 
            \begin{align*}
                \Pr_{S,S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})|\geq \delta\right] &= \sum_{s \leq (1-\epsilon_3)\frac{dk}{n}} \Pr_{S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \Pr_S\left[|S|=s\right] \\
                &+ 
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} \Pr_{S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \Pr_S\left[|S|=s\right]\\
                % &\leq \Pr_{S}\left[ |S| \leq (1-\epsilon_3)\frac{dk}{n} \right] + \Pr_{S'}\left[\right]
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} 6\exp\left( - \frac{2\delta^2s}{81} \right) \Pr_S\left[|S|=s\right]\\
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} 6\exp\left( - \frac{2\delta^2(1-\epsilon_3)dk}{81n} \right) \Pr_S\left[|S|=s\right]\\
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                6\exp\left( - \frac{2\delta^2(1-\epsilon_3)dk}{81n} \right)\\
                % 6\exp\left(-\frac{2\delta^2}{s}\right)
            \end{align*}
            Setting $\epsilon_3 = \frac{\delta}{5}$, the two terms inside exp become $\frac{\delta^2dk}{50n}$ and $\frac{2\delta^2(5-\delta)dk}{405n}$. Upper bounding $\delta$ by $1$ in the latter, the two terms become $\frac{0.02\delta^2dk}{n}$ and $\approx\frac{0.01975\delta^2dk}{n}$. Lower bounding each term by $\frac{0.019\delta^2dk}{n}$, which upper bounds the negative exp term, we get,
            \begin{align*}
                \Pr_{S,S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})|\geq \delta\right] &\leq 7\exp\left( -\frac{0.019\delta^2dk}{n} \right)
            \end{align*}
        \end{proof}
        \noindent Combining \cref{eq:classampTTbar} with \cref{subclaim:classampTS}, we get,
        \begin{align*}
            \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta_1 + \delta_2 \right] &\leq 2\exp\left(-\frac{k\delta_1^2}{2}\right) + 7\exp\left(-\frac{0.019\delta_2^2dk}{n}\right)
        \end{align*}
        Setting $\delta = \delta_1+\delta_2$, we get,
        \begin{align*}
            \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] &\leq 2\exp\left(-\frac{k(\delta-\delta_2)^2}{2}\right) + 7\exp\left(-\frac{0.019\delta_2^2dk}{n}\right)
        \end{align*}
        Setting $\delta_2 = \frac{\delta}{\left(1 + \sqrt{0.038\frac{d}{n}}\right)}$ to get the two exp terms as equal, we get,
        \begin{align*}
            &\Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] \leq 9\exp\left(-\frac{0.019\delta^2dk}{\left(1 + \sqrt{\frac{0.038d}{n}}\right)^2n}\right)\leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)\\
            \implies &\epsilon^\delta_{\mathsf{classical}} \leq \max_\strq \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] \leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)
            % \implies &\epsilon^\delta_{\mathsf{classical}} \leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)
        \end{align*}
        proving the required subclaim.
        % where we used that\footnote{We note that our focus here is not to find the tightest parameters, but show that the values are practical.\nishant{to edit?}} $\frac{d}{n}\leq 1$.
    \end{proof}
    \noindent To finish the proof of \cref{subclaim:tau}, we get $\epsilon$ in \cref{eq:taueq1} is s.t.\
    \[
        \epsilon \leq \epsilon^\delta_{\mathsf{quantum}} \leq \sqrt{\epsilon^\delta_{\mathsf{classical}}} = 3\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)
        % \epsilon \leq \epsilon^\delta_{\mathsf{quantum}} \leq \sqrt{\epsilon^\delta_{\mathsf{classical}}} = 3\exp\left(-\frac{3\delta^2dk}{576n}\right)
    \]
    which gives using \cref{eq:taueq1} that:
    \[
        \Tr(\Pi_{\mathsf{bad}}^\delta \tau) \leq (2q+1)^2 \left[3\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}} \right]
    \]
    Substituting $\delta = 19/200, \secp_\com = 4\secp, k = B\secp, d = C\secp, n = (A+B)\secp$, where $A = 10^6, B = 8 \times 10^5, C = 5 \times 10^4$, we get,
    \[
        \Tr(\Pi_{\mathsf{bad}}^{19/200} \tau) \leq (2q+1)^2\left[\frac{3}{2^{2\secp}} + \frac{8q}{2^{2\secp}} \right]
    \]
    which for $q \geq 5$ implies $(2q+1)^2 \leq 5q^2$ and $8q+3 \leq 9q$, giving, 
    \[
        \Tr(\Pi_{\mathsf{bad}}^{19/200} \tau) \leq 
        \frac{45q^3}{2^{2\secp}}
    \]
    \end{proof}
    Thus, by gentle measurement (\cref{lemma:gentle-measurement}), the $\tau$ defined in \cref{subclaim:tau} is within trace distance $\frac{3\sqrt{10}q^{3/2}}{2^{\secp}}$ of a state $\tau_{\mathsf{good}}$ in the image of $\bbI - \Pi_\mathsf{bad}^{19/200}$.%, where $\alpha$ is defined below. 
    % \[
    %     \alpha = \sqrt{2}(2q+1)\left(\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}}\right)^{1/2} 
    % \]
    The following sub-claim completes the proof of \cref{claim:qot-3r-bb84-hyb34}.
    \begin{subclaim}
    If $h : \zo^{m} \times \zo^{\leq (n-k)} \rightarrow \zo^{\secp}$ is a universal family of hash functions, then conditioned on $\tau$ (defined in \cref{subclaim:tau}) being the image of $\bbI - \Pi_\mathsf{bad}^{19/200}$, and $A=10^6,B=8\times 10^5,C=5\times 10^4$, it holds that 
    \[
        % |\Pr[\Hyb_3=1]-\Pr[\Hyb_4=1]| \leq 2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
        |\Pr[\Hyb_3=1]-\Pr[\Hyb_4=1]| \leq {2^{-3002\secp}}
    \]
    where $h_b$ is the binary entropy function. \nishant{this should be there in prelims} 
    \end{subclaim}
    \begin{proof}
    Note that 
    \begin{align}
        &\bbI - \Pi_{\mathsf{bad}}^\delta = \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb,\\U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \left(\sum_{\substack{\bR \, : \, \bR_{S'} \neq \widetilde{\bR}_{S'} \text{ or } \Delta\left(\bR_{\overline{T}}, \widetilde{\bR}_{\overline{T}}\right) < \delta\\\text{where }T = \fsro(\bc),\\S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_{j}\}}}\ket{\bR_{\widetilde{\btheta}}}\bra{\bR_{\widetilde{\btheta}}}_{\cS}\right) \label{eq:3rseeded1}
    \end{align}
    Since $\tau$ is in the image of $\bbI - \Pi_{\mathsf{bad}}^{19/200}$, the state on register $\cS$ is in a superposition of states as in the summation above. However, note that if $T \neq \fsro(\bc)$ or if $\bR_{S'}\neq \widetilde{\bR}_{S'}$ (where $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$), then the sender side check will fail and the two hybrids are perfectly indistinguishable. So, it suffices to analyze states $\tau$ where the register containing $T$ equals $\fsro(\bc)$ and where $\bR_{S'}=\widetilde{\bR}_{S'}$.
    Hence, conditioned on the sender not aborting, 
    % $\tau$ being in the image of $\bbI - \Pi_{\mathsf{bad}}^\delta$, $T = \fsro(\bc)$, and $\bR_{S'}=\widetilde{\bR}_{S'}$, 
    the above equation implies that the register $\cS$ is in superposition of states \nishant{confusing notation} $\ket{\bR_{\widetilde{\btheta}}}$ s.t.\ $\bR_{S'} = \widetilde{\bR}_{S'}, \Delta(\bR_{\overline{T}},\widetilde{\bR}_{\overline{T}})<19/200$, for $S'$ as defined above.
    
    \nishant{this} Recall that the next thing the sender performs is to measure register $\cS$. Since by elementary properties of quantum mechanics, measurements on different subsystems commute, assume that the sender measures the registers $\cS_{{T}\cup U}$ first. Then, using the above this leaves the registers $\cS_{\overline{T} \setminus {U}}$ in a superposition of states $\ket{\left(\bR_{\overline{T}\setminus U}\right)_{\widetilde{\btheta}}}$ for $\bR_{\overline{T}\setminus U}$ s.t.\  $\Delta(\bR_{\overline{T}\setminus U},\widetilde{\bR}_{\overline{T}\setminus U}) < \frac{19(n-k)}{200(n-k-d)} = 1/10$ (for $A = 10^6,C=5\times 10^4,k=B\secp,d=C\secp,n=(A+B)\secp$).
    
    Next, to obtain $ct_{b'}$ for $b' \in \zo$, the sender measures registers $\cS_{i,d_i \oplus b'}$ in basis $d_i \oplus b'$ to obtain a string $\br'_{b'} \in \{0,1\}^{|\overline{T}\setminus U|}$. Then, $ct_{b'}$ is set as $m_{b'} \oplus h(s,\br'_{b'})$, where $s$ is uniformly sampled seed for a universal hash function $h$.
    Recall, in addition, in $\Hyb_4$ the sender defines $b$ as $\maj \{\widetilde{\btheta}_i \oplus d_i\}_{i \in \overline{T}\setminus U}$. We now prove a lower bound on the quantum min-entropy of $\br'_{b \oplus 1}$, which using the Leftover Hash lemma (\cref{impthm:privacy-amplification}) would imply our claim. 
    
    Consider the subset $W \subseteq \zo \times \overline{T}\setminus U$ defined as $W = \{i, d_i \oplus b \oplus 1\}_{i \in \overline{T}\setminus U}$ and consider again by the commuting property of measurements on different systems that registers $\cS_{\overline{T}\setminus (U \cup W)} = \{\cS_{i, d_i \oplus b}\}_{i \in \overline{T}\setminus U}$ are measured first, leaving the registers $\cS_W = \{\cS_{i, d_i \oplus b \oplus 1}\}_{i \in \overline{T}\setminus U}$ in a superposition of states $\ket{\br_{\widetilde{\btheta}_W}}$, where $\omega\left(\br, \widetilde{\bR}_{W}\right) < 1/10$. Hence, since $\br'_{b \oplus 1}$ is obtained by measuring registers $\cS_W = \{\cS_{i,d_i \oplus b \oplus 1}\}_{i \in \overline{T}\setminus U}$ in basis $d_i \oplus b \oplus 1$, majority of the bits of $\br'_{b \oplus 1}$ are obtained by measuring $\cS_W$ in basis $\widetilde{\btheta}_i \oplus 1$ (since $b$ was defined as $\maj \{\widetilde{\btheta}_i \oplus d_i\}_{i \in \overline{T}\setminus U}$, this means in the majority of the places in $\overline{T} \setminus U$, the following holds: $b = \widetilde{\btheta}_i \oplus d_i \iff d_i \oplus b \oplus 1 = \widetilde{\btheta}_i \oplus 1$).
    
    Therefore, registers $\cS_W$ are in a superposition of states $\ket{\br_{\widetilde{\btheta}_W}}$, where $\omega\left(\br, \widetilde{\bR}_{W}\right) < 1/10$, and then majority of them are measured in basis $\widetilde{\btheta}_i \oplus 1$. Using \cref{impthm:small-superposition}, we get,
    % since for $i \in \overline{T}\setminus U$, registers $\cS_{i,d_i \oplus b \oplus 1}$ are measured in basis $d_i \oplus b \oplus 1$ to obtain $\br'$, this means at least $|\overline{T}\setminus U|/2$ of the bits $\br'_i$ are obtained by measuring in $\widetilde{\btheta}_i \oplus 1$. Let $M \subseteq \overline{T}\setminus U$ be this set of size at least $\frac{|\overline{T}\setminus U|}{2}$, and define $\widetilde{\br} \in \{0,1\}^n$ such that $\widetilde{\br}_i = \widetilde{\bR}_{i,d_i \oplus b \oplus 1}$. We know from above that the register $\cS_M$ is in a superposition of states $\ket{{\br_M}_{\widetilde{\btheta}_M}}$ for $\br_M$ such that $\omega(\br_M,\widetilde{\br}_M) < \delta'$. Thus, with an appropriate change of basis, we can appeal to \cref{impthm:small-superposition} to argue the following:
    \begin{align*}
        \mathbf{H}_\infty(\br'_{b \oplus 1} \, | \, \cC,\cZ_1,\cZ_2,\cX) &\geq \frac{|\overline{T}\setminus U|}{2} - h_b\left(0.1\right)|\overline{T}\setminus U|\\
        &\geq \frac{n-k-d}{2} - h_b\left(0.1\right)(n-k).
    \end{align*}
    For $n=(A+B)\secp,k=B\secp,d=C\secp,A=10^6,B=8\times 10^5,C=5\times 10^4$, we get,
    \begin{align*}
        \mathbf{H}_\infty(\br'_{b \oplus 1} \, | \, \cC,\cZ_1,\cZ_2,\cX) &\geq 6004\secp.
    \end{align*}
    where $h_b$ is the binary entropy function, and we bound the number of strings of length $n$ with hamming weight at most $\delta'$ by $h_b(\delta')n$.
    If $U_p$ denotes a random variable chosen uniformly from $\zo^p$, using now the leftover hash lemma (\cref{impthm:privacy-amplification}) we get the statistical distance between $(U_m,h(U_m,\br'_{b\oplus 1}))$ and $(U_m,U_{\secp})$ is bounded by ${2^{-3002\secp}}$,
    % \[
    %     2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
    % \]
    hence proving the claim.
    \end{proof}
    
    \end{proof}
    
    \end{proof}
}\fi





















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse{
        %version with the exact bounds
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        %
        %
        %       Sender security
        %
        %
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \noindent\underline{\textbf{Sender security}}
        
        Let $\SimExt = (\SimExt.\RO,\SimExt.\Ext)$ be the simulator for the extractable commitment scheme from \cref{sec:uccomm}. Let $+$ refer to the computational basis and $\times$ to the hadamard basis \nishant{do we need to define this?}. Below we describe the simulator $\Sim[\sR^*]$ against a malicious receiver $\sR^*$ for \proref{fig:qot-3r-bb84}\nishant{these figures don't have protocol number in them ; fix later at all places}.
        
        \underline{$\Sim[\sR^*](\brho)$}:
        \begin{itemize}
            \item Initialize the on-the-fly random oracle simulator $\simro$ from \cref{impthm:extROSim}. Run $\sR^*(\brho)$ answering its oracle queries to $\fsro$ using $\simro$ and queries to $\comro$ using $\SimExt.\RO$.
            \item Sample $2n$ EPR pairs on registers $\{(\cE_{i,b,S},\cE_{i,b,R})\}_{i \in [n], b \in \zo}$ and send registers $\{\cE_{i,b,R}\}_{i \in [n],b \in \zo}$ to $\sR^*$. 
            \item When $\sR^*$ outputs $\{c_i\}_{i \in [n]}, T, \{(\widehat{r_i}^0, \widehat{r_i}^1, \widehat{\theta}_i)\}_{i \in T}, \{d_i\}_{i \in \overline{T}}$, then run $\{(\widetilde{r_{i}}^0,\widetilde{r_{i}}^{1},\widetilde{\theta}_i)\}_{i \in [n]} \leftarrow \SimExt.\Ext(\{c_i\}_{i \in [n]})$. 
            \item Run the ``check receiver message" part of the honest sender strategy, except do the following in place of the third check:
                \begin{itemize}
                    \item Sample subset $U \subset [n]$ of size $d$ and for each $i \in [n]$, sample bit $b_i \in \zo$. 
                    \item For each $i \in [n]$, do the following: 
                        \begin{itemize}
                            \item If $i \in U$, measure registers $\cE_{i,0,S}$ and $\cE_{i,1,S}$ in basis $+$ if $b_i = 0$, or else in basis $\times$ if $b_i = 1$, to get measurement outcomes $r_i^0$ and $r_i^1$ respectively. 
                            \item If $i \notin U$, then measure $\cE_{i,0,S}$ in basis $+$ and $\cE_{i,1,S}$ in basis $\times$ to get outcomes $r_i^0,r_i^1$ respectively. 
                        \end{itemize}
                    \item For each $i \in T\cap U$ such that $\widetilde{\theta}_i = b_i$, check that $\widetilde{r_i}^0 = r_i^0$ and $\widetilde{r_i}^1 = r_i^1$.
                \end{itemize}
            \item Set $b \coloneqq \maj(\{\widetilde{\theta}_i \oplus d_i\}_{ i\in \overline{T}\setminus U})$ and send $b$ to $\cF_{\OT[\secp]}$ to receive back $m_b$ \nishant{abort doubt}.
            \item Compute the last message using the honest sender strategy except for using $m_{1-b} \coloneqq 0^\secp$. 
            \item Run $\sR^*$ on this last message, output its state and terminate.
            \item Answer queries of distinguisher to $\fsro$ and $\comro$ using $\simro$ and $\SimExt.\RO$ respectively.
        \end{itemize}
        Let $(\sD,\bsigma)$ be a distinguisher s.t.\ $\sR^*,\sD$ make a total of $q$ queries to $\fsro$ and $\comro$. Consider the following sequence of hybrids:
        \begin{itemize}
            \item $\Hyb_0$: This is the real world interaction between $\sR^*$ and $\sS$. Using the notation of \cref{def:secure-realization}, this is a distribution over $\zo$ denoted by $\Pi[\brho,\bsigma,\sR^*,\sD,(m_0,m_1)]$.
            \item $\Hyb_1$: This is the same as the previous hybrid, except the following are run instead to generate the first sender message: (1) Sample $2n$ EPR pairs on registers $\{(\cE_{i,b,S},\cE_{i,b,R})\}_{i \in [n], b \in \zo}$. (2) Run the following algorithm: 
            
                \underline{\textbf{Algorithm Measure-EPR}}:
                \begin{itemize}
                    \item Sample subset $U \subset [n]$ of size $d$ and for each $i \in [n]$, sample bit $b_i \in \zo$. 
                    \item For each $i \in [n]$, do the following: 
                        \begin{itemize}
                            \item If $i \in U$, measure registers $\cE_{i,0,S}$ and $\cE_{i,1,S}$ in basis $+$ if $b_i = 0$, or else in basis $\times$ if $b_i = 1$, to get outcomes $r_i^0$ and $r_i^1$ respectively. 
                            \item If $i \notin U$, then measure $\cE_{i,0,S}$ in basis $+$ and $\cE_{i,1,S}$ in basis $\times$ to get outcomes $r_i^0,r_i^1$ respectively. 
                        \end{itemize}
                \end{itemize}
            Thereafter, registers $\{\cE_{i,b,R}\}_{i \in [n],b \in \zo}$ are sent over to $\sR^*$ and the rest of the experiment works as the previous hybrid.
            \item $\Hyb_2$: This is the same previous hybrid, except that the sender delays running the algorithm Measure-EPR to just before executing the third check in ``check receiver message" part of the honest sender strategy.
            \item $\Hyb_3$: This is the same as the previous hybrid, except for the following changes: queries of $\sR^*$ to $\comro$ are now answered using $\SimExt.\RO$. Once $\sR^*$ outputs its second message, the following is run: $\{(\widetilde{r_{i}}^0,\widetilde{r_{i}}^1,\widetilde{\theta}_i)\}_{i \in [n]} \leftarrow \SimExt.\Ext(\{c_i\}_{i \in [n]})$. Thereafter, $\{(\widetilde{r_i}^0,\widetilde{r_i}^1,\widetilde{\theta}_i)\}_{i \in T}$ are used for the third check in the ``check receiver part" of the honest sender strategy.
            \item $\Hyb_4$: This is the result of the interaction between $\Sim[\sR^*]$, $\cF_{\OT[\secp]}$ and honest sender $\sS$. Using the notation of \cref{def:secure-realization}, this is denoted by $\widetilde{\Pi}_{\cF_{\OT[\secp]}}[\brho,\bsigma,\Sim[\sR^*],\sD,(m_0,m_1)]$.
        \end{itemize}
        We prove the indistinguishability between the hybrids using the following claims:
        \begin{claim} $\Pr[\Hyb_0=1] = \Pr[\Hyb_1=1]$
        \end{claim}
        \begin{proof}
            This follows from elementary properties of EPR pairs. In either hybrid, the distribution of the states sent from sender to receiver is a completely mixed state. \nishant{elaborate more}
        \end{proof}
        \begin{claim} $\Pr[\Hyb_1=1] = \Pr[\Hyb_2=1]$
        \end{claim}
        \begin{proof}
            This also follows using elementary properties of quantum mechanics, i.e.\ that the measurements on different sub-systems commute. \nishant{todo elaborate more}
        \end{proof}
        \begin{claim} $|\Pr[\Hyb_2=1] - \Pr[\Hyb_3=1]| \leq \frac{148(q+3\secp+1)^3+1}{2^{\secp}} + \frac{8qn}{2^{\secp/2}}$
        \end{claim}
        \begin{proof}
            This follows by a reduction to the $\frac{148(q+3\secp+1)^3+1}{2^{\secp}} + \frac{8qn}{2^{\secp/2}}$ \nishant{todo}.
        \end{proof}
        \begin{claim}
        \label{claim:qot-3r-bb84-hyb34}
        \begin{align*}
            |\Pr[\Hyb_3=1] - \Pr[\Hyb_4=1]| \leq &\sqrt{2}(2q+1)\left(\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}}\right)^{1/2} \\ &+ 2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
        \end{align*}
        \end{claim}
        \begin{proof}
        The only difference between $\Hyb_3$ and $\Hyb_4$ is that $m_{1-b} = 0^\secp$, where $b = \maj(\{\widetilde{\theta}_i \oplus d_i\}_{i \in \overline{T}})$. Intuitively we show that the mask of $m_{1-b}$ is a uniformly random string from the point of view of $\sR^*$ in either hybrid, which would imply the given claim. 
        \fflater{\nishant{There }}
        \paragraph{Notation:} We setup some notation before proceeding.
        \begin{itemize}
        \item Let $\bc \coloneqq (c_1,\dots,c_n)$ be the classical commitments and $\bb \coloneqq (b_1,\dots b_n)$ be the bits sampled by the sender while executing its checks.
        \nishant{there is a small notational inconsistency here between $\bb_i$ vs $b_i$}
        \item Write the classical extracted values $\{(\widetilde{r_i}^0,\widetilde{r_i}^1,\widetilde{\theta}_i)\}_{i \in [n]}$ as matrices
        \[
            \widetilde{\bR} \coloneqq \begin{bmatrix}\widetilde{r_1}^0 \ \dots \ \widetilde{r_n}^0 \\ \widetilde{r_1}^1 \ \dots \ \widetilde{r_n}^1\end{bmatrix}, 
            \widetilde{\btheta} \coloneqq \begin{bmatrix}\widetilde{\theta}_{1} \ \dots \ \widetilde{\theta}_{n} 
            % \\ \widetilde{\theta}_{1} \ \dots \ \widetilde{\theta}_n
            \end{bmatrix}.
        \]
        \item Given any $\bR \in \{0,1\}^{2 \times n}$, $\btheta \in \zo^n$, define $\ket{\bR_{\btheta}}$ as a state on $n$ $4$-dimensional registers, where register $i$ contains the state \nishant{ch} $\ket{\bR_{i,0},\bR_{i,1}}$ prepared in the $(\btheta_{i},\btheta_{i})$-basis. \nishant{define what this means}
        \item Given $\bR,\widetilde{\bR} \in \{0,1\}^{2 \times n}$ and a subset $T \subseteq [n]$, define $\bR_T$ be the columns of $\bR$ indexed by $T$, and define $\Delta\left(\bR_T,\widetilde{\bR}_{T}\right)$ as the fraction of columns $i \in T$ such that $(\bR_{i,0},\bR_{i,1}) \neq (\widetilde{\bR}_{i,0},\widetilde{\bR}_{i,1})$.
        \item For $T \subset [n]$, let $\overline{T} \coloneqq [n] \setminus T$.
        \item Given $\widetilde{\bR} \in \{0,1\}^{2 \times n}, \widetilde{\btheta} \in \zo^n$, $T \subseteq [n]$, $U \subseteq [n]$, $\bb \in \zo^n$, and $\delta \in (0,1)$, define
        \[
            \Pi^{\widetilde{\bR},\widetilde{\btheta},T,U,\bb,\delta} \coloneqq \sum_{\substack{\bR \, : \, \bR_{S'} = \widetilde{\bR}_{S'}, \Delta\left(\bR_{\overline{T}}, \widetilde{\bR}_{\overline{T}}\right) \geq \delta\\\text{where }S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_{j}\}}}\ket{\bR_{\widetilde{\btheta}}}\bra{\bR_{\widetilde{\btheta}}}.
        \]
    \end{itemize}
    
    \noindent Now, consider the following projection, which has hard-coded the description of $\fsro$:
    
    \[
        \Pi_{\mathsf{bad}}^\delta \coloneqq \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb,\\U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \Pi^{\widetilde{\bR},\widetilde{\btheta},\fsro(\bc),U,\bb,\delta}_{\cS},
    \]
    where $\cC$ is the register holding the classical commitments, $\cZ_1$ is the register holding the output of $\SimExt.\Ext$, $\cZ_2$ is the register holding the subset $U$ and bits $\bb$ sampled by sender, and $\cS$ is the register holding the sender's halves of EPR pairs.
    
    \begin{subclaim}\label{subclaim:tau}
    Let 
    \[
        \tau \coloneqq \sum_{\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb}p^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)} \tau^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)},
    \] 
    where 
    \[
        \tau^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)} = \ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)}_{\cS,\cX}
    \] 
    is the entire state of $\Hyb_3$ right after $\rcv^*$ outputs its message (which includes $\bc$), $\SimExt.\Ext$ is run to get $\widetilde{\bR},\widetilde{\btheta}$, and sender samples the set $U \subseteq [n]$ of size $d$ and bits $\bb \in \zo^n$. Here, each $p^{(\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb)}$ is the probability that the string $\bc,\widetilde{\bR},\widetilde{\btheta},U,\bb$ is contained in the registers $\cC,\cZ_1,\cZ_2$. Also, $\cS$ is the register holding the sender's halves of EPR pairs and $\cX$ is a register holding remaining state of the system, which includes the rest of the receiver's classical message and its private state. Then, 
    \[
        \Tr(\Pi_{\mathsf{bad}}^\delta \tau) \leq (2q+1)^2 \left[\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}} \right].
    \]
    \end{subclaim}
    \begin{proof}
    Define $\Adv_{\rcv^*}^{\fsro}$ to be the oracle machine that runs $\Hyb_3$ until $\rcv^*$ outputs $\bc$ (and the rest of its message), then runs $\SimExt.\Ext$ to obtain $\ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}$, followed by sampling the set $U \subseteq [n]$ of size $d$, and bits $\bb \in \zo^n$ in the register $\cZ_2$, and finally outputting the remaining state $\rho_{\cS,\cX}$. Consider running the measure-and-reprogram simulator $\Sim[\Adv_{\rcv^*}]$ from \cref{thm:measure-and-reprogram}, which simulates $\fsro$ queries, measures and outputs $\bc$, then receives a uniformly random subset $T \subset [n]$ of size $k$, and then continues to run $\Adv_{\rcv^*}$ until it outputs $\ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}$. Letting 
    \[
        \Pi_{\mathsf{bad}}^{\delta}[T] \coloneqq \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb \\ U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \Pi^{\widetilde{\bR},\widetilde{\btheta},T,U,\bb,\delta}_{\cS},
    \] for $T \subset [n]$, \cref{thm:measure-and-reprogram} implies that \begin{align*}
    &\Tr\left(\Pi_\mathsf{bad}^{\delta}\tau\right) \\ &\leq (2q+1)^2 \E\left[\Tr\left(\Pi_{\mathsf{bad}}^{\delta}[T]\left(\ket{\bc}\bra{\bc}_\cC \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}\otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}\right)\right): \begin{array}{r}(\bc,\state) \gets \Sim[\Adv_{\rcv^*}] \\ T \gets S_{n,k} \\ \left(\substack{\widetilde{\bR},\widetilde{\btheta},U,\\\bb,\rho_{\cS,\cX}}\right) \gets \Sim[\Adv_{\rcv^*}](T,\state)\end{array}\right],\end{align*} 
    where $S_{n,k}$ is the set of all subsets of $[n]$ of size $k$.
    
    Now, recall that one of the last things that $\Adv_{\rcv^*}$ does in $\Hyb_3$ is run $\SimExt.\Ext$ on $\bc$ to obtain $(\widetilde{\bR},\widetilde{\btheta})$. Consider instead running $\SimExt.\Ext$ on $\bc$ immediately after $\Sim[\Adv_{\rcv^*}]$ outputs $\bc$. Note that $\SimExt.\Ext$ only operates on the register holding $\bc$ and its own private state used for simulating $\comro$, so since $\Com^{\comro}$ \nishant{$\comro$} has a $\frac{8}{2^{{\secp_\com}/2}}$-commuting simulator (\cref{def:fextractable}), we have that, 
    
    \begin{align}
    \Tr\left(\Pi_\mathsf{bad}^{\delta}\tau\right) &\leq (2q+1)^2\left(\epsilon + \frac{8q}{2^{{\secp_\com}/2}}\right) \label{eq:taueq1}
    \end{align}
    % &\leq (2q+1)^2\left(\right) \\ 
    % &\coloneqq (2q+1)^2\left(\epsilon + \frac{8q}{2^{{\secp_\com}/2}}\right), \nonumber
    % \end{align}
    where 
    \[
        \epsilon \coloneqq \E\left[\Tr\left(\Pi_{\mathsf{bad}}^{\delta}[T]\left(\ket{\bc}\bra{\bc}_\cC  \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1}\otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \rho_{\cS,\cX}\right)\right): \begin{array}{r}(\bc,\state) \gets \Sim[\Adv_{\rcv^*}] \\ (\widetilde{\bR},\widetilde{\btheta}) \gets \SimExt.\Ext(\bc) \\ T \gets S_{n,k} \\ \left(\substack{\widetilde{\bR},\widetilde{\btheta},U,\\\bb,\rho_{\cS,\cX}}\right) \gets \Sim[\Adv_{\rcv^*}](T,\state)\end{array}\right].
    \]
    Now, consider the following quantum sampling game.
    
    \begin{itemize}
        \item Fix a state on register $\cS$ (and potentially other registers of arbitrary size), where $\cS$ is split into $n$ registers $\cS_1,\dots,\cS_n$ of dimension 4, and fix matrices $\widetilde{\bR}\in \{0,1\}^{2 \times n},\widetilde{\btheta} \in \zo^n$.
        \item Sample a uniformly random subset $T \subset [n]$ of size $k$.
        \item Sample a subset $S' \subseteq T$ \nishant{later at all places - $\subset$ vs $\subseteq$} as follows:    \begin{itemize}
            \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
            \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
        \end{itemize}
        \item For each $i \in S'$, measure the register $\cS_i$ in basis  $\widetilde{\btheta}_{i}$ to get $\bR_{S'} \in \zo^{2 \times |S'|}$. \nishant{sizeof} Output $\Delta(\bR_{S'},\widetilde{\bR}_{S'})$. 
        %as the estimate for the ``closeness''\footnote{The notion of closeness to a quantum state is not defined here, but is captured by the quantum error probability as defined in \cref{def:quantum-error-probability}.} of the state on registers $\cS_{\overline{T}}$ to $\ket{{\widetilde{\bR}_{\overline{T}}}_{\widetilde{\btheta}_{\overline{T}}}}$.
        
        
        %Register $\cE_S$, when written in the $\btheta^*$-basis, has non-zero amplitude on some string $\br$ such that $\br_{\widehat{T}} = \br^*_{\widehat{T}}$, but $\omega\left(\br_{\overline{\widehat{T}}} \oplus \br^*_{\overline{\widehat{T}}}\right) \geq \delta$.
    \end{itemize}
    
    \nishant{this can use some more explanation}
    The quantum error probability $\epsilon^{\delta}_{\mathsf{quantum}}$ (\cref{def:quantum-error-probability}) of the above game corresponds to the trace distance between the initial state on register $\cS$ and an ``ideal'' state (as defined in \cref{def:quantum-error-probability}). By definition of the above sampling game, for any $(T,\widetilde{\bR},\widetilde{\btheta})$, this ideal state is orthogonal to the subspace $\Pi^{\widetilde{\bR},\widetilde{\btheta},T,\delta}_\cS$ since for any vector $\ket{\bR_{\widetilde{\btheta}}}$ in the ideal state, if $\Delta(\bR_T,\widetilde{\bR}_T) = 0$, then $\Delta(\bR_{\overline{T}},\widetilde{\bR}_{\overline{T}}) < \delta$. Thus, noting that the trace inside the expectation defining $\epsilon$ would be 0 for any state orthogonal to this subspace, it follows that $\epsilon$ is bounded by $\epsilon^{\delta}_{\mathsf{quantum}}$.
    
    Thus, by \cref{impthm:error-probability}, $\epsilon$ is then bounded by $\sqrt{\epsilon^\delta_{\mathsf{classical}}}$, where $\epsilon^\delta_{\mathsf{classical}}$ is the \emph{classical} error probability (\cref{def:classical-error-probability}) in the following classical sampling game. \nishant{i think its better to say this just outputs $\widetilde{\delta}$}
    \begin{itemize}
        \item Let $\bR, \widetilde{\bR} \in \{0,1\}^{2 \times n}$ s.t.\ $\bR$ is the matrix on which we are running the sampling and $\widetilde{\bR}$ is an an arbitrary matrix.
        \item Sample a uniformly random subset $T \subset [n]$ of size $k$.
        \item Sample a subset $S' \subset T$ as follows: 
        \begin{itemize}
            \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
            \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
        \end{itemize}
        \item Output $\Delta(\bR_{S'},\widetilde{\bR}_{S'})$.
    \end{itemize}
    
    We analyze the classical error probability of the above game by looking at the same, but with sampling happening on a string $q \in \zo^n$ as follows:
    \paragraph{Analysis of the corresponding classical sampling strategy}
    For a string $\strq \in \zo^n$ and $S \subset [n]$, let $\strq_S = \{\strq_i \, | \, i \in S\}$. Consider the following classical sampling strategy to determine the relative hamming weight of a string $\strq \in \zo^n$.
    \begin{itemize}
        \item Choose a random subset $T \subset [n]$ of size $k$.
        \item Choose a subset $S' \subset T$ as follows: 
            \begin{itemize}
                \item Sample a uniformly random subset $U \subset [n]$ of size $d$ and bits $\bb \in \zo^n$. 
                \item Set $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$.
            \end{itemize}
        \item Output $\omega(\strq_{S'})$ as the estimate of the hamming weight of $\strq$.
    \end{itemize}
    This defines the corresponding classical sampling strategy, with $P_T$ as the distribution induced by sampling subset $T \subset [n]$ of size $k$ without replacement. $P_S$ is the distribution induced by sampling $S' \subset T$ as above, and $f(T,\strq_T,S') = \omega(\strq_{S'})$. We then prove the following for this classical sampling strategy:
    \begin{lemma}
        $\epsilon^\delta_{\mathsf{classical}} \leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) $ for $0 < \delta < 1$.
        % \coloneqq \max_{\bq \in A^n}\Pr_{t \gets P_T,s \gets P_S}\left[\bq \notin B_{t,s}^\delta(\Psi)\right]
    \end{lemma}
    \begin{proof}
        Let $S = T \cap U$ in the above sampling strategy. We have,
        \begin{align*}
            \epsilon^\delta_{\mathsf{classical}} &= \max_\strq \Pr_{T \leftarrow P_T, S' \leftarrow P_S}\left[\strq \notin B_{T,S'}^\delta\right]\\
            &= \max_\strq \Pr_{T \leftarrow P_T, S' \leftarrow P_S}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right]\\
            &\leq \max_\strq \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{T})| + |\omega(\strq_{{T}}) - \omega(\strq_{S'})| \geq \delta\right]
        \end{align*}
        Considering the sampling of $T$ as a separate sampling strategy, we know from the analysis in \cite[Appendix B.1]{C:BouFeh10}, for $0 < \delta < 1$,
        \begin{align}
            \max_\strq \Pr_{T \leftarrow P_T, |T|=k} \left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{T})| \geq \delta \right] \leq 2\exp\left( - \frac{k\delta^2}{2} \right)
            \label{eq:classampTTbar}
        \end{align}
        We prove the following sub-claim:
        \begin{subclaim}
            For any given string $\strq$,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right] \leq 6\exp\left( -\frac{2\delta^2 s}{81} \right)
            \]
        \end{subclaim}
        \begin{proof}
            Note that $|\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \implies |\omega(\strq_T) - \omega(\strq_{S})| + |\omega(\strq_S) - \omega(\strq_{S'})| \geq |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta$ (using triangle inequality). Therefore,
            \begin{align}
                \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right] \leq \Pr_{S,S'}\left[ |\omega(\strq_T) - \omega(\strq_{S})| + |\omega(\strq_S) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S| = s \right]
                \label{eq:classampeq1}
            \end{align}
            Given $|S| = |T \cap U| = s$, sampling $S'$ in the sampling game above is equivalent to first sampling a set $S \subset T$ of size $s$, then sampling $\theta \leftarrow \zo^{|S|}$ to define $S'$. Using Heoffding's inequality \nishant{add it - its tighter than chernoff}, for sampling $S \subset T$ of size $s$ at random without replacement, we have, for $\epsilon_1 > 0$,
            \begin{align*}
                \Pr_{S}\left[ |\omega(\strq_{T}) - \omega(\strq_S)| \geq \epsilon_1 \, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right)
            \end{align*}
            Also, since sampling of $S'$ from $S$ is equivalent to sampling a random subset of $S$, using \cite[Appendix B.2]{C:BouFeh10}, for $0 < \epsilon_2 < 1$, \nishant{this is not tight + if we get time, we should give a tighter analysis of even B.4} \nishant{todo - $S \setminus S'$}
            \begin{align*}
                &\Pr_{S'}\left[ |\omega(\strq_{S}) - \omega(\strq_{S'})| \geq \epsilon_2 \, \Big| \, |S|=s \right] \leq 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)\\
            % Noting that $|\omega(\strq_{S \setminus S'}) - \omega(\strq_{S'})| \geq \epsilon_2 \implies |\omega(\strq_{S}) - \omega(\strq_{S'})| =  \geq \epsilon_2$
                \implies &\Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_S)| \geq \epsilon_1 \wedge |\omega(\strq_{S}) - \omega(\strq_{S'})| \geq \epsilon_2 \, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)\\
                \implies &\Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq (\epsilon_1 + \epsilon_2)\, \Big| \, |S|=s \right] \leq 2\exp\left(-2\epsilon_1^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right) \quad \text{(using \cref{eq:classampeq1})}
            \end{align*}
            Setting $\delta = \epsilon_1 + \epsilon_2$, we get,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \leq 2\exp\left(-2(\delta - \epsilon_2)^2 s\right) + 4\exp\left(-\frac{\epsilon_2^2s}{32}\right)
            \]
            Setting $\epsilon_2 = \frac{8\delta}{9}$, we get the two exponents as equal to get,
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \leq 6\exp\left(- \frac{2\delta^2 s}{81}\right)
            \]
        \end{proof}
        \begin{subclaim}
            \label{subclaim:classampTS}
            \[
                \Pr_{S,S'}\left[ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \right] \leq 7\exp\left(- \frac{0.019 \delta^2  d  k}{n}\right)
            \]
        \end{subclaim}
        \begin{proof}
            We do this by noting the distribution of $S = T \cap U$. We use a Chernoff Bound for sampling with replacement. Let $U$ be drawn with replacement after $T$ is sampled, and let for all $i \in [d], X_i = 1$ iff the $i^{th}$ draw lands in $T$. Then, $\Pr[X_i=1] = \frac{k}{n}$. Let $X = \sum_{i=0}^d X_i$. $\E[X] = \frac{kd}{n}$. Since $X_i$ are independently drawn binary random variables, we get using Chernoff bound, for $0 < \epsilon_3 < 1$,
            \begin{align*}
                \Pr[X \leq (1-\epsilon_3)\frac{dk}{n}] &\leq \exp\left( -\frac{\epsilon_3^2 dk}{2n} \right)\\
                \implies \Pr_{S}\left[ \, |S| \leq (1-\epsilon_3)\frac{dk}{n}\right] &\leq \exp\left( -\frac{\epsilon_3^2 dk}{2n} \right)
            \end{align*}
            Therefore, 
            \begin{align*}
                \Pr_{S,S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})|\geq \delta\right] &= \sum_{s \leq (1-\epsilon_3)\frac{dk}{n}} \Pr_{S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \Pr_S\left[|S|=s\right] \\
                &+ 
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} \Pr_{S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})| \geq \delta \, \Big| \, |S|=s \right] \Pr_S\left[|S|=s\right]\\
                % &\leq \Pr_{S}\left[ |S| \leq (1-\epsilon_3)\frac{dk}{n} \right] + \Pr_{S'}\left[\right]
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} 6\exp\left( - \frac{2\delta^2s}{81} \right) \Pr_S\left[|S|=s\right]\\
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                \sum_{s > (1-\epsilon_3)\frac{dk}{n}} 6\exp\left( - \frac{2\delta^2(1-\epsilon_3)dk}{81n} \right) \Pr_S\left[|S|=s\right]\\
                &\leq \exp\left(-\frac{\epsilon_3^2
                dk}{2n}\right) +
                6\exp\left( - \frac{2\delta^2(1-\epsilon_3)dk}{81n} \right)\\
                % 6\exp\left(-\frac{2\delta^2}{s}\right)
            \end{align*}
            Setting $\epsilon_3 = \frac{\delta}{5}$, the two terms inside exp become $\frac{\delta^2dk}{50n}$ and $\frac{2\delta^2(5-\delta)dk}{405n}$. Upper bounding $\delta$ by $1$ in the latter, the two terms become $\frac{0.02\delta^2dk}{n}$ and $\approx\frac{0.01975\delta^2dk}{n}$. Lower bounding each term by $\frac{0.019\delta^2dk}{n}$, which upper bounds the negative exp term, we get,
            \begin{align*}
                \Pr_{S,S'}\left[ \ |\omega(\strq_{T}) - \omega(\strq_{S'})|\geq \delta\right] &\leq 7\exp\left( -\frac{0.019\delta^2dk}{n} \right)
            \end{align*}
        \end{proof}
        \noindent Combining \cref{eq:classampTTbar} with \cref{subclaim:classampTS}, we get,
        \begin{align*}
            \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta_1 + \delta_2 \right] &\leq 2\exp\left(-\frac{k\delta_1^2}{2}\right) + 7\exp\left(-\frac{0.019\delta_2^2dk}{n}\right)
        \end{align*}
        Setting $\delta = \delta_1+\delta_2$, we get,
        \begin{align*}
            \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] &\leq 2\exp\left(-\frac{k(\delta-\delta_2)^2}{2}\right) + 7\exp\left(-\frac{0.019\delta_2^2dk}{n}\right)
        \end{align*}
        Setting $\delta_2 = \frac{\delta}{\left(1 + \sqrt{0.038\frac{d}{n}}\right)}$ to get the two exp terms as equal, we get,
        \begin{align*}
            &\Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] \leq 9\exp\left(-\frac{0.019\delta^2dk}{\left(1 + \sqrt{\frac{0.038d}{n}}\right)^2n}\right)\leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)\\
            \implies &\epsilon^\delta_{\mathsf{classical}} \leq \max_\strq \Pr_{T,S'}\left[ |\omega(\strq_{\overline{T}}) - \omega(\strq_{S'})| \geq \delta \right] \leq 9\exp\left(-\frac{3\delta^2dk}{200\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)\\
            \implies &\epsilon^\delta_{\mathsf{classical}} \leq 9 \exp\left(-\frac{3\delta^2dk}{288n}\right)
        \end{align*}
        where we used that\footnote{We note that our focus here is not to find the tightest parameters, but show that the values are practical.\nishant{to edit?}} $\frac{d}{n}\leq 1$.
    \end{proof}
    \noindent To finish the proof of \cref{subclaim:tau}, we get $\epsilon$ in \cref{eq:taueq1} is s.t.\
    \[
        \epsilon \leq \epsilon^\delta_{\mathsf{quantum}} \leq \sqrt{\epsilon^\delta_{\mathsf{classical}}} = \sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right)
    \]
    which gives using \cref{eq:taueq1} that:
    \[
        \Tr(\Pi_{\mathsf{bad}}^\delta \tau) \leq (2q+1)^2 \left[\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}} \right]
    \]
    \end{proof}
    Thus, by gentle measurement (\cref{lemma:gentle-measurement}), the $\tau$ defined in \cref{subclaim:tau} is within trace distance $\alpha$ of a state $\tau_{\mathsf{good}}$ in the image of $\bbI - \Pi_\mathsf{bad}^{\delta}$, where $\alpha$ is defined below. 
    \[
        \alpha = \sqrt{2}(2q+1)\left(\sqrt{9}\exp\left(-\frac{3\delta^2dk}{400\left(1 + \sqrt{\frac{d}{25n}}\right)^2n}\right) + \frac{8q}{2^{\secp_\com/2}}\right)^{1/2} 
    \]
    The following sub-claim completes the proof of \cref{claim:qot-3r-bb84-hyb34}.
    \begin{subclaim}
    If $h : \zo^{m} \times \zo^{\leq (n-k)} \rightarrow \zo^{\secp}$ is a universal family of hash functions, then conditioned on $\tau$ (defined in \cref{subclaim:tau}) being the image of $\bbI - \Pi_\mathsf{bad}^{\delta}$, it holds that 
    \[
        |\Pr[\Hyb_3=1]-\Pr[\Hyb_4=1]| \leq 2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
    \]
    where $h_b$ is the binary entropy function. \nishant{this should be there in prelims} 
    \end{subclaim}
    \begin{proof}
    Note that 
    \begin{align}
        &\bbI - \Pi_{\mathsf{bad}}^\delta = \sum_{\substack{\bc,\widetilde{\bR},\widetilde{\btheta},\bb,\\U \subseteq [n], |U|=d}}\ket{\bc}\bra{\bc}_{\cC} \otimes \ket{\widetilde{\bR},\widetilde{\btheta}}\bra{\widetilde{\bR},\widetilde{\btheta}}_{\cZ_1} \otimes \ket{U\bb}\bra{U\bb}_{\cZ_2} \otimes \left(\sum_{\substack{\bR \, : \, \bR_{S'} \neq \widetilde{\bR}_{S'} \text{ or } \Delta\left(\bR_{\overline{T}}, \widetilde{\bR}_{\overline{T}}\right) < \delta\\\text{where }T = \fsro(\bc),\\S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_{j}\}}}\ket{\bR_{\widetilde{\btheta}}}\bra{\bR_{\widetilde{\btheta}}}_{\cS}\right) \label{eq:3rseeded1}
    \end{align}
    Since $\tau$ is in the image of $\bbI - \Pi_{\mathsf{bad}}^\delta$, the state on register $\cS$ is in a superposition of states as in the summation above. However, note that if $T \neq \fsro(\bc)$ or if $\bR_{S'}\neq \widetilde{\bR}_{S'}$ (where $S' = \{j \, | \, j \in T \cap U \, \wedge \, \bb_j = \widetilde{\btheta}_j \}$), then the sender side check will fail and the two hybrids are perfectly indistinguishable. So, it suffices to analyze states $\tau$ where the register containing $T$ equals $\fsro(\bc)$ and where $\bR_{S'}=\widetilde{\bR}_{S'}$.
    Hence, conditioned on the sender not aborting, 
    % $\tau$ being in the image of $\bbI - \Pi_{\mathsf{bad}}^\delta$, $T = \fsro(\bc)$, and $\bR_{S'}=\widetilde{\bR}_{S'}$, 
    the above equation implies that the register $\cS$ is in superposition of states \nishant{confusing notation} $\ket{\bR_{\widetilde{\btheta}}}$ s.t.\ $\bR_{S'} = \widetilde{\bR}_{S'}, \Delta(\bR_{\overline{T}},\widetilde{\bR}_{\overline{T}})<\delta$, for $S'$ as defined above.
    
    \nishant{this} Recall that the next thing the sender performs is to measure register $\cS$. Since by elementary properties of quantum mechanics, measurements on different subsystems commute, assume that the sender measures the registers $\cS_{{T}\cup U}$ first. Then, using the above this leaves the registers $\cS_{\overline{T} \setminus {U}}$ in a superposition of states $\ket{\left(\bR_{\overline{T}\setminus U}\right)_{\widetilde{\btheta}}}$ for $\bR_{\overline{T}\setminus U}$ s.t.\  $\Delta(\bR_{\overline{T}\setminus U},\widetilde{\bR}_{\overline{T}\setminus U}) < \delta' $ where $\delta' = \frac{\delta(n-k)}{n-k-d}$.
    
    Next, to obtain $ct_{b'}$ for $b' \in \zo$, the sender measures registers $\cS_{i,d_i \oplus b'}$ in basis $d_i \oplus b'$ to obtain a string $\br'_{b'} \in \{0,1\}^{|\overline{T}\setminus U|}$. Then, $ct_{b'}$ is set as $m_{b'} \oplus h(s,\br'_{b'})$, where $s$ is uniformly sampled seed for a universal hash function $h$.
    Recall, in addition, in $\Hyb_4$ the sender defines $b$ as $\maj \{\widetilde{\btheta}_i \oplus d_i\}_{i \in \overline{T}\setminus U}$. We now prove a lower bound on the quantum min-entropy of $\br'_{b \oplus 1}$, which using the Leftover Hash lemma (\cref{impthm:privacy-amplification}) would imply our claim. 
    
    Consider the subset $W \subseteq \zo \times \overline{T}\setminus U$ defined as $W = \{i, d_i \oplus b \oplus 1\}_{i \in \overline{T}\setminus U}$ and consider again by the commuting property of measurements on different systems that registers $\cS_{\overline{T}\setminus (U \cup W)} = \{\cS_{i, d_i \oplus b}\}_{i \in \overline{T}\setminus U}$ are measured first, leaving the registers $\cS_W = \{\cS_{i, d_i \oplus b \oplus 1}\}_{i \in \overline{T}\setminus U}$ in a superposition of states $\ket{\br_{\widetilde{\btheta}_W}}$, where $\omega\left(\br, \widetilde{\bR}_{W}\right) < \delta'$. Hence, since $\br'_{b \oplus 1}$ is obtained by measuring registers $\cS_W = \{\cS_{i,d_i \oplus b \oplus 1}\}_{i \in \overline{T}\setminus U}$ in basis $d_i \oplus b \oplus 1$, majority of the bits of $\br'_{b \oplus 1}$ are obtained by measuring $\cS_W$ in basis $\widetilde{\btheta}_i \oplus 1$ (since $b$ was defined as $\maj \{\widetilde{\btheta}_i \oplus d_i\}_{i \in \overline{T}\setminus U}$, this means in the majority of the places in $\overline{T} \setminus U$, the following holds: $b = \widetilde{\btheta}_i \oplus d_i \iff d_i \oplus b \oplus 1 = \widetilde{\btheta}_i \oplus 1$).
    
    Therefore, registers $\cS_W$ are in a superposition of states $\ket{\br_{\widetilde{\btheta}_W}}$, where $\omega\left(\br, \widetilde{\bR}_{W}\right) < \delta'$, and then majority of them are measured in basis $\widetilde{\btheta}_i \oplus 1$. Using \cref{impthm:small-superposition}, we get,
    % since for $i \in \overline{T}\setminus U$, registers $\cS_{i,d_i \oplus b \oplus 1}$ are measured in basis $d_i \oplus b \oplus 1$ to obtain $\br'$, this means at least $|\overline{T}\setminus U|/2$ of the bits $\br'_i$ are obtained by measuring in $\widetilde{\btheta}_i \oplus 1$. Let $M \subseteq \overline{T}\setminus U$ be this set of size at least $\frac{|\overline{T}\setminus U|}{2}$, and define $\widetilde{\br} \in \{0,1\}^n$ such that $\widetilde{\br}_i = \widetilde{\bR}_{i,d_i \oplus b \oplus 1}$. We know from above that the register $\cS_M$ is in a superposition of states $\ket{{\br_M}_{\widetilde{\btheta}_M}}$ for $\br_M$ such that $\omega(\br_M,\widetilde{\br}_M) < \delta'$. Thus, with an appropriate change of basis, we can appeal to \cref{impthm:small-superposition} to argue the following:
    \begin{align*}
        \mathbf{H}_\infty(\br'_{b \oplus 1} | \cC,\cZ_1,\cZ_2,\cX) &\geq \frac{|\overline{T}\setminus U|}{2} - h_b(\delta')|\overline{T}\setminus U|\\
        &\geq \frac{n-k-d}{2} - h_b(\delta')(n-k)
    \end{align*}
    where $h_b$ is the binary entropy function, and we bound the number of strings of length $n$ with hamming weight at most $\delta'$ by $h_b(\delta')n$.
    If $U_p$ denotes a random variable chosen uniformly from $\zo^p$, using now the leftover hash lemma (\cref{impthm:privacy-amplification}) we get the statistical distance between $(U_m,h(U_m,\br'_{b\oplus 1}))$ and $(U_m,U_{\secp})$ is bounded by:
    \[
        2^{-1-\frac{1}{2}\left(\frac{n-k-d}{2} - h_b\left(\frac{\delta (n-k)}{n-k-d}\right)(n-k)\right)+\secp}
    \]
    hence proving the claim.
    \end{proof}
    
    \end{proof}
    
    \end{proof}

}\fi

==> old-qot-4r-bb84-construction.tex <==
\section{Four-round QOT in the QROM}

\james{define OT fuctionality}

We provide our construction of a QOT protocol in the $\idealcom$ hybrid in \figureref{fig:qot-4r-bb84-construction}. Below we provide the theorem for its security and prove it over the next two subsections.

\begin{theorem}
    \label{thm:piot-four-round}
    $\piotfourhyb$ statistically quantum stand-alone realizes $\idealot$ in the $\idealcom$-hybrid.
\end{theorem}

\begin{corollary}
    $\piotfourcomp$ statistically quantum stand-alone realizes $\idealot$ in the QROM with query-dependent simulation and using only 4 rounds of communication.
\end{corollary}
\begin{proof}
    We have from the above theorem that $\piotfourhyb$ statistically QSA realizes $\idealot$ in the $\idealcom$ hybrid, and also from Theorem~\ref{thm:rom-commitment} that $\picom$ statistically QSA realizes $\idealcom$ in the QROM with query-dependent simulation. Using Theorem~\ref{thm:malc-qrom-composition}, it then follows that $\piotfourcomp$ statistically QSA realizes $\idealot$ in the QROM with query-dependent simulation. 
    
    Note that $\picom$ (Figure~\ref{fig:idealcomm-protocol}) requires only a single round of communication during each of its commit and reveal phases. Hence, in the composed protocol $\piotfourcomp$ from Figure~\ref{fig:qot-4r-bb84-construction}, the following steps can be combined together and performed in one round since they all involve communication from $R$ to $S$ -  (steps~\ref{itm:4rqot-recv-first-msg-a} and~\ref{itm:4rqot-recv-first-msg-b}) and (steps~\ref{itm:4rqot-recv-third-msg-a} and~\ref{itm:4rqot-recv-third-msg-b}).
    
    Therefore, the composed protocol $\piotfourcomp$ involves 4 rounds of communication.
\end{proof}

\protocol
{\proref{fig:qot-4r-bb84-construction}, $\piotfourhyb$}
{QOT protocol $\piotfourhyb$ in the $\idealcom$ hybrid. $h : \zo^{k(\secp)} \times \zo^{\leq 7\secp} \rightarrow \zo^\secp$ is a universal hash function family with seed length $k(\secp)$. Steps marked out with \nblue{blue} indicate those which involve communication and those \textbf{black} indicate local computation.}
{fig:qot-4r-bb84-construction}
{

\begin{tabular}{ l l }
\textbf{Sender $S$ Input:} $m_0,m_1 \in \zo^\secp$ & \textbf{Receiver $R$ Input:} Bit $b \in \{0,1\}$ \\
 \textbf{Sender $S$ Output:} $\perp$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
\end{tabular}


\begin{enumerate}
\item 
\textbf{State preparation:} $R$ chooses $x \leftarrow \{0, 1\}^{16\secp}$, $\theta \leftarrow \{+, \times \}^{16\secp}$ and prepares the state $\ket{x}_{\theta}$.

\item \textbf{\nblue{Commitments}:}
    \begin{enumerate}
        \item \label{itm:4rqot-recv-first-msg-a}
        $R$ sends to $S$ the state $\ket{x}_{\theta}$.

        \item \label{itm:4rqot-recv-first-msg-b}
        $R,S$ then invoke $\idealcom$ with $R$ as committer and $S$ as receiver. $R$ sends $(\mathsf{Commit},(x_1,\theta_1, \ldots x_{16\secp},\theta_{16\secp}))$ to $\idealcom$ and $S$ receives $\mathsf{Receipt}$ from $\idealcom$.
    \end{enumerate}

\item \label{itm:4rqot-recv-second-msg} 
\textbf{\nblue{Measurements}:} $S$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{16\secp}$ and measures the received state $\ket{x}_\theta$ in basis $\widehat{\theta}$ to get measurement outcome $\widehat{x}$. It samples a set $T \leftarrow [16\secp]$ s.t. $|T|=8\secp$. It sends $T, \{\widehat{\theta}_i\}_{i \in \overline{T}}$ to $R$, where $\overline{T} \coloneqq [16\secp]\setminus T$.

\item 
\textbf{Opening preparation:} $R$ divides $\overline{T}$ into 2 disjoint subsets $S_0, S_1$ in the following way - $S_0 = \{ i | i \in \overline{T} \wedge \theta_i = \widehat{\theta}_i \}, S_1 = \{ i | i \in \overline{T} \wedge \theta_i \ne \widehat{\theta}_i \}$. It sets $I_b = S_0$ and $I_{1-b} = S_1$. It also sets $T' = \bigcup_{i \in T} (\text{indices of } x_i, \theta_i \text{ in the set } \{x_1, \theta_1 \ldots x_{16\secp}, \theta_{16\secp}\}) = \bigcup_{i \in T} \{2i-1,2i\}$. 

\item \textbf{\nblue{Openings}:}
    \begin{enumerate}
        \item \label{itm:4rqot-recv-third-msg-a}
        $R$ sends to $S$ the sets - $I_0,I_1$.
        \item \label{itm:4rqot-recv-third-msg-b}
        $R,S$ run the reveal phase of $\idealcom$ and $R$ sends $(\mathsf{Reveal},T')$ to $\idealcom$. $S$ receives $(\mathsf{Reveal},T',\{x_i,\theta_i\}_{i \in T})$ from $\idealcom$.
    \end{enumerate}

\item \label{itm:4rqot-sender-checks}
\textbf{Local checks:} $S$ then performs the following actions: 
    \begin{enumerate}
        \item \label{itm:4rqot-sender-checks-a}
        Abort if $T' \neq \bigcup_{i \in T}\{2i-1,2i\}$.
        
        \item \label{itm:4rqot-sender-checks-b}
        Abort if $|I_0|<\secp$ or $|I_1|<\secp$.
        
        \item \label{itm:4rqot-sender-checks-c}
        Abort if $\exists i \in T$ s.t. $\theta_i = \widehat{\theta}_i$ but $x_i \neq \widehat{x}_i$.
        
        % \item $\forall i \in T$, let $ \ket{\psi_i} = \ket{x_i}_{\theta_i}$ and measure the $i^{th}$ qubit received in Step~\ref{itm:4rqot-recv-first-msg} of the protocol in basis $\{\dyad{\psi_i}{\psi_i}, \bbI- \dyad{\psi_i}{\psi_i}\}$. If any of the measured outcomes don't match with $\dyad{\psi_i}{\psi_i}$, then abort.

        \item Choose $\widehat{s} \leftarrow \zo^{k(\secp)}$ and let $\widehat{x}_0$ be $\widehat{x}$ restricted to the set of indices in $I_0$ and $\widehat{x}_1$ be $\widehat{x}$ restricted to indices in $I_1$. Prepare the following message - \[\widehat{s}, ct_0 = m_0 \oplus h(\widehat{s} || \widehat{x}_0) ,ct_1 = m_1 \oplus h(\widehat{s} || \widehat{x}_1).\]
    \end{enumerate}

\item 
\textbf{\nblue{Chosen inputs}:} $S$ sends to $R$ the message prepared above - $\widehat{s},ct_0,ct_1$. $R$ sets $x_b$ as $x$ restricted to indices in $I_b$, computes $\widetilde{m_b} = ct_b \oplus h(\widehat{s} || x_b)$ and outputs $(b, \widetilde{m_b})$.

\end{enumerate}
}

We now prove Theorem~\ref{thm:piot-four-round} over the next two subsections.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Sender Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sender Security in $\piotfourhyb$}
In the following, we describe the simulator $\simurecv$ against a malicious receiver $\malrecv$. 

\begin{enumerate}
    \item \label{itm:4rqot-sender-security-sim-step1}
    $\simurecv(\brho)$ invokes $\malrecv(\brho)$ and waits to receive $16\secp$ qubits from $\malrecv$.
    
    \item It starts the commit phase of $\idealcom$ with $\malrecv$, simulating $\idealcom$ itself and intercepting $\malrecv$'s messages meant for it. It receives message $(\mathsf{Commit},(x_1,\theta_1, \ldots x_{16\secp},\theta_{16\secp}))$ from $\malrecv$.
    
    \item As in Step~\ref{itm:4rqot-recv-second-msg} of \proref{fig:qot-4r-bb84-construction} it chooses $\widehat{\theta} \leftarrow \zo^{16\secp}$ and measures all the received qubits in bases $\widehat{\theta}$ to get measurement outcome $\widehat{x}$. It also samples a random subset $T \leftarrow [16\secp]$ s.t. $|T|=8\secp$. It sends $T,\{\widehat{\theta}_i\}_{i \in \overline{T}}$ to $\malrecv$, where $\overline{T} \coloneqq [16\secp]\setminus T$.
    
    \item It receives $(I_0,I_1)$ from $\malrecv$, where $I_0 \subseteq \overline{T}$ and $I_1 = \overline{T}\setminus I_0$. It invokes the reveal phase of $\idealcom$ with $\malrecv$. It receives message $(\mathsf{Reveal},T')$ from $\malrecv$.
    
    \item It performs the checks as in Steps~\ref{itm:4rqot-sender-checks-a},~\ref{itm:4rqot-sender-checks-b} and~\ref{itm:4rqot-sender-checks-c} of \proref{fig:qot-4r-bb84-construction} - i.e. it checks $T' = \bigcup_{i \in T}\{2i-1,2i\}$, if $|I_0|,|I_1| \geq \secp$ and if $\forall i \in T$, whether whenever $\theta_i=\widehat{\theta}_i$ if $x_i=\widehat{x}_i$. If any check fails, it stops and outputs the state of $\malrecv$.

    \item \label{itm:4rqot-simurecv-bset}
    It finds the set $Q = \{i : i \in I_0 \wedge \theta_i \neq \widehat{\theta}_i\}$. If $|Q| \geq 3\secp/2$, then it sets $b=1$, else it sets $b=0$.
    
    \item It sends $b$ to $\idealot$ and receives back $m_b$ in return. It sets $m_{1-b}=0^\secp$, samples $\widehat{s} \leftarrow \zo^{k(\secp)}$ and computes \[ct_b = m_b \oplus h(\widehat{s}||\{\widehat{x}_i\}_{i \in I_b}), ct_{1-b} = m_{1-b} \oplus h(\widehat{s}||\{\widehat{x}_i\}_{i \in I_{1-b}})\] It sends $\widehat{s},ct_0,ct_1$ to $\malrecv$ and outputs whatever it outputs.
    
\end{enumerate}

To argue real/ideal indistinguishability, first consider a hybrid world $\Hyb$, where $\simurecv(\brho)$ runs $\malrecv(\brho)$ as in the real world, but simulating $\idealcom$ for it, i.e. it now intercepts the message $(\mathsf{Commit},(x_1,\theta_1, \ldots x_{16\secp},\theta_{16\secp}))$ and $(\mathsf{Reveal},T')$ from $\malrecv$. $\Hyb \equiv $ the real world, since the view of $\malrecv$ in either case is identical. 

To argue why $\Hyb \approx_s $ ideal world, note that the view of $\malrecv$ in the two worlds are the same, except that in the ideal world, $\simurecv$ sets $m_{1-b} = 0^\secp$, for $b$ which it decides in Step~\ref{itm:4rqot-simurecv-bset}. Therefore, we need to aruge that $ct_{1-b}$ looks like a uniformly random string to $\malrecv$ in either worlds. We do this by making use of the quantum sampling lemma~\cite{C:BouFeh10,BCKM2021}.

\paragraph{Quantum Sampling~\cite{C:BouFeh10,BCKM2021}}
Consider the following interaction between a player $P$ and a challenger $C$.
\begin{enumerate}
    \item $P$ prepares an arbitrary quantum state $\ket{\psi}_{\gray{X}\gray{Y}}$ where $\gray{X}$ is a $2n$-qubit register and $\gray{Y}$ is an arbitrary-sized register of $P$'s choice. It sends the contents of $\gray{X}$ to $C$ along with two length-$2n$ classical strings ${x} \in \{0,1\}^{2n}$ and ${\theta} \in \{+,\times\}^{2n}$.
    
    \item \label[step]{step:check-T} $C$ samples a uniformly random set of $n$ indices $T \subset [2n]$ as well as a uniformly random $\widehat{\theta} \in \{+,\times\}^{2n}$.
    For each $i \in T$, it measures the $i^{th}$ qubit of $\gray{X}$ in basis $\widehat{\theta}_i$. If there exists $i \in T$ s.t. $\theta_i=\widehat{\theta}_i$ but $x_i \neq \widehat{x}_i$, then $C$ aborts the experiment and outputs $\bot$. Otherwise, it sends $\overline{T}, \{\widehat{\theta}_i\}_{i \in \overline{T}}$ to $P$, where $\overline{T} \coloneqq [2n]\setminus T$.
    
    \item $P$ responds with a subset $S \subseteq \overline{T}$. 
    
    \item\label[step]{step:measure} $C$ measures the indices of $\gray{X}$ specified by $S$, obtaining a length-$|S|$ bitstring $\widehat{X}_S$ of measurement outcomes; let $s$ denote the number of indices $i \in S$ where $\theta_i \neq \widehat{\theta}_i$.
\end{enumerate}

\nishant{ask to correct the typos in BCKM20 so that we can defer the proof to there?}

\begin{lemma}[\cite{C:BouFeh10} Quantum Sampling Lemma]
\label{lemma:sampling}
For any computationally unbounded player $P$ and a constant $0 < \varepsilon < 1$, the probability the sampling experiment does not abort and
\[ \mathbf{H}_{\infty}(\widehat{X}_S \mid \gray{X}_{\bar{S}}, \gray{Y}) \leq s- \varepsilon \cdot |S|. \]
is at most $\negl(|S|^2/n)$.
\end{lemma}
Since we make use of exactly the same sampling lemma, we refer the reader to~\cite{BCKM2021} for the proof of the above.

We now use the above lemma to argue $ct_{1-b}$ is a uniformly random string from $\malrecv$'s view in both $\Hyb$ and ideal world, and hence, $\Hyb \approx_s $ ideal world. Note that the above quantum sampling game exactly captures the interaction in our hybrids with register $\gray{X}$ denoting the $16\secp$ qubits sent by $\malrecv$ and received by $\simurecv$, and $\gray{Y}$ denoting the residual state of $\malrecv$. Setting some notation, for any set $A \subseteq [16\secp]$, let $wt(A) \coloneqq |\{i : i \in A \wedge \theta_i \neq \widehat{\theta}_i\}|$ and let $\widehat{X}_A = \{\widehat{x}_i\}_{i \in A}$. 
We have two cases then : 
\begin{enumerate}
    \item If $wt(I_0) \geq 3\secp/2$, the set $S$ in the quantum sampling game is set as $I_0$. By the quantum sampling lemma then, $\mathbf{H}_{\infty}(\widehat{X}_{I_0} \mid \widehat{X}_{I_1},\gray{Y}) \geq \mathbf{H}_{\infty}(\widehat{X}_{I_0} \mid \gray{X}_{I_1}, \gray{Y}) > wt(I_0) - \varepsilon |I_0| = 3\secp/2 - \varepsilon |I_0|$ \nishant{what is the quantum lemma being used to argue the first inequality - i.e. that entropy always increases on measurement - whats the citation?} except with probability $negl(|I_0|^2/\lambda)$. Since $\secp \leq |I_0| \leq 7\secp$ if the game didn't abort, setting $\varepsilon$ appropriately, we then have that $\mathbf{H}_{\infty}(\widehat{X}_{I_0} \mid \widehat{X}_{I_1},\gray{Y}) > 1.4\secp$, except with probability $negl(\lambda)$. Invoking the leftover hash lemma (Lemma~\ref{thm:privacy-amplification}), we then have that $(\widehat{s},h(\widehat{s},\widehat{X}_{I_0}))$ is statistically close to a uniformly random string from $\malrecv$'s view.
    
    \item If $wt(I_0) < 3\secp/2$, (since $\widehat{\theta}$ was sampled uniformly by $\simurecv$ from $\zo^{16\secp}$), using Hoeffding's inequality, except with negl probability, $wt(I_1) > 3\secp/2$ and the same argument as above works but showing that $\mathbf{H}_{\infty}(\widehat{X}_{I_1} \mid \widehat{X}_{I_0},\gray{Y}) > 1.4\secp$ except with probability $negl(\secp)$. Invoking the leftover hash lemma (Lemma~\ref{thm:privacy-amplification}) as before, $(\widehat{s},h(\widehat{s},\widehat{X}_{I_1}))$ is statistically close to uniformly random string from $\malrecv$'s view.
\end{enumerate}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Receiver Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Receiver Security in $\piotfourhyb$}

\nishant{Todo on Amit to update this section to be consistent with the updated protocol and updated MPC framework}
We first describe the construction of our simulator for a malicious sender $S^*$. In what we describe, $\simu$ will take control of the $\idealcom$ and will answer queries on its behalf to $S^*$. %We assume the following interface for an ideal commitment malicious receiver simulator: i) $\simu.Commit()$ - Generates a commitment string $c$, ii) $\simu.Reveal(c, v)$ - Generates the decommitment message for commitment string $c$ and plaintext value $v$.
%\james{talked to Amit about this: we don't need explicit algorithms here, the OT simulator should simply be controlling the commitment ideal functionality}


$\simu$:

\begin{enumerate}
    \item Prepare $[16 \secp]$ EPR pairs $\{ \ket{\phi^+}^{SR}_i \}_{i \in [16 \secp]}$ where $\ket{\phi^+}^{SR} = \frac{\ket{00} + \ket{11}}{\sqrt{2}}$. Send first half of each EPR pair and $\idealcom$ receipt message $(Receipt, R, S^*)$ to $S^*$.
    
    \item Receive $T, \{ \widehat{\theta_i} \}_{i \in \overline{T}}$ from $S^*$.
    
    \item For all $i \in T$, sample $\theta_i \leftarrow \{+, \times \}$ and measure the second half of each $\ket{\phi^+}^{SR}_i$ in the basis $\theta_i$ to obtain outcome $x_i$. Use $\{ x_i, \theta_i \}_{i \in T}$ to prepare the openings.
    
    For all $i \in \overline{T}$, sample $\theta_i \leftarrow \{+, \times \}$ and use it to prepare the sets $S_0, S_1$ as per the honest receiver strategy i.e. $S_0 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} = \theta_i \}, S_1 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} \ne \theta_i \}$. Set $I_0 := S_0$ and $I_1 := S_1$.
    
    Finally, send $(I_0, I_1)$, and $\idealcom$ Reveal message $(Reveal, R, S^*, \{x_i, \theta_i\}_{i \in T})$ to $S^*$.
    
    \item On receiving $\widehat{s}, y_0, y_1$ from $S^*$:
    
    \begin{itemize}
        \item For all $i \in \overline{T}$, measure the second half of each $\ket{\phi^+}^{SR}_i$ in the basis $\widehat{\theta_i}$ (received from $S^*$ in Round 2) to obtain outcome $\widetilde{x_i}$.
        \item Compute $\widetilde{m_0} = y_0 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_0})$
        \item Compute $\widetilde{m_1} = y_1 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_1})$
        \item Send $\widetilde{m_0}, \widetilde{m_1}$ to the OT ideal functionality
    \end{itemize}
\end{enumerate}

Having defined the $\simu$, we will now show that the real distribution is indistinguishable from the ideal distribution using a sequence of hybrids. In our sequence, $\Hyb_0$ will correspond to the real distribution and the last hybrid, $\Hyb_6$, will correspond to the ideal simulated distribution. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             Real        Hyb1                Hyb2                Hyb3                     Hyb4                            Hyb5                     Hyb6
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%                                         EPR-to-BB84
% --------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Round 1             Ideal Com           
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Round 2
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%                                                             Delay measure T
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Round 3             Ideal Open                              Open measured T
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
% Round 4
% ---------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%                                                                                     Delay measure T'         Extract and send               Remove receiver choice bit
%                                                                                                             m0 and m1 to ideal func.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\begin{itemize}{
    \item $\Hyb_0:$ This corresponds to the Real World. The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
%    \item $\Hyb_1:$ We introduce a commitment receiver $R_{\com}$ for the ideal commitment $\idealcom$ which sits between whose task is to receive messages from $\idealcom$ and the forward it to $S^*$. 
    
    \item $\Hyb_1$ [\textbf{$\simu$ controls $\idealcom$}]: Same as the previous hybrid except that the simulator takes control of $\idealcom$ functionality and answers its queries towards $S^*$. However, the way in which $\simu$ answers these queries is no different from how the queries was answered by $\idealcom$ functionality in the previous hybrid.
    
    
    %Instead of running the honest commitment strategy, we will invoke the simulator for a malicious receiver in the Ideal Commitment model. The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    %Before doing so, we first define a commitment receiver $R_{\com}$ for the ideal commitment $\idealcom$ whose task is to receive messages from $\idealcom$ and the forward it to $S^*$. 
    
    %In the reveal phase, the ideal commitment simulator would reveal exactly what an honest committer in the previous hybrid would have revealed. 
    %\amit{Define a malicious receiver for the ideal commitment (using a part of the malicious OT sender - build a wrapper) and invoke the ideal commitment simulator for this malicious commitment receiver}
    
    \item $\Hyb_2 [\textbf{Switching BB84 to EPR pair}]:$ Same as the previous hybrid except the following change: In Step 1, $\simu$ prepares each BB84 states using Algorithm EPR-to-BB84 i.e. For all $i \in [16 \secp]$, run Algorithm EPR-to-BB84$(i)$ to obtain $\ket{x_i}_{\theta_i}$.  The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
    \textbf{Algorithm EPR-to-BB84 $(i)$:}
    \begin{enumerate}
        \item Sample an EPR pair $\ket{\phi^+}^{SR}_i = \frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$
        \item Randomly sample a basis $\theta_i \leftarrow \{+, \times\}$
        \item Measure only second half of the EPR pair, i.e. System R of $\ket{\phi^+}^{SR}_i$, in the basis $\theta_i$ and let the outcome be $x_i$
        \item Use the first half of the post measurement state of $\ket{\phi^+}^{SR}_i$, i.e. System S , as a BB84 state $\ket{x_i}_{\theta_i}$
    \end{enumerate}
    
    It can be shown that the first half of the EPR pair collapses to one of the following four quantum states with uniform probaility : $\{ \ket{0}, \ket{1}, \ket{+}, \ket{-} \}$. This exactly matches the description of a valid single qubit BB84 state.
    
    
    \item $\Hyb_3$ [\textbf{Delayed Measurement of $T$}]: Same as the previous hybrid, except Step 2 and 3 of Algorithm EPR-to-BB84 is performed after Round 2 of the protocol for all $i \in T$. Use the $\{x_i, \theta_i \}_{i \in T}$ so obtained (as a result of performing Step 2 and Step 3 of Algorithm EPR-to-BB84) exactly as they would have been used in the previous hybrid to perform the opening in Protocol Round 5 (by answering $\idealcom$ Reveal query using  $\{x_i, \theta_i \}_{i \in T}$ towards $S^*$).  The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
    \amit{An efficient $\simu$ can't selectively delay only the measurement of challenge set $T$. In other words, an efficient $\simu$ will have to delay the measurement of both $T$ and $\overline{T}$ because $T$ is unknown in Step 1. However, since this is just a hybrid, it might be fine to do so - Check this}
    % \amit{\begin{itemize}
    %     \item For challenge set $T$, the situation is exactly similar to previous hybrid because $S$ has not measured his part of the BB84 state.
    %     \item For the non-challege set $T$, approximately half of the $\theta$ sampled by $\simu$ would match the $\widehat{\theta}$ sampled by $S$ in Step 2 of the protocol. The places where $\theta$ and $\widehat{\theta}$ match are also the places where the sender measurements $\widehat{x}$ and $\simu$ measurements $x$ would also exactly match (by virtue of EPR pair, or a different way to think about this is to imagine $S$ sending BB84 states to $\simu$ by performing Step 2-4 of Algorithm EPR-to-BB84 on $S$ side)
    % \end{itemize}}
    
    % \amit{The density matrix on malicious sender side will be same in both hybrids because the measurement outcomes }
    
    
    \item $\Hyb_4$ [\textbf{Delayed Measurement of $\overline{T}$}]: Same as the previous hybrid, except for the following change: For non-challenge set $\overline{T}$, instead of measuring in a randomly sampled basis (as dictated by Step 3 of Algorithm EPR-to-BB84), delay the measurement until Step 7 of the protocol. Note that for all $i \in \overline{T}$, $\simu$ still samples random $\theta_i \leftarrow \{+, \times\}$ in Algorithm EPR-to-BB84 and uses it to define the sets $S_0, S_1$ in QOT protocol Step 4 as prescribed. 
    
    On receiving $ct_0$, $ct_1$ from $S^*$ in Protocol Step 7, for all $i \in \overline{T}$, measure second half of EPR pairs in the basis $\{ \widehat{\theta} \}_{i \in \overline{T}}$ sent by $S$ in Step 3 and let the outcomes be $\{ \widetilde{x_i} \}_{i \in \overline{T}}$. Use $\{ \widetilde{x_i} \}_{i \in I_b}$ in Step 7 to compute $\widetilde{m_b}$ as $\widetilde{m_b} := ct_b \oplus h(\widehat{s} || \{\widetilde{x}_i\}_{i \in I_b})$.  The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
    %i.e. set $\{ \theta \}_{i \in \overline{T}} := \{ \widehat{\theta} \}_{i \in \overline{T}}$
    
  %  \amit{Define $I_0$ and $I_1$ for this }
    
    % \amit{\begin{itemize}
    %     \item This will ensure that the measurment outcomes $\{x_i\}_{i \in \overline{T}}$ exactly match $\{\widehat{x_i}\}_{i \in \overline{T}}$ conditioned on the $S$ sending the right basis $\widehat{\theta}$ i.e. $S$ is sending the exact same basis in which he measured the $\overline{T}$ qubits
    %     \item A malicious sender $S$ who sends the incorrect basis $\widehat{\theta}$ is not really an issue - because in the case, the real-world receiver will not receive the correct message as OT output, so it is fine in ideal world for the simulator to also fail at extracting the correct messages.
    % \end{itemize}
    % }
    
    
    \item $\Hyb_5 [\textbf{OT sender message extraction}]:$ Same as the previous hybrid, except for the following change: Instead of performing step 7 of the protocol, perform the following steps on receiving $\widehat{s}, ct_0, ct_1$ from $S^*$:
    
    \begin{itemize}
        \item Compute $\widetilde{m_0} = ct_0 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_0})$
        \item Compute $\widetilde{m_1} = ct_1 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_1})$
        \item Send $\widetilde{m_0}, \widetilde{m_1}$ to the OT ideal functionality
    \end{itemize}
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.
    
    
    \item $\Hyb_6 [\textbf{Removing the receiver choice bit}]:$  $\simu$ behaves exactly as $\Hyb_5$ except that in Step 4, instead of using $b$ to define the sets $I_0$ and $I_1$, it instead sets $I_0 := S_0$ and $I_1 := S_1$. It then completes the remaining steps as mentioned in the previous hybrid.
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.
   
}
    
\end{itemize}


We will now argue the computational indistinguishability of each pair of consecutive hybrids in the above sequence.


\begin{itemize}

    \item $\Hyb_0 \approx_c \Hyb_1:$ Follows from the computational sender security of the ideal commitment. \amit{Should composition theorem be invoked to argue this indistinguishability ?}
    \dakshita{write a reduction; i.e. an adversary $\cA$ that breaks the equivocality game}
    
    \item $\Hyb_1 = \Hyb_2:$ Follows from the fact that the distribution of the BB84 states in $\Hyb_1$ is identical to the distribution of BB84 states obtained via EPR-to-BB84 algorithm in $\Hyb_2$.
    
    Suppose the basis $\theta_i$ selected in Step 2 of Algorithm EPR-to-BB84 is the computational basis $+$. Then, Step 3 corresponds to applying the projector set $\{ \identity^S \otimes \ketbra{0}{0}^R, \identity^S \otimes \ketbra{1}{1}^R \}$ on $\ket{\phi^+}^{SR}$. Then the post measurement state $\ket{\omega}^{SR}_{\theta = +}$ can be described as follows:
    \[
        \ket{\omega}^{SR}_{\theta = +} = 
    \begin{cases}
        \ket{00}^{SR},& \text{with probability} \frac{1}{2}\\
        \ket{11}^{SR},& \text{with probability} \frac{1}{2}
    \end{cases}
    \]
    
    If the basis $\theta_i$ selected in Step 2 of Algorithm EPR-to-BB84 is the Hadamard basis $\times$, then Step 3 corresponds to applying the projector set $\{ \identity^S \otimes \ketbra{+}{+}^R, \identity^S \otimes \ketbra{-}{-}^R \}$ on $\ket{\phi^+}^{SR}$. Then the post measurement state $\ket{\omega}^{SR}_{\theta = \times}$ can be described as follows:
    \[
        \ket{\omega}^{SR}_{\theta = \times} = 
    \begin{cases}
        \ket{++}^{SR},& \text{with probability} \frac{1}{2}\\
        \ket{--}^{SR},& \text{with probability} \frac{1}{2}
    \end{cases}
    \]
    
    Combining the above two cases with the classical probability of selecting the basis $\theta_i$, the desity matrix of the final post measurement state in Step 4 of Algorithm EPR-to-BB84 can be described as follows:
    \begin{align*}
        \rho^{SR} &= \frac{1}{4} \ketbra{00}{00} + \frac{1}{4} \ketbra{11}{11} + \frac{1}{4} \ketbra{++}{++} + \frac{1}{4} \ketbra{--}{--}\\
    \end{align*}
    
    Now the partial desity matrix for the System $S$ can be computed by tracing out System $R$ as follows:
    
    \begin{align*}
        \rho^S &= \Tr_R[\rho^{SR}] = \Tr_R[\frac{1}{4} \ketbra{00}{00} + \frac{1}{4} \ketbra{11}{11} + \frac{1}{4} \ketbra{++}{++} + \frac{1}{4} \ketbra{--}{--}]\\
        &= \frac{1}{4} (\ketbra{0}{0} + \ketbra{1}{1} + \ketbra{+}{+} + \ketbra{-}{-}) = \frac{\identity}{2}\\
    \end{align*}
    
    Hence, the partial density matrix on the malicious sender side is identical to the previous hybrid where $S^*$ was receiving actual BB84 states. Therefore the view of $S^*$ in $\Hyb_2$ is identical to $\Hyb_1$.


    \item $\Hyb_2 = \Hyb_3:$ Follows from the fact that the measurement operations (i.e. Step 2 and Step 3 of Algorithm EPR-to-BB84) applied by the simulator on the second halves of EPR pairs in set $T$ are completely independent of any action performed by the adversary in both the hybrids. Hence the output distribution of measurement outcomes of the second halves of EPR pairs in set $T$ is identical between the two hybrids.

    \item $\Hyb_3 = \Hyb_4:$ Note that the transcript distribution is identical in both hybrids because the information about operations performed on second EPR halves for all $i \in \overline{T}$ is never used anywhere in the protocol except the last Step 7 (which is local to the receiver). Hence, all we need to show is that the output distribution of $R$ doesn't change. This follows from the fact the distribution of $\{ x_i \}_{i \in I_b}$ in $\Hyb_3$ is identical to the distribution of $\{ \widetilde{x_i} \}_{i \in I_b}$ in $\Hyb_4$. Hence the distribution of receiver's output $\widetilde{m_b}$ is identical in $\Hyb_3$ and $\Hyb_4$.
    
    
    \item $\Hyb_4 = \Hyb_5:$ Note that there is no difference in these hybrids with respect to the simulation of $S^*$ view. The only difference is in how we define the output of the honest receiver. In $\Hyb_4$, the receiver's output is computed by the simulator as $\widetilde{m_b} := ct_b \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_b})$. In $\Hyb_5$, the receiver's output is derived via the OT ideal functionality which receives sender's input strings $(\widetilde{m_0} := ct_0 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_0}), \widetilde{m_1} := ct_1 \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_1}))$ from the $\simu$ and ideal-world receiver choice bit $b$. The OT ideal functionality sends $\widetilde{m_b} := ct_b \oplus h(\widehat{s} || \{ \widetilde{x_i} \}_{i \in I_b})$ to the ideal world receiver which it then outputs. Hence, the output distribution of the receiver is identical in both the hybrids.
    
    % Correctness of the extraction procedure follows from the EPR measurement correlation property on set $\overline{T}$.
    % \amit{Handle the case where $x_i$}
    
    % \amit{The definition of $I_b$ is not changing between two hybrids and so $m_b$ would not change}
    
    
    \item $\Hyb_5 =\Hyb_6:$ We first observe that the distribution of $S_0 = S_1$ as long as $\{ \theta_i \}_{i \in \overline{T}}$ is private (which is in fact the case from the point of view of malicious sender and the distinguisher). This is because $\{ \theta_i \}_{i \in \overline{T}}$ is sampled uniformly at random, and hence $\{ S_0, S_1 \}$ form a uniformly random partition of the set $\overline{T}$. Hence, the distribution of $(S_0, S_1)$ is identical to $(S_1, S_0)$.

    Note that the protocol transcript contains $(I_0, I_1)$ which would be equal to $(S_b, S_{1-b})$ for an honest receiver strategy (and hence also for $\simu$ strategy until $\Hyb_5$). However, for the $\simu$ strategy in $\Hyb_6$, $(I_0, I_1)$ is always equal to $(S_0, S_1)$. Hence, if $b = 0$, the distribution of $(I_0, I_1)$ in $\Hyb_5$ would be identical to $\Hyb_6$. On the other hand, if $b = 1$, the distribution of $(I_0, I_1)$ in $\Hyb_5$ would be perfectly indistinguishable from $\Hyb_6$ (following from the fact that the distribution of $(S_0, S_1) = (S_1, S_0)$). Putting together these two observations, it easily follows that $\Hyb_5 = \Hyb_6$.
\end{itemize}

==> old_rom_commit.tex <==
\section{Old Equivocal and extractable commitments in the QROM}
\label{sec:oldeecom}

In this section, we define and construct non-interactive equivocal and extractable commitments in the quantum random oracle model.

\subsection{Definition}

We first define a non-interactive bit commitment scheme with selective opening in the quantum random oracle model. Such a scheme consists of a commit algorithm $\Commit^H$, an open algorithm $\Open^H$, and a receive algorithm $\Rec^H$, each with access to a random oracle $H$.\footnote{In our scheme, these algorithms will be entirely classical, and in particular will only need to query $H$ classically.} The scheme is parameterized by a polynomial $n = n(\secp)$ which determines the number of bits to be committed. The algorithms have the following syntax.

\begin{itemize}
    \item $\Com^H(1^\secp,\{b_i\}_{i \in [n]}) \to (\state,\{\com_i\}_{i \in [n]})$. The commit algorithm takes as input the security parameter $1^\secp$ and $n$ bits $\{b_i\}_{i \in [n]}$, and outputs a committer state $\state$ and a set of commitments $\{\com_i\}_{i \in [n]}$.
    \item $\Open^H(\state,T) \to \{b_i,r_i\}_{i \in T}$. The open algorithm takes as input the committer state $\state$ and a subset $T \subseteq [n]$ and outputs a set of openings $\{b_i,r_i\}_{i \in T}$.
    \item $\Rec^H(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T}) \to \{\{b_i\}_{i \in T}, \bot\}$. The receive algorithm takes as input a set of commitments $\{\com_i\}_{i \in [n]}$ and a set of openings $\{b_i,r_i\}_{i \in T}$ and outputs either the bits $\{b_i\}_{i \in T}$ or $\bot$.
\end{itemize}

\begin{definition}\label{def:extractable}
A non-interactive bit commitment scheme with selective opening, parameterized by $n = n(\secp)$, is \emph{extractable in the QROM} if for any function $q(\secp)$, there exists a stateful simulator $\cS_\Ext \coloneqq \cS_\Ext[q(\secp)]$, such that for any non-uniform family of quantum oracle algorithms $\{\rho_\secp,\cA_\secp = (\cA_{\Commit,\secp},\cA_{\Open,\secp},\cA_{\Dist,\secp}))\}_{\secp \in \bbN}$ where  $q(\secp)$ is an upper bound on the number of oracle queries $\cA_\secp$ makes, and where for any $T \coloneqq \{T_\secp \subseteq [n(\secp)]\}_{\secp \in \bbN}$, it holds that (where the state of $\cS_\Ext$ is kept implicit in the following)

\begin{align*}\bigg|&\Pr_{H}\left[\cA_{\Dist,\secp}^H(\rho_\out,R_\out) = 1: \begin{array}{r}(\rho_\state,\{\com_i\}_{i \in [n]}) \gets \cA_{\Commit,\secp}^H(\rho_\secp)\\ (\rho_\out,\{b_i,r_i\}_{i \in T}) \gets \cA_{\Open,\secp}^H(\rho_\state,T) \\ R_\out \gets \Rec^H(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T})\end{array}\right]\\
&-\Pr\left[\cA_{\Dist,\secp}^{\cS_\Ext}(\rho_\out,R_\out) = 1: \begin{array}{r}(\rho_\state,\{\com_i\}_{i \in [n]}) \gets \cA_{\Commit,\secp}^{\cS_\Ext}(\rho_\secp)\\ \{b_i^*\}_{i \in [n]} \gets \cS_\Ext(\{\com_i\}_{i \in [n]}) \\ (\rho_\out,\{b_i,r_i\}_{i \in T}) \gets \cA_{\Open,\secp}^{\cS_\Ext}(\rho_\state,T) \\ R_\out \gets \Rec^H(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T}) \\ R_\out \coloneqq \mathsf{FAIL} \text{ if } R_\out \notin \{\{b_i^*\}_{i \in T},\bot\}\end{array}\right]\bigg| = \negl(\secp).
\end{align*}

\end{definition}

\begin{definition}\label{def:equivocal}
A non-interactive bit commitment scheme with selective opening, parameterized by $n = n(\secp)$, is \emph{equivocal in the QROM} if for any function $q(\secp)$, there exists a stateful simulator $\cS_\Equ \coloneqq \cS_\Equ[q(\secp)]$, such that for any non-uniform family of algorithms $\{\rho_\secp,\cA_{\Rec,\secp}\}_{\secp \in \bbN}$ where $\cA_{\Rec,\secp}$ makes at most $q(\secp)$ oracle queries, and any $\{b_i\}_{i \in [n]} \coloneqq 
%\{T_\secp \subseteq [n(\secp)],
\{b_{i,\secp}\}_{i \in [n],\secp \in \bbN}$, it holds that  (where the state of $\cS_\Equ$ is kept implicit in the following) 

\begin{align*}
    \bigg|&\Pr_H\left[\cA_{\Rec,\secp}^H(\rho_\secp,\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}) = 1 : \begin{array}{r}(\state,\{\com_i\}_{i \in [n]}) \gets \Com^H(1^\secp,\{b_i\}_{i \in [n]}) \\ \{b_i,r_i\}_{i \in [n]} \gets \Open^H(\state) \end{array}\right] \\
    &-\Pr\left[\cA_{\Rec,\secp}^{\cS_\Equ}(\rho_\secp,\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}) = 1: \begin{array}{r}\{\com_i\}_{i \in [n]} \gets \cS_\Equ(1^\secp) \\ \{b_i,r_i\}_{i \in [n]} \gets \cS_\Equ(\{b_i\}_{i \in [n]})\end{array}\right] \bigg| = \negl(\secp).
\end{align*}

\end{definition}



%\subsection{Old definition}

%We first define the ideal functionality $\idealcom$ for secure bit commitment with selective opening in \figureref{fig:idealcomm-func}. This ideal functionality was also used in~\cite{GLSV}. Then, we give a protocol in the QROM ($\picom$, \proref{fig:idealcomm-protocol}) that statistically QOSA implements the functionality $\idealcom$. 

%\begin{theorem}
    %\label{thm:rom-commitment}
    %$\picom$ statistically quantum oracle stand-alone realizes %$\idealcom$ in the QROM with query-dependent simulation.
%\end{theorem}

%We provide the proof of this theorem in the following subsections, where we provide simulators against malicious receivers and malicious committers.

\protocol
{$\idealcom$}
{Ideal functionality for bit commitment with selective opening}
{fig:idealcomm-func}
{
Parameters : security parameter $\secp$, number of commitments $n(\secp)$\\
Parties : Committer $C$, Receiver $R$

\begin{itemize}
    \item \textbf{Commit Phase}: $C$ sends a query $(\mathsf{Commit},(m_1,m_2, \ldots m_{n(\secp)}))$ to $\idealcom$, where each $m_i \in \zo$. $\idealcom$ records $(m_1,m_2, \ldots m_{n(\secp)})$ and sends $\mathsf{Receipt}$ to $R$.
    
    \item \textbf{Reveal Phase}: $\idealcom$ receives a query $(\mathsf{Reveal},I)$ from $C$, where $I \subseteq [n(\secp)]$. If no $(m_1,m_2, \ldots m_{n(\secp)})$ is recorded, then it ignores the message, else it sends $(\mathsf{Reveal},I,\{m_i\}_{i \in I})$ to $R$.
    
    \amit{The previous statement is unclear, what does ``no $(m_1,m_2, \ldots m_{n(\secp)})$ is recorded'' mean - is it all the $m$'s or atleast one of the $m$'s ? Also, I think it should rather be checking just whether the indices in set $I$ are recorded (instead of checking $[n(\secp)]$)}
\end{itemize}
}

\protocol
{\proref{fig:idealcomm-protocol}, $\picom$}
{Protocol $\picom$ for implementing bit commitment functionality $\idealcom$ in QROM}
{fig:idealcomm-protocol}
{
Parties : Committer $C$, Receiver $R$\\
Random Oracles : $H:\zo^{\secp+1} \rightarrow \zo^{\secp+1}, G:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$

\begin{itemize}
    \item \textbf{Commit Phase}
    
    $C(m_1,m_2 \ldots m_{n(\secp)}), R(\bot)$: $C$ chooses $r_i \leftarrow \zo^\secp, \forall i \in [n(\secp)]$ and sends $\{c_1^i = H(m_i||r_i), c_2^i = G(m_i||r_i)\}_{i \in [n(\secp)]}$ to $R$. $C$ outputs $\{m_i,r_i\}_{i \in [n(\secp)]}$, and $R$ outputs $\{c_1^i,c_2^i\}_{i \in [n(\secp)]}$.
    
    \item \textbf{Reveal Phase} 
    
    $C(I,\{m_i,r_i\}_{i \in [n(\secp)]}), R(\{c_1^i,c_2^i\}_{i \in [n(\secp)]})$: $C$ sends $(I,\{m_i,r_i\}_{i \in I})$ to $R$. $R$ sets $J = \emptyset$ and for each $i \in I$, if $H(m_i||r_i)=c_1^i \wedge G(m_i||r_i) = c_2^i$, it sets $J = J \cup \{i\}$. $R$ outputs $J,\{m_j\}_{j \in J}$, and $C$ outputs $\bot$.
\end{itemize}
}

\subsection{Committer Security}
For every malicious receiver $\malrecv$ and bound on the environment's total oracle queries as $q_\cZ$, we define a simulator $\simu[\malrecv,q_\cZ]$, which takes input $\brho$ and performs the following actions: (we use shorthand $\simurecv$ for $\simu[\malrecv,q_\cZ]$)

\begin{enumerate}
    \item If $q_{\malrecv}$ is a bound on the total number of oracle queries by $\malrecv$, $\simurecv$ sets $q = q_\cZ+q_\malrecv$. It then chooses $r_i \leftarrow \zo^\secp, \forall i \in [n]$, and samples hash functions $h_{H},h_{G}$, at random from a $2q$-wise independent hash function family. It uses $h_H,h_G$ to answer oracle queries to $H,G$ below. It invokes $\malrecv(\brho)$ giving it access to the following two oracles: 
        \begin{itemize}
            \item $\puncrom{H}$: defined as $\puncrom{H}(\cdot) = H(\cdot)$ except $\forall i \in [n], \puncrom{H}(\cdot||r_i)$ is remapped to a fresh random value, i.e. $\puncrom{H}(0||r_i) = r^{H,i}_0$ and $\puncrom{H}(1||r_i) = r^{H,i}_1$, where $r^{H,i}_0,r^{H,i}_1 \leftarrow \zo^{\secp+1}$.
            \item $\puncrom{G}$: Similarly, $\puncrom{G}(\cdot) = G(\cdot)$ except $\forall i \in [n], \puncrom{G}(0||r_i) = r^{G,i}_0$ and $\puncrom{G}(1||r_i) = r^{G,i}_1$, where $r^{G,i}_0,r^{G,i}_1 \leftarrow \zo^{\secp+1}$.
        \end{itemize}
    
    Concretely, $\simurecv$ creates a circuit wrapper over $h_H,h_G$ to do this and answers the queries of $\malrecv$.
    
    \item \label{itm:romcom-comm-sec-sampleci}
    On receiving $\mathsf{Receipt}$ from $\idealcom$, it chooses $c^H_i, c^G_i \leftarrow \zo^{\secp+1}, \forall i \in [n]$ and sends $\{c^H_i,c^G_i\}_{i \in [n]}$ to $\malrecv$. 
    
    \item On receiving $(\mathsf{Reveal},I,\{m_i\}_{i \in I})$ from $\idealcom$, it does the following: 
        \begin{itemize}
            \item It defines $\puncrom{H}_R,\puncrom{G}_R$ as:
                \begin{itemize}
                    \item $\puncrom{H}_R(\cdot) = {H}(\cdot)$, except $\forall i \in I,\puncrom{H}_R(m_i||r_i) = c^H_i$.

                    \item $\puncrom{G}_R(\cdot) = {G}(\cdot)$, except $\forall i \in I,\puncrom{G}_R(m_i||r_i) = c^G_i$.

                \end{itemize}
                Concretely, to define $\puncrom{H}_R,\puncrom{G}_R$, it defines a circuit wrapper over ${H}$ and ${G}$ which does the required remapping of inputs.
                
            \item It runs the Reveal phase with $\malrecv$, but now answering its RO queries using $\puncrom{H}_R,\puncrom{G}_R$, and providing $I,\{m_i,r_i\}_{i \in I}$ to $\malrecv$.
        \end{itemize}
    
    \item It outputs whatever $\malrecv$ outputs.
\end{enumerate}

We argue indistinguishability using the following sequence of hybrids: 
\begin{itemize}
    \item $\Hyb_0$: This is the real world.
    
    \item $\Hyb_1$: In this hybrid, $\simurecv$ takes the role of honest $C$ and answers all RO queries of $\malrecv$ using ROs - $H,G$.
    
    \item $\Hyb_2$: This is the same as last hybrid, except $\simurecv$ first chooses the randomness used during commitment $r_i \in \zo^\secp, \forall i \in [n]$, and then invokes $\malrecv(\brho)$ and continues the protocol as in the last hybrid.

    \item $\Hyb_3$: In this hybrid, $\simurecv(\brho)$ acts as in the previous hybrid, except in how it answers the RO queries of $\malrecv$. It first chooses the commitment randomness $r_i \leftarrow \zo^\secp, \forall i \in [n]$ as in the last hybrid. It then defines the oracles (using circuit wrappers) $\puncrom{H}, \puncrom{G}$ as follows: $\puncrom{H}(\cdot) = H(\cdot)$, except $\forall i \in [n], \puncrom{H}(0||r_i) = r^{H,i}_0, \puncrom{H}(1||r_i) = r^{H,i}_1$, where $r^{H,i}_0,r^{H,i}_1 \leftarrow \zo^{\secp+1}$ (similarly for $\puncrom{G}$). 
    
    It invokes $\malrecv(\brho)$, answering RO queries of $\malrecv$ using $\puncrom{H},\puncrom{G}$ and then executes the commit phase with $\malrecv$, sending it $\{H(m_i||r_i),G(m_i||r_i)\}_{i \in [n]}$, all the while answering RO queries using $\puncrom{H},\puncrom{G}$. Thereafter, it runs the reveal phase with $\malrecv$, sending it $I,\{m_i,r_i\}_{i \in I}$, but now answering its RO queries using $H,G$.
    
    \item $\Hyb_4$: In this hybrid, $\simurecv$ chooses $r_i \leftarrow \zo^\secp, \forall i \in [n]$. It answers any RO queries of $\malrecv$ using $\puncrom{H},\puncrom{G}$ (defined using $\{r_i\}_{i \in [n]}$ as in the last hybrid), followed by executing the commit phase by first sampling $c^H_i \leftarrow \zo^{\secp+1}, c^G_i \leftarrow \zo^{\secp+1}, \forall i \in [n]$, and then sending to $\malrecv$ the values - $\{c^H_i,c^G_i\}_{i \in [n]}$. Thereafter it defines oracles $\puncrom{H}_R,\puncrom{G}_R$ as follows:
    
        \begin{itemize}
            \item $\puncrom{H}_R(\cdot) = {H}(\cdot)$, except $\forall i \in I,\puncrom{H}_R(m_i||r_i) = c^H_i$.

            \item $\puncrom{G}_R(\cdot) = {G}(\cdot)$, except $\forall i \in I, \puncrom{G}_R(m_i||r_i)=c^G_i$.
        \end{itemize}
        
    It then runs the reveal phase with $\malrecv$ by sending it $I,\{m_i,r_i\}_{i \in I}$, and answering any RO queries of it using $\puncrom{H}_R,\puncrom{G}_R$.
        
    \item $\Hyb_5$: This is the same as last hybrid, except $\simurecv$ now begins interacting with $\idealcom$ to get $I,\{m_i\}_{i \in I}$ in Reveal phase. In particular, on input $\brho$, it samples $r_i, \forall i \in [n]$ (as in the last hybrid), invokes $\malrecv(\brho)$ answering its RO queries with $\puncrom{H},\puncrom{G}$ (defined using $\{r_i\}_{i \in [n]}$ as done in last hybrid). On receiving $\mathsf{Receipt}$ from $\idealcom$ it begins the commit phase with $\malrecv$, by first sampling $c^H_i,c^G_i, \forall i \in [n]$ as in the last hybrid and then sending $\malrecv$ the values $\{c^H_i,c^G_i\}_{i \in [n]}$. On receiving the message $(\mathsf{Reveal},I,\{m_i\}_{i \in I})$, it begins the reveal phase with $\malrecv$ using the corresponding $I,\{m_i\}_{i \in I}$ it got from $\idealcom$, sending $\malrecv$ the values $I,\{m_i,r_i\}_{i \in I}$ and answering any of the RO queries of $\malrecv$ using $\puncrom{H}_R,\puncrom{G}_R$ (defined using $\{m_i,r_i\}_{i \in I}$ as in the last hybrid).
    
    \item $\Hyb_6$: This is the same as last hybrid, except $\simurecv$ now replaces its usage of ROs - $H,G$ by sampling hash functions $h_H,h_G$ at random from a $2q$-wise independent hash function family (where $q=q_\cZ+q_\malrecv$ is a bound on the total number of RO queries asked by $(\cZ,\malrecv)$) and using them to define the required oracles ($\puncrom{H},\puncrom{G},\puncrom{H}_R,\puncrom{G}_R$) by using circuit wrappers appropriately. Note that this is also the ideal world.

\end{itemize}
\nishant{add a remark that our simulator doesn't need access to random oracle?}

We now argue indistinguishability between the different hybrids: 
\begin{itemize}
    \item $\Hyb_0 \equiv \Hyb_1$: Since $\malrecv$'s queries are answered using ROs - $H,G$ in either hybrids, the output distributions in both cases is identical.
    
    \item $\Hyb_1 \equiv \Hyb_2$: In $\Hyb_2$, $r_i, \forall i \in [n]$ is now sampled at the beginning of the protocol. But since its not used at any place until the commit phase, this doesn't change $\malrecv$'s view in the protocol and hence the distributions are identical.
    
    \item $\Hyb_2 \approx_s \Hyb_3$: The difference between the two hybrids is in how $\simurecv$ answers the RO queries of $\malrecv$. In $\Hyb_3$, it uses random oracles $\puncrom{H},\puncrom{G}$ until before the reveal phase, while in $\Hyb_2$, it uses ${H},{G}$ for this. Consider an intermediate hybrid $\Hyb_{2.5}$, where $\simurecv$ only switches its usage of oracle $H$ to $\puncrom{H}$ and not of $G$ (i.e. in $\Hyb_{2.5}$ it uses $\puncrom{H},G$ to answer RO queries of $\malrecv$ until before the reveal phase). We show that $\Hyb_2 \approx_s \Hyb_{2.5}$. $\Hyb_{2.5} \approx_s \Hyb_3$ where $\simurecv$ switches its usage of $G$ to $\puncrom{G}$ follows by a similar argument. 
    
    Assume then for the sake of contradiction that $\exists$ an environment $\cZ^*=(\cZ_0^*,\cZ_1^*)$, s.t. $(\cZ^*,\malrecv)$ distinguish the output of $\Hyb_2$ from $\Hyb_3$ with non-negl probability $\varepsilon$. We show a contradiction using the one-way-to-hiding lemma (theorem~\ref{impthm:ow2h}). In particular, consider the following OW2H adversary $\cA$ having oracle access to $O$: 
    
    $\cA^O(H,G,\{r_i\}_{i \in [n]})$: It runs $\cZ_0^*$ to get $\brho,(m_1,m_2,\ldots, m_n),I,\bsigma$. It then runs $\malrecv(\brho)$ and acts as $\simurecv$ does in either hybrids with the commitment message being $(m_1,m_2,\ldots m_n)$ and the index set to reveal in reveal phase being $I$. It answers the RO queries of $\malrecv$ to $H$ till before the reveal phase using external oracle $O$. In more detail, it first invokes $\malrecv(\brho)$, answering its RO queries to $H$ using $O$ (and RO queries to $G$ using the full description it has), starts the commit phase, sending $\malrecv$ the values $\{H(m_i||r_i),G(m_i||r_i)\}_{i \in [n]}$ (note that it knows $\{r_i\}_{i \in [n]}$ from its input, $\{m_i\}_{i \in [n]}$ from $\cZ_0^*$, and it has full descriptions of $H,G$). Thereafter, it starts the reveal phase, sending $\malrecv$ the values $I,\{m_i,r_i\}_{i \in I}$ (again it knows $\{r_i\}_{i \in [n]}$ from its input and $I,\{m_i\}_{i \in [n]}$ from $\cZ_0^*$), and answering its RO queries using $H,G$. Once $\malrecv$ outputs, it runs $\cZ_1^*(\bsigma,\cdot)$ with input ($\bot,\malrecv$'s output state) and finally outputs whatever $\cZ_1^*$ outputs.
    
    Now as a challenger to the OW2H adversary $\cA$, we give it access to one of two oracles - $H$ or $\puncrom{H}$, where $\puncrom{H}$ is defined by first sampling $r_i \leftarrow \zo^\secp, \forall i \in [n]$ and setting $\puncrom{H}(\cdot) = H(\cdot)$, except $\forall i \in [n], \puncrom{H}(0 || r_i) = r^{H,i}_0 $ and $\puncrom{H}(1 || r_i) = r^{H,i}_1$, where $r^{H,i}_0,r^{H,i}_1 \leftarrow \zo^{\secp+1}$. 
    Now note that since $\cA^H$ exactly simulates the game in $\Hyb_2$, while $\cA^{\puncrom{H}}$ simulates the one in $\Hyb_{2.5}$, if $z=\{H,G,\{r_i\}_{i \in [n]}\}$ is the input to $\cA$, then $|Pr[\cA^H(z)] - Pr[\cA^{\puncrom{H}}(z)]| = \varepsilon$.
    
    Then by theorem~\ref{impthm:ow2h}, we have $\exists$ adversary $\cB^{\puncrom{H}}$, which works as follows - if $q$ denotes the number of oracle queries made by $\cA$, it picks $i \leftarrow [q]$, runs $\cA^{\puncrom{H}}$ till just before the $i^{th}$ query, measures the query register and outputs the measurement outcome $x_0$. If set $S = \bigcup_{i \in [n]}\{0||r_i,1||r_i \}$, defines all the points at which $H$ and $\puncrom{H}$ differ, we have that by theorem~\ref{impthm:ow2h}, $$Pr[x_0 \in S | x_0 \leftarrow \cB^{\puncrom{H}}(z)] \geq \varepsilon^2/{4q^2}$$
    
    But note that the only queries made by $\cA$ to its oracle $O$ are the ones made by $\malrecv$ till before the reveal phase. This means that measuring $i^{th}$ query made by $\malrecv$ during the commit phase results in $x_0 \in S = \bigcup_{i \in [n]} \{0||r_i,1||r_i\}$. 
    
    But if we note the view of $\malrecv$ during the commit phase, we see that it received $\{H(m_i||r_i)\}_{i \in [n]}$, and only had access to $\puncrom{H}$. But $\forall i \in [n], \puncrom{H}(0||r_i),\puncrom{H}(1||r_i)$ are fresh random strings uncorrelated with $H(m_i||r_i)$. We then have that given access to a uniform oracle $\puncrom{H}$ and uncorrelated random strings $\{H(m_i||r_i)\}_{i \in [n]}$, measuing the $i^{th}$ query of $\malrecv$ results in a point $\in S$ (and hence giving $r_j$ for some $j \in [n]$), with probability $\varepsilon^2/4q^2$, which is non-negl (since $q$ is $poly(\secp)$ and $\varepsilon$ is non-negl$(\secp)$).
    
    But since $\puncrom{H}$ is a uniform oracle and $\forall j \in [n], r_j$ was chosen uniformly from $\zo^\secp$, this can only happen with negl probablity. Hence, a contradiction.
    
    \item $\Hyb_3 \equiv \Hyb_4$: We argue that the view of $\malrecv$ in either hybrids is identical, and hence the outputs of the two hybrids are identical. Note that in $\Hyb_3$, during the commit phase, $\malrecv$ sees $\{c^H_i = H(m_i||r_i),c^G_i = G(m_i||r_i)\}_{i \in [n]}$ while having access to $\puncrom{H},\puncrom{G}$. Since $\forall i \in [n], \puncrom{H}(0||r_i),\puncrom{H}(1||r_i),\puncrom{G}(0||r_i),\puncrom{G}(1||r_i)$ are fresh random strings uncorrelated with $H,G$, during the commit phase, $c^H_i,c^G_i$ look as fresh random strings to $\malrecv$. During the reveal phase, $\malrecv$ gets access to oracles $H,G$, which are consistent with the ones it had access to in commit phase, except $H(m_i||r_i)=c^H_i$ and $H(1-m_i||r_i)$ is a fresh random string (similarly for $G$ and $c^G_i$).
    
    In $\Hyb_4$, $\malrecv$ gets uncorrelated uniformly drawn random strings $c^H_i,c^G_i, \forall i \in [n]$ during the commit phase, while having access to $\puncrom{H},\puncrom{G}$. During the reveal phase, it gets access to $\puncrom{H}_R,\puncrom{G}_R$, where $\puncrom{H}_R$ is defined to be consistent with $H$ everywhere, except $\forall i \in I, \puncrom{H}_R(m_i||r_i)=c^H_i$ (similarly for $\puncrom{G}_R$).
    
    The view of $\malrecv$ in either hybrids is then fresh random strings (uncorrelated with the oracle it has access to) which it receives during the commit phase and during the reveal phase, a RO consistent at $\{m_i||r_i\}_{i \in I}$ with the string is received during commit phase.
    
    Hence, the view of $\malrecv$ in either hybrids is identical.
    
    \item $\Hyb_4 \equiv \Hyb_5$: Note that in $\Hyb_4$, though $\simurecv$ had its messages $m_1,m_2 \ldots m_n$ during the commit phase, it did not use them until the Reveal phase. And during the Reveal phase, while in $\Hyb_4$, $\simurecv$ uses its own $I,\{m_i\}_{i \in I}$, in $\Hyb_5$, it gets the same from $\idealcom$. Hence, the view of $\malrecv$ in either hybrids is identical. The only other difference is that in $\Hyb_4$, $\simurecv$ acts as the honest $C$ and the output of the hybrid is (output of $\simurecv$, view of $\malrecv$) ; while in $\Hyb_5$, it is (the output of the honest committer interacting with $\idealcom$ and the output of $\simurecv$ outputting the view of $\malrecv$). Since the output of honest committer in either hybrids is $\bot$, the joint distributions in either hybrids is also identical.
    
    \item $\Hyb_5 \equiv \Hyb_6$: This follows from Theorem~\ref{impthm:simRO}, which shows that a quantum oracle algorithm making some $q'$ queries to a random oracle behaves identically if instead it is given access to a hash function sampled from a $2q'$-wise independent hash family. In our case, in $\Hyb_6$, $\simurecv$ sets $q$ as the bound on the total number of RO queries made by $(\cZ,\malrecv)$ to both the oracles - $H,G$, and then uses hash functions drawn randomly from $2q$-wise independent hash family. We can then replace the use of ROs $H,G$ one by one by the corresponding hash function chosen from the $2q$-wise independent hash family, and since the number of RO queries to any of them is bounded by $q$, we have that $\Hyb_5 \equiv \Hyb_6$.


\end{itemize}

\subsection{Receiver security}
For every malicious committer $\malcomm$ and bound on the environment's total oracle queries as $q_\cZ$, we define simulator $\simu[C^*,q_\cZ]$, which takes input $\brho$ and does the following: (we use shorthand $\simucomm$ for $\simu[C^*,q_\cZ]$)

\begin{enumerate}
    \item If $q_{C^*}$ is a bound on the total number of oracle queries made by $\malcomm$, $\simucomm$ sets $q = q_{C^*} + q_\cZ$ and samples hash functions - $h_H$ at random from a $2q$-wise independent hash function family and $h_G$ from a $2(q+2qn+n)$-wise independent hash family. It then invokes $\malcomm(\brho)$, answering its RO queries using the sampled hash functions - $h_H,h_G$. In particular, it chooses univariate polynomials of degree $k-1$ with coefficients in $GF(2^{\secp+1})$ as a $k$-wise independent hash function family~\cite{lemire2016faster,wegman1981new}. 
    % \james{what do these citations show?}\nishant{was trying to show that polynomials of degree $d-1$ are $d$-wise independent hash family, citations from wikipedia article on $k$ wise independence; maybe we can remove this if its clear}. 
    Let $p_H(x)$ be the chosen polynomial for $h_H$.
    
    \item It starts the commit phase with $\malcomm$ and on receiving $\{c_1^i,c_2^i\}_{i \in [n]}$ from $\malcomm$, it performs the following actions $\forall i \in [n]$: 
        \begin{enumerate}
            \item Find $R_i = \{x | x \in GF(2^{\secp+1}) \wedge p_H(x) = c_1^i \}$ by finding all roots of the polynomial equation $p_H(x)=c_1^i$ in polynomial time~\cite{berlekamp1967factoring}.
            
            \item Find $F_i = \{x | x \in R_i \wedge h_G(x) = c_2^i \}$ by checking for each $x \in R_i$ whether $h_G(x) = c_2^i$. If $|F_i| > 1$, then output \textsf{FAIL} and stop. If $|F_i| = 0$, set $m'_i = 0$. If $|F_i| = 1$ and $F_i = \{x_i\}$, then parse $x_i=a||b$ (where $|a|=1,|b|=\secp$) and set $m'_i=a$.
            
            % then set $m'_i = \bot$ \james{here we could say that if $|F_i| = 0$, set $m'_i = 0$? Not sure if the ideal functionality expects any $\bot$s. And to be more clear, we can say that if any $|F_i| > 1$, then the entire experiment aborts and outputs $\bot$, since this is a negl probability event.} else  
        \end{enumerate}
        
        % \amit{How will we convert a simulator which fails with negligible probability to one which fails with zero probability (at the cost of potentially running in expected polynomial time) ? Will this involve the invocation of Watrous quantum rewinding lemma ?}
        
    \item Send $(\mathsf{Commit},(m'_1,m'_2 \ldots m'_n))$ to $\idealcom$.
    
    \item Invoke the Reveal phase of $\malcomm$ to get message $(I,\{m_i,r_i\}_{i \in I})$ from $\malcomm$. Initialize $J \leftarrow \emptyset$ and $\forall i \in I$, check if $p_H(m_i||r_i) = c_1^i \wedge h_G(m_i||r_i) = c_2^i$, if so set $J = J \cup \{i\}$. Send $(\mathsf{Reveal},J)$ to $\idealcom$, and output whatever $\malcomm$ outputs.
\end{enumerate}

We now define a sequence of hybrids to prove that the real and ideal worlds are indistinguishable: 

\begin{itemize}
    \item $\Hyb_0$: This is the real world.
    
    \item $\Hyb_1$: In this hybrid, $\simucomm(\brho)$ invokes $\malcomm(\brho)$, playing the role of honest receiver for $\malcomm$  and answering all RO queries of $\malcomm$ using ROs - $H,G$.
    
    \item $\Hyb_2$: This is the same as last hybrid, except in how $\simucomm$ answers queries of $\malcomm$ to RO $H$. If $q_{C^*}$ is the bound on the total oracle queries made by $\malcomm$, it sets $q = q_{C^*}+q_\cZ$, samples hash function $h_H$ from a $2q$-wise independent hash function family and uses $h_H$ to answer $\malcomm$'s queries to oracle $H$. In particular, it uses the family of polynomials of degree $2q-1$ with coefficients in $GF(2^{\secp+1})$ as the $2q$-wise independent hash family. Suppose the polynomial it picks for $h_H$ is $p_H(x)$. It continues to answer RO queries to $G$ using RO $G$.
    
    \item $\Hyb_3$: This is the same as last hybrid, except $\simucomm$ uses a random permutation $\widetilde{G}:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$ to answer any of $\malcomm$'s queries to $G$. 
    
    \item $\Hyb_4$: This is the same as last hybrid, except that at the end of Commit phase, on receiving messages $\{c_1^i,c_2^i\}_{i \in [n]}$, $\simucomm$ performs the following actions $\forall i \in [n]$:
        \begin{itemize}
            \item Define $R_i = \{x | x \in GF(2^{\secp+1}) \wedge p_H(x) = c_1^i\}$ by solving the polynomial equation $p_H(x) = c_1^i$ in polynomial time~\cite{berlekamp1967factoring}. 
            
            \item Define $F_i = \{ x | x \in R_i \wedge \widetilde{G}(x) = c_2^i \}$ by checking $\forall x \in R_i$, whether $\widetilde{G}(x) = c_2^i$. 
            
            \item If $|F_i| > 1$, then output \textsf{FAIL} and stop. If $|F_i|=0$, then set $m'_i = 0$. If $|F_i|=1$ and $F_i = \{x_i\}$, parse $x_i = a||b$, where $|a|=1,|b|=\secp$ and set $m'_i=a$.
            
            % \item If $|F_i| \neq 1$, then set $m'_i = \bot$, else if $x_i \in F_i$, parse $x_i=a||b$ (where $|a|=1,|b|=\secp$) and set $m'_i=a$.
        \end{itemize}
    
    Even though $\simucomm$ defines the values $\{m'_i\}_{i \in [n]}$, it doesn't use it anywhere.
        
    \item $\Hyb_5$: In this hybrid, $\simucomm$ starts interacting with $\idealcom$. In particular, it answers the RO queries of $\malcomm$ as in the last hybrid, and at the end of commit phase either outputs \textsf{FAIL} and stops or defines $\{m'_i\}_{i \in [n]}$ as in the last hybrid. It then sends $(\mathsf{Commit},(m'_1,m'_2 \ldots m'_n))$ to $\idealcom$ and thereafter starts running the reveal phase with $\malcomm$. On receiving $(I,\{m_i,r_i\}_{i \in I})$ from $\malcomm$, it does the following - set $J = \emptyset$ and $\forall i \in I$ check if $p_H(m_i||r_i)=c_1^i \wedge \widetilde{G}(m_i||r_i) = c_2^i$ and if the check passes, then set $J = J \cup \{i\}$. It then sends $(\mathsf{Reveal},J)$ to $\idealcom$ and outputs whatever $\malcomm$ outputs.
    
    \item $\Hyb_6$: This is the same as last hybrid, except that $\simucomm$ replaces the use of $\widetilde{G}$ with a random oracle $G$ to answer $\malcomm$'s queries to $G$.
    
    \item $\Hyb_7$: This is the same as last hybrid, except now $\simucomm$ replaces the use of $G$ with a hash function $h_G$ sampled at random from a $2(q+2qn+n)$-wise independent hash function family and uses that to answer any of $\malcomm$'s queries to $G$. This is the ideal world.
\end{itemize}

Note that in $\Hyb_3,\Hyb_4,\Hyb_5$, $\simucomm$ runs inefficiently since it needs to sample and use $\widetilde{G}$. But in the end hybrids - $\Hyb_0,\Hyb_7$, it still runs in polynomial time. We now argue the indistinguishability of these hybrids: 

\begin{itemize}
    \item $\Hyb_0 \equiv \Hyb_1$: This follows because in either hybrids the oracle queries of $\malcomm(\brho)$ are answered using oracles $H,G$ and hence the views of $\malcomm$ in either hybrids is identical. 
    
    \item $\Hyb_1 \equiv \Hyb_2$: This follows by Theorem~\ref{impthm:simRO}, which states that a quantum oracle algorithm making $q'$ queries to the oracle, cannot distinguish between a random function and a hash function sampled from $2q'$-wise independent hash function family. In $\Hyb_2$, $\simucomm$ replaces the use of the RO $H$ by a hash function sampled from a $2q$-wise independent hash function family, where $q = q_{C^*}+q_\cZ$ is an upper bound on the total RO queries asked by $\malcomm$ and $\cZ$.
    
    \item $\Hyb_2 \approx_s \Hyb_3$: This follows from Theorem~\ref{impthm:ROinjective}, which states that a quantum oracle algorithm making some $q'$ queries to a random oracle cannot distinguish the oracle from a random injective function as long as domain and codomain sizes of the oracle are the same, except with probability $q'^3/|\text{codomain}|$. In our case, since $|Domain(G)|=|Codomain(G)|=2^{\secp+1}$, and the random permutation $\widetilde{G}$ is also a random injective function, it follows that $\malcomm/\cZ$ cannot distinguish $\simucomm$'s usage of random oracle $G$ in $\Hyb_2$ and its usage of a random permutation $\widetilde{G}$ in $\Hyb_3$ except with probability $q^3/2^{\secp+1}$, where $q$ as in the last hybrid is an upper bound on the total queries of $\malcomm$ and $\cZ$. Since $q=poly(\secp)$, we have $\Hyb_2 \approx_s \Hyb_3$.
    
    \item $\Hyb_3 \equiv \Hyb_4$: The difference between the two hybrids is that in $\Hyb_4$, at the end of commit phase, $\simucomm$ outputs \textsf{FAIL} and stops or defines values $\{m'_i\}_{i \in [n]}$ using $\widetilde{G}$ and  $p_H$. First, note that $\simucomm$ outputs \textsf{FAIL} only if for some $i$, $|F_i| > 1$. But $|F_i|>1$ only happens if there are more than one root to $\widetilde{G}(x)=c_2^i$. Since $\widetilde{G}$ is a permutation this cannot happen and hence in $\Hyb_4$, $\simucomm$ never outputs \textsf{FAIL}. Second, note that the only other computation done by $\simucomm$ sets up $\{m'_i\}_{i \in [n]}$ - which is not used anywhere in the protocol. Hence, $\Hyb_4 \equiv \Hyb_5$.
    
    \item $\Hyb_4 \equiv \Hyb_5$: The difference between the two hybrids is that instead of outputting the honest $R$'s output as in $\Hyb_4$, $\simucomm$ in $\Hyb_5$ starts interacting with $\idealcom$. 

    In $\Hyb_4$, note that when $\malcomm$ sends $I,\{m_i,r_i\}_{i \in I}$ during the reveal phase, $\simucomm$ checks $\forall i \in I$, if $H(m_i||r_i)=c_1^i \wedge \widetilde{G}(m_i||r_i) = c_2^i$ and outputs $J,\{m_j\}_{j \in J}$, where $J \subseteq I$ is the set of indices for which the check passes. But since $\widetilde{G}$ is a permutation, for every $i \in I$, either there is a unique value of $m_i||r_i$ which passes the checks and which $\malcomm$ provides, or the check fails and $\simucomm$ doesn't include index $i$ in its output.
    
    In $\Hyb_5$, $\simucomm$ on receiving $\{c_1^i,c_2^i\}_{i \in [n]}$ at the end of the commit phase, finds that unique value $x_i$ (if it exists) which satisfies $H(x_i)=c_1^i \wedge \widetilde{G}(x_i) = c_2^i$, by first finding all the roots $x \in GF(2^{\secp+1})$ s.t. $p_H(x) = c_1^i$ and checking for all such $x$ if $\widetilde{G}(x) = c_2^i$. Since $\widetilde{G}$ is a permutation, there can be at most one such value, and hence it never outputs \textsf{FAIL}. If no such value is found, it sets $m'_i=0$, else parses $x_i=a||b$ (where $|a|=1,|b|=\secp$) and sets $m'_i=a$. During the reveal phase, $\forall i \in I$ it checks if $\malcomm$ sent the unique opening and if so includes it in a set $J$. Finally, it sends $J$ to $\idealcom$. 
    
    $\forall i \in I$, there are two cases then - either $\exists$ a unique opening to $c_1^i,c_2^i$ or it doesn't. If it doesn't exist, then in both hybrids, $\malcomm$ fails to provide a valid opening and $\simucomm$ doesn't include index $i$ in its output/message to $\idealcom$. If a unique opening exists, and $\malcomm$ does provide it during the reveal phase, then in $\Hyb_4$ $\simucomm$ includes $i,m_i$ in its output, while in $\Hyb_5$, $\simucomm$ finds the unique opening at the end of commit phase and includes $i$ into the set $J$ sent to $\idealcom$, which allows the honest $R$ to also include $i,m_i$ in its output. If however the unique opening exists, but $\malcomm$ doesn't provide it during the reveal phase, in both hybrids, $\simucomm$ doesn't include index $i$ in its output/message to $\idealcom$.

    Hence, in either case, $\forall i \in I$, the outputs of $\simucomm$ in $\Hyb_4$ and that of honest $R$ in $\Hyb_5$ match. Therefore, since the views of $\malcomm$ is also identical in either hybrids, we have that $\Hyb_4 \equiv \Hyb_5$.

    \item $\Hyb_5 \approx_s \Hyb_6$: The difference between the two hybrids is that $\simucomm$ replaces its use of random permutation $\widetilde{G}$ with RO $G$ in $\Hyb_6$. We show then that $\Hyb_5 \approx_s \Hyb_6$ using Theorem~\ref{impthm:ROinjective}, which states a quantum oracle algorithm cannot distinguish a RO from a random injective function, except with a small probability, as long as sizes of domain and codomain of the oracle are same. 
    
    In particular, suppose for the sake of contradiction that $\exists$ an environment $\cZ^*=(\cZ_0^*,\cZ_1^*)$ s.t. $(\cZ^*,\malcomm)$ together distinguish the output of $\Hyb_5$ from $\Hyb_6$. We then build a quantum oracle algorithm $A^O$ which acts as follows:
    
    $A^O$ runs $\cZ_0^*$ to get $(\brho,\bsigma)$, then runs $\malcomm(\brho)$ acting just as $\simucomm$ does in either hybrids and answering its oracle queries to $G$ using the outer oracle $O$ and simulating $\idealcom$ and the honest $R$ itself. Note that $\simucomm$ also makes some queries to $G$, which are again answered using external oracle $O$. Once this execution finishes, it runs $\cZ_1^*(\bsigma,\cdot)$ on the outputs of $\simucomm$ and the honest $R$ and outputs whatever $\cZ_1^*$ outputs. 
    
    Now as a challenger, either we run $A^{\widetilde{G}}(\cdot)$ or $A^G(\cdot)$. Note that $A^{\widetilde{G}}$ simulates exactly the game in $\Hyb_5$, while $A^G$ exactly the one in $\Hyb_6$. Hence, if $(\cZ^*,\malcomm)$ distinguish $\Hyb_5,\Hyb_6$ with non-negl probability $\varepsilon$, $A$ distinguishes the oracles it is given access to also with non-negl probability $\varepsilon$.
    
    However, we know from theorem~\ref{impthm:ROinjective} that since $\widetilde{G}$ is a random injective function and $|Range(G)|=|Codomain(G)|=2^{\secp+1}$, no quantum oracle algorithm can distinguish $\widetilde{G}$ from $G$ except with probability $q'^3/2^{\secp+1}$, where $q'$ is the number of RO queries made to $G$ by $A$. Since $q' \leq q+2qn+n$ ($q$ by $(\cZ^*,\malcomm)$ and $\leq 2q$ for each $i \in [n]$ made by $\simucomm$ during extraction at the end of commit phase, and $\leq n$ made during the checks by $\simucomm$ during the reveal phase), and $q=poly(\secp),n=poly(\secp)$, we have that $q'=poly(\secp)$ and hence this is a contradiction.
    
    \item $\Hyb_6 \approx_s \Hyb_7$: This follows from Theorem~\ref{impthm:simRO} using a similar argument as the last hybrid. In particular, if the use of RO $G$ is replaced by hash function $h_G$ in $\Hyb_7$ and $\exists (\cZ^*,\malcomm)$ which distinguish output of $\Hyb_6$ from $\Hyb_7$, this implies a distinguisher which can distinguish oracle access to $G$ vs $h_G$ with same probability. But since $h_G$ is sampled from a $2q'=2(q+2qn+n)$-wise independent hash family, and the total number of queries made by to the external oracle by $\cZ^*,\malcomm$ and $\simucomm$ in total is bounded by $q'=q+2qn+n$ (as in the last hybrid), we have a contradiction.

\end{itemize}

==> ot-text.tex <==
%%pasted text here from other work
%%look for macros in headers.tex and move them to macros.tex if this doesn't compile

\subsection{Statistical Hiding}
\label{subsec:stat-hiding}

In this subsection, we prove that our extractable commitment scheme described in~\cref{fig:ext-com} is statistically hiding, assuming that $\eqcommit$ is a statistically binding (equivocal) commitment scheme.

Our proof closely follows techniques of~\cite{C:BouFeh10}, who developed techniques for analyzing~\cite{FOCS:CreKil88}-style oblivious transfer protocols based on quantum sampling techniques. We import a lemma from~\cite{C:BouFeh10}.

\paragraph{\cite{C:BouFeh10} Quantum Sampling.} 

Consider the following interaction between a player $P$ and a challenger $C$.
\begin{enumerate}
    \item $P$ prepares an arbitrary quantum state $\ket{\psi}_{\gray{X}\gray{Y}}$ where $\gray{X}$ is a $2n$-qubit register and $\gray{Y}$ is an arbitrary-size register of $P$'s choice. 
    
    $P$ sends the contents of $\gray{X}$ to $C$ along with two length-$2n$ classical strings $\hat{x} \in \{0,1\}^{2n}$ and $\hat{\theta} \in \{+,\times\}^{2n}$.
    
    \item\label[step]{step:check-T} $C$ samples a uniformly random set of $n$ indices $T \subset [2n]$ as well as a uniformly random $\theta \in \{+,\times\}^{2n}$.
    
    For each $i \in T$ it measures the $i$th qubit of $\gray{X}$ in basis $\hat{\theta}_i$. If there exists $i \in T$ where $\theta_i = \hat{\theta}_i$ and the measurement outcome does not match $\hat{x}_i$, then $C$ aborts the experiment and outputs $\bot$. Otherwise, $C$ sends $\overline{T} \coloneqq [2n] \setminus T$ to $P$.
    
    \item $P$ responds with a subset $S \subseteq \overline{T}$. 
    
    \item\label[step]{step:measure} $C$ measures the indices of $\gray{X}$ specified by $S$, obtaining a length-$|S|$ bitstring $X_S$ of measurement outcomes; let $s$ denote the number of indices $i \in S$ where $\theta_i \neq \hat{\theta}_i$. 
\end{enumerate}

\begin{lemma}[\cite{C:BouFeh10} Quantum Sampling Lemma]
\label{lemma:sampling}
For any computationally unbounded player $P$ and $0 < \varepsilon < 1$, the probability the sampling experiment does not abort and
\[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\bar{S}}, \gray{Y}) > s- \varepsilon \cdot |S|. \]
is at most $\negl(|S|^2/n)$.
\end{lemma}


\begin{proof}(Sketch.)
This lemma follows readily from techniques developed in~\cite{C:BouFeh10} to relate quantum sampling to classical sampling. Following~\cite{C:BouFeh10}, it suffices to analyze the case where $\hat{x} = 0^{2n}$ and $\hat{\theta} = +^{2n}$, since all other settings of $\hat{x}$ and $\hat{\theta}$ follow from an identical argument under a change of basis. 

In \cref{step:check-T} of the quantum sampling experiment, $C$ verifies that for every index in a random choice of $n$ indices $T \subset [2n]$, measuring the corresponding qubit in the computational basis yields $0$. As observed in~\cite{C:BouFeh10}, this is a natural quantum analogue of the following classical sampling experiment (\cite[Example 4]{C:BouFeh10}) on a length-$2n$ bitstring $X$:
\begin{enumerate}
    \item randomly select a size-$n$ subset $T \subset [2n]$,
    \item randomly select a string $\theta \in \{0,1\}^{2n}$,
    \item verify that $X_i = 0$ on each index $i \in T$ where $\theta_i = 1$, and abort otherwise.
\end{enumerate}
Let $X_{\overline{T}}$ denote the string $X$ restricted to the $n$ indices $\overline{T} = [2n] \setminus T$. For any initial bitstring $X$, the ``classical error probability'' is the probability that the sampling experiment succeeds and $X_{\overline{T}}$ has relative Hamming weight $\geq \delta$ is at most $6e^{-n \delta^2/50}$ (bound derived in \cite[Appendix B.4]{C:BouFeh10}).

\cite[Theorem 3]{C:BouFeh10} demonstrates that the ``quantum error probability'' is at most the square root of the classical error probability. That is, if the verification in \cref{step:check-T} passes, then the residual state on $\gray{X}$ restricted to $\overline{T}$ is within trace distance $\sqrt{6e^{-n \delta^2/50}}$ of a superposition of states with relative Hamming weight at most $\delta$.

Suppose for a moment that the state were \emph{exactly} a superposition of states with relative Hamming weight at most $\delta$. Now consider the restriction of $\gray{X}$ to a subset of indices $S \subset \overline{T}$ where exactly $s$ positions have $\hat{\theta}_i \neq \theta_i$. The relative Hamming weight of the state when restricted to $S$ is at most $\delta n/ |S|$. As long as $\delta n/ |S| < 1/2$, by~\cite[Corollary 1]{C:BouFeh10}, we have
\[ \mathbf{H}_{\infty}(X_S \mid \gray{X}_{\overline{S}}, \gray{Y}) > s - h(\delta n/|S|)\cdot |S|\]
where $h: [0,1] \rightarrow [0,1]$ is the binary entropy function defined as $h(p) = p \log (p) + (1-p) \log (1-p)$ for $0 < p < 1$ and as $0$ for $p = 0$ or $1$. For any desired $\varepsilon \in (0,1)$, there exists an $\epsilon' \in (0,1/2)$ such that $h(\varepsilon') = \varepsilon$, so we can plug in $\delta = \varepsilon' |S|/n$ to achieve the stated min-entropy lower bound of $s - \varepsilon \cdot |S|$.
\end{proof}

% Before we apply this lemma to prove statistical hiding of our extractable commitments, we provide some brief intuition behind the~\cite{C:BouFeh10} techniques used to prove this lemma. At a very high level, the main result of~\cite{C:BouFeh10} is that up to polynomial factors, ``quantum sampling'' behaves like classical sampling.

\paragraph{Proof of Statistical Hiding.} We now prove statistical hiding of our extractable commitment scheme in~\cref{fig:ext-com}. The core proof idea is due to~\cite{C:BouFeh10}.

Consider a \emph{purification} of the committer's strategy from~\cref{fig:ext-com}, where instead of sampling random $x \gets \{0,1\}^{2\secp^3}, \theta \gets \{+,\times\}^{2\secp^3}$ and sending $\ket{x}_\theta$ to $\mathcal{R}$ in~\cref{step:sample}, the committer $\mathcal{C}$ generates $2\secp^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$, and sends $\mathcal{R}$ one half of each pair. This change has no effect on the receiver's view. In this modification of~\cref{step:sample}, the committer will still sample random $\theta \gets \{+,\times\}^{2\secp^3}$ but does not use it to perform any measurements (and hence $x$ is not yet determined). We now recast~\cref{step:sample,step:open,step:commit,step:challenge,step:verify} of~\cref{fig:ext-com}, i.e., the ``measurement-check subprotocol'' to correspond with this undetectable modification of the committer's behavior:

% \begin{enumerate}
% \item The committer (inefficiently) opens the commitments to recover the receiver's choice of $(\hat{\theta},\hat{x})$.
% \item Rather than checking that 
% \end{enumerate}

\begin{enumerate}
\item $\cC$ chooses $2\lambda^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$ and sends $\mathcal{R}$ one half of each pair. The committer samples random $\theta \gets \{+,\times\}^{2\lambda^3}$ but does not perform any measurements (and hence $x$ is not yet determined).
\item $\cR$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{2\lambda^3}$
and obtains $\widehat{x} \in \{0, 1\}^{2\lambda^3}$ by measuring its $2\lambda^3$ EPR pair halves in bases specified by $\widehat{\theta}$.

$\cR$ commits to $\widehat{\theta}$ and $\widehat{x}$ using \emph{statistically binding commitments}.

\item $\cC$ sends a random test subset $T \subset [{2\lambda^3}]$ of size ${\lambda^3}$ to $\cR$. 

\item For every $i \in T$, $\cR$ decommits to $(\widehat{\theta}_i,\widehat{x}_i)$, and $\cC$ aborts if any decommitment is invalid.

\item $\cC$ checks that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $\cC$ proceeds with the protocol,
otherwise, $\cC$ aborts. 
\end{enumerate}

Notice that $\cC$'s messages are completely independent of its bit $b$ up to this point. If $\cR$ passes the check above, then $\cC$ will obtain a $\secp^3$-bit string $x$ by measuring its qubits (i.e., EPR pair halves) in positions $\overline{T} \coloneqq [2\secp] \setminus T$ in the bases specified in $\theta$. $\cC$ then partitions $x$ into $\secp$ different $\secp^2$-bit strings strings $x^{(1)},\dots,x^{(\secp)}$ and sends the receiver
\[ (s_1,b \oplus h(s_1,x^{(1)})),\dots,(s_\secp,b \oplus h(s_\secp,x^{(\secp)})), \]
where each $s_1,\dots,s_\secp$ is a random seed for the universal hash function $h$. By the leftover hash lemma (\cref{thm:privacy-amplification}), $b$ will be statistically hidden if each $x^{(\ell)}$ has sufficient independent min-entropy.

To that end, observe (following~\cite[Section 5]{C:BouFeh10}) that the committer decides to accept the receiver's commitment openings $(\hat{\theta}_i,\hat{x}_i)_{i \in [T]}$ \emph{only if} a certain ``quantum sampling experiment'' succeeds. Since the commitments are statistically binding, the values of $\hat{x},\hat{\theta}$ that $\mathcal{C}$ would accept are statistically determined after $\mathcal{R}$ commits. Let $\ket{\psi}_{\gray{X}\gray{Y}}$ be the joint state of the committer and receiver where $\gray{X}$ corresponds to the committer's $2\secp^3$ registers, and $\gray{Y}$ corresponds to the receiver's state. Then the committer's check can only pass if the sampling strategy of~\cref{lemma:sampling} succeeds for the committed values of $\hat{x},\hat{\theta}$. We remark that while no efficient $\mathcal{C}$ can actually \emph{perform} this sampling strategy (as it involves breaking the computational hiding of the underlying equivocal commitments), its behavior is statistically indistinguishable from $\mathcal{C}$ that does perform this sampling. 

By applying~\cref{lemma:sampling}, we conclude that each $x^{(\ell)}$ must therefore have min-entropy $\Omega(\lambda^2)$ conditioned on $\mathcal{R}$'s view and on all $x^{(j)}$ for $j \neq \ell$, since by Hoeffding's inequality, $\theta$ and $\hat{\theta}$ differ in at least $\Omega(\lambda^2)$ places within the $\lambda^2$ indices corresponding to $x^{(\ell)}$ with $1-\negl(\lambda)$ probability. Applying~\cref{thm:privacy-amplification} (leftover hash lemma) one by one to each $x^{(\ell)}$, this implies that each $(s_\ell,h(s_\ell,x^{(\ell)}))$ is statistically indistinguishable from uniform even given the receiver's view, and thus $b$ is statistically hidden.

==> overview.tex <==
%\section{Technical overview - old}
%\label{sec:overview}


%\subsection{Background}
%Crepeau and Kilian~\cite{FOCS:CreKil88} first proposed a template for achieving quantum oblivious transfer based on Wiesner's conjugate encoding scheme~\cite{Wiesner}, and their template is described in Figure \ref{fig:template}. The scheme begins with the sender transmitting single qubit states encoding either $0$ or $1$ in either the computational or Hadamard basis. Crucially, measuring (or essentially attempting to copy the encoded bit) in the wrong basis completely destroys information about the encoded bit. This allows a sender and receiver to establish two channels, where the capacity of one is larger than that of the other. The sender can then transmit one message over each channel, encoded at a rate that is intermediate to the capacity of both channels. To enforce that the receiver measure transmitted states (and hence delete some information by measuring in the wrong bases), the protocol requires the sender and receiver to run a {\em measurement-check subprotocol}. This is essentially a game where the receiver commits to their measurement outcomes and the sender checks a subset of these commitments. 

We begin by reviewing the Crepeau-Kilian~\cite{FOCS:CreKil88} OT template.
%in Figure~\ref{fig:template}.
Their template makes crucial use of the fact that having Bob send random BB84 states, and Alice honestly measure them in random bases, after which Bob reveals the correct bases -- sets up a secure erasure channel between them where the probability of erasure is exactly $\frac{1}{2}$. Between Bob sending BB84 states and revealing his bases, Alice convinces Bob that she measured these states in some combination of $+/\times$ bases via a cut-and-choose masurement check.
%The measurement check subprotocol in the figure is simply a way to enforce that the receiver indeed (mostly) performed measurements when they were supposed to, leading to a erasure channel (with some security loss due to imperfect measurements by the receiver).
Then the rest of the protocol can be viewed as a conversion from the resulting erasure channels to OT.
%, again following~\cite{FOCS:CreKil88}.
%The sender first transmits BB84 states, next the receiver ``proves'' that these states were measured, and next the sender reveals their true bases. At this point, the receiver recovers the indices where information was transmitted and where it was erased, forming two channels, and sending them back to the sender -- and finally, the sender sends an encoding of each of their two messages over each of these channels.
\iffalse{
\begin{figure}[ht!]
     \begin{framed}
    
    {\bf Sender $\cS$ Input: } Messages $m_0, m_1 \in \{0,1\}^\lambda$.
    {\bf Receiver $\cR$ Input: } Choice bit $b \in \{0,1\}$.\\
    
    For classical bits $(x,\theta)$, let $\ket{x}_\theta$ denote $\ket{x}$ if $\theta = 0$, and $(\ket{0} + (-1)^x\ket{1})/\sqrt{2}$ if $\theta = 1$. Let $\com(\cdot)$ denote an ideal commitment scheme, $h:\{0,1\}^{3\lambda/2} \rightarrow \{0,1\}^{\lambda}$ denote a pairwise independent hash function. 


    \begin{enumerate}
    
    \item  {\bf Sender Message.}
    %  , i.e. the choice of $z$ specifies whether to interpret $y$ as a computational or Hadamard basis vector. Let $\lambda$ denote the security parameter. 
    %
    $\cS$ samples two random $2\lambda$-bit strings $x$ and $\theta$, and sends $(\ket{x_i}_{\theta_i})_{i \in [2\lambda]}$ to $\cR$. 
    
    \item {\bf Measurement Check Subprotocol.}
    \begin{enumerate}
        \item $\cR$ samples a $2\lambda$-bit string $\widehat{\theta}$, measures each $\ket{x_i}_{\theta_i}$ in the basis specified by $\widehat{\theta}_i$ to obtain measurement result $\widehat{x}_i$.
        $\cR$ sends $\{\com(\widehat{x}_i), \com(\widehat{\theta}_i)\}_{i \in [2\lambda]}$ to $\cS$.
        \item $\cS$ sends $\cR$ a random $T \subset [2\lambda]$ of size $\lambda$.
        %, and challenges Alice to open the corresponding commitments.
        \item For every $i \in T$, $\cR$ sends $(\widehat{\theta}_i,\widehat{x}_i)$ along with the corresponding commitment opening to $\cS$. 
    \end{enumerate}
    
    
    \item {\bf Sender Message.} 
    $\cS$ verifies each commitment opening, and checks that $\widehat{x}_i = x_i$ for each $i \in T$ where $\widehat{\theta}_i = \theta_i$. If any of these checks fail, $\cS$ aborts.

    The tested positions are discarded by both parties: $S$ and $R$ restrict $x$ and $\theta$, respectively $\widehat{x}$ and $\widehat{\theta}$, to the $\lambda$ indices $i \in [2\lambda] \setminus {T}$.
    $S$ sends $\theta$ to $R$.

    \item {\bf Receiver Message.} $R$ partitions the positions of $\overline{T}$ into two parts: the ``good'' subset $I_b = \{i : \theta_i = \widehat{\theta}_i\}$ and the ``bad'' subset $I_{1-b} = \{i : \theta_i \neq \widehat{\theta}_i\}$. $R$ sends $(I_0,I_1)$ to $S$.

    \item {\bf Sender Message.} $S$ samples $s_0,s_1 \leftarrow \{0,1\}^{\lambda}$ and sends $\left(s_0,h(s_0,x_0) \oplus m_0,s_1,h(s_1,x_1) \oplus m_1\right)$, where $x_0$ is $x$ restricted to the set of indices $I_0$ and $x_1$ is $x$ restricted to the set of indices $I_1$.

    \item {\bf Receiver Output.} $R$ decrypts $s_b$ using $\widehat{x}_b$, the string $\widehat{x}$ restricted to the set of indices $I_b$.
    

    \end{enumerate}
     \end{framed}
    \caption{The~\cite{FOCS:CreKil88,C:BBCS91} OT template.}
    \label{fig:template}
\end{figure}
%e suggestion in~\cite{CK88}



As written, the protocol in Figure \ref{fig:template} requires $7$ messages of back-and-forth interaction between the sender and receiver. These can be reduced to 5 messages, by merging messages 2(b) and 3, and messages 2(c) and 4.
}\fi
%Reversing some parts of the protocol leads to an even more round-efficient protocol, as we describe next.
%We show in Appendix \ref{app:}
%First, one can see that messages sent in rounds $2(b)$ and $2(c)$ can be parallelized with messages in rounds $3$ and $4$ respectively, and sender checks from Step 3 can be deferred to Step 5, shaving off $2$ rounds.
%\amit{I don't see how $2(a)$ and $2(c)$ can be parallelized since the opening set $T$ is only known after $2(b)$}
%We now outline an approach to shave off another round, yielding a $4$ round OT protocol from extractable and equivocal commitments.



\paragraph{Reverse Crepeau-Kilian OT.} %\label{overview:reversebbcs}
%But there can be an alternative approach to establishing erasure channels between $\cS$ and $\cR$, where it is the {\em receiver} that sends BB84 states and the {\em sender} that measures them.
Suppose instead that Alice sends random BB84 states $\{\ket{x_i}_{\theta_i}\}_{i \in [n]}$ for $x_i \leftarrow \{0,1\}, \theta_i \leftarrow \{+,\times\}$, after which Bob measures these states in random bases $\{\widehat{\theta}_i\}_{i \in [n]}$.
Now instead of waiting to obtain the ``correct'' bases $\theta_i$, Bob simply sends $\{\widehat{\theta}_i\}_{i \in [n]}$ to Alice. 
When $\theta_i$ and $\widehat{\theta}_i$ match, $x_i = \widehat{x}_i$, and when $\theta_i$ and $\widehat{\theta}_i$ do not match, then $x_i$ and $\widehat{x}_i$ should be uncorrelated: again establishing an erasure channel on which Bob can send Alice messages. However, unlike CK88, the player that is performing measurements in random bases {\em need not wait to learn the right bases}, and instead simply announces his own bases to set up a reverse erasure channel.
Note that with this modification, Bob does not need to send a measurement check message anymore!
%, and can announce the random bases he used to perform measurements to set up a channel. 
%and helps reduce a round of interaction because . 

%\amit{I think the following attack is for a malicious receiver (and not the sender)}
However, this protocol leads to new avenues of attack for a malicious Alice: in particular, Alice can send halves of EPR pairs in the first round and given $\{\widehat{\theta}_i\}_n$, perform measurements to determine all $x_i$ values. 
Such attacks can be prevented by means of a ``reverse'' measurement check: namely, Alice {\em commits to all $x_i$ and $\theta_i$ values} in the first message, and given a random $T \subset [2\lambda]$ of size $\lambda$ picked by Bob, reveals all committed values $\{x_i, \theta_i\}_{i \in T}$. 
Given Alice's openings, for every $i \in [T]$, Bob performs a projective measurement of the states obtained in round $1$ onto $\{\dyad{\psi_i}{\psi_i}, \mathbb{I}- \dyad{\psi_i}{\psi_i}\}$ where $\psi_i = \ket{x_i}_{\theta_i}$, and aborts if any of the outcomes don't match $\dyad{\psi_i}{\psi_i}$. The resulting three round random-input OT protocol is summarized in Figure \ref{fig:3-round}. 



\begin{figure}[ht!]
      \begin{framed}
%\protocol
%{\proref{fig:qot-4r-bb84-construction}}
%{A 4-round QOT protocol. $h : \{0,1\}^{k(\lambda)} \times \cX \rightarrow \{0,1\}^\lambda$ is a universal hash function family with seed length $k(\lambda)$, and domain $\cX = \{0,1\}^{\leq 7\lambda}$. $IdealCom$ is an ideal commitment scheme. \nishant{todo - elaborate more}}
%{fig:qot-4r-bb84-construction}
%{

%\begin{tabular}{ l l }
%{\bf Bob input:} Messages $m_0,m_1 \in \{0,1\}^\lambda$. 
{\bf Alice input:} Choice bit $b \in \{0,1\}$, message $m \in \{0,1\}$. \\
\vspace{-4mm}
% \textbf{Sender $S$ Output:} $\perp$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
%\end{tabular}

%For classical bits $(x,\theta)$, let $\ket{x}_\theta$ denote $\ket{x}$ if $\theta = 0$, and $(\ket{0} + (-1)^x\ket{1})/\sqrt{2}$ if $\theta = 1$. Let $\com(\cdot)$ denote an ideal commitment scheme, $h:\{0,1\}^{3\lambda/2} \rightarrow \{0,1\}^{\lambda}$ denote a pairwise independent hash function. 


%\amit{The following protocol needs to be rewritten based on the last discussion. Specifically, the sender will measure \emph{all} of the qubits before Round 2 and perform a slightly different measurement check after Round 3.}
\begin{enumerate}
\item {\bf Alice message.}
Alice samples $x \leftarrow \{0,1\}^{\lambda}$ and $\theta \leftarrow \{+,\times\}^{\lambda}$, and sends qubits $(\ket{x_i}_{\theta_i})_{i \in [\lambda]}$ to Bob.
Alice also sends $\{\com(x_i), \com(\theta_i)\}_{i \in [\lambda]}$ to Bob.
%$R,S$ then invoke $\idealcom$ with $R$ as committer and $S$ as receiver. $R$ sends $(Commit,R,S,(x_1,\theta_1, \ldots x_{16\lambda},\theta_{16\lambda}))$ to $\idealcom$.

\item {\bf Bob Message.} 
Bob chooses $\widehat{\theta} \leftarrow \{0,1\}^{2\lambda}$ and samples a random ``large enough'' $T \subset [\lambda]$.
For $i \in [\lambda] \setminus T$, he measures the $i^{th}$ qubit received in basis $\widehat{\theta}_i$ to obtain $\widehat{x}_i$. He sends $T, \{\widehat{\theta}_i\}_{i \in [\lambda] \setminus T}$ to Alice.
%$\forall i \in \overline{T}$ it measures the $i^{th}$ qubit received from $R$ in basis $\widehat{\theta}_i$ and obtains measurement outcome $\widehat{x}_i$. It sends $T, \{\widehat{\theta}_i\}_{i \in \overline{T}}$ to $R$.

\item {\bf Alice Message.}
Alice divides $\overline{T}$ into 2 disjoint subsets $S_0, S_1$ in the following way - $S_0 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} = \theta_i \}, S_1 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} \ne \theta_i \}$. She sets $I_b = S_0$ and $I_{1-b} = S_1$ and sends $(I_0,I_1)$ to Bob.

For every $i \in T$, Alice also reveals $(x_i, \theta_i)$ along with the corresponding commitment openings to Bob. Finally, Alice sends $(x_0, x_1)$ to Bob where $x_b = m \oplus \mathsf{Extractor}(\{\widehat{x}_i\}_{i \in I_b})$ and $x_{1-b} \leftarrow \{0,1\}$.

\item {\bf Bob Output.}
For every $i \in T$, Bob measures the $i^{th}$ qubit received in Step 1 in basis $\{\dyad{\psi_i}{\psi_i}, \mathbb{I}- \dyad{\psi_i}{\psi_i}\}$ where $\psi_i = \ket{x_i}_{\theta_i}$. If any of the measured outcomes don't match $\dyad{\psi_i}{\psi_i}$, Bob aborts. Otherwise, Bob generates output $(m_0, m_1)$ as $m_0 = x_0 \oplus \mathsf{Extractor}(\{\widehat{x}_i\}_{i \in I_0}),
m_1 = x_1 \oplus \mathsf{Extractor}(\{\widehat{x}_i\}_{i \in I_1})
$.

%Bob chooses
%$s \leftarrow \{0,1\}^{k(\lambda)}$ and sends $s, y_0 = m_0 \oplus h(s || \{\widehat{x}_i\}_{i \in I_0}), y_1 = m_1 \oplus h(s || \{\widehat{x}_i\}_{i \in I_1})$ to Alice.

%\item {\bf Alice Output.} Alice computes $\widetilde{m_b} = y_b \oplus h(s || \{{x}_i\}_{i \in I_b})$ and outputs $(b, \widetilde{m_b})$.
\end{enumerate}
      \end{framed}
    \caption{Three-message random-input OT from commitments.}
    \label{fig:3-round}
\end{figure}

Unfortunately, this protocol as stated requires Bob to maintain quantum memory and store the states sent by Alice until the end of round $3$. So we modify the protocol to have Bob immediately measure all $2\lambda$ qubits in random bases $\widehat{\theta}_i$ and obtain outcomes $\widehat{x}_i$, immediately upon receiving qubits at the end of round 1. At the end of round 3, Bob checks that all indices $i \in [T]$ where $\theta_i = \widehat{\theta}_i$ satisfy $x_i = \widehat{x}_i$.
In Section \ref{sec:ot-eecom} we formally prove security of this modified protocol in the QROM, assuming that the underlying commitment scheme is {\em extractable and equivocal}. 
\dakshita{make sure this is the one we prove secure.}


\iffalse{
\begin{informaltheorem}
Assuming extractable and equivocal commitments, the protocol in Figure~\ref{fig:4-round} satisfies correctness, and security against malicious senders and receivers with negligible error.
\end{informaltheorem}

Informally, equivocality allows a simulator interacting with an arbitrary receiver to open a commitment to any given message.
Extractability allows an extractor to efficiently extract the message committed in any commitment.
As a contribution of independent interest, we build extractable and equivocal commitments in the quantum random oracle model; we summarize this construction in the next subsection.
}\fi

\iffalse{
\subsection{Extractable and Equivocal Commitments in the QROM}

To realize the reverse Crepeau-Kilian style OT mentioned in Section \ref{overview:reversebbcs} in a provably secure way, it is required that the bit commitments sent by the receiver in round 1 satisfy two additional properties (apart from the usual hiding and binding guarantees) which we now describe informally:
i) Equivocality: This property ensures that the commitment schemes admits an efficient simulator, let's say $\cS_\Equ$, which can sample commitment strings that are indistinguishable from commitment string generated honestly and later, during the opening phase, provide valid openings for both possible bits i.e. $0$ and $1$.
ii) Extractability: This property ensures that the commitment schemes admits an efficient extractor, let's say $\cS_\Ext$, which, given access to the committer, can output the bit value underlying the generated commitment string during the commitment phase.


The need for these two additional properties is not new to our work. Indeed, Damgard, Fehr, Lunemann, Salvail, and Schaffner \cite{C:DFLSS09} proved that bit commitment schemes, satisfying extraction and equivocation, suffice to instantiate the original \cite{FOCS:CreKil88,C:BBCS91} QOT template. \cite{C:DFLSS09} called their commitments dual-mode commitments, and provided a construction based on the quantum hardness of the learning with errors (QLWE) assumption. In two recent works \cite{BCKM2021, GLSV}, a construction of such commitment schemes was achieved by relying on the minimal assumption of one-way functions (in addition to quantum communication). 

%In this work, we investigate the following question:\\
%\hspace{3cm} \emph{Can we base the construction of QOT on information theoretic assumptions ?}\\


%We answer this question in the affirmative in the QROM model against a query-bounded adversary. To do this, 

In this work, we prove that the commitment scheme in Figure \ref{fig:abc} satisfies extractability and equivocality in the QROM against query bounded adversaries. 

\begin{figure}[H]
    \begin{framed}
    {Committer $\cC$ input:} $m$, 
    {Receiver $\cR$ input:} $\bot$, $H:\{0,1\}^{\lambda+2} \rightarrow \{0,1\}^{\lambda+1}$ is a random oracle.

\begin{itemize}
    \item \textbf{Commit Phase.}
    $\cC$ chooses $r \leftarrow \{0,1\}^\lambda$ and sends $c = H(0||m||r)||H(1||m||r)$ to $\cR$. 

    \item \textbf{Reveal Phase.} 
    $\cC$ sends $r$ to $R$. 
    $\cR$ outputs $m$ if $c = H(0||m||r)||H(1||m||r)$, and $\bot$ otherwise.
\end{itemize}
    \end{framed}
    \caption{Extractable and Equivocal Commitments in the QROM}
    \label{fig:abc}
\end{figure}

To argue that these commitments are equivocal, we rely on the one-way-to-hiding lemma of~\cite{Unruh15,ambainis2019quantum}, and to argue that the commitments are extractable against query-bounded adversaries, we rely on efficient simulation of random oracles by $k$-wise independent hash functions~\cite{zhandry12qwise}.
%the compressed oracle technique of~\cite{C:Zhandry16}.
%\dakshita{todo: @amit add more explanation here.}
%Later, we plug these special commitments in the reverse Crepeau-Kilian style OT mentioned in Section \ref{overview:reversebbcs} to achieve a 4 round QOT protocol which is information theoretically secure against query bounded adversaries. 

%Apart from the information theoretic security, two practically useful benefits of our special commitment scheme is that it is 
We note that in addition to simplicity, our scheme is entirely classically realizable and non-interactive. In particular, unlike \cite{BCKM2021, GLSV}, our special commitment does not involve multiple rounds or quantum communication between the committer and the receiver. We envision that this may be useful in the future as a standalone primitive for constructing provably secure post-quantum and quantum protocols in the QROM.
%and practically efficient realizations of such protocols. 

In the next section, we discuss how this scheme also helps obtain a qualitatively different unconditional OT protocol in three rounds, with specious security against senders and malicious security against receivers, in the quantum random oracle model.
}\fi

\iffalse{
\subsection{Quantum OT from Entanglement}
Next, we ask: can quantum communication help achieve unconditional OT with minimal round complexity? While the CK88 and our reverse CK88 templates seems to fundamentally require at least $4$ rounds of interaction, perhaps it is possible to go down to the (minimal) two rounds, by {\em departing} from this template, and potentially relying on entanglement\footnote{It is relatively hard but feasible to physically realize entanglement given current quantum technology, nevertheless we consider this part of our contribution to primarily be of theoretical interest.}?

We first consider the following natural candidate method of obliviously transferring one out of two strings from a sender to a receiver:
the sender samples uniform $r_0, r_1 \leftarrow \{0,1\}$, builds the quantum state $\ket{\psi} = \frac{{\ket{0 r_0} + \ket{1 r_1}}}{\sqrt{2}}$ and sends $\ket{\psi}$ to the receiver.
The receiver must measure this state in the computational basis and parse the measurement outcome as $b , x$ for $b, x \in \{0,1\}$, thereby realizing the OT functionality. While this protocol satisfies correctness, it is {\em insecure} against malicious receivers that can measure in arbitrary bases to obtain partial information about both $r_0$ and $r_1$. More generally, protocols of this form cannot exist because of the impossibility of quantum one-time programs. 
Nevertheless, all that is required to ensure security is to force the receiver to perform a measurement in the computational basis. This can be achieved using a single ``measurement-check'' response from the receiver.

To understand this step, consider a version of the protocol where the sender sends {\em many} independently sampled $\ket{\psi}_i$'s in parallel, where each $\ket{\psi}_i = \frac{\ket{0 r_{0,i}} + \ket{1 r_{1,i}}}{\sqrt{2}}$. The receiver is required to measure each of them in the computational basis, and then commit to the measurement outcomes. Then the sender could pick a random large enough subset $T$ of the commitments, ask the receiver to open this set, and check for each of the receiver's responses $(b_i, x_i)$ for $i \in T$ that $x_i = r_{b,i}$. If this is the case, (intuitively) the sender is convinced that the receiver indeed measured the remaining indices (outside the set $T$) in the computational basis. 
In fact, the measurement check can be computed using a single (non-interactive) message from the receiver, by making use of the Fiat-Shamir transform. At this point, the sender and receiver obtain a set of OT's of which all are secure against a malicious sender, and {\em most} are secure against a malicious receiver. Finally, the sender uses the third protocol message to encode both its inputs and transmit the encoded values to the receiver. 
This protocol is summarized in Figure \ref{fig:entqot}, and formally analyzed in Section \ref{sec:three-round}.

%(eg., a Hadamard basis measurement would yield \dakshita{check and fill}).



%\dakshita{discuss possible use of entanglement. impossibility of one-time programs rules out noninteractive OT, leading into what about extra round to ensure receiver measured.}

%\subsection{A 2-round protocol for Quantum Oblivious Transfer}


%\dakshita{motivate 2-round setting. talk about what the protocol does.}

\begin{figure}[ht!]
    \begin{framed}
    
    
%\protocol
%{\proref{fig:qot-2r-construction}}
%{2 round QOT protocol secure against specious sender and malicious receiver}
%{fig:qot-2r-construction}
%{

%\begin{tabular}{ l l }
%\textbf{Sender $S$ Input:} $\perp$\\ %\textbf{Sender $S$ Output:} $R_0,R_1 \in \{0,1\}$ \\
%\textbf{Receiver $R$ Input:} Bit $c \in \{0,1\}$ \\
%\textbf{Receiver $R$ Output:} $c,R_c$ \\
%\textbf{Public Random Oracles:} $\comro, \fsro, \maskro$ \\
%\end{tabular}

%\textbf{Receiver $\cR$ input: } Choice bit $c$. $H:\{0,1\}^{\lambda+2} \rightarrow \{0,1\}^{\lambda+1}$ is a random oracle. 

\begin{enumerate}

\item {\bf Sender Message.}
For $i \in [\lambda]$, $\cS$ samples uniform $r_0^i \leftarrow \{0,1\}, r_1^i \leftarrow \{0,1\}$, builds the quantum state $\ket{\psi^i} = ({\ket{0 r_0^i} + \ket{1 r_1^i}})/{\sqrt{2}}$ and sends $\{\ket{\psi^i}\}_{i \in [\lambda]}$ to $R$.

\item {\bf Receiver Message.}
$\cR$ measures each $\ket{\psi^i}$ in the computational basis $\{ \ket{00}, \ket{01}, \ket{10}, \ket{11} \}$ to obtain $\{\widehat{b}_i, \widehat{r}_i\}_{i \in [\lambda]}$. It then prepares a measurement check proof $\pi$ as follows:
\begin{enumerate}
    \item Commitment: For all $i \in [\lambda]$, $\com_i = H(\widehat{b}_i || \widehat{r}_i || \widehat{s}_i)$ where $\widehat{s}_i \leftarrow \{0, 1\}^\lambda$.
    
    \item Challenge: Use $H(\com_1, \ldots, \com_\lambda)$ to obtain random $T \subset [\lambda]$ of size $\lambda/2$.
    %$Y = \fsro(com_1 || \ldots || com_{4\lambda})$. 
    %Set T = $RandSubset_{[4\lambda],2\lambda}(Y)$.

    \item Response: Set $\pi = (\{\com_i\}_{i \in [\lambda]}, T, \{ \widehat{b}_i || \widehat{r}_i || \widehat{s}_i \}_{i \in T})$.
\end{enumerate}

It sends $\pi, \{c \oplus \widehat{b}_j \}_{j \in [2\lambda]\setminus T}$ for $c \leftarrow \{0,1\}$ to $\cS$, computes $R = \bigoplus_{j \in [2\lambda] \setminus T} \widehat{r}_j$ and outputs $(c,H(R))$.

\item {\bf Sender Message.}
$\cS$ parses $\pi,\{y_j\}_{j \in [2\lambda] \setminus T}$ and aborts if $T \neq H(\com_1, \ldots, com_{\lambda})$, or if $\com_i \neq H(\widehat{b}_i || \widehat{r}_i || \widehat{s}_i)$ for any $i \in [T]$, or if $\widehat{r}_i \neq r_{\widehat{b}_i}^i$ for any $i \in [T]$.

Otherwise it computes for $b \in \{0,1\}, R_b = \bigoplus_{i \in [\lambda] \setminus T} r_{y_j \oplus b}^i$ and sends $y_0 = m_0 \oplus H(R_0), y_1 = m_1 \oplus H(R_1)$ to $\cR$.

\item {\bf Receiver Output.} $\cR$ outputs $m_b = y_b \oplus R_b$.


\end{enumerate}

\end{framed}
    \caption{Three-Round Quantum 
    OT against Specious Senders and Malicious Receivers}
    \label{fig:entqot}
\end{figure}

%\dakshita{talking about converting to chosen-input OT. can we obtain 2-round chosen input OT.}


\begin{figure}
\begin{framed}
\dakshita{this should be commented out.}



\begin{enumerate}
\item {\bf Sender message.}
$\cS$ samples strings $c = c_1 c_2 \ldots c_\lambda \leftarrow \{0,1\}^\lambda$ and $d = d_1 d_2 \ldots d_\lambda \leftarrow \{0,1\}^{n\lambda}$.

$\cS$ sends $(\ket{d_i}_{0}, \ket{d_i \oplus c_i}_{1} )_{i \in [n\lambda]}$ to $\cR$.
%$R,S$ then invoke $\idealcom$ with $R$ as committer and $S$ as receiver. $R$ sends $(Commit,R,S,(x_1,\theta_1, \ldots x_{16\lambda},\theta_{16\lambda}))$ to $\idealcom$.

\item {\bf Receiver Message.} 
$\cR$ chooses $b \leftarrow \{0,1\}^{n\lambda}$ and measures the $i^{th}$ pair of qubits in basis $b_i$ to obtain $\widehat{a}_i, \widehat{a'}_i$. We stress that both qubits are measured in the same basis.

For every $i \in [n\lambda]$, if $b_i = 0$, set $a_i = \widehat{a}_i$ otherwise set $a_i = \widehat{a'}_i$.

\dakshita{add a measurement check message to ensure both measured in the same basis.}

Relabel the remaining indices to $[1, \ldots \frac{n}{2}\lambda]$, and cluster all the $a_i, b_i, d_i$ values into $n/2$ strings of length $\lambda$ each. Note that these strings will satisfy that for every $i \in [n/2]$, $d_i = a_i \oplus c_i b_i$.

Output $A = H(\{a_i\}_{i \in [n/2]})$ and $B = H(\{b_i\}_{i \in [n/2]})$.


\item {\bf Sender Output.}
\dakshita{$\cS$ checks the measurement check,} 
then outputs $C = \bigoplus_{i \in [n/2]} c_i$ and $D = H(\{c_i d_i\}_{i \in [n/2]})$.
\dakshita{Can also possibly move the computation of $C$ and $D$ to earlier in the protocol by not discarding the measurement check positions.}
\end{enumerate}
     \end{framed}
    \caption{Two Round  Random Choice Bit Chosen Sender Strings OT}
    \label{fig:2otstring}
\end{figure}
}\fi

==> ow2h-adaptive.tex <==
\section{Adaptive one-way to hiding lemma}

\nishant{Following is a conjecture for a stronger version of the one-way to hiding lemma, which would suffice in all of our use cases}

\begin{lemma}
Let $H : M \rightarrow N$ be a random oracle for finite sets $M,N$. Consider the following algorithms: 
    \begin{enumerate}
        \item $(\rho,x) \leftarrow A_0^H()$ : oracle algorithm $A_0$ has oracle access to $H$, makes some $q_0$ queries to $H$, and outputs quantum state $\rho$ and a value $x \in M$.
        \item $b' \leftarrow A_1^H(\rho,x,y)$ : oracle algorithm $A_1$ which has oracle access to $H$, makes some $q_1$ queries to $H$, gets as input the state $\rho$, $x \in M$ and $y \in N$, and outputs a single bit $b'$.
        \item $x' \leftarrow C^H(\rho,x,y,j)$ : oracle algorithm $C$ which has oracle access to $H$, runs $A_1^H(\rho,x,y)$ until (just before) the $j^{th}$ query, measures the $j^{th}$ query in computational basis, and outputs the measurement outcome (when $A_1$ makes $< j$ queries, $C$ outputs $\perp$).
    \end{enumerate}
    
    Let 
    $$P_A^1 = Pr[b'=1 : H \leftarrow (M \rightarrow N), (\rho,x) \leftarrow A_0^H(), b' \leftarrow A_1^H(\rho,x,H(x)]$$
    $$P_A^2 = Pr[b'=1 : H \leftarrow (M \rightarrow N), (\rho,x) \leftarrow A_0^H(), B \leftarrow N, b' \leftarrow A_1^H(\rho,x,B)]$$
    $$P_C = Pr[x=x' : H \leftarrow (M \rightarrow N), (\rho,x) \leftarrow A_0^H(), B \leftarrow N, j \leftarrow [q1], x' \leftarrow C^H(\rho,x,y,j)]$$
    
Then, if $H_\infty(x | \rho) \geq k$, then $|P_A^1 - P_A^2| \leq f(q_0,q_1,k,P_C)$, for some function $f$.
    
\end{lemma}

==> parameters.tex <==
\section{Notes on Parameters}

We want to achieve $\frac{\poly(q\secp)}{2^\secp}$ security, where $q$ is the number of random oracle queries. In all of our protocols, we will have some number of check positions $A\secp$ and some number of used positions $B\secp$, for some constants $A,B$. Let $\delta$ always correspond to the relative Hamming weight of the used positions we want to obtain via the quantum sampling game.

\subsection{Random basis protocols}

\amit{Our 4 round random basis protocol is currently not written in an extractor agnostic form. We are specifically applying the seeded extractor in the protocol.}

\noindent\paragraph{Seeded extractor.}

Constraints:
\begin{itemize}
    \item According to \cite[Theorem 2]{C:BouFeh10}, we need the quantum conditional min-entropy $H_\infty$ of the measured string to be $3\secp$ in order to extract $\secp$ bits of entropy.
    \item Since each party chooses their own sets of bases uniformly at random, we need to use Chernoff to bound the number $X$ of used positions where their bases differ. Using the bound $\Pr[X \leq (1-\epsilon)\E[X]] \leq e^{-\epsilon^2\E[X]/2}$, we need that \[\Pr[X \leq (1-\epsilon)\frac{B\secp}{2}] \leq e^{-\epsilon^2 B \secp/4} \leq 1/2^\secp.\]
    \item Let $s$ be the number of positions where their bases differ, so that the string that we want to claim is random has at least $s/2$ such positions. Then, by \cite[Corollary 1]{C:BouFeh10}, we have \[H_\infty \geq s/2 - h(\delta)B\secp.\]
    \item By \cite[Appendix B.4]{C:BouFeh10} and \cite[Theorem 3]{C:BouFeh10}, we need that \[\sqrt{6}/e^{-A\secp \delta^2/100} \leq 1/2^\secp.\] 
\end{itemize}

Tightening the second constraint gives \[\epsilon = \sqrt{\frac{4}{B \log e}}\] which means that \[s = \left(1-\sqrt{\frac{4}{B \log e}}\right)\frac{B\secp}{2}.\] Combining with the first and third constraints, we have that \[\left(1-\sqrt{\frac{4}{B \log e}}\right)\frac{B \secp}{4}-h(\delta)B\secp \geq 3\secp,\] which simplifies to \[h(\delta) \leq \frac{1}{4} - \frac{(1/\sqrt{\log e})}{2\sqrt{B}} - \frac{3}{B}.\] Thus, for $B \geq 1284$, we have that \[B \geq \left(\frac{1}{2(1/4 - h(\delta))}\right)^2.\]

By the fourth constraint, we have that \[A \geq \frac{100}{\delta ^ 2\log e }.\]

Optimizing by hand, we can set $\delta = 0.04$, giving \[A = 43322, B = 4208,\] for a total of $47630\secp$ qubits.

\amit{In the random basis framework 4-round protocol that we have currently, it is not explicit why using XOR extractor while reduce the number of rounds}

\noindent\paragraph{XOR extractor.} Here we are only extracting one bit, but without the extra round of interaction. Instead of the first and third constraint above, we have that \[s/4 \geq \delta B\lambda.\] This leads to the constraint that \[B \geq \left(\frac{\sqrt{\log e}}{4(1/8 - \delta)}\right)^2.\] Optimizing by hand, we can set $\delta = 0.11$, giving \[A = 5729, B = 401,\] for a total of $6130\secp$ qubits.

\noindent\paragraph{Random oracle extractor.} Here we can extract $\secp$ bits without an additional round of interaction. The adaptive re-programming lemma, showing an distinguishing advantage of $\frac{O(q)|L|}{2^{n/2}}$, gives the constraint \[s/4 \geq h(\delta)B\secp + \secp,\] since $|L| \leq 2^{h(\delta)B\secp}$ and $n \geq s/2$. This leads to the constraint that \[B \geq \left(\frac{.31}{1/8 - h(\delta)}\right)^2,\] for $B \geq 10000$. Optimizing by hand, we can set $\delta = 0.017$, giving \[A = 239844, B = 169937,\] for a total of $409781\secp$ qubits.

\noindent\paragraph{Notes.} The main constraint that separates these three extractors is
\begin{itemize}
    \item XOR: $s \geq 4\delta B \secp$.
    \item Seeded: $s \geq 2h(\delta)B\secp + 6\secp$.
    \item Random oracle: $s \geq 4h(\delta)B\secp + 4\secp$.
\end{itemize}

\james{I'm not sure if the Chernoff bound $(\Pr[X \leq (1-\epsilon)\E[X]] \leq e^{-\epsilon^2\E[X]/2})$ or the classical sampling game bound $(6/2^{A\secp \delta^2/50})$ are as tight as possible, but the rest of the analysis seems pretty tight.}

\dakshita{afaik the best known Chernoff bound is $(\Pr[X \leq (1-\epsilon)\E[X]] \leq \frac{e^{-\epsilon\E[X]}}{(1-\epsilon)^{(1-\epsilon)\E[X]}})$}


\subsection{Fixed basis protocols}

==> qot-3r-specious.tex <==
\section{Three-round QOT in the QROM}
\label{sec:three-round}
\subsection{Construction}

Our construction of three-round QOT (\proref{fig:qot-3r-construction}) makes use of the following.

\begin{itemize}
    \item A non-interactive extractable and equivocal commitment scheme $(\Com^H,\Open^H,\Rec^H)$ (\cref{sec:eecom}) which satisfies \emph{extraction with stateless simulation}. We will use this commitment scheme to commit to a set of strings of length $\secp + 1$, and open some subset $T$ of the strings. This ``string commitment with selective opening'' functionality can easily be obtained from the bit commitment with selective opening described in \cref{sec:eecom}.   
    \item Random oracles $\comro,\fsro,\maskro$. $\comro$ is the random oracle used by the commitment scheme. $\fsro$ is used for Fiat-Shamir, and its domain is the space of $\secp$ commitments and its range is all $(\secp/2)$-size subsets of $[\secp]$. $\maskro$ is used to mask the sender's messages and has domain $\{0,1\}^{\secp + \secp(\secp/2)}$ and range $\{0,1\}^\secp$.
    %\item A universal hash function $h: \{0,1\}^{k(\secp)} \otimes \{0,1\}^\secp \to \{0,1\}$ with seed length $k(\secp) = \poly(\secp)$.
\end{itemize}

 

\protocol
{\proref{fig:qot-3r-construction}}
{Three-round QOT protocol secure against specious senders and malicious receivers.}
{fig:qot-3r-construction}
{

\begin{tabular}{ l l }
\textbf{Sender $S$ Input:} $m_0,m_1 \in \{0,1\}^\secp$\\
\textbf{Receiver $R$ Input:} $b \in \{0,1\}$ \\
\textbf{Random Oracles:} $\comro, \fsro, \maskro$ \\
\end{tabular}


\begin{enumerate}

\item First message from $S$.
\begin{enumerate}
    \item For each $i \in [\secp]$, sample $r_{i,0},r_{i,1} \gets \{0,1\}^\secp$ and prepare $\ket{\psi_i} = \frac{\ket{0, r_{i,0}} + \ket{1, r_{i,1}}}{\sqrt{2}}$.
\end{enumerate}
$S$ sends $\{\ket{\psi_i}\}_{i \in [\secp]}$ to $R$.

\item Second message from $R$.
\begin{enumerate}
    \item Measure each $\ket{\psi_i}$ in the computational basis to obtain $\{\widehat{b}_i, \widehat{r}_i\}_{i \in [\secp]}$.
    \item Compute $(\state,\{\com_i\}_{i \in [\secp]}) \gets \Com^{\comro}(\{\widehat{b}_i,\widehat{r}_i\}_{i \in [\secp]}).$
    \item Compute $T = \fsro(\com_1,\dots,\com_{\secp})$, where $T \subset [\secp]$ and $|T| = \secp/2$.
    \item Compute $\{(\widehat{b}_i,\widehat{r}_i),s_i\}_{i \in T} \gets \Open^\comro(\state,T)$.
\end{enumerate}

$R$ sets $c_i \coloneqq b \oplus \widehat{b}_i$ for $i \in \overline{T}$ and sends $(\{\com_i\}_{i \in [\secp]},T,\{ (\widehat{b}_i, \widehat{r}_i),s_i \}_{i \in T}, \{c_i\}_{i \in \overline{T}})$ to $S$.

%$R$ sends $\pi, \{c \oplus \widehat{b}_j \}_{j \in \overline{T}}$ to $S$, computes $R = \bigoplus_{j \in \overline{T}} \widehat{r}_j$ and outputs $(c,\maskro(R))$.

\item Third message from $S$.
\begin{enumerate}
    \item Abort if $T \neq \fsro(\com_1,\dots,\com_{\secp})$.
    
    \item Abort if $\Rec^\comro(\{\com_i\}_{i \in T},\{(\widehat{b}_i,\widehat{r}_i),s_i\}_{i \in T}) = \bot$ or for any $i \in T$, $\widehat{r}_i \neq r_{i,\widehat{b}_i}$.

    \item Otherwise, set $\{\tilde{r}_{i,b} \coloneqq r_{i,c_i \oplus b}\}_{i \in \overline{T}, b \in \{0,1\}}$ and define $R_0 = \{\tilde{r}_{0,i}\}_{i \in \overline{T}}, R_1 = \{\tilde{r}_{1,i}\}_{i \in \overline{T}}.$
    
    \item Sample seeds $t_0,t_1 \gets \{0,1\}^{\secp}$.
\end{enumerate}

$S$ sends $(t_0,m_0 \oplus \maskro(t_0,R_0),t_1,m_1 \oplus \maskro(t_1,R_1))$ to $R$.

\item $R$ parses $S$'s message as $(t_0,d_0,t_1,d_1)$ and outputs $m_b = d_b \oplus \maskro(t_b,\{\widehat{r}_i\}_{i \in \overline{T}})$.

\end{enumerate}
}


\subsection{Sender Security}

In this section, we show simulation security against a malicious receiver. First, we give a high-level overview of the proof.

The goal will be to show that any malicious receiver $\cR$ that obtains information about both of the sender strings $m_0,m_1$ can be used to construct an algorithm $G$ such that
\[\Pr_{r_0,r_1 \gets \{0,1\}^\secp}\left[(r_0,r_1) \gets G\left(\frac{\ket{0,r_0} + \ket{1,r_1}}{\sqrt{2}}\right)\right] = 1/\poly(\secp).\]

However, such a $G$ cannot exist, as we show in \cref{claim:trace-distance}.

%since the mixed state $\frac{\ket{0,r_0} + \ket{1,r_1}}{\sqrt{2}}$ for $r_0,r_1 \gets \{0,1\}^\secp$ is within negligible trace distance of the mixed state that is $\ket{0,r_0}$ with probability 1/2 and $\ket{1,r_1}$ with probability 1/2, 

Towards constructing $G$, we first use the random oracle $\maskro$ to show that if $\cR$ learns information about some $m_b$, then it must be able to predict $R_b$ with some $1/\poly(\secp)$ probability. This follows via an application of an appropriate One-Way to Hiding lemma. Let $E_b$ be the machine, defined based on $\cR$, that predicts $R_b$ with $1/\poly(\secp)$ probability.

Next, we make use of the extractor for the commitment scheme to obtain some values $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$ from the commitments $\{\com_i\}_{i \in [\secp]}$ that $\cR$ sends in the second round. Now, if the sender doesn't abort, we know that for all $i \in T$ (the ``measurement check'' subset), it holds that $\widetilde{r}_i = r_{i,\widetilde{b}_i}$. On the other hand, we have no a priori guarantee on $\widetilde{r}_i$ for $i \in \overline{T}$, since $\cR$ samples $T$ along with $\{\com_i\}_{i \in [\secp]}$. However, since $T$ is defined as a random oracle hash of $\{\com_i\}_{i \in [\secp]}$, $\cR$ should not have too much control over the subset $T$. To formalize this intuition, we use the Measure-and-Reprogram lemma to show that $T$ can be sampled uniformly at random \emph{after} the message $\{\com_i\}_{i \in [\secp]}$ is determined (and thus, after the extracted values $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$ are determined), with some polynomial loss in how well $E_b$ predicts the value $R_b$.

Now, once $T$ is sampled after $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$, we can argue that if $\widetilde{r}_i = r_{i,\widetilde{b}_i}$ for all $i \in T$, this must also hold for (almost) all $i \in \overline{T}$, except with negligible probability. Thus, for some bit $b^*$, we can argue that with $1/\poly(\secp)$ probability, there must exist $i^* \in \overline{T}$ such that the commitment extractor outputs $\widetilde{r}_{i^*} = r_{i^*,b^*}$, and $E_{1-b^*}$ outputs $R_{1-b^*}$, which contains $r_{i^*,1-b^*}$. This observation can finally be used to construct the algorithm $G$ with takes as input a single state $\frac{\ket{0,r_0} + \ket{1,r_1}}{\sqrt{2}}$, inserts it into the sender's first message at position $i^*$, and then runs $\cR$ (with modifications made by the Measure-and-Reprogram simulator, the One-Way to Hiding predictor, and the extractor for the commitment scheme) to produce both $r_0$ and $r_1$.

Full details are given in the proof of the theorem below.



\begin{theorem}
Say that $\Com$ is $\mu_\Com(\secp,q(\secp))$-extractable. Then \proref{fig:qot-3r-construction} $\left(\mu_\Com(\secp,q(\secp)) + 5q^2\left(\frac{3}{4}\right)^{\secp/4} + 8q^{3/2}\left(\frac{1}{2}\right)^{\secp/2}\right)$-securely realizes $\cF_{\mathsf{OT}}$ with query-bounded simulation in the QROM against malicious receivers (\cref{def:secure-realization}). 
\end{theorem}

\begin{proof}

This proof considers infinite families of quantum advice and quantum machines, parameterized by $\secp$, but we drop the $\secp$ to avoid notational clutter.

For any query bound $q$ and malicious receiver $\cR$, we describe a simulator $\cS$.

\begin{itemize}
    \item Let $\cS_\Ext = \cS_\Ext[q]$ be the extractor for the commitment scheme.
    \item Run the honest sender algorithm to produce a first message $\{\ket{\psi_i}\}_{i \in [\secp]}$, which it sends to $\cR$. Answer $\cR$'s queries to $\comro$ using $\cS_\Ext$ and queries to $\fsro,\maskro$ honestly (by forwarding them to $\fsro,\maskro$).
    \item When $\cR$ outputs $(\{\com_i\}_{i \in [\secp]},T, \{ \widehat{b}_i, \widehat{r}_i,s_i \}_{i \in T}, \{c_i\}_{i \in \overline{T}})$, run $\cS_\Ext$ on $\{\com_i\}_{i \in [\secp]}$ to obtain $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$. Set $b^*$ to be the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$.
    \item Query the ideal funtionality with $b^*$ and receive $m_{b^*}$.
    \item Run the honest sender algortihm to produce a third message, except that $d_{1-b^*}$ is sampled as a uniformly random string.
    \item Run the final stage of $\cR$ and the distinguisher $\cD$, answering $\comro$ queries with $\cS_\Ext$ and $\fsro,\maskro$ queries honestly.
\end{itemize}

Now, for any $(\brho,\bsigma,\cR,\cD,(m_0,m_1))$, consider the following hybrids. Let $\Pi$ be \proref{fig:qot-3r-construction}. 

%Let $q = q + q_\cR$ be an upper bound on the number of oracle queries made by $\cR$ and $\cD$ throughout the experiment.

\begin{itemize}
    \item $\Hyb_0$: This is the execution of the real world $\Pi[\brho,\bsigma,\cR,\cD,(m_0,m_1)]$.
    \item $\Hyb_1$: This is the execution of the real world, except that 
    \begin{itemize}
        \item all of $\cR$'s and $\cD$'s queries to $\comro$ are answered with $\cS_\Ext = \cS_\Ext[q]$,
        \item $\cS_\Ext$ is run on $\{\com_i\}_{i \in [\secp]}$ to obtain $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$,
        %\item $b^*$ is defined to be the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$),
        \item and $S$ now aborts if for any $i \in T$, $\widetilde{r}_i \neq r_{i,\widetilde{b}_i}$ rather than if $\widehat{r}_i \neq r_{i,\widehat{b}_i}$.
    \end{itemize}
    \item $\Hyb_2$: Define $\maskro^\bot = \maskro$ except that for any input $x$ of the form $(t_0,\cdot)$ or $(t_1,\cdot)$, $\maskro^\bot(x) = \bot$. In this hybrid, all of $\cR$'s queries to $\maskro$ are instead answered with $\maskro^\bot$ until right after $S$'s final message is sent, at which point all queries to $\maskro$ are answered with $\maskro$.
    \item $\Hyb_3$: Define $b^*$ to be the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$. In this hybrid, $d_{1-b^*}$ is set to $m_{1-b^*} \oplus u$, where $u \gets \{0,1\}^\secp$.
    \item $\Hyb_4$: This is the execution of the ideal world $\widetilde{\Pi}_{\cF_{\mathsf{OT}}}[\brho,\bsigma,\cS,\cD,(m_0,m_1)]$.
\end{itemize}

\begin{lemma}
$|\Pr[\Hyb_0 = 1] - \Pr[\Hyb_1 = 1]| \leq \mu_\Com(\secp,q(\secp)).$
\end{lemma}

\begin{proof}
This follows directly from the extractability of the commitment scheme (\cref{def:extractable}).
\end{proof}

\begin{lemma}\label{lemma:1-2}
$|\Pr[\Hyb_1 = 1] - \Pr[\Hyb_2 = 1]| \leq 4q^{3/2} / 2^{\secp/2}.$
\end{lemma}

\begin{proof}
This follows from an application of One-Way to Hiding (\cref{impthm:ow2h}), by setting $O_1 = \maskro$ and $O_2 = \maskro^\bot$. Indeed, since $t_0,t_1$ are uniformly sampled $\secp$-bit strings, it follows that $P_{guess} = 2q/2^\secp$. Thus, $|\Pr[\Hyb_1 = 1] - \Pr[\Hyb_2 = 1]| \leq 2q \sqrt{2q/2^\secp} \leq 4q^{3/2}/2^{\secp/2}.$
\end{proof}

In order to prove the next indistinguishability, we will make use of the following claim.

\nishant{claim updated below -- update rest of hte proof}
\begin{claim}
\label{claim:trace-distance}
For any quantum algorithm $G$, 
\[
    \Pr_{r_0,r_1 \gets \{0,1\}^\secp}\left[(r_0,r_1) \gets G\left(\frac{\ket{0,r_0}+\ket{1,r_1}}{\sqrt{2}}\right)\right] \leq \frac{3}{2^{\frac{\secp}{2}+1}}.
\]
%Let $\brho_0 = \left\{\frac{1}{2^{2\secp}},\frac{\ket{0,r_0} + \ket{1,r_1}}{\sqrt{2}}\right\}_{r_0,r_1 \in \{0,1\}^\secp}$ and $\brho_1 = \left\{\frac{1}{2^{\secp + 1}},\ket{b,r}\right\}_{b \in \{0,1\},r \in \{0,1\}^\secp}$. Then it holds that $\TD(\brho_0,\brho_1) = \frac{1}{2^\secp}$.
\end{claim}

\begin{proof}
Assume there exists a $G$ that outputs $(r_0,r_1)$ with $> 3/2^{1+(\secp/2)}$ probability. Consider the following mixed states \begin{align*}&\brho_0 = \left\{\frac{1}{2^{2\secp}},\frac{\ket{0,s_0,r_0} + \ket{1,s_1,r_1}}{\sqrt{2}}\ket{s_0 \oplus s_1}\right\}_{s_0,s_1,r_0,r_1 \in \{0,1\}^{\secp/2}}, \\ &\brho_1 = \left\{\frac{1}{2^{2\secp + 1}},\ket{b,s_b,r_b}\ket{s_0 \oplus s_1}\right\}_{b \in \{0,1\},s_0,s_1,r_0,r_1 \in \{0,1\}^{\secp/2}},\end{align*} and let $G'$ be the algorithm that takes $\brho_c$ for $c \in \{0,1\}$ as input, runs $G$ on the first $\secp+1$ qubits to obtain some output $((\widetilde{s}_0,\widetilde{r}_0), (\widetilde{s}_1,\widetilde{r}_1))$, and then outputs 1 if $\widetilde{s}_0 \oplus \widetilde{s}_1$ is equal to the classical string held in the final $\secp/2$ qubits. Note that by definition, $\Pr[G'(\brho_0) = 1] > 3/2^{1+(\secp/2)}$. On the other hand, it is easy to see that $\Pr[G'(\brho_1) = 1] = 1/2^{\secp/2}$, since $s_{1-b}$ can be sampled after $G$ has already been applied to the first registers. Hence, $|\Pr[G'(\brho_0) = 1] - \Pr[G'(\brho_1) = 1]| > 1/2^{1+(\secp/2)}$

Now, to reach a contradiction, we show that for any $G'$, $|\Pr[G'(\brho_0) = 1] - \Pr[G'(\brho_1) = 1]| \leq 1/2^{1+(\secp/2)}$, hence giving us a contradiction. In fact we will show something stronger, that for each fixed $s_0,s_1 \in \{0,1\}^{\secp/2}$, $|\Pr[G'(\brho_{0,s_0,s_1}) = 1] - \Pr[G'(\brho_{1,s_0,s_1}) = 1]| \leq 1/2^{1+(\secp/2)}$, where
\begin{align*}
    &\brho_{0,s_0,s_1} = \left\{\frac{1}{2^\secp},\frac{\ket{0,s_0,r_0} + \ket{1,s_1,r_1}}{\sqrt{2}}\right\}_{r_0,r_1 \in \{0,1\}^{\secp/2}},\\
    &\brho_{1,s_0,s_1} = \left\{\frac{1}{2^\secp},\frac{1}{2}\dyad{0,s_0,r_0}{0,s_0,r_0} + \frac{1}{2}\dyad{1,s_1,r_1}{1,s_1,r_1}\right\}_{r_0,r_1 \in \{0,1\}^{\secp/2}}.
\end{align*}
To show this, we prove in Appendix~\ref{app:tracedistance} that $\TD(\brho_{0,s_0,s_1},\brho_{1,s_0,s_1}) = \frac{1}{2^{\frac{\secp}{2}+1}}$.\\
Note that each $b \in \zo$, 
\[
    \brho_b = \frac{1}{2^\secp} \sum_{s_0,s_0 \in \zo^{\secp/2}} \brho_{b,s_0,s_1} \otimes \dyad{s_0 \oplus s_1}{s_0 \oplus s_1}
\]
Hence, \nishant{todo: expand more on the below?}
\begin{align*}
    % \TD(\brho_0,\brho_1) &= \frac{1}{2} \Tr \left( \sqrt{\left( \brho_0 - \brho_1 \right)^2} \right)\\
    % &= \frac{1}{2} \Tr \left( \sqrt{\left( \frac{1}{2^\secp} \sum_{s_0,s_1 \in \zo^{\secp/2}} (\brho_{0,s_0,s_1}-\brho_{1,s_0,s_1}) \otimes \dyad{s_0 \oplus s_1}{s_0 \oplus s_1} \right)^2} \right)\\
    % &= \TD \left( \brho_{0,s_0,s_1},\brho_{1,s_0,s_1} \right)\\
    \TD(\brho_0,\brho_1) &= \frac{1}{2^{\frac{\secp}{2}+1}}
\end{align*}
And since trace distance corresponds to the minimum error state discrimination probability \nishant{citation?}, we get that for any $G'$, $|\Pr[G'(\brho_0) = 1] - \Pr[G'(\brho_1) = 1]| \leq 1/2^{1+(\secp/2)}$, hence giving us a contradiction.


\end{proof}

\begin{lemma}
$|\Pr[\Hyb_2 = 1] - \Pr[\Hyb_3 = 1]| \leq 5q^2\left(\frac{3}{4}\right)^{\secp/4}.$
\end{lemma}

\begin{proof}

First, define $\epsilon \coloneqq |\Pr[\Hyb_2 = 1] - \Pr[\Hyb_3 = 1]|.$ Note that the only difference between $\Hyb_2$ and $\Hyb_3$ is the value of $\maskro(t_{1-b^*},R_{1-b^*})$, which is only given to $\cR$ after the final message from $S$. This observation implies the following.

\begin{itemize}
    \item If these hybrids are distinguishable with $\epsilon$ probability, then it must be the case that $S$ does not abort with probability $\geq \epsilon$, since this message is not given to $\cR$ if $S$ aborts. Define $\epsilon_{\mathsf{no-abort}}$ to be the probability of abort in both $\Hyb_2$ and $\Hyb_3$.
    \item The difference between these hybrids can be captured by a difference in the oracle given to $(\cR,\cD)$ after $S$'s final message is sent. That is, define $\Hyb_3'$ to be the same as $\Hyb_3$ except that $d_{1-b^*} = m_{1-b^*} \oplus \maskro(t_{1-b^*},R_{1-b^*})$, and $(\cR,\cD)$ is given access to the oracle $\maskro'$, which is equal to $\maskro$ except that $\maskro'(t_{1-b^*},R_{1-b^*}) = v$ for a freshly sampled $v \gets \{0,1\}^\secp$. This is identically distributed to $\Hyb_3$. Indeed, before $S$'s final message is sent, $\cR$ has no access to (the uniformly random string) $\maskro(t_{1-b^*},R_{1-b^*})$ since $\maskro$ was ``punctured'' at all points of the form $(t_{1-b^*},\cdot)$.
\end{itemize}

Next, define $\epsilon_{\mathsf{dist}} \coloneqq |\Pr[\Hyb_2 = 1 | \text{no abort}] - \Pr[\Hyb_3 = 1 | \text{no abort}]|,$ and note that $\epsilon = \epsilon_{\mathsf{no-abort}} \cdot \epsilon_{\mathsf{dist}}$.

%Now, assume for contradiction that $|\Pr[\Hyb_2 = 1] - \Pr[\Hyb_3 = 1]| = 1/\poly(\secp).$ 

\begin{claim}\label{claim:guessing}
Let $(\btau_{\mathsf{na}},\bsigma)$ be the joint state of $(\cR,\cD)$ after $S$ sends its final message in $\Hyb_3$, conditioned on the event that $S$ did not abort. There exists an oracle machine $E^{\fsro}$ that makes at most $q$ queries to $\fsro$ such that $\Pr[E^{\fsro}(\btau_{\mathsf{na}},\bsigma) = R_{1-b^*}] \geq (\epsilon_\mathsf{dist}/2q)^2$. 
\end{claim}

\begin{proof}

First, define $(\btau'_{\mathsf{na}},\bsigma)$ to be the joint state of $(\cR,\cD)$ in $\Hyb_3'$ after $S$ sends its final message, conditioned on $S$ not aborting. Let $F^{\fsro,\maskro'}[\cS_\Ext,\cR,\cD]$ be the quantum machine that completes the execution of $\Hyb_3'$ and outputs a single bit. By the above two observations, we know that \[|\Pr[F^{\fsro,\maskro'}[\cS_\Ext,\cR,\cD](\btau'_{\mathsf{na}},\bsigma)] - \Pr[F^{\fsro,\maskro}[\cS_\Ext,\cR,\cD](\btau'_{\mathsf{na}},\bsigma)]| = \epsilon_{\mathsf{dist}}.\]

Thus, by setting $O_1 = \maskro'$, $O_2 = \maskro$, and $z$ equal to a (potentially inefficient) classical description of $(\btau'_{\mathsf{na}},\bsigma)$, it follows from \cref{impthm:ow2h} that there exists $E$ that makes at most $q$ queries to $\fsro$ such that \[\Pr[E^{\fsro,\maskro'}(\btau'_{\mathsf{na}},\bsigma) = R_{1-b^*}] \geq (\epsilon_{\mathsf{dist}}/2q)^2.\] %We know that $E$ only makes $\poly(\secp)$ oracle queries to $\fsro$ since $F$ only made $\poly(\secp)$ queries to $\fsro$, and $E$ is defined to simply run $F$ and measure a random query to $\maskro'$. 
%Since $S$ does not abort with probability $1/\poly(\secp)$, this implies that \[\Pr[E^{\fsro,\maskro'}(\btau',\bsigma) = R_{1-b^*}] = 1/\poly(\secp),\] where $(\btau',\bsigma)$ is the joint state of $(\cR,\cD)$ after $S$ sends its final message in $\Hyb_3'$. 

Thus, we have that 

\[\Pr[E^{\fsro,\maskro}(\btau_{\mathsf{na}},\bsigma) = R_{1-b^*}] \geq (\epsilon_{\mathsf{dist}}/2q)^2,\] which follows from the definitions of $\Hyb_3,\Hyb_3',\maskro,\maskro'$ given above. Finally, we can re-define $E$ to include a full description of $\maskro$, and only give it oracle access to $\fsro$. \end{proof}


%Moreover, let $(\btau,\bsigma)$ be the joint state of $\cR$ and $\cD$ after $S$ sends its final message in $\Hyb_3$, conditioned on $S$ not aborting. By \cref{impthm:ow2h}, there exists a quantum oracle machine $E^{\fsro,\maskro}$ such that $E^{\fsro,\maskro}(\btau,\bsigma) = R_{1-b^*}$ with probability $1/\poly(\secp)$.

Now, consider the oracle machine $M^{\fsro}(\brho,\bsigma)$ that does the following.

\begin{itemize}
    \item Run $\Hyb_3$ coherently, forwarding any $\fsro$ queries to its external oracle, and sampling $\maskro$ internally, until right after $S$ sends the final message of the protocol.
    \item Run $E^{\fsro}$ coherently on the joint state of the receiver and distinguisher.
    \item Measure the appropriate registers to obtain the honest sender's initial randomness $\{r_{i,0},r_{i,1}\}_{i \in [\secp]}$, (part of) $\cR$'s classical message $(\{\com_i\}_{i \in [\secp]},T, \{c_i\}_{i \in \overline{T}})$, $\cS_\Ext$'s output $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$, and $E^{\fsro}$'s output $\widetilde{R}_{1-b^*}$.
\end{itemize}

Let $x \coloneqq \{\com_i\}_{i \in [\secp]}$, $z \coloneqq (\{r_{i,0},r_{i,1}\}_{i \in [\secp]},T, \{c_i\}_{i \in \overline{T}},\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]},\widetilde{R}_{1-b^*})$, and consider the predicate $V(x,H(x),z)$ that checks the following.

\begin{enumerate}
    \item $H(x) = T$,
    \item for each $i \in [T]$, $\widetilde{r}_{i} = r_{i,\widetilde{b}_i}$, and 
    \item $\widetilde{R}_{1-b^*} = \{r_{i,c_i \oplus b^* \oplus 1}\}_{i \in \overline{T}}$, where $b^*$ is the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$.
\end{enumerate}

We have established above that \[\Pr[V(x,H(x),z)) : (x,z) \gets M^{\fsro}(\brho,\bsigma)] \geq \epsilon_{\mathsf{no-abort}} \cdot (\epsilon_\mathsf{dist}/2q)^2 \geq \epsilon^2 / 2q^2,\] since  the first two conditions must hold if $S$ does not abort, and \cref{claim:guessing} shows that the third condition holds with probability $(\epsilon_\mathsf{dist}/2q)^2$, conditioned on $S$ not aborting. Thus, by \cref{thm:measure-and-reprogram}, there exists a two-stage $\cS[M]$ (that runs $M^{\fsro}$ honestly, except that it responds to $\fsro$ queries and introduces an extra measurement of one of $M$'s registers), such that 

\[\Pr\left[V(x,T',z) = 1 : \begin{array}{r} (x,\btau) \gets \cS[M](\brho,\bsigma) \\ T' \gets \cT_{\secp,\secp/2} \\ z \gets \cS[M](\btau,T') \end{array}\right] \geq \epsilon^2/2q^2(2q+1)^2,\]

where $\cT_{\secp,\secp/2}$ is the set of subsets of $[\secp]$ of size $\secp/2$. Now consider the predicate $V'(x,T',z)$ that checks the following.

\begin{itemize}
    \item $T' = T$,
    \item for at least $3\secp/4$ indices $i \in [\secp]$, it holds that $\widetilde{r}_{i} = r_{i,\widetilde{b}_i}$, and 
    \item $R_{1-b^*} = \{r_{i,c_i \oplus b^* \oplus 1}\}_{i \in \overline{T}}$, where $b^*$ is the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$.
\end{itemize}

\begin{claim}
It holds that \[\Pr\left[V'(x,T',z) = 1 : \begin{array}{r} (x,\btau) \gets \cS[M](\brho,\bsigma) \\ T' \gets \cT_{\secp,\secp/2} \\ z \gets \cS[M](\btau,T') \end{array}\right] \geq \epsilon^2/2q^2(2q+1)^2 - (3/4)^{\secp/2}.\]
\end{claim}

\begin{proof}

Consider any $x = \{\com_{i}\}_{i \in [\secp]}$ output by the first stage of $\cS[M]$, and note that $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]} \gets \cS_\Ext(x)$ may be determined at this point, since $\cS_\Ext$ is a stateless simulator. Consider the event $E_\mathsf{bad}$ that for at least $\secp/4$ indices $i \in [\secp]$, it holds that $\widetilde{r}_{i,\widetilde{b}_i} \neq r_{i,\widetilde{b}_i}$. We have that \[\Pr_{T' \gets \cT_{\secp,\secp/2}}\left[\forall \ i \in [T'], \widetilde{r}_{i} = r_{i,\widetilde{b}_i} \ | \ E_{\mathsf{bad}}\right] \leq \left(\frac{3}{4}\right)^{\secp/2},\] which implies that

\[\Pr\left[V(x,T',z) = 1  \wedge E_\mathsf{bad}: \begin{array}{r} (x,\btau) \gets \cS[M](\brho,\bsigma) \\ T' \gets \cT_{\secp,\secp/2} \\ z \gets \cS[M](\btau,T') \end{array}\right] \geq \epsilon^2/2q^2(2q+1)^2 - (3/4)^{\secp/2}.\] This completes the proof of the claim by plugging in the definition of $E_\mathsf{bad}$.

\end{proof}

Now, observe that whenever $V'$ holds, there must exist some index $i^*$ such that 
\begin{itemize}
    \item $b^* = c_{i^*} \oplus \widetilde{b}_{i^*}$, 
    \item $\widetilde{r}_{i^*} = r_{i^*,\widetilde{b}_{i^*}}$,
    \item and $R_{1-b^*}$ contains the string $r_{i^*,1-\widetilde{b}_{i^*}}$.
\end{itemize}

Thus, by a union bound, we have that there exists some fixed index $i^*$ such that the above conditions hold with probability $\epsilon^2/\secp2q^2(2q+1)^2 - (1/\secp)(3/4)^{\secp/2}$. Now consider the following machine $G$.

\begin{itemize}
    \item $G$ is initialized with $(\brho,\bsigma)$, and takes as input $\frac{\ket{0,r_0} + \ket{1,r_1}}{\sqrt{2}}$, where $r_0,r_1 \gets \{0,1\}^\secp$.
    \item $G$ runs $\cS[M]$, using its input state as the $i^*$th message from sender $S$ and sampling $\{r_{i,0},r_{i,1}\}_{i \neq i^*}$ uniformly at random. If $b^* \neq c_{i^*} \oplus \widetilde{b}_{i^*}$, abort. Otherwise, continue, and in the sender's third message, use $\widetilde{r}_{i^*}$ in place of $r_{i^*,c_{i^*} \oplus b^*}$. Note that in this case, $r_{i^*,c_{i^*} \oplus b^* \oplus 1}$ is not needed to run $\cS[M]$, since it is not needed to run $M$.
    \item Output $\widetilde{r}_{i^*}$, and $\widetilde{R}_{1-b^*}$.
\end{itemize}

We have that with $\epsilon^2/\secp2q^2(2q+1)^2 - (1/\secp)(3/4)^{\secp/2}$ probability, $G$'s output contains both $r_0$ and $r_1$. Thus, due to \cref{claim:trace-distance}, it must hold that 

\[\epsilon^2/\secp2q^2(2q+1)^2 - (1/\secp)(3/4)^{\secp/2} \leq 2/2^{\secp/2},\]

which gives that

\[\epsilon \leq 5q^2\left(\frac{3}{4}\right)^{\secp/4},\] completing the proof.

%To complete the proof, we'll follow these steps.

%\begin{itemize}
    %\item Use \cref{impthm:ow2h} to argue that there exists an oracle quantum operation $E^{\fsro}$ that can be applied to the joint state of receiver and distinguisher after round 3, and outputs $R_{1-b^*}$ with probability $1/\poly(\secp)$. 
    %\item Consider the predicate that outputs 1 if $S$ does not abort and $E$ outputs $R_{1-b^*}$. Change the experiment to invoke the measure-and-reprogram simulator. Appeal to measure-and-reprogram to say that this predicate still outputs 1 with noticeable probability.
    %\item Due to structure of the simulator, show that this implies that $\cS_\Ext$ outputs most correct $r_{i}$ with noticeable probability. This should follow because the query to $\fsro$ fixes these extracted values (not sure if this holds given our currect definition of extraction - may need the property that the extractor's behavior does not change from query to query).
    %\item Show that this violates \cref{claim:trace-distance}.
%\end{itemize}



\end{proof}

\begin{lemma}
$|\Pr[\Hyb_3 = 1] - \Pr[\Hyb_4 = 1]| \leq 4q^{3/2} / 2^{\secp/2}.$
\end{lemma}

\begin{proof}
The only difference between these two hybrids is that in $\Hyb_3$, $\maskro$ is punctured at inputs $(t_0,\cdot)$ and $(t_1,\cdot)$ until after $S$ sends its final message. Thus, this follows from the same argument used in \cref{lemma:1-2}.
\end{proof}


%\james{start of old argument based on universal hashing}
%Now, consider the following (part of the) state of the experiment $\Hyb_1$ after step $(c)$ of the computation of the third message by (honest) $S$. The state consists of registers that hold the classical strings $(R_0,R_1)$, the classical part of the transcript $(\{\com_i\}_{i \in [\secp]}, \{ (\widehat{b}_i, \widehat{r}_i),s_i \}_{i \in T}, \{c_i\}_{i \in \overline{T}})$, the output $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [\secp]}$ of $\cS_\Ext$, the classical description of the random oracles $\comro,\fsro$, the sender's input $(m_0,m_1)$, the malicious receiver $\cR$'s current state $\btau$, and the distinguisher's state $\bsigma$. If there was an abort in step (b), we instead define $R_0,R_1 \gets \{0,1\}^\secp$. We can also define the bit $b^*$ to be the most frequently occuring bit in $\{c_i \oplus \widetilde{b}_i\}_{i \in \overline{T}}$, define register $\gray{R}$ to hold the classical string $R_{1-b^*}$, and define register $\gray{Y}$ to hold the entire rest of the state. Letting $p_R$ be the probability the register $\gray{R}$ holds string $R \in \{0,1\}^\secp$ over the randomness of the experiment up until this point, the state can be written as

%\[\sum_{R \in \{0,1\}^\secp} p_R \ket{R}\bra{R}^{\gray{R}} \otimes \by_R^{\gray{Y}}.\]

%Now, due to \cref{thm:privacy-amplification} and the observation above about the difference between $\Hyb_1$ and $\Hyb_2$, it follows that if $\mathbf{H}_\infty(R \mid \mathbf{y}) = \omega(\log(\secp))$, then $|\Pr[\Hyb_1 = 1] - \Pr[\Hyb_2 = 1]| = \negl(\secp)$. Thus, assume for contradiction that $\mathbf{H}_\infty(R \mid \mathbf{y}) = O(\log(\secp))$. This implies the following.

%\begin{itemize}
    %\item Let $\mathsf{pass}$ be the event that $S$ does not abort in at step (b) during the preparation of the third message. Then $\Pr[{\mathsf{pass}}] = 1/\poly(\secp)$, since conditioned on an abort, $R$ is sampled uniformly and indendently of $\by$.
    %\item By \cref{lemma:guessing-probability}, this implies that there exists a quantum operation $E$ such that \[\Pr[\mathsf{guess}] \coloneqq \sum_{R \in \{0,1\}^\secp}p_R\Pr[E(\by_R) = R] = 1/\poly(\secp).\] Moreover, it must hold that $\Pr[\mathsf{guess} | \mathsf{pass}] = 1/\poly(\secp)$, again since $R$ is independent of $\by$ when $\mathsf{pass}$ does not occur.
    %\item Together, we have that $\Pr[\mathsf{guess} \wedge \mathsf{pass}] = 1/\poly(\secp)$.
%\end{itemize}

%Next, we define the event $\mathsf{extract}$ that for at least $3\secp/8$ of the $\{\widehat{b}_i,\widehat{r_i}\}_{i \in \overline{T}}$, it holds that $r_{i,\widehat{b}} = \widehat{r}_i$.


This completes the proof of our theorem.
\end{proof}

\subsection{Receiver Security}

\begin{theorem}
\proref{fig:qot-3r-construction} is private against specious adversaries corrupting the sender (\cref{def:specious-privacy}).
\end{theorem}

\begin{proof}

Consider a specious sender, specified by two quantum oracle machines $\widetilde{A}_1,\widetilde{A}_2$, and two recovery operations $F_1,F_2$, where each machine has oracle access to $\comro,\fsro,\maskro$. 

For any joint inputs $(m_0,m_1,b)$, let $\brho_{m_0,m_1,b}$ be the sender's private state output by $\widetilde{A}_2$ when the protocol is run on inputs $(m_0,m_1,b)$. We need to show that for any $q$, there exists a simulator $\cS$, such that for any $\cD$ that queries $\comro,\fsro,\maskro$ at most $q$ times, and any $m_0,m_1,b$,

\[\big|\Pr[\cD^{\comro,\fsro,\maskro}(\brho_{m_0,m_1,b}) = 1] - \Pr[\cD^{\cS}(\cS(m_0,m_1)) = 1]\big| = \negl(\secp).\]

We define $\cS$ as follows.
\begin{itemize}
    \item Let $\cS_\Equ = \cS_\Equ[q]$ be the equivocality simulator for the commitment scheme.
    \item Run $\widetilde{A}_1^{\cS_\Equ,\fsro,\maskro}$ to obtain a first-round message $\{\ket{\psi_i}\}_{i \in [\secp]}$ and private state $\btau$.
    \item Run $\{\com_i\}_{i \in [\secp]} \gets \cS_\Equ$, compute $T = \fsro(\com_1,\dots,\com_\secp)$, measure each $\{\ket{\psi_i}\}_{i \in T}$ in the computational basis to obtain $\{\widehat{b}_i,\widehat{r}_i\}_{i \in T}$, compute $\{s_i\}_{i \in T} \gets \cS_\Equ(\{\widehat{b}_i,\widehat{r}_i\}_{i \in T})$, and sample $c_i \gets \{0,1\}$ for $i \in \overline{T}$.
    \item Run $\widetilde{A}_2^{\cS_\Equ,\fsro,\maskro}$ on $\btau$ and $(\{\com_i\}_{i \in [\secp]},T,\{ (\widehat{b}_i, \widehat{r}_i),s_i \}_{i \in T}, \{c_i\}_{i \in \overline{T}})$ to obtain ouptut $\btau'$, which is given to $\cD$. Answer $\cD's$ oracle queries to $\comro$ using $\cS_\Equ$ and to $\fsro,\maskro$ honestly.
\end{itemize}

Consider the following hybrids.

\begin{itemize}
    \item $\Hyb_0:$ This is the real experiment $\cD^{\comro,\fsro,\maskro}(\brho_{m_0,m_1,b})$.
    \item $\Hyb_1:$ In this hybrid, we run $\cS$ above, except that all $\{\widehat{b}_i,\widehat{r}_i\}_{i \in [\secp]}$ are still obtained by measuring $\{\ket{\psi_i}\}_{i \in [\secp]}$, and the $c_i$ are still computed honestly based on $b$.
    \item $\Hyb_2:$ This is the simulated experiment $\cD^{\cS}(\cS(m_0,m_1))$.
\end{itemize}

\begin{claim}
$|\Pr[\Hyb_0 = 1] - \Pr[\Hyb_1 = 1]| = \negl(\secp)$.
\end{claim}

\begin{proof}
This follows directly from equivocality of the commitment scheme (\cref{def:equivocal}).
\end{proof}

\begin{claim}
$|\Pr[\Hyb_1 = 1] - \Pr[\Hyb_2 = 1]| = \negl(\secp)$.
\end{claim}

\begin{proof}
Consider the joint state $(\btau,\bsigma)$ output by $\widetilde{A}_1$, where $\btau$ is the state on $\widetilde{A}'s$ private memory register, and $\bsigma$ is the state sent to $R$ (and where $\btau,\bsigma$ may be entangled). Let $M_1$ be the quantum operation that $\Hyb_1$ applies to $\bsigma$ in order to produce $(\{\com_i\}_{i \in [\secp]},T,\{\widehat{b}_i\}_{i \in \overline{T}})$. Let $M_2$ be the same operation, except that $\{\widehat{b}_i\}_{i \in \overline{T}}$ is replaced with a uniformly sampled string $u \gets \{0,1\}^{\secp/2}$. Observe that it suffices to show that 
\begin{equation}
    \TD((\btau,M_1(\bsigma)),(\btau,M_2(\bsigma))) = \negl(\secp), \label{eq:TD1}
\end{equation}

since these joint distributions capture the difference between $\Hyb_1$ and $\Hyb_2$.

To see this, note that by the fact that $\widetilde{A}$ is specious (and in particular, due to the existence of the recovery operation $F_1$), there exists $\btau'$ such that

\begin{equation}
    \TD((\btau,\bsigma),(\btau',\bsigma')) = \negl(\secp), \label{eq:TD2}
\end{equation} where $\bsigma'$ is a distribution over $\secp$ states of the form $\frac{\ket{0,r_{i,0}} + \ket{1,r_{i,1}}}{\sqrt{2}}$ (that is, the honest sender's distribution). Due to the structure of $\bsigma'$, each bit $\{\widehat{b}_i\}_{i \in \overline{T}}$ is the result of measuring an unentangled register in uniform superposition over $\ket{0}$ and $\ket{1}$. Thus, we have that 

\begin{equation}
    \TD((\btau',M_1(\bsigma')),(\btau',M_2(\bsigma'))) = 0. \label{eq:TD3}
\end{equation}

Finally, \cref{eq:TD1} follows directly from \cref{eq:TD2} and \cref{eq:TD3}.
\end{proof}
\end{proof}


==> qot-4r-2q-construction.tex <==
\section{A 4-round fully secure protocol for Quantum Oblivious Transfer}

\subsection{Construction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Variables used in the below construction
\newcommand{\numst}{\secp^3}
\newcommand{\numstf}{\secp^2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\protocol
{\proref{fig:qot-4r-construction}}
{4 round fully secure QOT protocol}
{fig:qot-4r-construction}
{

\begin{tabular}{ l l }
\textbf{Sender $S$ Input:} $M_0,M_1 \in \zo$ & \textbf{Sender $S$ Output:} $\perp$ \\
\textbf{Receiver $R$ Input:} Bit $B \in \{0,1\}$ & \textbf{Receiver $R$ Output:} $B,M_B$ \\
\textbf{Public Random Oracles:} $\comro, \fsro$ & \\
\end{tabular}


\begin{enumerate}

\item $R$ performs the following operation - $\forall i \in [4\numst]$, sample $r_0^i, r_1^i \leftarrow \zo$. Create the quantum state $\ket{\psi^i} = \frac{\ket{0 r_0^i} + \ket{1 r_1^i}}{\sqrt{2}}$ and send over all the quantum states $\{\ket{\psi^i}\}_{i \in [4\numst]}$ to $S$.

\item $S$ chooses set $T \leftarrow [4\numst]$ s.t. $|T|=2\numst$. It then performs the following operations: 

\begin{enumerate}

    \item It measures states in positions indexed by $\overline{T}$ in the computational basis $(\{ \ket{00}, \ket{01}, \ket{10}, \ket{11} \})$ to get $\{\widehat{b}_i, \widehat{r}_i\}_{i \in \overline{T}}$. It renames them to $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [2\numst]}$.
    
    \item It prepares a measurement check proof $\pi$ of the above measurement as follows:
        \begin{enumerate}
            \item Commitment: $\forall i \in [2\numst]$, $com_i = \comro(\widetilde{b}_i || \widetilde{r}_i || \widetilde{s}_i)$ where $\widetilde{s}_i \leftarrow \{0, 1\}^\secp$. 
            
            \item Challenge: $Y = \fsro(com_1 || \ldots || com_{2\numst})$ and set $T' = RandSubset_{[2\numst],\numst}(Y)$.
        
            \item Openings: Set $\pi = (\{com_i\}_{i \in [2\numst]}, Y, \{ \widetilde{b}_i || \widetilde{r}_i || \widetilde{s}_i \}_{i \in T'})$.
        \end{enumerate}
    
    \item Take $\{\widetilde{b}_i,\widetilde{r}_i\}_{i \in [2\numst] \setminus T'}$ and divide them into $\numstf$ buckets of $\secp$ each and rename them to $\{b'_{ij},r'_{ij}\}_{i \in [\numstf], j \in [\secp]}$. $\forall i \in [\numstf]$, sample $c_i \leftarrow \{0,1\}$. Finally, compute $\forall i \in [\numstf], j \in [\secp]$ $d_{ij} = c_i \oplus b'_{ij}$ and send to $R$ the following - $T,\pi,\{d_{ij}\}_{i \in [\numstf],j \in [\secp]}$.
    
    \item Set $\forall i \in [\numstf], \widetilde{R}_i = \bigoplus_{j \in [\secp]} r'_{ij}$.
    \item Set $\forall i \in [\numstf], \forall b \in \zo, \widetilde{y}^i_b = \widetilde{R}_i \oplus bc_i $.
\end{enumerate}

\item $R$ parses the received message as $T,\pi,\{d_{ij}\}_{i \in [\numstf],j \in [\secp]}$, and performs the following actions: 
    \begin{enumerate}
        \item It checks $\pi$ as follows and aborts if any of the checks fail.
            \begin{enumerate}
                \item Check if $Y = \fsro(com_1 || \ldots || com_{2\numst})$. If so, set $T' = RandSubset_{[2\numst],\numst}(Y)$.
                \item Check if $\forall i \in T', com_i = \comro(\widetilde{b}_i || \widetilde{r}_i || \widetilde{s}_i)$. Also, $\forall i \in T'$, $\widetilde{r}_i = r_{\widetilde{b}_i}^i$.
            \end{enumerate}
        \item Take $\{(r^i_0,r^i_1)\}_{i \in [4\numst] \setminus T}$, in the remaining positions discard the ones indexed by $T'$, divide the remaining into $\numstf$ buckets of $\secp$ each and rename the same to get $\{r^{ij}_0,r^{ij}_1\}_{i \in [\numstf],j \in [\secp]}$.
        \item Compute $\forall i \in [\numstf], \forall j \in [\secp], \forall b \in \zo$, $R^{ij}_b = r^{ij}_{b \oplus d_{ij}}$.
        \item Compute $\forall i \in [\numstf], \forall b \in \zo, x^i_b = \bigoplus_{j \in [\secp]} R^{ij}_b$.
        \item Compute $\forall i \in [\numstf], w_i = x^i_0 \oplus x^i_1, z_i = x^i_0$.
        \item Send to $S$ the following - $\{r^i_0,r^i_1\}_{i \in T}, \{B \oplus w_i\}_{i \in [\numstf]}$.
    \end{enumerate}
        
\item $S$ parses the received message as $\{r^i_0,r^i_1\}_{i \in T}, \{\omega_i\}_{i \in [\numstf]}$. It then does the following:
    \begin{enumerate}
        \item $\forall i \in T$, prepare quantum state $\ket{\phi^i} = \frac{\ket{0 r_0^i} + \ket{1 r_1^i}}{\sqrt{2}}$ and measure the quantum state (received in the first message) in basis $\{\dyad{\phi^i}{\phi^i}, \bbI - \dyad{\phi^i}{\phi^i}\}$. Abort if any measurement yields outcome $0$ (i.e. the quantum state projects onto $\bbI - \dyad{\phi^i}{\phi^i}\}$.
        
        \item Compute $\forall i \in [\numstf], \forall b \in \zo, \widetilde{p}^i_b = \widetilde{y}^i_{b \oplus \omega_i} $.
        
        \item Compute $\forall b \in \zo$, $Y_b = \bigoplus_{i \in [\numstf]} \widetilde{p}^i_b$ and send to $R$, the following - $(M_0 \oplus Y_0, M_1 \oplus Y_1)$.
    \end{enumerate}
    
\item $R$ on receiving $(q_0,q_1)$ from $S$, computes $Z = \bigoplus_{i \in [\numstf]} z_i$ and output $q_B \oplus Z$.

\end{enumerate}
}



==> qot-5r-construction.tex <==
\section{Quantum Oblivious Transfer}


\subsection{Construction}
We describe the construction of our QOT protocol in \proref{fig:qot-5r-construction}.

u
\protocol
{\proref{fig:qot-5r-construction}}
{A 5-round QOT protocol. Here $RandSubset_{[2n],n}(x)$ is a deterministic function for mapping strings of sufficient length to subsets of $[2n]$ of size $n$, with the gurantee that if the input is uniformly random string, then the output is a random subset of $[2n]$ of size $n$. This can be instantiated in a canonical way - for example by interpretting the input string as indices into the array and doing sampling with replacement. \nishant{Move this last line description someplace else like prelims?} } 
{fig:qot-5r-construction}
{

\begin{tabular}{ l l }
\textbf{Sender $S$ Input:} $m_0,m_1 \in \zo^\secp$ & \textbf{Sender $S$ Output:} $\perp$ \\
\textbf{Receiver $R$ Input:} Bit $b \in \{0,1\}$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
\textbf{Public Random Oracles:} $\comro, \fsro, \maskro$ & \\
\end{tabular}



\begin{enumerate}
\item $S$ chooses $x \leftarrow \{0, 1\}^{16\secp}$ and $\theta \leftarrow \{+, \times \}^{16\secp}$ 
and sends $\{\ket{x_i}_{\theta_i}\}_{i\in[16\secp]}$ to $R$. 

\item \label{itm:qot-recv-measurement}
$R$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{16\secp}$
and obtains $\widehat{x} \in \{0, 1\}^{16\secp}$ by measuring $\{\ket{x_i}_{\theta_i}\}_{i\in[16\secp]}$
in basis $\widehat{\theta}$. 
$R$ then computes a measurement check proof $\pi$ as follows:

\begin{enumerate}
    \item \label{itm:qot-recv-meas-com}
    Commitment: $\forall i \in [16\secp]$, $com_i = \comro(\widehat{x}_i || \widehat{\theta}_i || \widehat{r}_i)$ where $\widehat{r}_i \leftarrow \{0, 1\}^\secp$.
    
    \item Challenge: $Y = \fsro(com_1 || \ldots || com_{16\secp})$, $T = RandSubset_{[16\secp],8\secp}(Y)$.

    \item Set $\pi = (\{com_i\}_{i \in [16\secp]}, Y, \{\widehat{x}_i, \widehat{\theta}_i, \widehat{r}_i \}_{i \in T})$, and send $\pi$ to $S$.
\end{enumerate}

\item \label{itm:qot-sendr-check}
$S$ checks proof $\pi$ using the following steps:

\begin{enumerate}
    \item Check if $Y = \fsro(com_1 || \ldots || com_{16\secp})$. If so, set $T = RandSubset_{[16\secp],8\secp}(Y)$.
    
    \item Check if $\forall i \in T, com_i = \comro(\widehat{x}_i || \widehat{\theta}_i || \widehat{r}_i)$.
    
    \item Check if $\forall i \in T$ that satisfy $\widehat{\theta}_i = \theta_i$, whether $\widehat{x}_i = x_i$.
\end{enumerate}

If all the above checks pass, send $\{ \theta_i \}_{i \in \overline{T}}$ to $R$, where $\overline{T} = [16\secp] \setminus T$, otherwise abort.

\item  \label{itm:qot-recv-bit-encoding}
$R$ encodes bit $b$ into 2 sets - $I_0,I_1$ in the following way and sends $(I_0,I_1)$ to $S$.
\begin{enumerate}
    \item Divide $\overline{T}$ into 2 disjoint subsets $S_0, S_1$ in the following way - $S_0 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} = \theta_i \}, 
    S_1 = \{ i | i \in \overline{T} \wedge \widehat{\theta_i} \ne \theta_i \}$.
    
    \item Set $I_b = S_0$ and $I_{1-b} = S_1$.
    
\end{enumerate}


\item \label{itm:qot-sendr-lastmsg}
If $|I_0|<\secp$ or $|I_1|<\secp$, $S$ aborts. Otherwise, it chooses $s \samp \zo^\secp$, computes $ct_0 = m_0 \oplus \maskro(s||\{x_i\}_{i \in I_0}), ct_1 = m_1 \oplus \maskro(s||\{x_i\}_{i \in I_1})$ and sends $s, ct_0, ct_1$ to $R$. 

\item $R$ outputs $m_b = ct_b \oplus \maskro(s||\{\widehat{x}_i\}_{i \in I_b})$.
\end{enumerate}
}



==> qot-5r-non-FS-construction.tex <==
\section{The CK88 Framework}

\james{maybe we keep this here for comparison / parameters?}


\subsection{Construction}
We describe the construction of our QOT protocol in \proref{fig:qot-5r-non-FS-construction}.

\protocol
{\proref{fig:qot-5r-non-FS-construction}}
{QOT protocol of Type-1 in the $\idealcom$ hybrid. \nishant{we can't write 5-round here now since its in the $\idealcom$ hybrid} $h : \zo^{k(\secp)} \times \cX \rightarrow \zo^\secp$ is a universal hash function family with seed length $k(\secp)$, and domain $\cX = \zo^{\leq 7\secp}$.}
{fig:qot-5r-non-FS-construction}
{

\begin{tabular}{ l l }
\textbf{Sender $S$ Input:} $m_0,m_1 \in \zo^\secp$ & \textbf{Receiver $R$ Input:} Bit $b \in \{0,1\}$ \\
\textbf{Sender $S$ Output:} $\perp$ & \textbf{Receiver $R$ Output:} $b,m_b$ \\
\end{tabular}


\begin{enumerate}
\item $S$ chooses $x \leftarrow \{0, 1\}^{16\secp}$ and $\theta \leftarrow \{+, \times \}^{16\secp}$ 
and sends $\ket{x}_{\theta}$ to $R$. \nishant{this notation should be there in prelims}

\item 
    \begin{enumerate}
        \item \label{itm:qot-recv-measurement} $R$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{16\secp}$ and obtains $\widehat{x} \in \{0, 1\}^{16\secp}$ by measuring $\ket{x}_{\theta}$ in basis $\widehat{\theta}$.
        
        \item $R,S$ execute the commit phase of $\idealcom$ with $R$ as the committer and $S$ as the receiver. $R$ sends $(Commit,R,S,(\widehat{x}_1,\widehat{\theta}_1,\ldots \widehat{x}_{16\secp},\widehat{\theta}_{16\secp}))$ to $\idealcom$.
    \end{enumerate}

\item $S$ chooses a random set $T \leftarrow [16\secp]$ s.t. $|T|=8\secp$ and sends $T,\{\theta_i\}_{i \in \overline{T}}$ to $R$.

\amit{In hindsight, we should have used different symbols for denoting what an honest sender is expected to send and what actually gets sent over the channel. For example, instead of saying that $S$ sends $\{ \theta_i \}_{i \in \overline{T}}$ to $R$, we should have written: $S$ sets $\{ \widetilde{\theta_i} \}_{i \in \overline{T}} := \{ \theta_i \}_{i \in \overline{T}}$ and then sends $\{ \widetilde{\theta_i} \}_{i \in \overline{T}}$ to $R$. The next step of $R$ would be defined as ``On receiving $\{ \widetilde{\theta_i} \}_{i \in \overline{T}}$ from $S$ \ldots''. This would have simplified the exposition of security proof because, for example, it enables us to write ``$\simu^{S^*}$ on receiving $\{ \widetilde{\theta_i} \}_{i \in \overline{T}}$ from $S^*$ \ldots'' without explicitly worrying about whether $\widetilde{\theta_i}$ matches $\theta_i$ or not. This idea is similar to how we are using $\widetilde{m_b}$ instead of $m_b$ to describe the output of honest $R$ in the current protocol.}

\item 
    \begin{enumerate}
        \item $R,S$ execute the reveal phase of $\idealcom$:
            \begin{enumerate}
                \item $R$ sets $T' = \bigcup_{i \in T} \{\text{indices of } \widehat{x}_i,\widehat{\theta}_i \text{ in the set } \{\widehat{x}_1,\widehat{\theta}_1,\ldots \widehat{x}_{16\secp},\widehat{\theta}_{16\secp}\}\} = \bigcup_{i \in T} \{2i-1,2i\}$. It also sets $b_i=1,\forall i \in T'$.
            
                \item $R$ sends $(Open,R,S,T',\{b_i\}_{i \in T'})$ to $\idealcom$. 
            
                \item \label{itm:qot-5r-non-fs-sender-checks}
                $S$ receives $(Open,R,S,T',\{\widehat{x_i},\widehat{\theta_i}\}_{i \in T})$ from $\idealcom$. It checks if $T' = \bigcup_{i \in T} \{2i-1,2i\}$, if $\forall i\in T, \widehat{x}_i,\widehat{\theta}_i$ are $\neq \bot$, and if $\forall i \in T$ s.t. $\theta_i = \widehat{\theta}_i$, whether $x_i = \widehat{x}_i$. If any check fails, it aborts.
            \end{enumerate}
            
        \item $R$ divides $\overline{T}$ into 2 disjoint subsets $S_0, S_1$ in the following way - $S_0 = \{ i | i \in \overline{T} \wedge \widehat{\theta}_i = \theta_i \}, S_1 = \{ i | i \in \overline{T} \wedge \widehat{\theta}_i \ne \theta_i \}$. It sets $I_b = S_0$ and $I_{1-b} = S_1$ and sends $(I_0,I_1)$ to $S$.
    \end{enumerate}

\item $S$ checks if $|I_0|<\secp$ or $|I_1|<\secp$, and aborts if so. Otherwise, it chooses $s \samp \zo^{k(\secp)}$, and sends to $R$ the following - \[s,m_0 \oplus h(s||\{x_i\}_{i \in I_0}), m_1 \oplus h(s||\{x_i\}_{i \in I_1})\]

\item $R$ on receiving $s,y_0,y_1$ computes $\widetilde{m}_b = y_b \oplus h(s||\{\widehat{x}_i\}_{i \in I_b})$. It outputs $(b,\widetilde{m}_b)$.

\end{enumerate}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Receiver Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Receiver Security}

We first describe the construction of our simulator for a malicious sender $S^*$. In our description, $\simu$ takes control of $\idealcom$ and answers its queries to $S^*$

$\simu$:

\begin{enumerate}
    \item Receive $\{ \ket{x_i}_{\theta_i} \}_{i \in [16\secp]}$ from $S^*$
    
    \item Sends $(Commit, R, S^*, 0^{32 \secp})$ to $\idealcom$ on behalf of the receiver and send $(Receipt, R, S^*)$ to $S^*$ on behalf of $\idealcom$
    
    \item Receive $T, \{ \theta_i \}_{i \in \overline{T}}$ from $S^*$.
    
    \item Performs delayed measurement of  $\{ \ket{x_i}_{\theta_i} \}_{i \in [16\secp]}$ in the following fashion:
    
    \begin{itemize}
        \item For all $i \in T$: sample $\widehat{\theta_i} \leftarrow \{ +, \times \}$, measure $\ket{x_i}_{\theta_i}$ in the basis $\widehat{\theta_i}$ to obtain outcome $\widehat{x_i}$. These outcomes and basis will be used to generate $\idealcom$ openings.
        
        \item For all $i \in \overline{T}$: measure $\ket{x_i}_{\theta_i}$ in the basis $\theta_i$ received from $S^*$ in Step 3, and let the outcome be $\widehat{x_i}$
    \end{itemize}
    
    Post this, complete Step 4 a) i and Step 4 a) ii honestly. In Step 4 a) iii, send $(Open, R, S^*, T', \{ \widehat{x_i}, \widehat{\theta_i} \}_{i \in T})$ to $S^*$, where  $\{ \widehat{x_i}, \widehat{\theta_i} \}_{i \in T}$ are the delayed measurements described above.  
    
    In Step 4 b), set $I_0 := S_0$ and $I_1 := S_1$. Send $(I_0, I_1)$ to $S^*$.
    
    
    \item Perform the following steps on receiving $s, y_0, y_1$ from $S^*$:
    
    \begin{itemize}
        \item Compute $\widetilde{m_0} = y_0 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_0})$
        \item Compute $\widetilde{m_1} = y_1 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_1})$
        \item Send $\widetilde{m_0}, \widetilde{m_1}$ to the OT ideal functionality
    \end{itemize}
    
    
\end{enumerate}


Having defined the $\simu$, we will now show that the real world is indistinguishable from the ideal world via a sequence of hybrids.

\begin{itemize}
    \item $\Hyb_0$: This corresponds to the Real World. The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
    \item $\Hyb_1$ \textbf{[$\simu$ controls $\idealcom$]}: In this hybrid, $\simu$ runs the honest $R$ protocol with $S^*$ and also starts controlling $\idealcom$ functionality. However, it sends $\idealcom$ replies to $S^*$ in exactly the same way as in previous hybrid.
    \amit{Replace with equivocal}
    
    \item $\Hyb_2$ \textbf{[Delayed Measurement]}: Same as the previous hybrid except for the following change: Instead of measuring $\{ \ket{x_i}_{\theta_i} \}_{i \in [16 \secp]}$ in Step 2a, $\simu$ delays the measurement until Step 4. Also, in Step 2b, it sends $(Commit, R, S^*, 0^{32 \secp})$ to $\idealcom$ and sends $(Receipt, R, S^*)$ to $S^*$ on behalf of $\idealcom$.
    
    On receiving $T, \{ \theta_i \}_{i \in \overline{T}}$ in Step 3, it performs the delayed measurement before executing Step 4a in the following fashion:
    
    \begin{itemize}
        \item For all $i \in T$: sample $\widehat{\theta_i} \leftarrow \{ +, \times \}$, measure $\ket{x_i}_{\theta_i}$ in the basis $\widehat{\theta_i}$ to obtain outcome $\widehat{x_i}$. These outcomes and basis will be used to generate $\idealcom$ openings.
        
        \item For all $i \in \overline{T}$: measure $\ket{x_i}_{\theta_i}$ in the basis $\theta_i$ received from $S^*$ in Step 3, and let the outcome be $\widehat{x_i}$
    \end{itemize}
    
    Post this, $\simu$ completes Step 4 a) i and Step 4 a) ii honestly. In Step 4 a) iii, it sends $(Open, R, S^*, T', \{ \widehat{x_i}, \widehat{\theta_i} \}_{i \in T})$ to $S^*$, where  $\{ \widehat{x_i}, \widehat{\theta_i} \}_{i \in T}$ are the delayed measurements described above. The remaining steps are completed as per the honest $R$ strategy.
    
    \item $\Hyb_3$ \textbf{[OT sender message extraction]}: Same as the previous hybrid except the following change: Instead of performing step 6 of the protocol, perform the following steps on receiving $s, y_0, y_1$ from $S^*$:
    
    \begin{itemize}
        \item Compute $\widetilde{m_0} = y_0 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_0})$
        \item Compute $\widetilde{m_1} = y_1 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_1})$
        \item Send $\widetilde{m_0}, \widetilde{m_1}$ to the OT ideal functionality
    \end{itemize}
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.

    
    \item $\Hyb_4$ \textbf{[Removing the receiver choice bit]}: $\simu$ behaves exactly as the previous hybrid except that in Step 4 b), instead of using $b$ to define the sets $I_0$ and $I_1$, it instead sets $I_0 := S_0$ and $I_1 := S_1$. It then completes the remaining steps as mentioned in the previous hybrid.
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.
\end{itemize}

Having defined the hybrids, we will now show the indistinguishability between each pair of hybrids.

\begin{itemize}
    \item $\Hyb_0 \approx_c \Hyb_1$: Follows from the computational security of $\idealcom$ functionality against a malicious commitment receiver. \amit{Should composition theorem be invoked here ?}
    
    \amit{Replace this with equivocality}
    
    \item $\Hyb_1 = \Hyb_2$: Follows from the following two observations: i) For all $i \in T$, the distribution of $\widehat{\theta_i}, \widehat{x_i}$ is identical in both hybrids, ii) For all $i \in \overline{T}$, the measurement outcomes $\widehat{x_i}$ are not present anywhere in the protocol transcript. Their only usage is in computing the receiver's output $\widetilde{m_b}$ locally in Step 6. Here we note that the distribution of $\{ \widehat{x_i} \}_{i \in I_b}$ is identical in both hybrids, hence the distribution of $\widetilde{m_b}$ is also identical.
    
    \item $\Hyb_2 = \Hyb_3:$ Note that there is no difference in these hybrids with respect to the simulation of $S^*$ view. The only difference is in how we define the output of the honest receiver. In $\Hyb_2$, the receiver's output is computed by the simulator as $\widetilde{m_b} := y_b \oplus h(s || \{ \widehat{x_i} \}_{i \in I_b})$. In $\Hyb_3$, the receiver's output is derived via the OT ideal functionality which receives sender's input strings $(\widetilde{m_0} := y_0 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_0}), \widetilde{m_1} := y_1 \oplus h(s || \{ \widehat{x_i} \}_{i \in I_1}))$ from the $\simu$ and ideal-world receiver choice bit $b$. The OT ideal functionality sends $\widetilde{m_b} := y_b \oplus h(s || \{ \widehat{x_i} \}_{i \in I_b})$ to the ideal world receiver which it then outputs. Hence, the output distribution of the receiver is identical in both the hybrids.
    
    % Correctness of the extraction procedure follows from the EPR measurement correlation property on set $\overline{T}$.
    % \amit{Handle the case where $x_i$}
    
    % \amit{The definition of $I_b$ is not changing between two hybrids and so $m_b$ would not change}
    
    
    \item $\Hyb_3 =\Hyb_4:$ We first observe that the distribution of $S_0 = S_1$ as long as $\{ \widehat{\theta_i} \}_{i \in \overline{T}}$ is private (which is in fact the case from the point of view of malicious sender and the distinguisher). This is because $\{ \widehat{\theta_i} \}_{i \in \overline{T}}$ is sampled uniformly at random, and hence $\{ S_0, S_1 \}$ form a uniformly random partition of the set $\overline{T}$. Hence, the distribution of $(S_0, S_1)$ is identical to $(S_1, S_0)$.

    Note that the protocol transcript contains $(I_0, I_1)$ which would be equal to $(S_b, S_{1-b})$ for an honest receiver strategy (and hence also for $\simu$ strategy until $\Hyb_3$). However, for the $\simu$ strategy in $\Hyb_4$, $(I_0, I_1)$ is always equal to $(S_0, S_1)$. Hence, if $b = 0$, the distribution of $(I_0, I_1)$ in $\Hyb_3$ would be identical to $\Hyb_4$. On the other hand, if $b = 1$, the distribution of $(I_0, I_1)$ in $\Hyb_3$ would be perfectly indistinguishable from $\Hyb_4$ (following from the fact that the distribution of $(S_0, S_1) = (S_1, S_0)$). Putting together these two observations, it easily follows that $\Hyb_3 = \Hyb_4$.
    
    
\end{itemize}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Sender Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sender security}

We prove the security our QOT protocol in \figureref{fig:qot-5r-non-FS-construction} here. We describe the simulator $\simurecv$ against a malicious receiver $\malrecv$ in the following : 

\begin{enumerate}
    \item $\simurecv(\rho)$ invokes $\malrecv(\rho)$. It samples $x \leftarrow \zo^{16\secp}, \theta \leftarrow \zo^{16\secp}$, prepares the state $\ket{x}_{\theta}$ and sends the same to $\malrecv$.
    
    \item It executes the commit phase with $\malrecv$, simulating $\idealcom$ for it, and intercepting the corresponding messages meant for $\idealcom$ by $\malrecv$. It receives message $(Commit,\malrecv,S,(\widehat{x}_1,\widehat{\theta}_1, \ldots \widehat{x}_{16\secp},\widehat{\theta}_{16\secp}))$ from $\malrecv$.
    
    \item It samples set $T \leftarrow [16\secp]$ s.t. $|T|=8\secp$ and sends $T,\{\theta_i\}_{i \in \overline{T}}$ to $\malrecv$. 
    
    \item It executes the reveal phase of $\idealcom$ with $\malrecv$, and receives message $(Open,R,S,T',\{b_i\}_{i \in T'})$ from $\malrecv$. It checks if $T' = \bigcup_{i \in T} \{2i-1,2i\}$, if $\forall i \in T', b_i=1$, and if $\forall i \in T$ s.t. $\theta_i = \widehat{\theta}_i$, whether $x_i = \widehat{x}_i$. If any check fails, it outputs $\bot$.
    
    \item It receives sets $(I_0,I_1)$ from $\malrecv$ and checks if $|I_0|,|I_1| \geq \secp$ and aborts if not. 
    
    \item It finds set $Q = \{i : i \in I_0 \wedge \theta_i \neq \widehat{\theta}_i\}$. If $|Q|>3\secp/2$, it sets $b=1$, else it sets $b=0$. 
    
    \item It sends $b$ to $\idealot$ and receives $m_b$ in return. It sets $m_{1-b}=0^\secp$, samples $s \leftarrow \zo^{k(\secp)}$ and sends to $\malrecv$: \[s,m_0 \oplus h(s||\{x_i\}_{i \in I_0}), m_1 \oplus h(s||\{x_i\}_{i \in I_1})\] It outputs whatever $\malrecv$ outputs.
\end{enumerate}

==> qot-5r-recv-security-alternative.tex <==
\subsection{Analysis: Receiver Security}
%Simulate malicious sender

\begin{itemize}
    \item $\Hyb_0:$ Real World
    
    \item $\Hyb_1:$ $\simu$ takes the role of honest $R$ and also transparently forwards all calls between $S^*$ and $\{\comro, \fsro, \maskro\}$
   
    \item $\Hyb_2$: $\simu$ behaves exactly as the previous hybrid in addition to privately sampling the following sets of size ${16\secp}$:
    
    $$ \mathbb{R}^{zero} = \{ r^{zero}_i | r^{zero}_i \uniformsample \zo^\secp \}$$
    $$ \mathbb{R}^{one} = \{ r^{one}_i | r^{zero}_i \uniformsample \zo^\secp \}$$
    
    \item $\Hyb_3$: $\simu$ behaves exactly as the previous hybrid except that it forms a wrapper $\comro'$ - parametrized using the sets $\mathbb{R}^{zero}, \mathbb{R}^{one}, \widehat{\theta}$ - around $\comro$ in the following way:
    
    $\comro'_{\mathbb{R}^{zero}, \mathbb{R}^{one}, \widehat{\theta}}(q)$:
    
    \begin{itemize}
    
        \item Parse query $q$ as $x || \theta || r$
        
        \item If $x = 1$ and $\exists i$ such that $\theta = \widehat{\theta}_i$ and $r = r^{one}_i$, then set $q_{new} = \bar{x} || \theta || r^{zero}_i$, else set $q_{new} = q$
        
        \item Return $\comro(q_{new})$
        
    \end{itemize}
    
    The above wrapper can be efficiently implemented by $\simu$ using just oracle access to $\comro$ and a quantum circuit that implements the above wrapper logic given the sets $\mathbb{R}^{zero}, \mathbb{R}^{one}, \widehat{\theta}$
    
    
    \item $\Hyb_4$: \amit{Delayed measurement and equivocation} $\simu$ behaves exactly as the previous hybrid except for the following changes:
    
    \begin{itemize}
        \item Instead of obtaining the measurement values $\widehat{x}$ honestly in Step \ref{itm:qot-recv-measurement}, it instead skips the measurement completely, and randomly samples $\widehat{x} \uniformsample \zo^{16\secp}$.
        
        \item  Additionally, it computes the measurement commitment using the following rule: $\forall i \in [16\secp], c_i = \comro'(\widehat{x}_i || \widehat{\theta}_i || r^{\widehat{x}_i}_i)$ where $r^{\widehat{x}_i}_i \in \mathbb{R}^{\widehat{x}_i}$. In the opening phase, $R$ actually performs the measurement of BB84 states only at indices represented by $T$ to obtain $\{ \widehat{x_i}^{measured} \}_{i \in T }$ and computes the respective openings as $\{ \widehat{x_i}^{measured}, \widehat{\theta_i}, r_i^{\widehat{x_i}^{measured}} \}_{i \in T}$
        
        \item In the beginning of Step \ref{itm:qot-recv-bit-encoding}, it measures all the remaining BB84 states (i.e. states at indices in $\overline{T}$) after it has received the correct basis $\{ \theta_i \}_{i \in \overline{T}}$ from $S^*$. For all $i \in \overline{T}$, it measures $\ket{x_i}_{\theta}$ in the basis $\theta_i$ to obtain $\{ \widehat{x_i}^{measured} \}_{i \in \overline{T}}$ 
        
        \item Then it forms subsets $S_0$ and $S_1$ by randomly splitting the indices in $\overline{T}$
        \amit{Check this subset formation rule. Make sure in passes Sender check in Step \ref{itm:qot-sendr-lastmsg}}
        \amit{Need to sample a random choice bit $b$ ?}
        
        \item Finally, in the last step, after receiving $ct_0, ct_1$ from $S^*$, it computes $m_0 = ct_0 \oplus \maskro(s || \{ \widehat{x_i}^{measured} \}_{i \in I_0})$ and $m_1 = ct_1 \oplus \maskro(s || \{ \widehat{x_i}^{measured} \}_{i \in I_1})$. It then sends $m_0, m_1$ to the OT Ideal functionality.
    \end{itemize}
    
\end{itemize}


We will now argue the computational indistinguishability of each pair of consecutive hybrids in the above sequence.

\begin{itemize}
    \item $\Hyb_0 = \Hyb_1$: The distribution of $\Hyb_0$ is identical to the distribution of $\Hyb_1$ by construction. Hence these two hybrids are perfectly indistinguishable.
    
    \item $\Hyb_1 = \Hyb_2$: Since the sets $\mathbb{R}^{zero}, \mathbb{R}^{one}$ are sampled privately and not used anywhere in the protocol, therefore the adversary's view is completely independent of them. Hence, these two distributions are also perfectly indistinguishable.
    
    \item $\Hyb_2 \approx_c \Hyb_3$: First we make the following observation: The wrapper $\comro'$ can be viewed as programmed version of $\comro$ where, for all $i \in [16\secp]$, the image of $1 || \widehat{\theta}_i || r^{one}_i$ is remapped to the image of $0 || \widehat{\theta}_i || r^{zero}_i$. 
    
    This wrappered oracle $\comro'$ is idecntically distributed to another oracle $\comro''$, which additionally takes in a parameter $\widehat{x}$ representing the (guessed) measurement results,  described as follows:
    
    $\comro''_{\mathbb{R}^{zero}, \mathbb{R}^{one}, \widehat{\theta}, \widehat{x}}(q)$:
    
    \begin{itemize}
    
        \item Parse query $q$ as $x || \theta || r$
        
        \item If $\exists i$ such that $\theta = \widehat{\theta}_i$:
        
        \begin{itemize}
            \item If $\widehat{x_i} = 0$ and $x = 1$ and $r = r^{one}_i$, then set $q_{new} = \bar{x} || \theta || r^{zero}_i$
            
            \item If $\widehat{x_i} = 1$ and $x = 0$ and $r = r^{zero}_i$, then set $q_{new} = \bar{x} || \theta || r^{one}_i$

        \end{itemize}
        
        \item Else set $q_{new} = q$
        
        \item Return $\comro(q_{new})$
        
    \end{itemize}
    
\amit{Performing the mapping in such a way so that only 
%\st{non-openings}
incorrect measurement points (which we will be decided by delayed measurement) are remapped to the 
%\st{openings}
correct measurement points. For e.g. If delayed measurement of $i^{th}$ BB84 state resulted in 1, then remap $0||\theta||r^{zero}_i$ to the image of $1||\theta||r^{one}_i$. If the measurement was 0, vice-versa. This will ensure that the equivocal commitment openings have disjoint (and completely uncorrelated randomness) from the points which are remapped.}

\amit{Note that implementing the wrapper $\comro''$ is inefficient. In particular, it requires knowing the (delayed) measurement outcomes
%\st{and set $T$}
ahead of time. However, this is not an issue since $\comro''$ will not be used by the actual $\simu$. We introduce it just for proving indistinguishability}

Intuitively, $\comro''$ implements the same wrapper as $\comro'$ except %\st{for the indices in set $T$ where it flips the logic}
the following change: Instead of remapping the image of $1 || \widehat{\theta}_i || r^{one}_i$ to the image of $0 || \widehat{\theta}_i || r^{zero}_i$, it remaps the image of $\overline{\widehat{x}_i} || \widehat{\theta}_i || r^{\overline{\widehat{x}_i}}_i$ to the image of $\widehat{x}_i || \widehat{\theta}_i || r^{\widehat{x}_i}_i$, where $\widehat{x}_i$ are the (guessed) measurement results.

Having framed such a (wrappered) oracle $\comro''$, we can now say that an adversary which distinguishes between $\Hyb_2$ (where we are using $\comro$) and $\Hyb_3$ (where we are using $\comro'$) can also distinguish between $\Hyb_2$ (where we are using $\comro$) and $\Hyb_3'$ (where we use $\comro''$ instead of $\comro'$) - this is because $\comro''$ is identically distributed to $\comro'$ by construction.

Now we can invoke One Way to Hiding lemma on such an adversary to argue that there will exist a guessing adversary which successfully guesses the remapped points in $\comro''$, i.e. $\{ \overline{\widehat{x}_i} || \widehat{\theta}_i || r^{\overline{\widehat{x}_i}}_i \}_{i \in [16\secp]}$ with high probability. This implies that the adversary can guess $\{ r^{\overline{\widehat{x}_i}}_i \}_{i \in [16\secp]}$ with high probability. However, this is a contradiction since the randomness $\{ r^{\overline{\widehat{x}_i}}_i \}_{i \in [16\secp]}$ are totally uncorrelated with any of the protocol messages.

\amit{Need second pre-image resistance of $\comro''$ against a quantum adversary in order to rule out the guessing adversary of OW2H lemma ? The underlying game is (roughly) the following: Challenger samples $\comro$ and $r_1, r_2 \uniformsample \zo^\secp$. It then remaps $\comro(r_1)$ to $\comro(r_2)$ and sends $\comro$, $r_2, \comro(r_2)$ to the adversary. Adversary has to guess $r_1$}

\begin{theorem} [One-way to Hiding \cite{ambainis2019quantum}]
Let $S \subseteq X$ be an arbitrary subset. Let $G, H : X \rightarrow Y$ be arbitrary functions satisfying $\forall x \notin S, G(x) = H(x)$. Let $z$ be a arbitrary bitsring. ($S, G, H, z$ may have arbitrary joint distribution.)

$\forall$ quantum oracle algorithm $A^\mathcal{O}$ with query depth $d$ such that,

$$\Big| \Pr[b = 1 | b \leftarrow A^G(z)] - \Pr[b = 1 | b \leftarrow A^H(z)] \Big| = k$$

$\exists$ quantum oracle algorithm $B^\mathcal{O}_{A, d}$ such that,

$$ \Pr[S \cap T \ne \phi | T \leftarrow B^G_{A, d}] \ge \frac{k^2}{4d^2} $$

and

$$ \Pr[S \cap T \ne \phi | T \leftarrow B^H_{A, d}] \ge \frac{k^2}{4d^2} $$

\end{theorem}

Supoose there exists malicious sender-distinguisher pair $(S^*, D)$ which can distinguish between $\Hyb_2$ and $\Hyb_3'$. In our reduction, we will use the above OW2H lemma in the following way: We will set $G$ to be $\comro$, $H$ to be $\comro''$ and set $S$ to be $\overline{\widehat{x}_i} || \widehat{\theta}_i || r^{\overline{\widehat{x}_i}}_i$. Query algorithm $A_{OW2H}$ will be given access to either $G$ or $H$, and it will play the role of $\simu$ with $S^*$. In the end, $A_{OW2H}$ outputs whatever distinguisher $D$ outputs.

Therefore,

$$ \Pr[b = 1 | b \leftarrow A^G(z)] = \Pr[b = 1 | b \leftarrow D(\Hyb_2)] $$
$$ \Pr[b = 1 | b \leftarrow A^H(z)] = \Pr[b = 1 | b \leftarrow D(\Hyb_3')] $$

Hence,

$$ \Big| \Pr[b = 1 | b \leftarrow A^G(z)] - \Pr[b = 1 | b \leftarrow A^H(z)] \Big| = \Big| \Pr[b = 1 | b \leftarrow D(\Hyb_2)] - \Pr[b = 1 | b \leftarrow D(\Hyb_3')] \Big| \ge \frac{1}{\mathsf{poly}(\secp)}$$

By OW2H lemma, this implies the existence of an adversary $B^H_{A, d}$ which can guess the reporogrammed points in oracle $H$ with some inverse polynomial probabilty, and hence the randomness $\{ r^{\overline{\widehat{x}_i}}_i \}_{i \in [16\secp]}$. But this is a contradiction as these randomness are independent of any protocol messages.



\item $\Hyb_3 \approx_s \Hyb_4:$ These two distributions are statistically indistinguishable by construction.



\end{itemize}

==> qot-5r-recv-security.tex <==
\subsection{Analysis: Receiver Security}
%Simulate malicious sender

We first describe the construction of our simulator for a malicious sender $S^*$. In our construction, the $\simu$ will have oracle access to the random oracles $\{ \comro, \fsro, \maskro \}$. The $\simu$ will transparently forward all calls made by $S^*$ to the random oracles.\\

$\simu$:

\begin{enumerate}
    \item $\simu$ begins by executing $S^*$ to obtain BB84 states $\{ \ket{x_i}_{\theta} \}_{i \in [16\secp]}$ as described in Step 1 of the protocol.
    
    \item $\simu$ samples a set $Y_{\simu} \uniformsample \mathsf{Range}(\fsro)$ and sets $T_\simu := RandSubset_{[16\secp],8\secp}(Y_\simu)$. It also samples $\widehat{\theta} \leftarrow \{+, \times\}^{16\secp}$ and obtains $\widehat{x} \in \{0, 1\}$ by measuring only $\{ \ket{x_i}_{\theta} \}_{i \in T_\simu}$ in basis $\widehat{\theta_i}$. The remaining states $\{ \ket{x_i}_{\theta} \}_{i \notin T_\simu}$ are not measured. $\simu$ then computes a measurement check proof $\pi$ as follows:
    
    \begin{enumerate}
        \item Commitment: $\forall i \in T_\simu$, $com_i = \comro(\widehat{x}_i || \widehat{\theta}_i || \widehat{r}_i)$ where $\widehat{r}_i \leftarrow \{0, 1\}^\secp$. $\forall i \notin T_\simu$, $com_i = \comro(0 || \widehat{\theta}_i || \widehat{r}_i)$ where $\widehat{r}_i \leftarrow \{0, 1\}^\secp$
    
        \item Challenge: Program $\fsro$ at domain point $(com_1 || \ldots || com_{16\secp})$ so that $\fsro(com_1 || \ldots || com_{16\secp}) := Y_\simu$
    
        \item Set $\pi = (\{com_i\}_{i \in [16\secp]}, Y_\simu, \{\widehat{x}_i, \widehat{\theta}_i, \widehat{r}_i \}_{i \in T_\simu})$, and send $\pi$ to $S^*$.
    \end{enumerate}
    
    \item Receive the basis values $\{ \theta_i \}_{i \in \overline{T_\simu}}$ from $S^*$, where $ \overline{T_\simu} = [16 \secp] \setminus T_\simu$.
    
    \item Form sets $I_0$ and $I_1$ in the following way and send $(I_0, I_1)$ to $S^*$.
    
    \begin{enumerate}
        \item Divide $\overline{T_\simu}$ into 2 disjoint subsets $S_0, S_1$ in the following way - $S_0 = \{ i | i \in \overline{T_\simu} \wedge \widehat{\theta_i} = \theta_i \}, 
    S_1 = \{ i | i \in \overline{T_\simu} \wedge \widehat{\theta_i} \ne \theta_i \}$.
    
        \item Set $I_0 = S_0$ and $I_1 = S_1$.
    \end{enumerate}
    
    \item Receive $s, ct_0, ct_1$ from $S^*$.
    
    \item On receiving $s, ct_0, ct_1$ from $S^*$, performs the following steps:
    
    \begin{itemize}
        \item  $\forall i \in \overline{T_\simu}$, measure $\ket{x_i}_{\theta}$ in the basis $\theta_i$ (where $\theta_i \in \{ \theta_i \}_{i \in \overline{T_\simu}}$ are the basis values received from $S^*$ in Step 3) to obtain $\widehat{x_i}$
        
        \item Compute $m_0 = ct_0 \oplus \maskro(s || \{ \widehat{x_i} \}_{i \in I_0})$ and $m_1 = ct_1 \oplus \maskro(s || \{ \widehat{x_i} \}_{i \in I_1})$. 
        
        \item Send $m_0, m_1$ to the OT Ideal functionality.
    \end{itemize}
    
\end{enumerate}


Having defined the $\simu$, we will now show that the real distribution is indistinguishable from the ideal distribution using a sequence of hybrids. In our sequence, $\Hyb_0$ will correspond to the real distribution and the last hybrid, $\Hyb_6$, will correspond to the ideal simulated distribution. 


\begin{itemize}
    \item $\Hyb_0:$ This corresponds to the Real World. The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the honest receiver $R$.
    
    \item $\Hyb_1:$ $\simu$ takes the role of honest $R$ and also transparently forwards all calls between $S^*$ and $\{\comro, \fsro, \maskro\}$. The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the simulated receiver.
   
    
    \item $\Hyb_2$: $\simu$ behaves exactly as $\Hyb_1$ except the following additional steps between Step 2a and Step 2b:
    
    \begin{itemize}
        \item $\simu$ privately samples a set $Y_{\simu} \uniformsample \mathsf{Range}(\fsro)$
        
        \item $\simu$ programs $\fsro$ so that $\fsro(com_1 || \ldots || com_{16\secp}) = Y_{\simu}$, where $\{com_i\}_{i \in [16\secp]}$ are commitments generated in Step 2a.
    \end{itemize}
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the simulated receiver.
    
    \item $\Hyb_3$: $\simu$ behaves exactly as $\Hyb_2$ except that the sampling of $Y_{\simu}$ is shifted to the beginning of Step 2.
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the simulated receiver.
    
    \item $\Hyb_4$: $\simu$ behaves exactly as $\Hyb_3$ except that in Step 2a, the commitments $\{ com_i \}_{i \in \overline{T_\simu}}$, where $T_\simu = RandSubset_{[16\secp],8\secp}(Y_\simu)$ and $\overline{T_\simu} = [16\secp] \setminus T_\simu$, are generated as follows: $\forall i \in \overline{T_\simu}, com_i = \comro(0 || \widehat{\theta_i} || r_i)$
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the simulated receiver.

    
    \item $\Hyb_5$: $\simu$ behaves exactly as $\Hyb_4$ except that in Step 2, it doesn't measure $\{ \ket{x_i}_{\theta} \}_{i \in \overline{T_\simu}}$, where $T_\simu = RandSubset_{[16\secp],8\secp}(Y_\simu)$. Instead, it delays the measurement of these BB84 till Step 5. On receiving $s, ct_0, ct_1$ from $S$ in Step 5, it performs the following steps:
    
    \begin{itemize}
        \item  $\forall i \in \overline{T_\simu}$, it measures $\ket{x_i}_{\theta}$ in the basis $\theta_i$ (where $\theta_i \in \{ \theta_i \}_{i \in \overline{T_\simu}}$ are the basis values it receives from $S$ in Step 3) to obtain $\widehat{x_i}$
        
        \item It computes $m_0 = ct_0 \oplus \maskro(s || \{ \widehat{x_i} \}_{i \in I_0})$ and $m_1 = ct_1 \oplus \maskro(s || \{ \widehat{x_i} \}_{i \in I_1})$. 
        
        \item It then sends $m_0, m_1$ to the OT Ideal functionality.
    \end{itemize}
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.
    
    
    \item $\Hyb_6$: $\simu$ behaves exactly as $\Hyb_5$ except that in Step 4 b, instead of using $b$ to define the sets $I_0$ and $I_1$, it instead sets $I_0 := S_0$ and $I_1 := S_1$. It then completes the remaining steps as mentioned in the previous hybrid.
    
    The output of this hybrid consists of the final state of the malicious sender $S^*$ and the output of the ideal-world receiver.
    
    
\end{itemize}

We will now argue the computational indistinguishability of each pair of consecutive hybrids in the above sequence.

\amit{Pin down where exactly in the proof are we leveraging the fact that $I_0$ and $I_1$ are $\secp$ bits long.}
\nishant{I think this is required for $\Hyb_5 \rightarrow \Hyb_6$}
\amit{I don't think the size of $I_0$ and $I_1$ have any effect on receiver security; it only seems to be critical for sender security}

\begin{itemize}
    \item $\Hyb_0 = \Hyb_1$: The distribution of $\Hyb_0$ is identical to the distribution of $\Hyb_1$ by construction. Hence these two hybrids are perfectly indistinguishable.
    
    \item $\Hyb_1 \approx_c \Hyb_2$: \nishant{I think this is statistical? it seems the hardness of the ROM theorem comes from the poly queries a PPT adv can do to a RO?} \amit{I agree; will check with Dakshita once}
    Assume towards contradiction that there exists malicious sender $S^*$ and distinguisher $D$ such that:
    
    $$ \Big| \Pr[ b = 1 | b \leftarrow  D(\Hyb_1)] - \Pr[ b = 1 | b \leftarrow  D(\Hyb_2)] \Big| \ge \frac{1}{\poly(\secp)} $$
    
    We will show that there exists a triple of algorithms $A_0, A_C, A_2$ which contradicts the following theorem (presented as Corollary 6 in \cite{EC:Unruh15})
    
    \begin{theorem} [Adaptive ROM programming I] \label{thm: adaptiveROMprogramming}
    Let $M,N$ be finite sets and $H : M \rightarrow N$ be the random oracle. Let $A_0, A_C, A_2$ be algorithms, where $A^H_0$ makes at most $q$ queries to $H$, $A_C$ is classical, and the output of $A_C$ is in $M$ and has collision-entropy at least $k$ given $A_C$’s initial state. $A_0, A_C, A_2$ may share state. Then,
   
   \begin{align*}
    & \Big| \Pr[ b = 1 | H \uniformsample (M \rightarrow N), A^H_0(), x \leftarrow A_C(), B := H(x), b \leftarrow A_2^H(B)] \\
   & - 
    \Pr[ b = 1 | H \uniformsample (M \rightarrow N), A^H_0(), x \leftarrow A_C(), B \uniformsample N, H(x) := B, b \leftarrow A_2^H(B)] \Big| \le (4 + \sqrt{2}) \sqrt{q} 2^{-k/4}
   \end{align*} 
   
     \end{theorem}

    \begin{proof}
    
    Given $S^*, D$, we will now define the algorithms $A_0, A_C, A_2$. $A_0, A_2$ will have external oracle access to $H := \fsro$. Additionally $A_0, A_C, A_2$ will have internal oracle access to $\comro$ and $\maskro$
    
    ${A_0}^{\fsro}_{S^*}()$:
    
    \begin{itemize}
        \item Run $S^*$ to generate the first sender message of the protocol.
        
        \item Run honest $R$ algorithm to perform the measurement of BB84 states as mentioned in Step 2 to obtain $\{ \widehat{x_i} \}_{i \in [16\secp]}$
    \end{itemize}
    
    
    $A_C()$:
    
    \begin{itemize}
        \item Receive $\{ \widehat{x_i}, \widehat{\theta_i} \}_{i \in [16\secp]}$ as an initial classical state from $A_0$
        
        \item Sample $\widehat{r_i} \uniformsample \zo^\secp$ for all $i \in [16\secp]$
        
        \item Perform Step 2a of the honest $R$ algorithm to obtain $\{ com_i \}_{i \in [16\secp]}$ and output it.
    \end{itemize}
    
    ${A_2}^{\fsro}_{S^*, D}(B)$:
    
    \begin{itemize}
        \item Receive $\{ com_i, \widehat{x_i}, \widehat{\theta_i}, \widehat{r_i} \}_{i \in [16\secp]}$ as an initial classical state from $A_C()$
        
        \item Receive $\ket{\state_{S^*}}$ as the final state of sender at the end of $A_0$'s execution.
        
        \item Perform Step 2c of the protocol by setting $\pi := ( \{com_i\}_{i \in [16\secp]}, B, \{ \widehat{x_i}, \widehat{\theta_i}, \widehat{r_i} \}_{i \in T})$ where $T = RandSubset_{[16\secp],8\secp}(B)$
        
        \item Initialize $S^*$ using $\ket{\state_{S^*}}$ and send $\pi$ to it.
        
        \item Complete the remainder of protocol (starting from Step 3) between $S^*$ and honest receiver $R$
        
        \item Output the bit $b$ returned by the distinguisher $D$
    \end{itemize}
    
    
    Having defined $A_0, A_C, A_2$, we note that:
    
    \begin{align*}
    & \Pr[ b = 1 | \fsro \uniformsample (M \rightarrow N), A_0^{\fsro}(), \{ com_i \}_{i \in [16\secp]} \leftarrow A_C(), B := \fsro(\{ com_i \}_{i \in [16\secp]}), b \leftarrow {A_2}^{\fsro}(B)] \\
    & = \Pr[ b = 1 | b \leftarrow  D(\Hyb_1)]
    \end{align*}
    \begin{align*}
    & \Pr[ b = 1 | \fsro \uniformsample (M \rightarrow N), A_0^{\fsro}(), \{ com_i \}_{i \in [16\secp]} \leftarrow A_C(), B \uniformsample N, \fsro(\{ com_i \}_{i \in [16\secp]}) := B, b \leftarrow {A_2}^{\fsro}(B)] \\
    & = \Pr[ b = 1 | b \leftarrow  D(\Hyb_2)]
    \end{align*}
    
    Therefore,
    
    \begin{align*}
    &\Big| \Pr[ b = 1 | \fsro \uniformsample (M \rightarrow N), A_0^{\fsro}(), \{ com_i \}_{i \in [16\secp]} \leftarrow A_C(), B := \fsro(\{ com_i \}_{i \in [16\secp]}), b \leftarrow {A_2}^{\fsro}(B)] \\
    & - \Pr[ b = 1 | \fsro \uniformsample (M \rightarrow N), A_0^{\fsro}(), \{ com_i \}_{i \in [16\secp]} \leftarrow A_C(), B \uniformsample N, \fsro(\{ com_i \}_{i \in [16\secp]}) := B, b \leftarrow {A_2}^{\fsro}(B)] \Big| \\
    & = \Big| \Pr[ b = 1 | b \leftarrow  D(\Hyb_1)] - \Pr[ b = 1 | b \leftarrow  D(\Hyb_2)] \Big| \ge \frac{1}{\poly(\secp)}
    \end{align*}
    
    Now we will show how the above inference contradicts Theorem \ref{thm: adaptiveROMprogramming}. We first observe that the output $\{ com_i \}_{i \in [16\secp]}$ of $A_C$ has atleast $\poly(\secp)$ collision entropy for some fixed $\poly$. To prove this, we will measure the collision entropy of just $com_0$ and use it to lower bound the collision entropy of $\{ com_i \}_{i \in [16\secp]}$. Imagine two random variables - $com_0^{exec_0}$ and $com_0^{exec_1}$ - which denote the value of $com_0$ obtained by executing two independent executions of algorithm $A_C$ using the same fixed initial classical state. Now, the collision entropy of $com_0$ will be exactly equal to $-\log \Pr[com_0^{exec_0} = com_0^{exec_1}]$.
    
    \begin{align*}
        \Pr[com_0^{exec_0}= com_0^{exec_1}] &= \Pr[com_0^{exec_0}= com_0^{exec_1} | \widehat{r_0}^{exec_0} = \widehat{r_0}^{exec_1}] + \Pr[com_0^{exec_0}= com_0^{exec_1} | \widehat{r_0}^{exec_0} \ne \widehat{r_0}^{exec_1}] \\
        &= \Pr[\widehat{r_0}^{exec_0} = \widehat{r_0}^{exec_1}] \\
        &+ \Pr[\widehat{r_0}^{exec_0} \ne \widehat{r_0}^{exec_1}] \cdot \Pr[\comro(\widehat{x_0} || \widehat{\theta_0} || \widehat{r_0}^{exec_0}) = \comro(\widehat{x_0} || \widehat{\theta_0} || \widehat{r_0}^{exec_1}) | \widehat{r_0}^{exec_0} \ne \widehat{r_0}^{exec_1}]\\
        & \le \frac{1}{2^\secp} + (1 - \frac{1}{2^\secp}) \cdot \frac{1}{2^\secp}\\
        & \le \frac{1}{2^{\secp - 1}}
    \end{align*}
     
    Therefore, $-\log \Pr[com_0^{exec_0} = com_0^{exec_1}] \ge -\log \frac{1}{2^{\secp - 1}}$, and hence collision entropy of $com_0$ is atleast $\secp - 1$. It follows directly that the output of $A_C$ consisting of $\{ com_i \}_{i \in [16\secp]}$ also has a collision etropy of atleast $\secp - 1$.
    
    
    Since the output $\{ com_i \}_{i \in [16\secp]}$ of $A_C$ has collision entropy atleast $k = O(\secp)$, and $A_0$ makes atmost $q = \poly_{S^*}(\secp)$ number of queries to $\fsro$ (where $\poly_{S^*}$ is a fixed polynomial depending on the query complexity of given sender $S^*$), the distinguishing advantage as given by Theorem \ref{thm: adaptiveROMprogramming} should be $\negl(\secp)$. However, our reduction shows that the distinguishing advantage is noticeable which contradicts Theorem \ref{thm: adaptiveROMprogramming}.
    
    \end{proof}
    
\item $\Hyb_2 = \Hyb_3$: These two hybrids are identically distributed by construction, and hence perfectly indistinguishable.


\item $\Hyb_3 \approx_c \Hyb_4$: \nishant{I think this is also statistical?} \amit{I agree; will check with Dakshita once}
To prove this, we will introduce a sequence of intermediate hybrids - $\Hyb_{3, 1}, \ldots, \Hyb_{3, |\overline{T_\simu}|}$ - between $\Hyb_3$ and $\Hyb_4$. $\Hyb_{3, i}$ is exactly same as $\Hyb_{3, i-1}$ except that in Step \ref{itm:qot-recv-meas-com}, commitment $com_j$ is generated as $\comro(0 || \widehat{\theta_j} || r_j)$ instead of  $\comro(\widehat{x_j} || \widehat{\theta_j} || r_j)$, where $j$ refers to the element at the $i^{th}$ location in the sorted version of $\overline{T_\simu}$ (recall that $\overline{T_\simu}$ represents a subset of $[16 \secp]$ in the actual protocol where the commitments are not opened). Note that  $\Hyb_{3, \overline{T_\simu}}$ is identical to $\Hyb_4$.  We claim that $\Hyb_3 \approx_c \Hyb_{3, 1} \approx_c \ldots \approx_c \Hyb_{3, |\overline{T_\simu}|} = \Hyb_4$.

Assume towards contradiction that there exists $i \in [|\overline{T_\simu}|]$, a malicious sender $S^*$ and a distinguisher $D$ such that,

$$\Big| \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i})] - \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i - 1})] \Big| \ge \frac{1}{\poly(\secp)}$$

We will show that there exists an adverary $A$ which will contradict Lemma \ref{lemma:rom-hiding-commitment}. Before constructing such $A$, we note the following: Conditioned on the event where $\widehat{x_i} = 0$, $\Hyb_{3, i - 1}$ is identical to $\Hyb_{3, i}$ and hence perfectly indistinguishable. Therefore, we only focus on the case where $\widehat{x_i} = 1$. With that in mind, we build a reduction adversary $A$ as follows:

$A_{S^*, D}:$

\begin{enumerate}
    \item Receive oracle $H$ and a commitment string $c$ from the challenger
    
    \item Instantiate $\comro := H$ and begin executing the $\simu$ algorithm for $\Hyb_{3, i}$ with $S^*$ except the following change: Replace $com_j$ generated by the $\simu$ in Step \ref{itm:qot-recv-meas-com} with commitment $c$ that is received from the external challenger, where $j$ refers to the element at $i^{th}$ location in the sorted version of $\overline{T_\simu}$.
    
    \item Complete the protocol, run the distinguisher $D$, receive a bit $b$ from $D$ and return it to the challenger.
\end{enumerate}

Now we make the following observation: 

\begin{align*}
\Pr[b = 1 | H \uniformsample (\zo^* \rightarrow \zo^\secp), r \uniformsample \zo^\secp, c := H(0 || r), b \leftarrow A_{S^*, D}^H(c)] = \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i})] \\
\Pr[b = 1 | H \uniformsample (\zo^* \rightarrow \zo^\secp), r \uniformsample \zo^\secp, c := H(1 || r), b \leftarrow A_{S^*, D}^H(c)] = \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i - 1})]
\end{align*}

Therefore,

\begin{align*}
\Big| \Pr[b = 1 | H \uniformsample (\zo^* \rightarrow \zo^\secp), r \uniformsample \zo^\secp, c := H(0 || r), b \leftarrow A_{S^*, D}^H(c)] \\
- \Pr[b = 1 | H \uniformsample (\zo^* \rightarrow \zo^\secp), r \uniformsample \zo^\secp, c := H(1 || r), b \leftarrow A_{S^*, D}^H(c)] \Big| = \\
\Big| \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i})] - \Pr[b = 1 | b \leftarrow D(\Hyb_{3, i - 1})] \Big| \ge \frac{1}{\poly(\secp)}
\end{align*}

Hence, the reduction adversary $A_{S^*, D}$ contradicts Lemma \ref{lemma:rom-hiding-commitment}.

\amit{In the following hybrids, the ideal functionality is being invoked. Therefore, the output of the hybrid needs to be clarified (and explicity stated) that it contains the view of adversary + output of the honest party. In earlier hybrids, the hybrid output consists of the adversary's view + simulated receiver's output}

\item $\Hyb_4 = \Hyb_5$: Note that, in the previous hybrid, the values $\{ \widehat{x_i} \}_{i \in \overline{T_\simu}}$ have no effect on the distribution of transcript messages as these values are not used anywhere before Step 6. 
Hence, delaying the measurement of$\{ \ket{x_i}_{\theta} \}_{i \in \overline{T_\simu}}$ until the last step (as specified in $\Hyb_5$) doesn't have any effect on the distribution of $\Hyb_4$. To make sure that the output distribution of honest $R$ doesn't change, $\simu$ simply performs a delayed measurement as specified in $\Hyb_5$, extracts $\{ m_0, m_1 \}$ from $\{ ct_0, ct_1 \}$ and sends it to the OT ideal functionality. The correctness of this extraction procedure is implied by the perfect indistinguishability between $\Hyb_4$ and $\Hyb_5$ in all the prior steps of the protocol.

\item $\Hyb_5 \approx_s \Hyb_6$: 

\nishant{I think we should write a formal reduction in this step for reducing $(S_0,S_1) \approx_s (S_1,S_0)$ to a distinguisher distinguishing $\Hyb_5, \Hyb_6$. The fact that $\{\widehat{\theta}_i\}_{i \in \overline{T}}$ is not required for the reduction serves to show that $\{\widehat{\theta}_i\}_{i \in \overline{T}}$ is hidden from the adv}


We first observe that $S_0 \approx_s S_1$ as long as $\{ \widehat{\theta_i} \}_{i \in \overline{T}}$ is private (which is in fact the case from the point of view of malicious sender and the distinguisher). This is because $\{ \widehat{\theta_i} \}_{i \in \overline{T}}$ is sampled uniformly at random, and hence $\{ S_0, S_1 \}$ form a uniformly random partition of the set $\overline{T}$. Hence, $(S_0, S_1) \approx_s (S_1, S_0)$.

Note that the protocol transcript contains $(I_0, I_1)$ which would be equal to $(S_b, S_{1-b})$ for an honest receiver strategy (and hence also for $\simu$ strategy until $\Hyb_5$). However, for the $\simu$ strategy in $\Hyb_6$, $(I_0, I_1)$ is always equal to $(S_0, S_1)$. Hence, if $b = 0$, the distribution of $(I_0, I_1)$ in $\Hyb_5$ would be identical to $\Hyb_6$. On the other hand, if $b = 1$, the distribution of $(I_0, I_1)$ in $\Hyb_5$ would be statistically indistinguishable from $\Hyb_6$ (following from the fact that $(S_0, S_1) \approx_s (S_1, S_0)$). Putting together these two observations, it easily follows that $\Hyb_5 \approx_s \Hyb_6$.

\end{itemize}

==> qot-5r-sender-security.tex <==
\subsection{Analysis: Sender Security}

To simulate for a malicious receiver $\malrecv$ with advice $\brho$, $\simurecv(\brho)$ works as follows:

\begin{enumerate}
    \item $\simurecv(\brho)$ defines the following oracles.
        \begin{enumerate}
            \item \nishant{Need more details here} It initializes $\simuextrac$ and answers any queries to $\comro(x)$ as $\simuextrac.RO(x)$.
            \item It chooses hash functions $h_M$ and $h_{FS}$ randomly from a $2q$-wise independent hash function family where $q$ is an upper bound on the total number of queries made by $\malrecv$ on any of the ROs (which can be obtained by $\simurecv$ non-uniformly). Any queries to $\maskro(x)$ are answered as $h_M(x)$ and to $\fsro(x)$ as $h_{FS}(x)$.
            \item \label{itm:simr-sample-s} In addition, it samples $s \gets \zo^\secp$ and defines an oracle $\maskrop$ as follows: $\maskrop(s||\cdot) = \bot$, $\maskrop(x)=\maskro(x)$ otherwise. Concretely, it builds a circuit which checks if the input if of the form $s||\cdot$ and if so, answers with $\bot$, otherwise answers with $h_M$. 
        \end{enumerate}
    \item $\simurecv(\brho)$ starts executing the protocol with $\malrecv(\brho)$, answering any queries to $\comro$ and $\fsro$ as described above. However, any queries to $\maskro$ are answered with $\maskrop$. 
    \item As the first step of the protocol, it sends BB84 states $\ket{x}_\theta$ to $\malrecv$ just as the original sender would.
    \item In turn it receives the measurement check proof $\pi = (\{c_i\}_{i \in [16\secp]}, Y, \{\widehat{x_i}, \widehat{\theta_i}, \widehat{r_i} \}_{i \in T})$ from $\malrecv$ and performs the same checks as the sender in Step \ref{itm:qot-sendr-check} of \proref{fig:qot-5r-construction}. It then uses $\simuextrac$ to extract the corresponding $\widehat{x}_i,\widehat{\theta}_i$ from $c_i$, i.e. it sets $\widehat{x}_i||\widehat{\theta}_i||\widehat{r_i} = \simuextrac.E(c_i), \forall i \in \overline{T}$.
    \item It then continues the protocol with $\malrecv$ just as a honest sender, sending it $\{\theta_i\}_{i \in \overline{T}}$ and subsequently receives $(I_0,I_1)$ from $\malrecv$. Let $P$ be the indices in $I_0$ where $\theta_i \neq \widehat{\theta}_i$. If $|P| > 3\secp/2$, then it sets $b=1$, otherwise sets $b=0$.
    \item It queries $\fot$ with input $b$ to get $m_b$. It sets $ct_b = m_b \oplus \maskro(s || \{x_i\}_{i \in I_b}), ct_{1-b} = 0^\secp \oplus \maskro(s||\{x_i\}_{i \in I_{1-b}})$, where $s$ is the same string it chose earlier in Step \ref{itm:simr-sample-s}. 
    \item It reprograms the oracle $\maskro$ at the input $s||\{x_i\}_{i \in I_{1-b}}$ using a fresh random value. It calls this reprogrammed oracle $\maskror$. Concretely, it builds a circuit wrapper over its simulated $\maskro$ which does this. It then sends $s,ct_0,ct_1$ to $\malrecv$ and answers any queries to $\maskro$ made by $\malrecv$ using $\maskror$, instead of using $\maskrop$ as before. It then outputs $\malrecv$'s final state.
\end{enumerate}

We will now show that the joint output of honest sender - $\outsendr$ and $\simurecv$ in the ideal world is computationally close to one in the real game by going through a sequence of hybrids.

\begin{itemize}
    \item $Hyb_0$: This is the real world, where $\malrecv(\brho)$ is interacting with an honest sender $S$ and having all its RO queries answered by the real random oracles.
    
    \item $Hyb_1$: Same as $Hyb_0$, except now the RO queries made by $\malrecv$ are answered by the sender. The sender continues to use the respective real ROs to do this.
    
    \item $Hyb_2$: Same as $Hyb_1$, except the sender starts using a $2q$-wise independent hash function to answer the oracle queries for $\fsro$ and $\maskro$, where $q$ is the total number of queries made by $\malrecv$ to any of the three ROs (obtained non-uniformly by $S$). It still continues to use the real random oracle to answer queries to $\comro$. 
    
    \item $Hyb_3$: Same as $Hyb_2$, except the sender now answers the queries to $\comro$ using $\simuextrac.RO$.
    
    \item $Hyb_4$: Same as $Hyb_3$, except it now starts extracting $\widehat{\theta_i},\widehat{x_i}$ using $\simuextrac.E$ after receiving the measurement check proof from $\malrecv$ in the second message of the protocol. In particular, as done by $\simurecv$, it sets $\widehat{x}_i||\widehat{\theta}_i||\widehat{r_i} = \simuextrac.E(c_i), \forall i \in \overline{T}$. After receiving the sets $(I_0,I_1)$ from $\malrecv$ in the fourth message of the protocol, it finds the set $P$ as the indices in $I_0$ where $\theta_i \neq \widehat{\theta}_i$. If $|P| > 3\secp/2$, then it sets $b=1$, otherwise sets $b=0$. Even though it sets the value of $b$, it doesn't use it anywhere else in the protocol.
    
    \item $Hyb_5$: Same as $Hyb_4$, except the string $s$ sampled randomly from $\zo^\secp$ by $S$ while sending the last message of the protocol is now sampled at the beginning before it even starts the protocol execution.
    
    \item $Hyb_6$: Before starting the protocol, $S$ first defines the oracle $\maskrop$ as : $\maskrop(s||\cdot) = \bot, \maskrop(x) = \maskro(x)$ otherwise, where $s$ is $\secp$ length string sampled at the beginning of the protocol as in $Hyb_5$. Concretely, it uses a circuit to act as a wrapper over $\maskro$ to do this. It then continues the protocol as in $Hyb_5$, except in how it answers the RO queries to $\maskro$. It answers any queries to $\maskro$ made by $\malrecv$ using $\maskrop$ up until before sending the last message in \prostepref{itm:qot-sendr-lastmsg} of \proref{fig:qot-5r-construction}. After sending the last message, it answers any queries to $\maskro$ using its simulated $\maskro$ as was happening in $Hyb_5$.
    
    \item $Hyb_7$: This is the same as $Hyb_6$, except in how $S$ answers the RO queries to $\maskro$. As in $Hyb_6$, it continues to use $\maskrop$ to answer any queries to $\maskro$ before sending the last message to $\malrecv$. But to answer any queries to $\maskro$ after sending the last message to $\malrecv$, it defines a reprogrammed oracle $\maskror$ and uses that to answer any subsequent queries to $\maskro$. To define $\maskror$, it reprograms $\maskro$ at the point $s||\{x_i\}_{i \in I_{1-b}}$ with a fresh random value (concretely, using a circuit wrapper over its simulated $\maskro$).
    
    \item $Hyb_8$: Same as $Hyb_7$, except now $S$ sets $m_{1-b}=0^\secp$. 
    
    \item $Hyb_9$: This is the ideal world where $\simurecv$ acts as already defined.
\end{itemize}

We now argue the indistinguishability of the hybrids defined above. 
\begin{itemize}
    \item $Hyb_0 \rightarrow Hyb_1$: Since the RO queries continue to be answered by the real ROs, but are just redirected through $S$, we have that the output distributions in either hybrids are identical, i.e. $Hyb_0 \equiv Hyb_1$.
    
    \item $Hyb_1 \rightarrow Hyb_2$: $Hyb_2$ is same as $Hyb_1$ except $S$ uses hash functions chosen from $2q$-wise independent hash family to answer queries to $\comro$ and $\fsro$. But we know from \cite{zhandry12qwise} that any quantum algorithm making at most $q$ queries to a RO behaves identically given either the real RO or a hash function chosen from a $2q$-wise independent hash family. And since the $q$ chosen by $S$ in $Hyb_2$ is an upper bound on number of queries performed by $\malrecv$ to any of the ROs, we conclude $Hyb_1 \equiv Hyb_2$. \nishant{TODO: formalize this further after checking the ppr}
    
    \item $Hyb_2 \rightarrow Hyb_3$: This follows from \cite{DFMS21}. \nishant{TODO: fill in details after checking the ppr}.
    
    \item $Hyb_3 \rightarrow Hyb_4$: The only change when going from $Hyb_3$ to $Hyb_4$ is that $S$ now extracts $\widehat{\theta},\widehat{x_i}, \forall i \in \overline{T}$. That this extraction goes unnoticed by $\malrecv$ follows from \cite{DFMS21}. \nishant{TODO: fill in details after checking the ppr}
    
    \item $Hyb_4 \rightarrow Hyb_5$: The only change in $Hyb_5$ from $Hyb_4$ is that the $\secp$ length string $s$ is sampled at the beginning of the protocol rather then when needed while sending the last message to $\malrecv$. But since $s$ is only used while sending the last message to $\malrecv$ and nowhere before, it follows that the view of $\malrecv$ in either world is identical. Hence, $Hyb_4 \equiv Hyb_5$.
    
    \item $Hyb_5 \rightarrow Hyb_6$: We will prove the indistinguishability between $Hyb_5$ and $Hyb_6$ using the one-way to hiding theorem from \cite{ambainis2019quantum}.
    In particular, suppose for the sake of contradiction, that $\exists$ a pair of messages $m_0,m_1$, a malicious receiver $\malrecv(\brho)$, a distinguisher $\maldist(\bsigma)$ s.t. $\maldist(\bsigma,\cdot)$ distguishes between the outputs of $Hyb_5$ and $Hyb_6$. If we label the outputs in either hybrids by $\outsendr,\outmalrecv$ for output of $Hyb_5$ and $\outsendr',\outmalrecv'$ for output of $Hyb_6$, then this means $|Pr[\maldist(\bsigma, \outsendr, \outmalrecv)=1] - Pr[\maldist(\bsigma, \outsendr', \outmalrecv')=1]| = \epsilon$, where $\epsilon$ is the non-negligible advantage of $\maldist$ in distinguishing $Hyb_5$ and $Hyb_6$.
    
    Given the existance of such a $\maldist$, we will now build a one-way to hiding adversary $\cA$ which breaks the one-way to hiding theorem of \cite{ambainis2019quantum}. $\cA$ is given as input a string $s \gets \zo^\secp$ and the description sufficient for simulation of oracles $\comro,\fsro,\maskro$ \nishant{TODO: don't know the description behind the exRO}, in addition to the advice strings for $\malrecv$ and $\maldist$ - $\brho,\bsigma$. $\cA$ also gets oracle access to one of two oracles - $O_1,O_2$. Here $O_1 = \maskro$ and $O_2 = \maskrop$ where $\maskro$ is the actual RO as in either of $Hyb_5$ or $Hyb_6$ and $\maskrop$ is defined similar to $Hyb_6$, i.e. $\maskrop(s||\cdot) = \bot, \maskrop(x) = \maskro(x)$ otherwise, and where $s$ is the same $\secp$ length string given as input to $\cA$. Note that to fit the description of the O2H theorem, $\cA$ is given access to the actual (full) ROs - $\maskro$ and $\maskrop$, and not the simulated ones as in $Hyb_5$ or $Hyb_6$. But again this would not matter since by $\cite{zhandry12qwise}$ the behaviour of $\cA$ doesn't change when given the real RO or the one simulated using a hash function chosen from $2q$-wise independent hash family.
    
    $\cA^O(s,\comro,\fsro,\maskro,\brho,\bsigma)$ executes the protocol with $\malrecv(\brho)$ acting as the sender from $Hyb_5$. It answers any queries to $\comro,\fsro$ by simulating the corresponding RO as in $Hyb_5$ or $Hyb_6$ (and using the descriptions provided to it as input). Also, it answers any queries to $\maskro$ by $\malrecv$ using the oracle $O$, up until before sending the last message to $\malrecv$. In computing the last message to be sent to $\malrecv$ and answering oracle queries to $\maskro$ subsequently, $\cA$ uses the description of $\maskro$ provided to it as input. At the end of the protocol execution, $\cA$ outputs $\maldist(\bsigma, \outsendr, \outmalrecv)$, where $\outsendr$ is $\mathsf{end}$ and $\outmalrecv$ is the final state of $\malrecv$ at the end of the protocol execution.
    
    Now note that if $\cA$ is given oracle access to $O_1 = \maskro$, it is simulating exactly $Hyb_5$ for the corresponding $\malrecv$ and if given oracle access to $O_2 = \maskrop$, it is simulating exactly $Hyb_6$ for $\malrecv$, except the tiny difference that in this case it is using the actual ROs for simulating $\maskro/\maskrop$, while in $Hyb_5/Hyb_6$ the same was being simulated using a $2q$-wise independent hash function. But as explained earlier, by \cite{zhandry12qwise}, the output distribution in either case is identical \nishant{give actual hybrids?}. Hence, $Pr[\cA^{O_1}(s,\comro,\fsro,\maskro,\brho,\bsigma)=1] = Pr[\maldist(\bsigma,\outsendr,\outmalrecv)=1]$ and $Pr[\cA^{O_2}(s,\comro,\fsro,\maskro,\brho,\bsigma)=1] = Pr[\maldist(\bsigma,\outsendr',\outmalrecv')=1]$ and hence $\cA$ distinguishes between the two oracles with non-negl probability $\epsilon$. 
    
    Therefore, by the O2H theorem of \cite{ambainis2019quantum}, $\exists$ adversary $\cB^{O_1}$, who works by choosing a query $i \gets \{1,2 \ldots q_M\}$ at random, where $q_M$ is the number of oracle queries made by $\cA$, running $\cA$ up until that point of query and measuring all the query input registers till then in computational bases, and outputting the set $T$ of measurement outcomes. Note that between the two oracles $O_1,O_2$ given to $\cA$, the set of points in which they differ is given by $S=\{s||y, \forall y\}$. The O2H theorem of \cite{ambainis2019quantum} then guarantees that $Pr[S \cap T \neq \emptyset] \geq \frac{\epsilon}{4q}$, which is still non-negl. But since the set $T$ is the result of measuring queries of $\cA$, which exactly corresponds to the set of queries made by $\malrecv$ during the run by $\cA$ before sending the last message, this means running $\malrecv$ up until some $i^{th}$ query and measuring all those queries in computational bases gave some point prefixed by $s$ with non-negl probability. But since $\malrecv$ doesn't get to know $s$ before the last message and $s$ was chosen uniformly at random from $\zo^\secp$, this can only happen with probability $\frac{1}{2^\secp}$, and hence we overall get a contradiction. \nishant{TODO: unsatisfying, there is a final logical step missing in going from measurement to knowing, there has to be something to capture that the queries by $\malrecv$ can be superposition queries, but they collapse to some point in $S$ with only negl prob unless $\malrecv$ knows $s$ + there should be something to capture that for example $\malrecv$ can't just find some point which evaluates to $\bot$ by doing quantum queries to $\maskrop$} 
    
    \item $Hyb_6 \rightarrow Hyb_7$:  We will use the O2H lemma from \cite{ambainis2019quantum} to do a direct reduction to the EPR protocol as described in \sectionref{subsec:epr-protocol}.
    
    Suppose for the sake of contradiction, that $\exists$ a pair of messages $m_0,m_1$, a malicious receiver $\malrecv(\brho)$, a distinguisher $\maldist(\bsigma)$ s.t. $\maldist(\bsigma,\cdot)$ distguishes between the outputs of $Hyb_6$ and $Hyb_7$. Labelling the outputs of $Hyb_6$ by $\outsendr,\outmalrecv$ and output of $Hyb_7$ by $\outsendr',\outmalrecv'$, we have $|Pr[\maldist(\bsigma, \outsendr, \outmalrecv)=1] - Pr[\maldist(\bsigma, \outsendr', \outmalrecv')=1]| = \epsilon$, where $\epsilon$ is the non-negligible advantage of $\maldist$ in distinguishing $Hyb_6$ and $Hyb_7$.
    
    Next, we construct a one-way to hiding adversary $\owhadv$. At a high level, $\owhadv$ will run a particular part of $\malrecv$ - one which is supposed to take in the last message from the sender and output the final state. More concretely, $\owhadv$ takes as input a state $\outmalrecv^{temp}$, string $s \in \zo^\secp$, two messages $msg_0,msg_1 \in \zo^\secp$, the (possibly quantum) descriptions required to simulate oracles $\comro,\fsro$ \nishant{the exRO description is indeed quantum actually and might have been disturbed in extracting} and the advice string for $\maldist$ - $\bsigma$. In addition, $\owhadv$ is given oracle access to one of two oracles - $O_1$ or $O_2$, where $O_1(\cdot) = \maskro(\cdot)$ and $O_2(\cdot) = O_1(\cdot)$, except that $O_2(x')$ is redefined to be a fresh random value, where $x' = s||\{x_i\}_{i \in I_{1-b}}$. Note that here the differing point $x'$ is defined only once $x_i$ and $I_{1-b}$ get defined. Indeed, the run of $\owhadv$ only makes sense once a sender has completed execution till before sending the last message to $\malrecv(\brho)$. 
    
    $\owhadv^O(\outmalrecv^{temp},s,msg_0,msg_1,\comro,\fsro,\bsigma)$ starts $\malrecv$ in state $\outmalrecv^{temp}$ \nishant{describe in the quantum ITM model?} and sends it $s,msg_0,msg_1$, while answering its oracle queries as follows : it answers the queries to $\comro,\fsro$ by using the (possibly quantum) descriptions provided to it as part of its input. For answering queries to $\maskro$, it uses the oracle $O$ to which it is given oracle access. Finally, once $\malrecv$ finishes execution and outputs state $\outmalrecv$, it outputs $\maldist(\bsigma,\outsendr,\outmalrecv)$, where $\outsendr=\mathsf{end}$ representing the output of an honest sender as in $Hyb_6$ or $Hyb_7$. \nishant{fix the input to D in an earlier place as well + we need O2H which works with mixed state as well + can we solve this problem by having a new interactive O2H theorem?}
    
    At a later point in the proof, we will invoke the O2H theorem from \cite{ambainis2019quantum} with $\owhadv$ as the O2H adversary. Correspodingly then, we have the quantum algorithm $\owhadvb^O$ which takes in the same inputs as $\owhadv$, and chooses some $i \gets [q_M]$, where $q_M$ is the number of oracle queries made by $\owhadv$ (and hence by the part of $\malrecv$ which runs after the last message from sender), runs $\owhadv$ till the $i^{th}$ query, then measures the input query registers till that point in the computational bases and outputs that as set $T$.
    
    We will now use the quantum algorithm $\owhadvb$ to do a reduction to EPR protocol from \sectionref{subsec:epr-protocol}. Our reduction algorithm $\cR$ acts as the receiver $B$ in the EPR protocol from \proref{subsec:epr-protocol} and interacts with $\malrecv,\owhadvb$ to break the protocol.
    
    \begin{enumerate}
        \item \label{itm:reduction-sample-s}
        $\cR$ initializes $\malrecv(\brho)$ and starts interacting with the EPR sender $A$, while forwarding messages to $\malrecv$. It answers the oracle queries to $\malrecv$ in the same way as done by $S$ in $Hyb_6$, i.e. it answers queries to $\comro,\fsro$ using $\simuextrac.RO$ and a hash function chosen from $2q$-wise independent hash family. And it answers quries of $\malrecv$ to $\maskro$, by first sampling string $s \gets \zo^\secp$, and using the oracle $\maskrop$, where $\maskrop$ is as defined in $Hyb_6$.
        
        \item When $\cR$ gets $m=16\secp$ halves of EPR pairs from $A$, it forwards the same to $\malrecv$. 
        
        \item \label{itm:epr-reduction-m-and-r}
        $\cR$ now applies the measure-and-reprogram strategy~\cite{don2019security} to reprogram the RO $\fsro$. More concretely, it samples $i \gets [q'_{FS}+1]$, where $q'_{FS}$ is the total number of queries made by $\malrecv$ from after receiving the halves of the EPR pairs to before returning the measurement check proof. \nishant{is bound on the \#queries really sufficient? reservoir sampling doesn't work ; same problem in classical case as well? + this needs more careful analysis for the q+1 in m\&r result}. It then answers queries to $\fsro$ for $\malrecv$, except on the turn of the $i^{th}$ query, it measures the query in the computational bases to get some string $c$. It parses $c$ as $c_1||c_2|| \ldots c_{16\secp}$, where $\forall i, |c_i| = |\comro(x)|$. It uses $\simuextrac$ to get $\widehat{x_i}||\widehat{\theta_i}||\widehat{r_i} = \simuextrac.E(c_i), \forall i \in [16\secp]$. It passes $\widehat{x_i},\widehat{\theta_i}$ to the EPR sender $A$ and gets back the challenge set $T$ in return, which it uses to reprogram $\fsro(c) = T$. Call this new oracle $\fsror$. It answers the current $i^{th}$ query with either $\fsro(c)$ or $\fsror(c)$, with the choice being made at random, and answers the remaining queries to $\fsro$ by $\malrecv$ using $\fsror$. \nishant{IMP: IMP: IMP: does this really work? can the quantum predicate in m\&r depend on H as well? why did they have q+1 then?}
        
        \item Subsequently, $\malrecv$ returns the measurement check proof $\pi = (\{c_i'\}_{i \in [16\secp]}, Y', \{\widehat{x_i}', \widehat{\theta_i}', \widehat{r_i}' \}_{i \in T})$, at which point $\cR$ checks if $\forall i \in [16\secp], c_i'=c_i$, in addition to performing all the checks by the sender in \prostepref{itm:qot-sendr-check} of \proref{fig:qot-5r-construction}. If all checks pass, $\cR$ sends continue to EPR sender $A$, else sends abort to $A$ and aborts.
        
        \item Thereafter, $\cR$ receives $\{\theta_i\}_{i \in T}$ from $A$ and forwards the same to $\malrecv$. 
        
        \item $\malrecv$ in turns replies back with $(I_0,I_1)$, which $\cR$ forwards the same to $A$. Suppose the state of $\malrecv$ at this point is $\outmalrecv^{temp}$.
        
        \item Finally, $A$ sends $(h,x')$ to $\cR$. $\cR$ samples a fresh random oracle $O$ (using a $2q$-wise independent hash function) and sets $\maskro(s||\cdot)=O(\cdot), \maskro(x) = \maskrop(x)$ otherwise (this can again be done with a circuit wrapper over $\maskrop$). Next, it finds the set of indices $P$ in $I_0$ where $\theta_i \neq \widehat{\theta}_i$ and if $|P|>3\secp/2$, sets $b=1$, else sets $b=0$. Finally, it retrieves the string s (prepared in Step~\ref{itm:reduction-sample-s}), the strings $m_0,m_1$ for which $\maldist$ had worked, sets $msg_b = m_b \oplus \maskro(s||x'), msb_{1-b} = m_{1-b} \oplus r$, where $r$ is a freshly drawn random value. It then runs $\owhadvb$ to get $x''$, i.e. $x'' \gets \owhadvb^{\maskro}(\outmalrecv^{temp},s,msg_0,msg_1,\comro,\fsro,\bsigma)$~\footnote{Here by $\comro$ and $\fsro$, we mean the corresponding (possibly quantum) description $\cR$ was using to simulate the same.}, parses $x''$ as $s||x'''$ (abort if this is not so parseable) and outputs $h(x''')$.
        
    \end{enumerate}
    
    \begin{claim}
        The string output by $\cR = h(\{x_i\}_{i \in I_{1-b}})$ with non-negl probability, hence contradicting~\cref{lemma:epr-guarantee}. \nishant{change to cref at all places}
    \end{claim}
    \begin{proof}
        We first show that $\exists$ quantum algorithm $\cR'$ which can simulate either of $Hyb_6$ or $Hyb_7$ for $\maldist$, which would imply that $\owhadv$ (which runs $\maldist$ inside) distinguishes between the two oracles to which it is given access to ($O_1/O_2$) with a non-negl probability. 
        
        $\cR'$ works exactly as the sender $S$ in $Hyb_6$, initializing $\malrecv(\brho)$, simulating oracles $\comro,\fsro$ (using $\simuextrac.RO$ and a hash function from a $2q$-wise independent hash family as done by $S$ in $Hyb_6$) and answering oracle calls to $\maskro$ using $\maskrop$ (to define which it first chooses $s \gets \zo^\secp$ and thereafter defines it as in $Hyb_6$). It runs $\malrecv$ till before sending the last message to it, at which point it calls $\owhadv$ passing it the approprimate inputs and giving it oracle access to one of two oracles - $O_1(\cdot) = \maskro(\cdot)$ or $O_2(\cdot) = O_1(\cdot)$ except $O_2(x')$ is programmed to a fresh random value, where $x' = s||\{x_i\}_{i \in I_{1-b}}$. Thereafter $\cR'$ outputs whatever $\owhadv$ outputs. 
        
        Note that here when $\cR'$ gives $\owhadv$ access to $O_1$, it exactly simulates $Hyb_6$ for the underlying $\maldist$, and when it gives access to $O_2$, it exactly simulates $Hyb_7$ for $\maldist$. Since by assumption, $\maldist$ distinguishes between $Hyb_6$ and $Hyb_7$ with non-negl probability $\epsilon$, therefore $\owhadv$ distinguishes between the oracles $O_1/O_2$ with same non-negl probability $\epsilon$.
        
        Invoking the O2H lemma from~\cite{ambainis2019quantum}, we then have that $\owhadvb^{O_2}$ outputs $x'$ with probability $\geq \frac{\epsilon}{4q_{\cA}}$, where $q_{\cA}$ is the number of oracle queries made by $\owhadv$. \nishant{TODO : making the non-trivial jump of passing in mixed state to $\owhadv$ + $\owhadvb$ is given access to $O_2$} In other words, this means that we need to only simulate $Hyb_7$ for $\owhadvb$ (since by giving access to $O_2$, we are doing exactly that) and it can output the point $x'=s||\{x_i\}_{i \in I_{1-b}}$ with non-negl probability.
        
        Note that our EPR reduction algorithm $\cR$ runs exactly $\owhadvb^{O_2}$ (barring the difference due to measuring and programming the RO). To see further from here, note that performing the measure and reprogram step in Step~\ref{itm:epr-reduction-m-and-r} by $\cR$ only changes $\owhadvb$'s behaviour by a factor of $O(q_{FS}'^2)$~\cite{don2019security} (since all the checks performed by $\cR$ after Step~\ref{itm:epr-reduction-m-and-r} can be captured a quantum predicate). Otherwise the actions of $\cR$ is identical to one of $\cR'$ above, which means $\owhadvb$ succeeds in outputting $x'$ with probability $\geq \frac{\epsilon}{4q_{\cA}O(q_{FS}'^2)}$, which is still non-negligible. \nishant{TODO: this whole part of reduction to measure and reprogram needs to be done more properly} 
    \end{proof}
    
    
    \item $Hyb_7 \rightarrow Hyb_8$: The thing which changes between $Hyb_7$ and $Hyb_8$ is that $S$ sets $m_{1-b}=0^\secp$ in $Hyb_8$ rather than like an honest sender in $Hyb_7$. It suffices then to argue that the mask used while sending $m_{1-b}$ from the point of view of $\malrecv$ is a uniformly random mask, which would ensure that $\malrecv$ doesn't notice the difference between sending the actual $m_{1-b}$ and $0^\secp$. In either of the hybrids, the mask used while sending $m_{1-b}$ is $\maskro(s||\{x_i\}_{i \in I_{1-b}})$. Lets call $x'=s||\{x_i\}_{i \in I_{1-b}}$, which would mean the mask used is $\maskro(x')$. But notice that before sending the last message, any queries to $\maskro$ were answered by $S$ with $\maskrop$ which at the point $x'$ evaluated to $\maskrop(x') = \maskrop(s||\{x_i\}_{i \in I_{1-b}}) = \bot$. Also, after sending the last message, any queries to $\maskro$ were answered by $S$ using $\maskror$, which was reprogrammed at $x'$ before sending the last message so that $\maskror(x')$ was a fresh random value. Hence, the mask used in sending the message $m_{1-b}$ to $\malrecv = \maskro(x')$ is not used anywhere else in the protocol and hence looks uniformly drawn fresh random value from the point of view of $\malrecv$.
    
    \item $Hyb_8 \rightarrow Hyb_9$: The only difference in $Hyb_9$ compared to $Hyb_8$ is that instead of choosing $m_b$ itself as an honest sender, $\simurecv$ sends $b$ to $\fot$ to get back $m_b$. Hence, $Hyb_8 \equiv Hyb_9$.
    
\end{itemize}

==> re-programming.tex <==
\section{The random oracle extractor}

\iffalse
\subsection{Two-round sketch}

Below is a simple two-round random bit OT protocol that I think we can prove secure, along with a sketch of the proof.

\begin{itemize}
    \item Sender: 
    \begin{itemize}
        \item Prepare $2\secp$ EPR pairs, and send one half of each to the receiver.
    \end{itemize}
    \item Receiver (with input $b \in \{0,1\}$):
    \begin{itemize}
        \item Sample $\Theta_1,\dots,\Theta_\secp \gets \{0,1\}$.
        \item Split the $2\secp$ qubits received from the sender into $\secp$ pairs, and measure each pair $i$ in the computational basis if $\Theta_i = 0$ and in the Hadamard basis if $\Theta_i = 1$. Let $a_{1,0},a_{1,1},\dots,a_{\secp,0},a_{\secp,1}$ be the results.
        \item Prepare commitments $\Com(\Theta_1,a_{1,0},a_{1,1}),\dots,\Com(\Theta_\secp,a_{\secp,0},a_{\secp,1})$, query the random oracle to receive $T \subset [\secp]$ of size $\secp / 2$, and open the corresponding set of commitments.
        \item Send the commitments, the openings, and $\{c_i \coloneqq b \oplus \Theta_i\}_{i \in \overline{T}}$ to the sender. Output \[\left(b,m_b \coloneqq \bigoplus_{i \in \overline{T}}a_{i,b}\right).\]
    \end{itemize}    
    \item Sender: 
    \begin{itemize}
        \item Measure each pair $\{i\}_{i \in T}$ in the basis indicated by the commitment openings, and abort if any results don't match the commitment openings.
        \item Measure each pair $\{i\}_{i \in \overline{T}}$ in $(C,H)$ if $c_i = 0$ and in $(H,C)$ if $c_i=1$. Let $a'_{1,0},a'_{1,1},\dots,a'_{\secp,0},a'_{\secp,1}$ be the results. \item Output \[\left(m_0 \coloneqq \bigoplus_{i \in \overline{T}} a'_{i,0},m_1 \coloneqq \bigoplus_{i \in \overline{T}} a'_{i,1}\right).\]
    \end{itemize}  
\end{itemize}

\paragraph{Security against malicious receiver.}

\begin{itemize}
    \item Assume for now that the commitments are perfectly extractable, so that we can replace the commitments with the committed values themselves everywhere in the proof. 
    \item Given a sequence of bases $\Theta = \Theta_1,\dots,\Theta_n$, bits $b = b_1,\dots,b_n$, a subset $T \subset [n]$, and a constant $\delta > 0$, define the projection \[\Pi_{\Theta,b,T,\delta} = \sum_{c \in \{0,1\}^n: c_T = b_T, \cH\cW(c_{\overline{T}} \oplus b_{\overline{T}}) > \delta|\overline{T}|} \ket{c^\Theta}\bra{c^\Theta}.\] 
    \item Consider the joint state of the system right after the receiver sends its message, on register $\cR$ holding the receiver's private state, $\cZ$ holding the receiver's classical message $z$, and $\cS$ holding the sender's state. From message $z$, we can define a string of bases $\Theta_z = (\Theta_1,\Theta_1,\dots,\Theta_\secp,\Theta_\secp)$, a string of bits $a_z = (a_{1,0},a_{1,1},\dots,a_{\secp,0},a_{\secp,1})$, and $T_z \subset [2\secp]$. Consider the projection \[\Pi_\mathsf{Bad} = \sum_z \ket{z}\bra{z} \otimes \Pi_{\Theta_z,a_z,T_z,1/4}\] on registers $\cZ,\cS$.
    \item It follows from measure-and-reprogram that the probability $\Pi_\mathsf{Bad}$ accepts when $T$ is sampled uniformly at random after $a$ is determined is at most a polynomial factor higher than the probability it accept on $\cZ,\cS$ in the real game. Then, by BF10, this probability is negligible.
    \item Thus, by gentle measurement, we can project $\cZ,\cS$ onto $\bbI - \Pi_{\mathsf{bad}}$ with at most a negligible loss in trace distance. \item Now, the distinguisher gets $(\cR,\cZ)$ and a register $\cM$ that holds the result of applying the appropriate measurement to $\cS$, returning either $\bot$ or $(m_0,m_1)$. We can define the receiver's choice bit $b^*$ based on $\Theta$ and $a$, and argue that $m_{b^*}$ can be replaced with a uniformly random bit $r$, by the XOR extractor lemma below, and the fact that the state on $\cS$ is in the image of $\bbI-\Pi_{\mathsf{bad}}$.
\end{itemize}

\subsection{XOR extractor} \james{moved to prelims}



\subsection{Random oracle extractor}
\fi

In this section, we prove the following theorem.

\begin{theorem}
Let $H : \{0,1\}^n \to \{0,1\}^m$ be a random oracle. Consider a two-stage adversary $A_1^H, A_2^H$ that combined makes at most $q$ calls to $H$. Suppose that $A_1^H$ outputs a quantum state $\ket{\gamma}_{\cA,\cX}$ and classical strings $(T,\{x_i\}_{i \in T})$, where $T \subseteq [n]$, each $x_i \in \{0,1\}$, $\cA$ is a register of arbitary size, and $\cX$ is a register on $k = n-|T|$ qubits. Let $L$ be the smallest set of $k$-bit binary strings such that \[\ket{\gamma} = \sum_{u \in L}\ket{\psi_u}_\cA \otimes \ket{u}_\cX.\] Now consider the following two games.
\begin{itemize}
    \item $\mathsf{REAL}$: 
    \begin{itemize}
        \item $A_1^H$ outputs $\ket{\gamma}_{\cA,\cX},T,\{x_i\}_{i \in T}$.
        \item $\cX$ is measured in the Hadamard basis to produce a $k$-bit string, which is parsed as $\{x_i\}_{i \in \overline{T}}$. Define $x = (x_1,\dots,x_n)$.
        \item $A_2^H$ is given $\Tr_\cX(\ket{\gamma}\bra{\gamma}), T, \{x_i\}_{i \in T}, H(x)$, and outputs a bit.
    \end{itemize}
    \item $\mathsf{IDEAL}$: 
    \begin{itemize}
        \item $A_1^H$ outputs $\ket{\gamma}_{\cA,\cX},T,\{x_i\}_{i \in T}$.
        \item $r \gets \{0,1\}^m$.
        \item $A_2^H$ is given $\Tr_\cX(\ket{\gamma}\bra{\gamma}), T, \{x_i\}_{i \in T}, r$, and outputs a bit.
    \end{itemize}
\end{itemize}
Then, \[\left|\Pr[\mathsf{REAL} = 1] - \Pr[\mathsf{IDEAL} = 1]\right| \leq \frac{3\sqrt{2}\sqrt{q}|L| + 2q\sqrt{|L|}}{2^{k/2}} = \frac{O(q|L|)}{2^{k/2}}.\]
\end{theorem}

\begin{proof}

Consider the following hybrid game.
\begin{itemize}
    \item $\mathsf{HYBRID}$: 
    \begin{itemize}
        \item $A_1^H$ outputs $\ket{\gamma}_{\cA,\cX},T,\{x_i\}_{i \in T}$.
        \item $\cX$ is measured in the Hadamard basis to produce a $k$-bit string, which is parsed as $\{x_i\}_{i \in \overline{T}}$. Define $x = (x_1,\dots,x_n)$. Sample $r \gets \{0,1\}^m$, and re-program $H(x)$ to $r$.
        \item $A_2^H$ is given $\Tr_\cX(\ket{\gamma}\bra{\gamma}), T, \{x_i\}_{i \in T}, r$, and outputs a bit.
    \end{itemize}
\end{itemize}

\begin{claim}
\[|\Pr[\mathsf{REAL} = 1] - \Pr[\mathsf{HYBRID} = 1]| \leq \frac{3\sqrt{2}\sqrt{q}|L|}{2^{k/2}}.\]
\end{claim}

\begin{proof}
This follows from the adaptive reprogrammming lemma (\cref{lemma:adaptive-reprogramming}), along with the imported lemma (\cite[Lemma 2]{EC:AMRS20}, \cite[Lemma 1]{10.1007/978-3-030-92062-3_22}) establishing the structure of an adversary / random oracle state after at most $q$ queries.
\end{proof}

\begin{claim}
\[|\Pr[\mathsf{HYBRID} = 1] - \Pr[\mathsf{IDEAL} = 1]| \leq \frac{2q\sqrt{|L|}}{2^{k/2}}.\]
\end{claim}

\begin{proof}
This follows from an invocation of \cref{impthm:ow2h}. Consider the distribution over $(S,O_1,O_2,\ket{\psi})$ that results from the following. 
\begin{itemize}
    \item Sample $O_1$ as a random oracle $H$,
    \item run $A_1^H$ to obtain $\ket{\gamma}_{\cA,\cX},T,\{x_i\}_{i \in T}$,
    \item measure to obtain $x$ as in the $\mathsf{HYBRID}$ game and set $S = \{x\}$, 
    \item sample $r \gets \{0,1\}^m$, and let $O_2$ be the same as $O_1$, except that $O_2(x) = r$,
    \item and let $\ket{\psi}$ be the resulting state on register $\cA$ along with the classical strings $T,\{x_i\}_{i \in T},r$.
\end{itemize}

Then, $\Pr[\mathsf{IDEAL} = 1] = P_{\text{left}}$ and $\Pr[\mathsf{HYBRID} = 1] = P_{\text{right}}$, so it suffices to bound $P_{\text{guess}}$. However, $P_{\text{guess}}$ is upper bounded by $1/2^{\mathbf{H}_\infty}$, where $\mathbf{H}_\infty$ is the quantum conditional min-entropy of $x$ given $\Tr_\cX(\ket{\gamma}\bra{\gamma})$. By \cref{impthm:small-superposition}, and the fact that measuring an unentangled $k$-bit standard basis vector in the Hadamard basis gives $k$ bits of quantum conditional min-entropy, $P_\text{guess}$ is upper bounded by $\frac{|L|}{2^{k}}$. Thus, \cref{impthm:ow2h} gives the final bound of $\frac{2q\sqrt{|L|}}{2^{k/2}}$.

\end{proof}


\end{proof}

\iffalse
\noindent\paragraph{Setup.} Consider a state $\ket{\gamma}_{\cA,\cF,\cX}$ initially on three registers, $\cA$ for the adversary, $\cF$ for the random oracle (written in purified form), and $\cX$. The parts of the state on $\cF$ and $\cX$ satisfy some special properties: $\cF$ is the result of interacting with the QROM with at most $q$ queries, and $\cX$ is in a superposition of a small number of terms in the computational basis. Say that $\cX$ is measured in the Hadamard basis to produce $x$, and then $x$ is queried to the random oracle to obtain $y$, which is placed in register $\cY$. This produces a mixed state $\rho_{\cA,\cF,\cX,\cY}$. Ultimately, we want to prove the following claim:

\[\TD\left(\Tr_\cX(\rho),\Tr_{\cX,\cY}(\rho) \otimes \frac{1}{2^n}\sum_{y}\ket{y}\bra{y}^{\nishant{\cY}}\right) = \negl(n).\]

\nishant{$n$ not defined yet? + small question to ask} \james{yeah $n$ is just defined to be the size of the output of the random oracle, actually this should be $m$ to be consistent with what is below} Below, we show a different claim, which establishes at least that $y=H(x)$ is close to uniformly random from the adversary's perspective. In particular, we show that 

\[\TD\left(\rho,\rho^{\cF:x \to r}\right) = \negl(n),\]

where $\rho^{\cF:x \to r}$ indicates that $\cF$ has been re-rogrammed to uniformly random at index $x$, right after $\cX$ was measured to obtain $x$, but right before $y = H(x)$ was written to $\cY$. 
\fi


\noindent\paragraph{The adaptive re-programming claim.} In this section, we prove the following lemma.

\begin{lemma}\label{lemma:adaptive-reprogramming}
Let $\cF$ be a $(m \cdot 2^n)$-qubit register split into $2^n$ sub-registers $\{\cF_x\}_{x \in \{0,1\}^n}$ of size $m$. Let $\cA$ be an arbitrary register and $\cX$ be an $n$-qubit register. Consider any state $\ket{\gamma}_{\cF,\cA,\cX}$, set $L \subseteq \{0,1\}^n$, and integer $q \in \bbN$, such that $\ket{\gamma}$ can be written as 

\[\ket{\gamma} = \sum_{u \in L} a_u\ket{\psi_u}_{\cF,\cA} \otimes \ket{u}_\cX,\]

where each $a_u \in \bbR$, and each $\ket{\psi_u}$ is a unit vector such that 

\[\ket{\psi_u} = \sum_{S \subset \{0,1\}^n : |S| \leq q} \ket{\psi_{u,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}},\] where $\ket{\phi_0}_{\cF_x}$ is orthogonal to $\ket{\psi_{u,S}}$ for all $x \in S$.

Suppose that $\cX$ is measured in the Hadamard basis to produce $x \in \{0,1\}^n$. Then \[\TD\left(\Tr_{\cX}\left(\ket{\gamma}\bra{\gamma}\right) \otimes \ket{x}\bra{x}, \Tr_{\cX,\cF_x}\left(\ket{\gamma}\bra{\gamma}\right) \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x} \otimes \ket{x}\bra{x}\right) \leq \frac{3\sqrt{2q}|L|}{2^{n/2}}.\]

\end{lemma}



 %Let $L \subset \{0,1\}^n$ be such that $\frac{|L|}{2^{n/2}} = \negl(n)$, and $q = \poly(n)$. Consider any state \[\ket{\gamma} = \sum_{u \in L} \ket{\widehat{\psi}_u}_{\cF,\cA} \otimes \ket{u}_\cX\] where $\ket{\psi_u} \coloneqq \frac{\ket{\widehat{\psi}_u}}{\|\ket{\widehat{\psi}_u}\|}$ is such that \[\ket{\psi_u} = \sum_{S \subset \{0,1\}^n : |S| \leq q} \ket{\psi_{u,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}},\] and $\ket{\phi_0}_{\cF_x}$ is orthogonal to $\ket{\psi_{u,S}}$ for all $x \in S$. 

\begin{proof}
 
Consider apply Hadamard to register $\cX$ of $\ket{\gamma}$, producing

\[\sum_{u \in L, x \in \{0,1\}^\ell}\frac{(-1)^{u \cdot x}a_u}{2^{\ell/2}}\ket{\psi_u}_{\cF,\cA} \otimes \ket{x}_{\cX} \coloneqq \sum_{x \in \{0,1\}^\ell}\ket{\chi_x}_{\cF,\cA} \otimes \ket{x}_{\cX}\] and then measuring in the computational basis to produce $x$ and left-over state \[\sum_{x \in \{0,1\}^n}\ket{\chi_x}\bra{\chi_x}_{\cF,\cA}.\]

The lemma asks to bound the following quantity.


%\[\sum_{x \in \{0,1\}^n}\Tr_{\cF_{x}}[\ket{\chi_x}\bra{\chi_x}_{\cF,\cA}] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_{x}}.\]
%We also want to allow the adversary access to $x$. Thus, the distinguishing advantage corresponds to the quantity  


\begin{align*}
&\Bigg\|\sum_{x \in \{0,1\}^n}\ket{\chi_x}\bra{\chi_x}_{\cF,\cA} \otimes \ket{x}\bra{x} - \sum_{x \in \{0,1\}^n}\Tr_{\cF_{x}}[\ket{\chi_x}\bra{\chi_x}_{\cF,\cA}] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_{x}} \otimes \ket{x}\bra{x} \Bigg\|_1 \\
&= \Bigg\|\frac{1}{2^n}\sum_{x \in \{0,1\}^n}\sum_{u_1,u_2 \in L}(-1)^{(u_1 \oplus u_2) \cdot x}a_{u_1}a_{u_2}\ket{\psi_{u_1}}\bra{\psi_{u_2}} \otimes \ket{x}\bra{x} \\ 
&\ \ \ - \frac{1}{2^n}\sum_{x \in \{0,1\}^n}\Tr_{\cF_x}\left[\sum_{u_1,u_2 \in L}(-1)^{(u_1 \oplus u_2) \cdot x}a_{u_1}a_{u_2}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x} \otimes \ket{x}\bra{x}\Bigg\|_1 \\ 
&\leq \frac{1}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\left\|\sum_{x \in \{0,1\}^n}\left(\ket{\psi_{u_1}}\bra{\psi_{u_2}} - \Tr_{\cF_x}\left[\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right]\otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\right) \otimes \ket{x}\bra{x}\right\|_1 \\ 
&\leq \frac{1}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sum_{x \in \{0,1\}^n}\left\|\left(\ket{\psi_{u_1}}\bra{\psi_{u_2}} - \Tr_{\cF_x}\left[\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right]\otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\right) \otimes \ket{x}\bra{x}\right\|_1 \\ &= \frac{1}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sum_{x \in \{0,1\}^n}\left\|\ket{\psi_{u_1}}\bra{\psi_{u_2}} - \Tr_{\cF_x}\left[\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right]\otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\right\|_1,\end{align*}

where the inequalities use the linearity of partial trace and the homogeneity and triangle inequality of the trace norm.

Following \cite{10.1007/978-3-030-92062-3_22}, for any $u_1,u_2,$ and $x$, we can write \begin{align*}\ket{\psi_{u_1}}\bra{\psi_{u_2}} = &\bra{\phi_0}_{\cF_x}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{\phi_0}_{\cF_x} \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x} + \ket{\psi_{u_1}}\bra{\psi_{u_2}}(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\\ &+ (\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{\phi_0}\bra{\phi_0}_{\cF_x}\end{align*} and 
\begin{align*}
    \Tr_{\cF_x}\left[\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right]\otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x} = &\bra{\phi_0}_{\cF_x}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{\phi_0}_{\cF_x} \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\\ &+ \Tr_{\cF_x}\left[(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}
\end{align*}
so
\begin{align*}
    &\left\|\ket{\psi_{u_1}}\bra{\psi_{u_2}} - \Tr_{\cF_x}\left[\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right]\otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\right\|_1 \leq \|\ket{\psi_{u_1}}\bra{\psi_{u_2}}(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\|_1 \\ &+ \|(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{\phi_0}\bra{\phi_0}_{\cF_x}\|_1 + \|\Tr_{\cF_x}\left[(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\|_1.
\end{align*}

Now, let $\{\ket{i}\}_i$ be an orthonormal basis of $\cF_x$ that includes $\ket{\phi_0}$. Define $\alpha_{x,u,i} = \|\bra{i}_{\cF_x}\ket{\psi_{u}}\|$, and note that $\sum_i \alpha_{x,u,i}^2 = 1$. The first term above simplifies as 
\begin{align*}
    \|\ket{\psi_{u_1}}\bra{\psi_{u_2}}(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\|_1 = \|\bra{\psi_{u_2}}(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\| = \sqrt{1-\bra{\psi_{u_2}}\ket{\phi_0}\bra{\phi_0}\ket{\psi_{u_2}}} = \sqrt{1-\alpha_{x,u_2,
    \phi_0}^2}.
\end{align*}

The second term above simplifies as 

\begin{align*}
    &\|(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{\phi_0}\bra{\phi_0}_{\cF_x}\|_1 \leq \|(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\|_1 \\ &= \|(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\| = \sqrt{1-\bra{\psi_{u_1}}\ket{\phi_0}\bra{\phi_0}\ket{\psi_{u_1}}} = \sqrt{1-\alpha_{x,u_1,\phi_0}^2}.
\end{align*}

The third term above simplifies as 
\begin{align*}
    &\|\Tr_{\cF_x}\left[(\bbI - \ket{\phi_0}\bra{\phi_0}_{\cF_x})\ket{\psi_{u_1}}\bra{\psi_{u_2}}\right] \otimes \ket{\phi_0}\bra{\phi_0}_{\cF_x}\|_1 \\ &= \|\sum_{i}\bra{i}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{i} - \bra{i}\ket{\phi_0}\bra{\phi_0}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{i} \otimes \ket{\phi_0}\bra{\phi_0}\|_1 \\ &= \sum_{i \neq \phi_0} \|\bra{i}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{i}\|_1 \\ &= \sum_{i \neq \phi_0}\Tr\sqrt{\bra{i}\ket{\psi_{u_2}}\bra{\psi_{u_1}}\ket{i}\bra{i}\ket{\psi_{u_1}}\bra{\psi_{u_2}}\ket{i}} \\ &= \sum_{i \neq \phi_0} \alpha_{x,u_1,i}\Tr\sqrt{\bra{i}\ket{\psi_{u_2}}\bra{\psi_{u_2}}\ket{i}} \\ &= \sum_{i \neq \phi_0} \alpha_{x,u_1,i}\alpha_{x,u_2,i} \\ &= \sqrt{\sum_{i,j \neq \phi_0}\alpha_{x,u_1,i}^2\alpha_{x,u_2,j}^2} \\ &\leq \sqrt{1-\alpha_{x,u_1,\phi_0}^2\alpha^2_{x,u_2,\phi_0}}.
\end{align*}

Thus, the distinguishing advantage can be bounded by 

\begin{align*}
    &\frac{1}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sum_{x \in \{0,1\}^n}\sqrt{1-\alpha^2_{x,u_1,\phi_0}} + \sqrt{1-\alpha^2_{x,u_2,\phi_0}} + \sqrt{1-\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0}} \\ &\leq \frac{3}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sum_{x \in \{0,1\}^n}\sqrt{1-\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0}}
    \\ &\leq \frac{3}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sqrt{2^n\left(2^n - \sum_{x \in \{0,1\}^n}\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0}\right)},
\end{align*}
    
    %\\ &\leq \frac{3M}{2^\ell}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sqrt{2^n\left(2^n - \sum_{y \in \{0,1\}^n}\alpha^2_{y,u_1,\phi_0}\alpha^2_{y,u_2,\phi_0}\right)}.
    
    
    %&\leq \frac{1}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\left[\sqrt{2^n\left(2^n - \sum_{x \in \{0,1\}^n}\alpha^2_{x,u_1,\phi_0}\right)} + \sqrt{2^n\left(2^n - \sum_{x \in \{0,1\}^n}\alpha^2_{x,u_2,\phi_0}\right)} + \sqrt{2^n\left(2^n - \sum_{x \in \{0,1\}^n}\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0}\right)}\right]


where the second inequality is due to Cauchy-Schwartz. 

%Note that the third term in the summation is at least as large as the first two, so we can simplify to 

%\begin{align*}
    %\frac{3}{2^n}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2}\sqrt{2^n\left(2^n - \sum_{x \in \{0,1\}^n}\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0}\right)}.
%\end{align*}

Now, for any $u_1,u_2$,

\begin{align*}
    &\sum_{x \in \{0,1\}^n}\alpha^2_{x,u_1,\phi_0}\alpha^2_{x,u_2,\phi_0} \\ &= \sum_{x \in \{0,1\}^n} \| \bra{\phi_0}_{\cF_x}\ket{\psi_{u_1}}\|^2 \| \bra{\phi_0}_{\cF_x}\ket{\psi_{u_2}}\|^2 \\ &= \sum_{x \in \{0,1\}^n}\bigg\|\sum_{S \subset \{0,1\}^n : |S| \leq q} \bra{\phi_0}_{\cF_x}\ket{\psi_{u_1,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2\bigg\|\sum_{S \subset \{0,1\}^n : |S| \leq q} \bra{\phi_0}_{\cF_x}\ket{\psi_{u_2,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2 \\ &= \sum_{x \in \{0,1\}^n}\bigg\|\sum_{S \not\owns x} \ket{\psi_{u_1,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2\bigg\|\sum_{S \not\owns x} \ket{\psi_{u_2,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2,
\end{align*}

where the last equality follows since $\ket{\phi_0}_{\cF_x}$ is orthogonal to $\ket{\psi_{u,S}}$ for all $x \in S$, and $\ket{\phi_0}$ is normalized. Now, since each of the summands is pairwise orthogonal, we can write
    
    
\begin{align*} 
    &\sum_{x \in \{0,1\}^n}\bigg\|\sum_{S \not\owns x} \ket{\psi_{u_1,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2\bigg\|\sum_{S \not\owns x} \ket{\psi_{u_2,S}}_{\cA,\cF_S} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2
    \\ &= \sum_{S_1,S_2}\sum_{x \notin (S_1 \cup S_2)}\bigg\|\ket{\psi_{u_1,S_1}}_{\cA,\cF_{S_1}} \otimes \left(\ket{\phi_0}^{(2^n-|S_1|)}\right)_{\cF_{\overline{S_1}}}\bigg\|^2\bigg\|\ket{\psi_{u_2,S_2}}_{\cA,\cF_{S_2}} \otimes \left(\ket{\phi_0}^{(2^n-|S_2|)}\right)_{\cF_{\overline{S_2}}}\bigg\|^2 \\ &\geq (2^n-2q)\sum_{S_1,S_2}\bigg\|\ket{\psi_{u_1,S_1}}_{\cA,\cF_{S_1}} \otimes \left(\ket{\phi_0}^{(2^n-|S_1|)}\right)_{\cF_{\overline{S_1}}}\bigg\|^2\bigg\|\ket{\psi_{u_2,S_2}}_{\cA,\cF_{S_2}} \otimes \left(\ket{\phi_0}^{(2^n-|S_2|)}\right)_{\cF_{\overline{S_2}}}\bigg\|^2 \\ &= (2^n-2q)\bigg\|\sum_S \ket{\psi_{u_1,S}}_{\cA,\cF_{S}} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2\bigg\|\sum_S \ket{\psi_{u_2,S}}_{\cA,\cF_{S}} \otimes \left(\ket{\phi_0}^{(2^n-|S|)}\right)_{\cF_{\overline{S}}}\bigg\|^2 \\ &= (2^n - 2q)\|\ket{\psi_{u_1}}\|^2\|\ket{\psi_{u_2}}\|^2 \\ &= 2^n - 2q.
\end{align*}

Thus, the distinguishing advantage can be bounded by

\begin{align*}
    \frac{3}{2^n}\sqrt{2^n \cdot 2q}\sum_{u_1,u_2 \in L}a_{u_1}a_{u_2} \leq \frac{3\sqrt{2q}|L|}{2^{n/2}},
\end{align*}

by Cauchy-Schwartz.

\end{proof}



==> rom-commitments.tex <==
\section{Equivocal and extractable commitments in the QROM}
\label{sec:eecom}

In this section, we define and construct non-interactive equivocal and extractable commitments in the quantum random oracle model.

\subsection{Definition}

We first define a non-interactive bit commitment scheme with selective opening in the quantum random oracle model. Such a scheme consists of a commit algorithm $\Commit^H$, an open algorithm $\Open^H$, and a receive algorithm $\Rec^H$, each with access to a random oracle $H$.\footnote{In our scheme, these algorithms will be entirely classical, and in particular will only need to query $H$ classically.} The scheme is parameterized by a polynomial $n = n(\secp)$ which determines the number of bits to be committed. The algorithms have the following syntax. 

\begin{itemize}
    \item $\Com^H(1^\secp,\{b_i\}_{i \in [n]}) \to (\state,\{\com_i\}_{i \in [n]})$. The commit algorithm takes as input the security parameter $1^\secp$ and $n$ bits $\{b_i\}_{i \in [n]}$, and outputs a committer state $\state$ and a set of commitments $\{\com_i\}_{i \in [n]}$.
    \item $\Open^H(\state,T) \to \{b_i,r_i\}_{i \in T}$. The open algorithm takes as input the committer state $\state$ and a subset $T \subseteq [n]$ and outputs a set of openings $\{b_i,r_i\}_{i \in T}$.
    \item $\Rec^H(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T}) \to \{\{b_i\}_{i \in T}, \bot\}$. The receive algorithm takes as input a set of commitments $\{\com_i\}_{i \in [n]}$, and a set of openings $\{b_i,r_i\}_{i \in T}$ and outputs either the bits $\{b_i\}_{i \in T}$ or $\bot$.
\end{itemize}

\begin{definition}[$\mu(\lambda,q(\secp))$-Equivocality]\label{def:equivocal}
A non-interactive bit commitment scheme with selective opening, parameterized by $n = n(\secp)$, is \emph{equivocal in the QROM} if for any function $q(\secp)$, there exists a stateful
% \nishant{added efficient, confirm} \james{should we say, that runs in time $\poly(\secp,q(\secp))$, or some other bound? just saying ``efficient'' is not clear} \dakshita{yes, and the same edits below.}
simulator $\cS_\Equ \coloneqq \cS_\Equ[q(\secp)]$, running in time $\poly(\secp,q(\secp))$, such that for any non-uniform family of algorithms $\{\brho_\secp,\cA_{\Rec,\secp} = (\cA_{\RCommit,\secp},\cA_{\ROpen,\secp},\cA_{\Dist,\secp})\}_{\secp \in \bbN}$ where $\cA_{\Rec,\secp}$ makes at most $q(\secp)$ oracle queries, and any $\{b_i\}_{i \in [n]} \coloneqq 
%\{T_\secp \subseteq [n(\secp)],
\{b_{i,\secp}\}_{i \in [n],\secp \in \bbN}$, it holds that  (where the state of $\cS_\Equ$ is kept implicit in the following)

%\amit{The interface for $\Open$ is not correctly used here. In particualar, the interface requires set $T$ to be provided but it is missing in the usage below. One possible solution might be to quantify over all $T$ in the definition and use the quantified $T$ in the $\Open$ call}
%\dakshita{We should just say $\Open(\mathsf{st}, [n])$ below.}

\begin{align*}
    \bigg|&\Pr_H\left[\cA_{\Dist,\secp}^H(\brho_2,\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}) = 1 : \begin{array}{r}\brho_1 \gets \cA_{\RCommit,\secp}^H(\brho_\secp) \\ (\state,\{\com_i\}_{i \in [n]}) \gets \Com^H(1^\secp,\{b_i\}_{i \in [n]}) \\ \brho_2 \gets \cA_{\ROpen,\secp}^H(\brho_1,\{\com_i\}_{i \in [n]}) \\ \{b_i,r_i\}_{i \in [n]} \gets \Open^H(\state, [n]) \end{array}\right] \\
    &-\Pr\left[\cA_{\Dist,\secp}^{\cS_\Equ}(\brho_2,\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}) = 1: \begin{array}{r}\brho_1 \gets \cA^{\cS_\Equ}_{\RCommit,\secp}(\brho_\secp) \\ \{\com_i\}_{i \in [n]} \gets \cS_\Equ(1^\secp) \\ \brho_2 \gets \cA^{\cS_\Equ}_{\ROpen,\secp}(\brho_1,\{\com_i\}_{i \in [n]}) \\ \{b_i,r_i\}_{i \in [n]} \gets \cS_\Equ(\{b_i\}_{i \in [n]})\end{array}\right] \bigg| = \mu(\secp,q(\secp)).
\end{align*}
\end{definition}

\begin{definition}[$\mu(\lambda,q(\secp))$-Extractability]\label{def:extractable}
A non-interactive bit commitment scheme with selective opening, parameterized by $n = n(\secp)$, is \emph{extractable in the QROM} if for any function $q(\secp)$, there exists a stateful simulator $\cS_\Ext \coloneqq \cS_\Ext[q(\secp)]$, running in time $\poly(\secp,q(\secp))$, such that for any non-uniform family of quantum oracle algorithms $\{\brho_\secp,\cA_\secp = (\cA_{\Commit,\secp},\cA_{\Open,\secp},\cA_{\Dist,\secp}))\}_{\secp \in \bbN}$ where  $q(\secp)$ is an upper bound on the number of oracle queries $\cA_\secp$ makes, and where for any $T \coloneqq \{T_\secp \subseteq [n(\secp)]\}_{\secp \in \bbN}$, it holds that (where the state of $\cS_\Ext$ is kept implicit in the following) 
\fflater{\nishant{can strengthen the defn so that T is chosen adversarially - but not required for now} \amit{I think chosing set $T$ adversarially is a strenghtening of equivocality definition (not extractability). Also, the exisiting definition of extractability here is already quantified over \emph{all} $T$}}


\begin{align*}\bigg|&\Pr_{H}\left[\cA_{\Dist,\secp}^H(\brho_\out,R_\out) = 1: \begin{array}{r}(\brho_\state,\{\com_i\}_{i \in [n]}) \gets \cA_{\Commit,\secp}^H(\brho_\secp)\\ (\brho_\out,\{b_i,r_i\}_{i \in T}) \gets \cA_{\Open,\secp}^H(\brho_\state,T) \\ R_\out \gets \Rec^H(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T})\end{array}\right]\\
&-\Pr\left[\cA_{\Dist,\secp}^{\cS_\Ext}(\brho_\out,R_\out) = 1: \begin{array}{r}(\brho_\state,\{\com_i\}_{i \in [n]}) \gets \cA_{\Commit,\secp}^{\cS_\Ext}(\brho_\secp)\\ \{b_i^*\}_{i \in [n]} \gets \cS_\Ext(\{\com_i\}_{i \in [n]}) \\ (\brho_\out,\{b_i,r_i\}_{i \in T}) \gets \cA_{\Open,\secp}^{\cS_\Ext}(\brho_\state,T) \\ R_\out \gets \Rec^{\cS_\Ext}(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T}) \\ R_\out \coloneqq \mathsf{FAIL} \text{ if } R_\out \notin \{\{b_i^*\}_{i \in T},\bot\}\end{array}\right]\bigg| = \mu(\secp,q(\secp)).
\end{align*}

In addition, we say that the commitment scheme satisfies \emph{extraction with a stateless simulator} if $\cS_\Ext$ does not have to maintain state. That is, $\cS_\Ext$ can be written as two stateless algorithms $\cS_{\Ext,\mathsf{RO}},\cS_{\Ext,\mathsf{COM}}$, where $\cS_{\Ext,\mathsf{RO}}$ is used to respond to oracle queries made by $\cA$, and $\cS_{\Ext,\mathsf{COM}}$ is used to extract from a set of commitments.

\end{definition}


\subsection{Construction}
In \proref{fig:idealcomm-protocol}, we describe the construction of a non-interactive equivocal and extractable bit commitment scheme with selective opening\footnote{Our construction makes use of two random oracles $H,G:\zo^{\secp+1}\rightarrow \zo^{\secp+1}$, which as explained in Section~\ref{sec:prelims}, can be implemented by a single random oracle of sufficient input/output sizes.}.




%\subsection{Old definition}

%We first define the ideal functionality $\idealcom$ for secure bit commitment with selective opening in \figureref{fig:idealcomm-func}. This ideal functionality was also used in~\cite{GLSV}. Then, we give a protocol in the QROM ($\picom$, \proref{fig:idealcomm-protocol}) that statistically QOSA implements the functionality $\idealcom$. 

%\begin{theorem}
    %\label{thm:rom-commitment}
    %$\picom$ statistically quantum oracle stand-alone realizes %$\idealcom$ in the QROM with query-dependent simulation.
%\end{theorem}

%We provide the proof of this theorem in the following subsections, where we provide simulators against malicious receivers and malicious committers.

% \protocol
% {$\idealcom$}
% {Ideal functionality for bit commitment with selective opening}
% {fig:idealcomm-func}
% {
% Parameters : security parameter $\secp$, number of commitments $n(\secp)$\\
% Parties : Committer $C$, Receiver $R$

% \begin{itemize}
%     \item \textbf{Commit Phase}: $C$ sends a query $(\mathsf{Commit},(m_1,m_2, \ldots m_{n(\secp)}))$ to $\idealcom$, where each $m_i \in \zo$. $\idealcom$ records $(m_1,m_2, \ldots m_{n(\secp)})$ and sends $\mathsf{Receipt}$ to $R$.
    
%     \item \textbf{Reveal Phase}: $\idealcom$ receives a query $(\mathsf{Reveal},I)$ from $C$, where $I \subseteq [n(\secp)]$. If no $(m_1,m_2, \ldots m_{n(\secp)})$ is recorded, then it ignores the message, else it sends $(\mathsf{Reveal},I,\{m_i\}_{i \in I})$ to $R$.
    
%     \amit{The previous statement is unclear, what does ``no $(m_1,m_2, \ldots m_{n(\secp)})$ is recorded'' mean - is it all the $m$'s or atleast one of the $m$'s ? Also, I think it should rather be checking just whether the indices in set $I$ are recorded (instead of checking $[n(\secp)]$)}
% \end{itemize}
% }


% \protocol
% {\proref{fig:idealcomm-protocol}, $\picom$}
% {Protocol $\picom$ for implementing bit commitment functionality $\idealcom$ in QROM}
% {fig:idealcomm-protocol}
% {
% Parties : Committer $C$, Receiver $R$\\
% Random Oracles : $H:\zo^{\secp+1} \rightarrow \zo^{\secp+1}, G:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$

% \begin{itemize}
%     \item \textbf{Commit Phase}
    
%     $C(b_1,b_2 \ldots b_{n(\secp)}), R(\bot)$: $C$ chooses $r_i \leftarrow \zo^\secp, \forall i \in [n(\secp)]$ and sends $\{c_1^i = H(b_i||r_i), c_2^i = G(b_i||r_i)\}_{i \in [n(\secp)]}$ to $R$. $C$ outputs $\{b_i,r_i\}_{i \in [n(\secp)]}$, and $R$ outputs $\{c_1^i,c_2^i\}_{i \in [n(\secp)]}$.
    
%     \item \textbf{Reveal Phase} 
    
%     $C(T,\{b_i,r_i\}_{i \in [n(\secp)]}), R(\{c_1^i,c_2^i\}_{i \in [n(\secp)]})$: $C$ sends $(T,\{b_i,r_i\}_{i \in T})$ to $R$. $R$ sets $J = \emptyset$ and for each $i \in T$, if $H(b_i||r_i)=c_1^i \wedge G(b_i||r_i) = c_2^i$, it sets $J = J \cup \{i\}$. $R$ outputs $J,\{m_j\}_{j \in J}$, and $C$ outputs $\bot$.
% \end{itemize}
% }

\protocol
{\proref{fig:idealcomm-protocol}}
{Extractable and equivocal commitment scheme}
{fig:idealcomm-protocol}
{
Random Oracles : $H:\zo^{\secp+1} \rightarrow \zo^{\secp+1}, G:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$

\begin{itemize}
    \item {$\Com^{H,G}(1^\secp,\{b_i\}_{i \in [n]})$}: Sample $r_i \leftarrow \zo^\secp, \forall i \in [n]$. Set $\state = \{b_i,r_i\}_{i \in [n]}$ and $\forall i \in [n], c_1^i = H(b_i||r_i), c_2^i = G(b_i||r_i), \com_i = (c_1^i,c_2^i)$. Output $(\state, \{\com_i\}_{i \in [n]})$.
    
    \item $\Open^{H,G}(\state, T)$: Parse $\state$ as $\{b_i,r_i\}_{i \in [n]}$ and output $\{b_i,r_i\}_{i \in T}$. 
    
    \item $\Rec^{H,G}(\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in T})$: $\forall i \in [n], \text{parse } \com_i$ as $(c_1^i,c_2^i)$. Output $\bot$ if $\exists i \in T$ s.t. $H(b_i||r_i) \neq c_1^i$ or $G(b_i||r_i) \neq c_2^i$. Otherwise output $\{b_i\}_{i \in T}$.
\end{itemize}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Committer Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Equivocality}

\begin{theorem}
    \proref{fig:idealcomm-protocol} is a non-interactive $\mu(\lambda,\qlamb)$-equivocal bit commitment scheme with selective opening in the QROM satisfying Definition~\ref{def:equivocal}, where $\mu(\secp,\qlamb) = {\frac{\qlamb^{3/2} n^{1/2}}{2^{(\secp/2) - 1}}}$.
\end{theorem}

\begin{proof}

Let $\{\brho_\secp,\malrecvlamb=(\cR^*_{\RCommit,\secp},\cR^*_{\ROpen,\secp},\cR^*_{\Dist,\secp})\}$ be a malicious receiver.
We construct a simulator $\simuequ[\qlamb]$ as follows: 

\begin{enumerate}
    \item Let $n = n(\secp)$. Sample hash functions $h_H,h_G$ from a $2\qlamb$-wise independent hash function family. For all $i \in [n]$, sample $r_i \leftarrow \zo^\secp, r^{H,i}_0, r^{H,i}_1, r^{G,i}_0, r^{G,i}_1 \gets \zo^{\secp+1}$. Answer oracle queries of $\malrecvlamb$ to $H,G$ using oracles $\puncrom{H},\puncrom{G}$ respectively and which are defined as follows: 
    \[   
        \begin{array}{ll}
             \puncrom{H}(x) = 
             \begin{cases}
               r^{H,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
               r^{H,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
               H(x) & \, \text{otherwise} \\ 
             \end{cases}
        & 
            \puncrom{G}(x) = 
             \begin{cases}
               r^{G,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
               r^{G,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
               G(x) & \, \text{otherwise} \\ 
             \end{cases}
        \end{array}
    \]
    
    \item \label{itm:romcom-comm-sec-sampleci}
    To output commitments, for all $i \in [n]$, sample $c^H_i, c^G_i \leftarrow \zo^{\secp+1}$, set $\com_i = (c^H_i,c^G_i)$ and output $\{\com_i\}_{i \in [n]}$. 
    
    \item When given input $\{b_i\}_{i \in [n]}$, output $\{b_i,r_i\}_{i \in [n]}$. From here on, define the following two oracles $\puncrom{H}_R,\puncrom{G}_R$ and use them to answer oracle queries of $\malrecvlamb$ to $H,G$ respectively.
        \begin{itemize}
            \item $\puncrom{H}_R(x) = {H}(x)$, except for all $ i \in [n],\puncrom{H}_R(b_i||r_i) = c^H_i$.

            \item $\puncrom{G}_R(x) = {G}(x)$, except for all $ i \in [n],\puncrom{G}_R(b_i||r_i) = c^G_i$.
        \end{itemize}
\end{enumerate}

For a given $\malrecvlamb$, which makes at most $\qlamb$ oracle queries, and $\simuequ[\qlamb]$ defined as above, we define the following sequence of hybrids to show that \proref{fig:idealcomm-protocol} is an equivocal bit commitment scheme in QROM satisfying Definition~\ref{def:equivocal}.

\fflater{\nishant{I think in our proof adv need only be divided into 2 parts - before opening and after opening - but going with the 3 part defn for now}}

\begin{itemize}
    \item $\Hyb_0$: This hybrid outputs a distribution as follows: 
        \begin{itemize}
            \item $\brho_1 \gets \cR_{\RCommit,\secp}^{* \  H,G}(\brho_\secp)$
            \item $(\state, \{\com_i\}_{i \in [n]}) \gets \Com^{H,G}(1^\secp, \{b_i\}_{i \in [n]})$
            \item $\brho_2 \gets \cR_{\ROpen,\secp}^{* \  H,G}(\brho_1, \{\com_i\}_{i \in [n]})$
            \item $\{b_i,r_i\}_{i \in [n]} \gets \Open^{H,G}(\state)$
            \item Output $\cR_{\Dist,\secp}^{* \  H,G}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})$.
        \end{itemize}

    \item $\Hyb_1$: This is the same as previous hybrid, except in how the oracle queries of $\malrecvlamb$ are answered. Here $\simuequ$ is run to answer oracle queries of $\malrecvlamb$ and it does so using oracles $H,G,\puncrom{H}$ or $\puncrom{G}$. Concretely, this hybrid outputs a distribution as follows:
        \begin{itemize}
            \item $\simuequ$ samples for all $i \in [n],$ $r_i \leftarrow \zo^\secp, r^{H,i}_0,r^{H,i}_1,r^{G,i}_0,r^{G,i}_1 \gets \zo^{\secp+1}$ and defines oracles $\puncrom{H},\puncrom{G}$ as:
            \[   
                \begin{array}{ll}
                     \puncrom{H}(x) = 
                     \begin{cases}
                       r^{H,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
                       r^{H,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
                       H(x) & \, \text{otherwise} \\ 
                     \end{cases}
                & 
                    \puncrom{G}(x) = 
                     \begin{cases}
                      r^{G,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
                      r^{G,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
                      G(x) & \, \text{otherwise} \\ 
                     \end{cases}
                \end{array}
            \]
            \item $\brho_1 \gets \cR_{\RCommit,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_\secp)$
            \item $(\state, \{\com_i\}_{i \in [n]}) \gets \Com^{\simuequ^{{H},{G}}}(1^\secp, \{b_i\}_{i \in [n]} ; \{r_i\}_{i \in [n]})$ ($\{r_i\}_{i \in [n]}$ is the randomness used by $\Com$). \fflater{\nishant{technially can't pass a set, but will take care after deadline}}
            \item $\brho_2 \gets \cR_{\ROpen,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_1, \{\com_i\}_{i \in [n]})$
            \item $\{b_i,r_i\}_{i \in [n]} \gets \Open^{\simuequ^{{H},{G}}}(\state)$
            \item Output $\cR_{\Dist,\secp}^{* \  \simuequ^{{H},{G}}}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})$.
        \end{itemize}
    
    % \item $\Hyb_2$: This is the same as previous hybrid except for the following changes: 
    %     \begin{itemize}
    %         \item $\simuequ$ in addition to defining oracle $\puncrom{H}$, also defines oracle $\puncrom{G}$ by first sampling $r^{G,i}_0,r^{G,i}_1 \gets \zo^{\secp+1}$, along with sampling $r_i,r^{H,i}_0,r^{H,i}_1$ as in the previous hybrid. It defines oracle $\puncrom{H}$ as in the previous hybrid and oracle $\puncrom{G}$ as follows: 
    %         \[   
    %             \begin{array}{l}
    %                 %  \puncrom{H}(x) = 
    %                 %  \begin{cases}
    %                 %   r^{H,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
    %                 %   r^{H,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
    %                 %   H(x) & \, \text{otherwise} \\ 
    %                 %  \end{cases}
    %             % & 
    %                 \puncrom{G}(x) = 
    %                  \begin{cases}
    %                   r^{G,i}_0 & \, \text{if }x = 0||r_i \text{ for some }i \in [n]\\
    %                   r^{G,i}_1 & \, \text{if }x = 1||r_i \text{ for some }i \in [n]\\
    %                   G(x) & \, \text{otherwise} \\ 
    %                  \end{cases}
    %             \end{array}
    %         \]
            
    %         \item $\simuequ$ switches its use of oracle $G$ to $\puncrom{G}$ while answering queries of $\cR^*_{\RCommit,\secp},\cR^*_{\ROpen,\secp}$.
    %     \end{itemize}
    
    \item $\Hyb_2$: This is the same as previous hybrid, except that the call to $\Com^{\simuequ^{H,G}},\Open^{\simuequ^{{H},{G}}}$ are replaced with calls to $\simuequ$. In addition, $\simuequ$ defines oracles $\puncrom{H}_R,\puncrom{G}_R$ which it uses to answer oracle queries of $\cR_{\Dist,\secp}^*$. Concretely, the hybrid outputs a distribution as follows: 
        \begin{itemize}
            \item Sample, for all $i \in [n], r_i,r^{H,i}_0,r^{H,i}_1,r^{G,i}_0,r^{G,i}_1$ as in the previous hybrid and use them to define oracles $\puncrom{H},\puncrom{G}$.
            \item $\brho_1 \gets \cR_{\RCommit,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_\secp)$
            \item $\{\com_i\}_{i \in [n]} \gets \simuequ(1^\secp)$. To do this, $\simuequ$ samples for all $i \in [n], c^H_i,c^G_i \gets \zo^{\secp+1}$, sets $\com_i = (c^H_i,c^G_i)$ and outputs $\{\com_i\}_{i \in [n]}$.
            \item $\brho_2 \gets \cR_{\ROpen,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_1, \{\com_i\}_{i \in [n]})$
            \item $\{b_i,r_i\}_{i \in [n]} \gets \simuequ(\{b_i\}_{i \in [n]})$. In addition, $\simuequ$ defines oracles $\puncrom{H}_R,\puncrom{G}_R$ as follows.
                \begin{itemize}
                    \item $\puncrom{H}_R(x) = {H}(x)$, except for all $i \in [n],\puncrom{H}_R(b_i||r_i) = c^H_i$.
                    \item $\puncrom{G}_R(x) = {G}(x)$, except for all $i \in [n], \puncrom{G}_R(b_i||r_i)=c^G_i$.
                \end{itemize}
            \item Output $\cR_{\Dist,\secp}^{* \  \simuequ^{\puncrom{H}_R,\puncrom{G}_R}}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})$.
        \end{itemize}

    \item $\Hyb_3$: 
    % \nishant{@dakshita tried writing this clearly, do you still think we should be explicit about this hybrid or does this suffice?} 
    This is the same as previous hybrid, except that $\simuequ$ instead of making calls to external oracles $H,G$, first samples hash functions $h_H,h_G$ from a $2\qlamb$-wise independent hash function family and uses them for oracle calls to $H,G$. Note that oracles $\puncrom{H},\puncrom{G},\puncrom{H}_R,\puncrom{G}_R$ are defined using $H,G$ and hence $\simuequ$ no longer uses any external oracles. This hybrid distribution is also the final output distribution in Definition~\ref{def:equivocal}.

\end{itemize}

We show that for $\simuequ[\qlamb]$ defined as above and every $\malrecvlamb$ making at most $\qlamb$ queries, we have 
% for all i $\in [1,3]$ $|\Pr[\Hyb_i=1]-\Pr[\Hyb_{i-1}=1]| \leq \negl(\secp)$. And therefore, 
$|\Pr[\Hyb_3=1]-\Pr[\Hyb_0=1]| \leq \frac{\qlamb^{3/2} n^{1/2}}{2^{(\secp/2) - 1}}$, which along with noting that $\simuequ$ runs in time $\poly(\secp,\qlamb)$, implies that \proref{fig:idealcomm-protocol} is an equivocal bit commitment scheme according to Definition~\ref{def:equivocal}.

\begin{claim}
\label{claim:equivhyb01}
    $|\Pr[\Hyb_0=1]-\Pr[\Hyb_1=1]|\leq \frac{\qlamb^{3/2} n^{1/2}}{2^{(\secp/2) - 1}}$
\end{claim}

\begin{proof}
There are two differences between the hybrids - first, in $\Hyb_1$ the randomness $\{r_i\}_{i \in [n]}$ to be used by $\Com$ is sampled at the start of the experiment\nishant{todo-ideally this should be a separate hybrid, but keeping it low priority}. This however doesn't affect the output distribution since the randomness of $\Com$ was not used anywhere prior to its call in $\Hyb_0$. The second difference is in how oracle queries of $\malrecvlamb$ are answered. In $\Hyb_1$, $\simuequ$ answers queries to $H,G$ of $\cR_{\RCommit,\secp}^*$ and $\cR_{\ROpen,\secp}^*$ using oracles $\puncrom{H},\puncrom{G}$ respectively instead of $H,G$ as in $\Hyb_0$. All the other oracle calls are answered as in $\Hyb_0$.

Assume then for sake of contradiction that there exists 
% a polynomial $p(\cdot)$, 
some $(\brho_\secp,\malrecvlamb)$ and inputs $\{b_i\}_{i \in [n]}$ for which $|\Pr[\Hyb_1=1]-\Pr[\Hyb_0=1]| > \frac{\qlamb^{3/2} n^{1/2}}{2^{(\secp/2) - 1}}$. 
%\dakshita{$\frac{1}{\poly}$ was still undefined, so editing. This should actually be replaced by a concrete parameter.}
We show a contradiction using the One-Way to Hiding lemma (Imported Theorem~\ref{impthm:ow2h}). 
Consider the following oracle algorithms $\cA,\cB,\cC$, where $\cA,\cB$ are the corresponding ones in the One-Way to Hiding lemma and $\cC$ is a wrapper over $\cB$. We show $\cC$ succeeds in a particular task with more probability than possible, which gives us a final contradiction. 
\begin{remark}
\label{remark:singleoracle}
Throughout the claim of this proof, we assume oracle access of $\cA,\cB,\cC$ to oracles $X_1,X_2:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$, is implicitly implemented using a single oracle $X:\zo^{\secp+2} \rightarrow \zo^{\secp+1}$ s.t. $X(0||y) = X_1(y), X(1||y)=X_2(y)$, for all $y \in \zo^{\secp+1}$. For brevity, we overload notation and use $\cA^{X_1,X_2}$ to refer to $\cA^X$.
\end{remark}
% $\cA$ is the distinguisher adversary in the One-Way to Hiding lemma, $\cB$ is the one in the statement of the lemma, and $\cC$ is a wrapper over $\cB$. We analyze the probability of $\cC$ succeeding with noticeable probability in a particular experiment, from which we derive our contradiction. 

\vspace{-5pt}
\paragraph{\underline{$\cA^{X_1,X_2}((H,G),\{r_i\}_{i \in [n]})$}} %Run the same experiment as in $\Hyb_1$ starting with the call to $\cR^*_{\RCommit,\secp}$ and using the provided input $\{r_i\}_{i \in [n]}$ as the randomness for $\Com$, except that all oracle queries of $\cR^*_{\RCommit,\secp},\cR^*_{\ROpen,\secp}$ which are answered using $\puncrom{H},\puncrom{G}$ in $\Hyb_1$ are now answered using external oracles $X_1,X_2$ respectively. Answer any other oracle queries to $H,G$ in $\Hyb_1$ using the description of $H,G$ given as input.
\begin{itemize}
    \item $\brho_1 \gets \cR_{\RCommit,\secp}^{* \  X_1,X_2}(\brho_\secp)$
    \item $(\state, \{\com_i\}_{i \in [n]}) \gets \Com^{H,G}(1^\secp, \{b_i\}_{i \in [n]} ; \{r_i\}_{i \in [n]})$
    \item $\brho_2 \gets \cR_{\ROpen,\secp}^{* \  X_1,X_2}(\brho_1, \{\com_i\}_{i \in [n]})$
    \item $\{b_i,r_i\}_{i \in [n]} \gets \Open^{H,G}(\state)$
    \item Output $\cR_{\Dist,\secp}^{* \  H,G}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})$.
\end{itemize}

\vspace{-5pt}
\paragraph{\underline{$\cB^{X_1,X_2}((H,G),\{r_i\}_{i \in [n]})$}} Let $q' = q'(\lambda)$ denote (an upper bound on the) number of oracle queries of $\cA^{X_1,X_2}$.
\dakshita{Is this an upper bound? Is this over the randomness of sampling $\puncrom{H},\puncrom{G}$ or for a fixing of these? Note that for some fixings of $\puncrom{H},\puncrom{G}$, $q'$ may not be polynomial}
Pick $i \leftarrow [q']$, run $\cA^{X_1,X_2}$ till just before the $i^{th}$ query, measure the query registers and output the set $T$ of measurement outcomes. 

\vspace{-5pt}
\paragraph{\underline{$\cC^{X_1,X_2}((H,G),\{r_i\}_{i \in [n]})$}} Run $T \gets \cB^{X_1,X_2}((H,G),\{r_i\}_{i \in [n]})$, sample $x \in T$ at random, and parse $x$ as $b_1||b_2||r$, where $|b_1|=|b_2|=1,|r|=\secp$. Output $r$. 

\begin{subclaim}
\label{subclaim:ow2haboutC}
    Let oracle algorithms $\cA,\cB,\cC$ be as defined above. Sample oracles $H,G,\puncrom{H},\puncrom{G}$ as follows: sample $H,G:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$. For all $i \in [n]$, sample $r_i \leftarrow \zo^\secp, r^{H,i}_0, r^{H,i}_1,r^{G,i}_0, r^{G,i}_1 \gets \zo^{\secp+1}$ and define oracles $\puncrom{H},\puncrom{G}$ using these as in $\Hyb_1$. If $\qlamb$ denotes (an upper bound on the) number of oracle queries by $\cA^{\puncrom{H},\puncrom{G}}$, then for a fixed $H,G,\puncrom{H},\puncrom{G}$, we have, \fflater{\nishant{check}} 
    \[
    \Pr\left[y \in \{r_i\}_{i \in [n]} \ | \ y \gets \cC^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})\right] > {\frac{n}{2^\secp}}
    \]
\end{subclaim}
\begin{proof}
    To prove this claim, we prove the following subclaim about $\cB$:
    \begin{subclaim}
        \label{subclaim:ow2haboutB}
        Let quantum algorithms $\cA,\cB,\cC$ be as defined above, and oracles $H,G,\puncrom{H},\puncrom{G}$ along with query bound $\qlamb$ be as defined in SubClaim~\ref{subclaim:ow2haboutC}. Furthermore, in accordance with Remark~\ref{remark:singleoracle}, let $\{\puncrom{H},\puncrom{G}\}$ be implemented using a single oracle $O_1 : \zo^{\secp+2} \rightarrow \zo^{\secp+1}$, and similarly, $\{H,G\}$ using oracle $O_2 : \zo^{\secp+2} \rightarrow \zo^{\secp+1}$. If set $S = \bigcup_{b_1,b_2 \in \zo,i \in [n]}\{b_1||b_2||r_i\}$ is the set of points at which $O_1$ and $O_2$ differ, then for a fixed $H,G,\puncrom{H},\puncrom{G}$, we have \fflater{\nishant{this is really not over the randomness of oracle right?}}
        \[
            \Pr[S \cap T \neq \emptyset \ | \ T \leftarrow \cB^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})] > \frac{\qlamb n}{2^\secp}
        \]
    \end{subclaim}
    \begin{proof}
        Note that $\cA^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})$ exactly runs the experiment in $\Hyb_1$ (in $\Hyb_1$ oracle queries of $\malrecvlamb$ are routed through $\simuequ$, but answered using corresponding oracles only). Similarly, $\cA^{H,G}((H,G),\{r_i\}_{i \in [n]})$ exactly runs the experiment in $\Hyb_0$ (in $\Hyb_0$ the randomness used in $\Com$ is sampled during the execution of $\Com$, while in $\cA^{H,G}((H,G),\{r_i\}_{i \in [n]})$ it is passed as input to $\Com$. However, in either case $\{r_i\}_{i \in [n]}$ is not used before the call to $\Com$).
        
        As defined in the claim, mapping oracles $O_1,O_2$ to $\{\puncrom{H},\puncrom{G}\},\{H,G\}$ respectively, we have,
        \begin{align*}
            P_{\text{left}} &= \Pr[\cA^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})=1] = \Pr[\cA^{O_1}(O_2,\{r_i\}_{i \in [n]})] = \Pr[\Hyb_1=1] \\ 
            P_{\text{right}} &= \Pr[\cA^{H,G}((H,G),\{r_i\}_{i \in [n]})=1] = \Pr[\cA^{O_2}(O_2,\{r_i\}_{i \in [n]})] = \Pr[\Hyb_0=1] \\
            \therefore \Big|P_{\text{left}} - P_{\text{right}} \Big| &= \Big|\Pr[\Hyb_1=1]-\Pr[\Hyb_0=1] \Big| > \frac{\qlamb^{3/2} n^{1/2}}{2^{(\secp/2) - 1}}
        \end{align*}
        Invoking the One-Way to Hiding lemma (Imported Theorem~\ref{impthm:ow2h}), with $O_1,O_2$ being the two oracles under consideration, and noting the oracle algorithm $\cB$ defined in the lemma is exactly the same as the one in the current claim, along with the set of points at which $O_1,O_2$ differ being the set $S$ defined in the claim, we get
        \begin{align*}
            P_{\text{guess}} &= \Pr[S \cap T \neq \emptyset \ | \ T \leftarrow \cB^{O_1}(O_2,\{r_i\}_{i \in [n]})] \\
            &= \Pr[S \cap T \neq \emptyset \ | \ T \leftarrow \cB^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})] \\
            &\geq \frac{|P_{\text{left}}-P_{\text{right}}|^2}{4\qlamb^2} > \frac{\qlamb n}{2^{\secp}}
        \end{align*}
        Therefore, 
        \[
            \Pr[S \cap T \neq \emptyset \ | \ T \leftarrow \cB^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})] > \frac{\qlamb n}{2^{\secp}}
        \]
    \end{proof}
    
    \noindent To finish the proof of SubClaim~\ref{subclaim:ow2haboutC}, note that
    \begin{align*}
        \Pr\left[x \in S \ \Bigg| \ \begin{array}{r}
             T \leftarrow \cB^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]}) \\ 
             x \gets T 
        \end{array} \right] 
        & \geq \frac{1}{|T|} \Pr[S \cap T \neq \emptyset \ | \  T \leftarrow \cB^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]}] \\
        &> \frac{1}{\qlamb} \times \frac{\qlamb n}{2^{\secp}}\\
        &= \frac{n}{2^{\secp}}
    \end{align*}
    
    \noindent Finally, note that for any $x \in S$, $x$ is of the form $b_1||b_2||r$, where $|b_1|=|b_2|=1$ and $|r|=\secp$. Hence, parsing $x$ sampled from $T$ gives one of $\{r_i\}_{i \in [n]}$ with same probability. We get as claimed:
    \[
        \Pr\left[y \in \{r_i\}_{i \in [n]} \ | \ y \gets \cC^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]})\right] > \frac{n}{2^{\secp}}
    \]
\end{proof}

\fflater{\nishant{can the bound above be improved?}}
\noindent To complete the proof of Claim~\ref{claim:equivhyb01}, we show that the event in SubClaim~\ref{subclaim:ow2haboutC} can only happen with probability at most $n/2^\secp$, hence giving us the final contradiction.

First note that if SubClaim~\ref{subclaim:ow2haboutC} holds for any fixed $H,G,\puncrom{H},\puncrom{G}$, it also holds for a uniformly sampled $H,G,\puncrom{H},\puncrom{G}$, i.e. 

\begin{align*}
    \Pr\left[y \in \{r_i\}_{i \in [n]} \ \Bigg| \
    \begin{array}{r}
        \text{Sample } H,G,\{r_i,r^{H,i}_0,r^{H,i}_1, r^{G,i}_0,r^{G,i}_1\}_{i \in [n]} \text{ and define } \puncrom{H},\puncrom{G}\\
        y \gets \cC^{\puncrom{H},\puncrom{G}}((H,G),\{r_i\}_{i \in [n]}) 
    \end{array} \right]
    &> \frac{n}{2^{\secp}}
\end{align*}

Opening up the algorithm $\cC$ we get: 
\begin{align}
\label{eq:equiveq1}
    \Pr\left[y \in \{r_i\}_{i \in [n]} \  \left|\rule{0cm}{1.6cm}\right. \
    \begin{array}{r}
        \text{Sample } H,G,\{r_i,r^{H,i}_0,r^{H,i}_1, r^{G,i}_0,r^{G,i}_1\}_{i \in [n]} \text{ and define } \puncrom{H},\puncrom{G}\\
        i \gets [\qlamb] \text{ and run the below two steps till the }i^{th} \text{ query} \\
        \brho_1 \gets \cR_{\RCommit,\secp}^{* \  \puncrom{H},\puncrom{G}}(\brho_\secp) \\
        \brho_2 \gets \cR_{\ROpen,\secp}^{* \  \puncrom{H},\puncrom{G}}(\brho_1, \{H(b_i||r_i),G(b_i||r_i)\}_{i \in [n]})\\
        \text{Measure query registers to get }T\\
        x \gets T, \text{ parse }x = b_1||b_2||y \text{ where }|b_1|=|b_2|=1,|y|=\secp
    \end{array} \right]
    &> \frac{n}{2^{\secp}}
\end{align}

Since for all $i \in [n]$, $\puncrom{H}(b_i||r_i)=r^{H,i}_{b_i}$, while $H(b_i||r_i)$ is independently drawn uniform string (and similarly for $\puncrom{G}(b_i||r_i),G(b_i||r_i)$), we have the above implies: \nishant{what more explanation to give?}
\begin{equation}
    \label{eq:equiveq2}
    \Pr\left[y \in \{r_i\}_{i \in [n]} \  \left|\rule{0cm}{1.5cm}\right. \
    \begin{array}{r}
        \nblue{\text{Sample } O_1,O_2},\{r_i\}_{i \in [n]}, \nblue{\{c^H_i,c^G_i\}_{i \in [n]}}\\
        i \gets [\qlamb] \text{ and run the below two steps till the }i^{th} \text{ query} \\
        \nblue{\brho_1 \gets \cR_{\RCommit,\secp}^{* \  O_1,O_2}(\brho_\secp)} \\
        \nblue{\brho_2 \gets \cR_{\ROpen,\secp}^{* \  O_1,O_2}(\brho_1, \{c^H_i,c^G_i\}_{i \in [n]})}\\
        \text{Measure query registers to get }T\\
        x \gets T, \text{ parse }x = b_1||b_2||y \text{ where }|b_1|=|b_2|=1,|y|=\secp
    \end{array} \right]
    > \frac{n}{2^{\secp}}
\end{equation}

But note here $\{r_i\}_{i \in [n]}$ is not used throughout the experiment and is therefore uniform and independent of the rest of the experiment. Hence, the bound in Equation~\ref{eq:equiveq2} is at most $n/2^\secp$, while this is $>n/2^\secp$ by our assumption. 
Hence, a contradiction and this completes the proof of Claim~\ref{claim:equivhyb01}.

% To do so, note that algorithm $\cC$ works by choosing an element of the set $T$ output by $\cB$ at random. In turn, the set $T$ output by $\cB$ is obtained by measuring some oracle query of $\cA$ chosen randomly. $\cA$ in turn only queries its external oracle for queries of $\cR_{\RCommit,\secp}^{*}$ and $\cR_{\ROpen,\secp}^{*}$. 


% \begin{itemize}
%     \item The view of $\cR_{\RCommit,\secp}^{*}$ is ($\brho_\secp$, oracle access to $\puncrom{H},\puncrom{G}$), which is same as oracle access to two uniform oracles, and hence is independent of $\{r_i\}_{i \in [n]}$.
%     \item The view of $\cR_{\ROpen,\secp}^{*}$ is $(\brho_1, \{H(b_i||r_i),G(b_i||r_i)\}_{i \in [n]}$, oracle access to $\{\puncrom{H},\puncrom{G}\})$. Since $\brho_1$ is output of $\cR_{\RCommit,\secp}^{*}$ and is independent of $\{r_i\}_{i \in [n]}$, and $\puncrom{H},\puncrom{G}$ are uniformly random oracles with for each $i \in [n]$, $\puncrom{H}(b_i||r_i),\puncrom{G}(b_i||r_i)$ being uniform and independent of ${H}(b_i||r_i),{G}(b_i||r_i)$ respectively, we have the view of $\cR_{\ROpen,\secp}^{*}$ is identically distributed to $(\brho_1,\{s^H_i,s^G_i\}_{i \in [n]}$, oracle access to $\{O_1,O_2\})$, where $O_1,O_2$ are uniform oracles and for all $i \in [n]$, $s^H_i,s^G_i$ are uniform strings sampled independently of $O_1,O_2$. Hence, the view of $\cR_{\ROpen,\secp}^{*}$ is independent of $\{r_i\}_{i \in [n]}$.
% \end{itemize}
% Hence, measuring the $i^{th}$ query of $\cR^*_{\RCommit,\secp}$,$\cR^*_{\ROpen,\secp}$ can result in  one can query given only uniformly random strings and oracle access to uncorrelated uniform oracles, $\cR_{\ROpen,\secp}^{*}$ cannot do better than guessing and hence can only query a point in set $S$ with probability at most $n\qlamb/2^{\secp}=\negl(\secp)$, while we know from Equation~\ref{eqn:bhperp} that this happens with probability $\geq {1/\poly(\secp)}$. Hence, a contradiction. 

% \item $|\Pr[\Hyb_1=1]-\Pr[\Hyb_2=1]| \leq \negl(\secp)$

% In $\Hyb_1$, $\simuequ$ replaces the use of $G$ with $\puncrom{G}$ for oracle calls to $G$ of $\cR^*_{\RCommit,\secp},\cR^*_{\ROpen,\secp}$. Hence, the indistinguishability follows by the same reasoning as for $\Hyb_0,\Hyb_1$.
\end{proof}
    
\begin{claim} 
$\Pr[\Hyb_1=1]=\Pr[\Hyb_2=1]$
\end{claim} 
\begin{proof}
    \begin{align*}
        \Pr[\Hyb_1=1] &= \Pr\left[
            y = 1 \ \left|\rule{0cm}{2cm}\right. \
            \begin{array}{r}
                 \text{Sample } H,G,\{r_i,r^{H,i}_0,r^{H,i}_1, r^{G,i}_0,r^{G,i}_1\}_{i \in [n]} \text{ and define } \puncrom{H},\puncrom{G} \\
                 \brho_1 \gets \cR_{\RCommit,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_\secp)\\
                 \nblue{\forall i \in [n], \com_i = (H(b_i||r_i),G(b_i||r_i))}\\
                 \brho_2 \gets \cR_{\ROpen,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_1, \{\com_i\}_{i \in [n]})\\
                %  \{b_i,r_i\}_{i \in [n]} \gets \Open^{\nblue{\simuequ^{{H},{G}}}}(\state)\\
                y \gets \cR_{\Dist,\secp}^{* \  \nblue{\simuequ^{{H},{G}}}}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})
            \end{array}
        \right]
    \end{align*}
    \begin{align*}
        \Pr[\Hyb_2=1] &= \Pr\left[
            y = 1 \ \left|\rule{0cm}{2cm}\right. \
            \begin{array}{r}
                 \text{Sample } H,G,\{r_i,r^{H,i}_0,r^{H,i}_1, r^{G,i}_0,r^{G,i}_1\}_{i \in [n]} \text{ and define } \puncrom{H},\puncrom{G} \\
                 \brho_1 \gets \cR_{\RCommit,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_\secp)\\
                 \nblue{\text{ Sample } \{c^H_i,c^G_i\}_{i \in [n]}, \forall i \in [n], \com_i = (c^H_i,c^G_i)}\\
                 \brho_2 \gets \cR_{\ROpen,\secp}^{* \  \simuequ^{\puncrom{H},\puncrom{G}}}(\brho_1, \{\com_i\}_{i \in [n]})\\
                 \text{Define }\puncrom{H}_R,\puncrom{G}_R \text{ using }\{c^H_i,c^G_i,b_i,r_i\}_{i \in [n]}\\
                y \gets \cR_{\Dist,\secp}^{* \  \nblue{\simuequ^{\puncrom{H}_R,\puncrom{G}_R}}}(\brho_2,\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in [n]})
            \end{array}
        \right]
    \end{align*}

    In the above, the highlighted parts indicate the difference between the two hybrids. However, note that $\cR^*_{\ROpen,\secp}$ only sees uniform strings independent of the oracle it has access to in either hybrid. Also, $\cR^*_{\Dist,\secp}$ sees a uniform oracle consistent at $x_i=b_i||r_i$, together with an evaluation of the oracle at $x_i$ for each $i \in [n]$. Hence, the two distributions are in fact identical.  \fflater{\nishant{could have expanded more, but skipping for now}}

    % To show this, first note that the view of $\cR^*_{\RCommit,\secp}$
    % \dakshita{what does "the view of" mean? It'd be best to refer to random variables in the respective experiments of these hybrids, same for the next sentence.}
    % is identical in either hybrid. 
    % The view of $\cR^*_{\ROpen,\secp}$ in $\Hyb_1$ is $(\brho_1,\{H(b_i||r_i),G(b_i||r_i)\}_{i \in [n]}$, oracle access to $\puncrom{H},\puncrom{G})$, while in $\Hyb_2$ it is $(\brho_1,\{c^H_i,c^G_i\}_{i \in [n]}$, oracle access to $\puncrom{H},\puncrom{G})$. But these distributions are identical since distribution of $\brho_1$ (which is output of $\cR^*_{\RCommit,\secp}$) is identical and independent of $\{b_i,r_i\}_{i \in [n]}$ and for all $i \in [n]$, in $\Hyb_1$, $\{H(b_i||r_i),G(b_i||r_i)\}$ are uniform strings independent of the oracle $\puncrom{H},\puncrom{G}$, and in $\Hyb_2$ as well $\{c^H_i,c^G_i\}$ are uniform strings independent of the oracle $\puncrom{H},\puncrom{G}$.
    
    % % \nishant{these paras could use some more refining}
    % Similarly, the view of $\cR^*_{\Dist,\secp}$ in $\Hyb_1$ is $(\brho_2,\{H(b_i||r_i),G(b_i||r_i)\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}$, oracle access to ${H},{G})$. The same \dakshita{please dont use this phrase! "The same is"} in $\Hyb_2$ is $(\brho_2,\{c^H_i,c^G_i\}_{i \in [n]},\{b_i,r_i\}_{i \in [n]}$, oracle access to $\puncrom{H}_R,\puncrom{G}_R)$. But these distributions are in fact identical. To see this, first note that distribution of $\brho_2$, which was output by $\cR^*_{\ROpen,\secp}$ is identical as explained above. Second, for each $i \in [n]$, the distribution of $(H(b_i||r_i),G(b_i||r_i),b_i,r_i$, oracles $H,G)$ in $\Hyb_1$ is a uniform oracle and its evaluation at a $b_i||r_i$ \dakshita{this isn't accurate, this is evaluation first, then $b_i, r_i$, then the oracles themselves...which are exponential sized!}, while in $\Hyb_2$ the same is \dakshita{please do not use "the same"..was also in my comments two days ago} $(c^H_i,c^G_i,b_i,r_i$, oracles $\puncrom{H}_R,\puncrom{G}_R)$, which is again a uniform oracle and its evaluation at $b_i||r_i$.
    % Therefore, the view of $\malrecvlamb$ in either hybrid is identical and the claim follows.
\end{proof}
    

\begin{claim} 
$\Pr[\Hyb_2=1]=\Pr[\Hyb_3=1]$ 
\end{claim}
\begin{proof}
    This follows using Imported Theorem~\ref{impthm:simRO}, which shows that a quantum oracle algorithm making some $q'$ queries to the oracle behaves identically if given a uniform oracle or a function sampled randomly from a $2q'$-wise independent hash function family. Since $\malrecvlamb$ makes a total of $\qlamb$ queries, which is the bound used in $\Hyb_3$, the argument follows.
\end{proof}
This completes the proof of our theorem.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Receiver Security
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Extractability}

\begin{theorem}
    \proref{fig:idealcomm-protocol} is a non-interactive $\mu(\secp,\qlamb)$-extractable bit commitment scheme with selective opening in the QROM satisfying Definition~\ref{def:extractable}, where $\mu(\secp,\qlamb) = O(\qlamb^3/2^{\secp+1}) + O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$.
\end{theorem}

\begin{proof}
We construct a simulator $\Sim_\Ext[\qlamb]$ that works as follows: 

\begin{enumerate}
    \item Let $n=n(\secp)$. Sample hash functions - $h_H$ at random from a $2\qlamb$-wise independent hash function family and $h_G$ from a $2(\qlamb+2\qlamb n+n)$-wise independent hash function family. In particular, use the family of univariate polynomials of degree $k-1$ with coefficients in $\GF(2^{\secp+1})$ as a $k$-wise independent hash function family~\cite{wegman1981new,lemire2016faster}. Use $h_H,h_G$ to answer oracle queries to $H,G$ respectively throughout the execution.
    
    \item On input $\{\com_i\}_{i \in [n]}$, $\Sim_\Ext$ computes and outputs $\{b_i^*\}_{i \in [n]}$ as follows: for each $i \in [n]$, parse $\com_i$ as $(c_1^i,c_2^i)$. If the parsing fails, set $b_i^* = 0$. Otherwise, perform the following actions: 
        \begin{enumerate}
            \item Compute $R_i = \{x \ | \ x \in \GF(2^{\secp+1}) \wedge h_H(x) = c_1^i \}$ by finding all roots of the finite field polynomial equation $h_H(x)=c_1^i$ of degree $2\qlamb-1$ in polynomial time~\cite{berlekamp1967factoring}.
            
            \item Compute $F_i = \{x \ | \ x \in R_i \wedge h_G(x) = c_2^i \}$ by checking for each $x \in R_i$ whether $h_G(x) = c_2^i$. If $|F_i| \neq 1$, set $b_i^* = 0$. Otherwise let $F_i = \{x_i\}$, where $x_i=a||b,|a|=1,|b|=\secp$. Set $b_i^*=a$.
        \end{enumerate}
    
    % \item Finally output $b_i^*$ as the extracted commitment value. \nishant{@amit, sim is a stateful functionality in this defn - it outputs the b_i^* in point 2 above}
\end{enumerate}

For any malicious committer $\{\brho_\secp,\malcommlamb=(\cC_{\Commit,\secp}^{*},\cC_{\Open,\secp}^{*},\cC_{\Dist,\secp}^{*})\}_\secp$ and for $\Sim_\Ext[\qlamb]$ defined as above, we define a sequence of hybrids to show that \proref{fig:idealcomm-protocol} is an extractable bit commitment scheme in QROM according to Definition~\ref{def:extractable}.

\begin{itemize}
    \item $\Hyb_0$: This hybrid outputs a distribution defined as follows. 
        \begin{itemize}
            \item $(\brho_\state,\{\com_i\}_{i \in [n]}) \gets {\cC_{\Commit,\secp}^{* \ {H,G}}}(\brho_\secp)$
            \item $(\brho_\out,\{b_i,r_i\}_{i \in T}) \gets \cC_{\Open,\secp}^{* \ H,G}(\brho_\state,T)$
            \item $R_\out \gets \Rec^{H,G}(\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in T})$
            \item Output $\cC_{\Dist,\secp}^{* \ H,G}(\brho_\out,R_\out)$.
        \end{itemize}
    
    \item $\Hyb_1$: Here, all oracle queries of $\malcommlamb$ are answered by $\Sim_\Ext^G[\qlamb]$. To do so, $\Sim_\Ext^G[\qlamb]$ first samples a hash function $h_H$ from a $2\qlamb$-wise independent hash function family and uses $h_H$ to answer $\malcommlamb$'s queries to oracle $H$. In particular, it uses the family of polynomials of degree $2\qlamb-1$ with coefficients in $\GF(2^{\secp+1})$ as the $2\qlamb$-wise independent hash function family. It continues to answer oracle queries to $G$ using external oracle $G$. Rest of the experiment is identical to $\Hyb_0$.
    
    \item $\Hyb_2$: This is same as previous hybrid, except $G$ is replaced with a random permutation on $\zo^{\secp+1}$.
    % $\simucomm$ uses a random permutation $\widetilde{G}:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$ to answer any of $\malcomm$'s queries to $G$. 
    
    \item $\Hyb_3$: This is same as previous hybrid, except for the following changes: 
    \begin{itemize}
        \item After running $(\brho_\state, \{\com_i\}_{i \in [n]}) \gets  {\cC_{\Commit,\secp}^{* \ \Sim_\Ext^{G}}}(\brho_\secp)$, $\Sim_\Ext^G$ is run on inputs $\{\com_i\}_{i \in [n]}$. $\Sim_\Ext^G$ for each $i \in [n]$ parses $\com_i$ as $(c_1^i,c_2^i)$. If the parsing fails, it sets $b_i^* = 0$, otherwise performs the following actions:
        \begin{itemize}
            \item Compute $R_i = \{x \ | \ x \in \GF(2^{\secp+1}) \wedge h_H(x) = c_1^i\}$ by solving the finite field polynomial equation $h_H(x) = c_1^i$ of degree $2\qlamb-1$ in polynomial time~\cite{berlekamp1967factoring}. 
            
            \item Compute $F_i = \{ x \ | \ x \in R_i \wedge {G}(x) = c_2^i \}$ by checking for each $x \in R_i$, whether ${G}(x) = c_2^i$. 
            
            \item If $|F_i| \neq 1$, then set $b_i^* = 0$. Otherwise, let $F_i = \{x_i\}$, where $x_i = a||b,|a|=1,|b|=\secp$. Set $b_i^*=a$.
            
            % \item If $|F_i| \neq 1$, then set $m'_i = \bot$, else if $x_i \in F_i$, parse $x_i=a||b$ (where $|a|=1,|b|=\secp$) and set $m'_i=a$.
        \end{itemize}
        
        $\Sim_\Ext^G$ outputs $\{b_i^*\}_{i \in [n]}$.
        
        \item After running $R_{\out} \gets \Rec^{\Sim_\Ext^{G}}(\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in T})$, the following is computed: \\$R_\out \coloneqq \mathsf{FAIL} \text{ if } R_\out \notin \{\{b_i^*\}_{i \in T},\bot\}$.
    \end{itemize}
        
    % \item $\Hyb_5$: In this hybrid, $\simucomm$ starts interacting with $\idealcom$. In particular, it answers the RO queries of $\malcomm$ as in the last hybrid, and at the end of commit phase either outputs \textsf{FAIL} and stops or defines $\{m'_i\}_{i \in [n]}$ as in the last hybrid. It then sends $(\mathsf{Commit},(m'_1,m'_2 \ldots m'_n))$ to $\idealcom$ and thereafter starts running the reveal phase with $\malcomm$. On receiving $(I,\{m_i,r_i\}_{i \in I})$ from $\malcomm$, it does the following - set $J = \emptyset$ and $\forall i \in I$ check if $p_H(m_i||r_i)=c_1^i \wedge \widetilde{G}(m_i||r_i) = c_2^i$ and if the check passes, then set $J = J \cup \{i\}$. It then sends $(\mathsf{Reveal},J)$ to $\idealcom$ and outputs whatever $\malcomm$ outputs.
    
    \item $\Hyb_4$: This is same as previous hybrid, except that $G$ is replaced with a random oracle $\zo^{\secp+1} \rightarrow \zo^{\secp+1}$. 
    
    \item $\Hyb_5$: Here, $\Sim_\Ext[\qlamb]$, in addition to first sampling $h_H$, also samples $h_G$ from a $2(\qlamb + 2\qlamb n + n)$-wise independent hash function family and replaces the use of $G$ throughout its execution with $h_G$. Rest of the hybrid is identical to the previous one. Note that the experiment in this hybrid is identical to the final experiment in Definition~\ref{def:extractable}.
\end{itemize}

While in intermediate hybrids $\Sim_\Ext$ is given access to a random permutation\fflater{\nishant{Check if this doesn't make sense to others}}, in the final hybrid, $\Sim_\Ext$ does not make use of any external oracle. Below we show that for $\Sim_\Ext[\qlamb]$ defined as above, and for every $\malcommlamb$ making at most $\qlamb$ oracle queries 
% and for all $i \in [1,5]$, we have $|\Pr[\Hyb_i=1] - \Pr[\Hyb_{i-1}=1]| \leq \negl(\secp)$.
% And therefore 
$|\Pr[\Hyb_5=1] - \Pr[\Hyb_{0}=1]| \leq O(\qlamb^3/2^{\secp+1}) + O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$, which along with noting that $\Sim_\Ext$ runs in time $\poly(\secp,\qlamb)$, implies that \proref{fig:idealcomm-protocol} is an extractable bit commitment scheme according to definition~\ref{def:extractable}.

\begin{claim}
     $\Pr[\Hyb_0=1] = \Pr[\Hyb_1=1]$ 
\end{claim}
\begin{proof}
    % \nishant{D's comment - is this clear or need more exlanation?}
    This follows by Imported Theorem~\ref{impthm:simRO}, which states that a quantum oracle algorithm making $q'$ queries to the oracle, cannot distinguish between a random function and a hash function sampled from $2q'$-wise independent hash function family. In $\Hyb_1$, $\Sim_\Ext$ while answering oracle queries of $\malcommlamb$, replaces the use of the random oracle $H$ by a hash function sampled from a $2\qlamb$-wise independent hash function family. Since $\malcommlamb$ makes at most $\qlamb$ queries, the argument follows.
\end{proof}

\begin{claim}
    $|\Pr[\Hyb_1=1] - \Pr[\Hyb_2=1]| \leq O(\qlamb^3/2^{\secp+1})$
\end{claim}
\begin{proof}
    This follows using Imported Theorem~\ref{impthm:ROinjective}, which implies that a quantum oracle algorithm making some $q'$ queries to a random oracle$:\zo^\ell \rightarrow \zo^\ell$ cannot distinguish the oracle from a random injective function on $\zo^\ell$, except with probability $O(q'^3/2^\ell)$. Thus it follows that the usage of random oracle $G$ in $\Hyb_1$ and that of random permutation $G$ in $\Hyb_2$ are indistinguishable except with probability $O(\qlamb^3/2^{\secp+1})$.
\end{proof}

\begin{claim}
    $\Pr[\Hyb_2=1] = \Pr[\Hyb_3=1]$
\end{claim}
\begin{proof}
    There are two differences between $\Hyb_2$ and $\Hyb_3$: first, after the call to ${\cC_{\Commit,\secp}^{* \ \Sim_\Ext^{G}}}(\brho_\secp)$, $\Sim_\Ext^G$ is run on inputs $\{\com_i\}_{i \in [n]}$ to get $\{b_i^*\}_{i \in [n]}$, and second, after running $R_{\out} \gets \Rec^{\Sim_\Ext^G}(\ldots)$, $R_{\out}$ is set as $\mathsf{FAIL}$ if $R_{\out} \notin \{\{b_i^*\}_{i \in T}, \bot\}$. We show this cannot happen - i.e. $\Pr[R_{\out} \notin \{\{b_i^*\}_{i \in T}, \bot\}]=0$, where $R_{\out} \gets \Rec^{\Sim_\Ext^G}(\ldots)$. 
    
    From \proref{fig:idealcomm-protocol}, $\Rec^{\Sim_\Ext^G}(\ldots)$ outputs either $\bot$ or $\{b_i\}_{i \in T}$. If it outputs $\bot$, $R_\out = \bot$ and our claim above follows. Otherwise $R_\out = \{b_i\}_{i \in T}$. We show that in this case for all $i \in T, b_i = b_i^*$. From the description of $\Sim_\Ext^G(\{\com_i\}_{i \in [n]})$ in $\Hyb_3$, $\Sim_\Ext$ does the following for each $i \in T$: 
    
    \begin{itemize}
        \item If parsing of $\com_i$ as $(c_1^i,c_2^i)$ fails, it sets $b_i^*=0$. However, in this case, $\Rec^{\Sim_\Ext^G}(\{\com_i\}_{i \in [n]}, \{b_i,r_i\}_{i \in T})$ would output $\bot$, which we assumed does not happen.
        \item After computing $F_i$, if $|F_i| \neq 1$, $b_i^*$ is set as $0$. There are two cases here: 
            \begin{enumerate}
                \item $|F_i|>1$: We show this cannot happen. $F_i$ is computed as $\{x \ | \ x \in \GF(2^{\secp+1}) \wedge G(x) = c_2^i\}$. Since $G$ is a permutation on $\zo^{\secp+1}$, for any $c_2^i$, there can be at most one value which satisfies $G(x)=c_2^i$ and hence $|F_i| \leq 1$.
                \item $|F_i|=0$: We show in this case $\Rec^{\Sim_\Ext^G}(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T})$ outputs $\bot$, which we assumed does not happen. If $\Rec^{\Sim_\Ext^G}(\ldots) \neq \bot$, by the checks defined in $\Rec^{\Sim_\Ext^G}$, for $x_i = b_i||r_i$, we have $h_H(x_i)=c_1^i$ and $G(x_i)=c_2^i$. But this would mean $x_i \in F_i$, since $\Sim_\Ext^G$ exhaustively looked at all roots of the polynomial equation $h_H(x)=c_1^i$. Hence, since we assumed $|F_i|=0$, this cannot happen.
            \end{enumerate}
            
        \item If $|F_i|=1$ and $F_i=\{x_i\}$ where $x_i = a||b,|a|=1,|b|=\secp$, $b_i^*$ is set as $a$. We show in this case that $b_i$ must be equal to $a$ as well. If $b_i \neq a$, we have by the checks performed by $\Sim_\Ext$ while computing $F_i$ and that performed in $\Rec^{\Sim_\Ext^G}$, that there exists at least two different roots to $G(x)=c_2^i$, which cannot happen since $G$ is a permutation.
    \end{itemize}
\end{proof}

\begin{claim}
    $|\Pr[\Hyb_3=1] - \Pr[\Hyb_4=1]| \leq O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$
\end{claim}
\begin{proof}
    This follows using Imported Theorem~\ref{impthm:ROinjective} in a similar way as was used to argue indistinguishability between $\Hyb_1$ and $\Hyb_2$.
    In particular, suppose for some $\malcommlamb$ we have $|\Pr[\Hyb_3=1] - \Pr[\Hyb_4=1]| > O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$. Consider then a quantum oracle algorithm $\cA^O$ which runs the experiment in $\Hyb_3$, but answers all oracle queries of $\Sim_\Ext$ to $G$ (and hence also oracle queries of $\malcommlamb$ to $G$) using its external oracle $O$.
    
    % $A^O$ runs $\cZ_0^*$ to get $(\brho,\bsigma)$, then runs $\malcomm(\brho)$ acting just as $\simucomm$ does in either hybrids and answering its oracle queries to $G$ using the outer oracle $O$ and simulating $\idealcom$ and the honest $R$ itself. Note that $\simucomm$ also makes some queries to $G$, which are again answered using external oracle $O$. Once this execution finishes, it runs $\cZ_1^*(\bsigma,\cdot)$ on the outputs of $\simucomm$ and the honest $R$ and outputs whatever $\cZ_1^*$ outputs. 
    
    The challenger sets $O=G$ or $\widetilde{G}$, where $G$ is a random function$:\zo^{\secp+1} \rightarrow \zo^{\secp+1}$ and $\widetilde{G}$ is a random permutation on $\zo^{\secp+1}$. Hence, $\Pr[\cA^{\widetilde{G}}=1]=\Pr[\Hyb_3=1]$ and $\Pr[\cA^{{G}}=1]=\Pr[\Hyb_4=1]$. We therefore get $|\Pr[\cA^{\widetilde{G}}=1] - \Pr[\cA^{{G}}=1]| > O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$.
    
    However, we know from Imported Theorem~\ref{impthm:ROinjective} that this can only happen with probability $O(q'^3/2^{\secp+1})$, where $q'$ is the number of oracle queries made by $\cA$ to its external oracle. The number of oracle queries by $\cA \leq \qlamb+2\qlamb n+n$ ($\qlamb$ by $\malcommlamb$ and $\leq 2\qlamb$ for each $i \in [n]$ made by $\Sim_\Ext$ when called with inputs $\{\com_i\}_{i \in [n]}$, and $\leq n$ made during call to $\Rec^{\Sim_\Ext^G}(\{\com_i\}_{i \in [n]},\{b_i,r_i\}_{i \in T})$. Hence, we have the probability of distinguishing $G$ and $\widetilde{G}$ can be at best $O(\left(\qlamb+2\qlamb n + n \right)^3/2^{\secp+1})$, hence giving us a contradiction.
\end{proof}

\begin{claim}
    $\Pr[\Hyb_4=1] = \Pr[\Hyb_5=1]$
\end{claim}
\begin{proof}
    In $\Hyb_5$, $\Sim_\Ext$ replaces the calls to random oracle $G$ with a hash function $h_G$ sampled from a $2q'_\secp$-wise independent hash function family, where $q'_\secp = \qlamb + 2\qlamb n + n$. The distinguishability of $\Hyb_4$ and $\Hyb_5$ can then be reduced to distinguishability of a random oracle and $h_G$ by using a similar reduction as in the last hybrid. Since $\Sim_\Ext$ and $\malcommlamb$ make total oracle queries bounded by $q'_\secp$, using Imported Theorem~\ref{impthm:simRO}, which states that a quantum algorithm making some $q$ queries to the oracle cannot distinguish between a random oracle and a hash function sampled from a $2q$-wise independent hash family, the claim follows.
\end{proof}


\end{proof}

==> sec-equivocality.tex <==
\renewcommand{\extcommit}{\mathsf{Commit}}
\renewcommand{\extdecommit}{\mathsf{Decommit}}

\section{A Quantum Equivocality Compiler}
\label{sec: equivocal commitment}

In this section, we show a generic black-box compiler that takes any quantum-secure bit commitment scheme and produces a quantum-secure \emph{equivocal} bit commitment scheme. 

\ifsubmission
The compiler is described in \proref{fig:eqextcom}, where $(\extcommit,\extdecommit)$ denotes some statistically binding and computationally hiding bit commitment scheme. We describe how to equivocally commit to a single bit, and note that commitment to an arbitrary length string follows by sequential repetition. 
\else
The compiler is described in \proref{fig:eqextcom}, where $(\extcommit,\extdecommit)$ denotes some statistically binding and computationally hiding bit commitment scheme satisfying Definitions \ref{def:hiding} and \ref{def:binding}. We describe how to equivocally commit to a single bit, and note that commitment to an arbitrary length string follows by sequential repetition. 
\fi

%For ease of presentation, the protocol is presented assuming that $(\extcommit,\extdecommit)$ has a non-interactive decommitment phase.

\ifsubmission
Furthermore, we show that if the underlying commitment $(\extcommit,\extdecommit)$ is \emph{extractable}, then the resulting commitment is both extractable and equivocal.
\else
Furthermore, we show that if the underlying commitment $(\extcommit,\extdecommit)$ is \emph{extractable} according to~\cref{def:extcom}, then the resulting commitment is both extractable and equivocal (\cref{def:eqcom}).
\fi

These results are captured in the following theorems.
%Both of these properties are satisfied by our construction in \cref{section: extractable com}.


%We let $(\extcommit,\extdecommit)$ denote a hiding (computational hiding suffices) and extractable commitment scheme satisfying Definitions \ref{def: hiding} and \ref{def:extcom}. We will use this to build an extractable equivocal commitment satisfying Definition \ref{def:eecom}. The commitment is described in \proref{fig:eqextcom}. Again, it is shown how to commit to a single bit, and commitment to an arbitrary length string follows by sequential repetition. Furthermore, for ease of presentation, the protocol is presented assuming that $(\extcommit,\extdecommit)$ has a non-interactive decommitment phase, and that the honest receiver's state $\by_\com$ after the commitment phase is classical. Both of these properties are satisfied by our construction in \cref{section: extractable com}.

\renewcommand{\view}{\rho}

\protocol
{\proref{fig:eqextcom}}
{Equivocal Bit Commitment.}
{fig:eqextcom}
{
\textbf{Committer $\cC$ Input:} Bit $b \in \{0,1\}$.

\underline{\textbf{The Protocol: Commit Phase}}
\begin{enumerate}
\item $\cC$ samples uniformly random bits $d_{i,j}$ for $i \in [\lambda]$ and $j \in \zo$.
\item For every $i \in [\lambda]$, $\cC$ and $\cR$ sequentially perform the following steps.
\begin{enumerate}
\item $\cC$ and $\cR$ execute four sessions sequentially, namely:
\begin{itemize}
    \item $\bx_{0,0}, \by_{0,0} \leftarrow \extcommit \langle \cC(d_{i,0}), \cR \rangle$,
    \item $\bx_{0,1}, \by_{0,1} \leftarrow \extcommit \langle \cC(d_{i,0}), \cR \rangle$, 
    \item $\bx_{1,0}, \by_{1,0} \leftarrow \extcommit \langle \cC(d_{i,1}), \cR \rangle$ and 
    \item $\bx_{1,1}, \by_{1,1} \leftarrow \extcommit \langle \cC(d_{i,1}), \cR \rangle$.
\end{itemize}
\item $\cR$ sends a choice bit $c_i \leftarrow \zo$.
\item $\cC$ and $\cR$ execute two decommitments, obtaining the opened bits:
\begin{itemize}
\item $u \leftarrow \extdecommit \langle \cC(\bx_{c_i,0}), \cR(\by_{c_i,0}) \rangle$ and
\item $v \leftarrow \extdecommit \langle \cC(\bx_{c_i,1}), \cR(\by_{c_i,1}) \rangle$. 
\end{itemize}
%At the end of these two phases, $R$ obtains two bits $b'_{c,0}$ and $b'_{c,1}$ that  correspond to the decommitment of each of the two sessions. 
 If $u \neq v$, $\cR$ aborts.
 Otherwise, $\cC$ and $\cR$ continue.
\end{enumerate}
\item For $i \in [\lambda]$, 
$\cC$ sets $e_i = b \oplus d_{i, 1-c_i}$ and
sends $\{e_i\}_{i \in [\lambda]}$ to $R$.
\end{enumerate}

\underline{\textbf{The Protocol: Decommit Phase}}
\begin{enumerate}
    \item $\cC$ sends $b$ to $\cR$. In addition,
    \begin{itemize}
    \item For $i \in [\lambda]$, 
    $\cC$ picks $\alpha_i \gets \zo$ and sends it to $\cR$. 
    \item $\cC$ and $\cR$ execute  $\widehat{d}_i \leftarrow \extdecommit \langle \cC(\bx_{1-c_i,\alpha_i}), \cR(\by_{1-c_i,\alpha_i}) \rangle$.
    \end{itemize}
    \item $\cR$ accepts the decommitment and outputs $b$ if for every $i \in [\lambda]$, $\widehat{d}_i = b \oplus e_i$.
\end{enumerate}
}

% \begin{theorem}
% \label{thm:qecom}
% \proref{fig:eqextcom} describes a  quantum statistically binding and equivocal commitment (satisfying Definitions \ref{def:binding} and \ref{def:eqcom}) whenever $\extcommit$ is instantiated with any quantum statistically binding, computationally hiding commitment (satisfying Definitions \ref{def:binding} and \ref{def:hiding}).
% \end{theorem} \james{if Commit is statistically hiding, then resulting commitment is statistically equivocal}

% \begin{theorem}
% \label{thm:qeecom}
% \proref{fig:eqextcom} describes a quantum extractable and equivocal commitment (satisfying Definition \ref{def:eecom}) whenever $\extcommit$ is instantiated with any quantum extractable, computationally hiding commitment (satisfying Definitions \ref{def:extcom} and \ref{def:hiding}).
% \end{theorem}

\ifsubmission
\begin{theorem}
\label{thm:equiv-compiler}
For $\mathcal{X} \in \{\text{quantum extractability},\text{statistical binding}\}$ and $\mathcal{Y} \in$ \\ $\{\text{computationally},\text{statistically}\}$, if $\extcommit$ is a $\mathcal{Y}$-hiding quantum bit commitment satisfying $\mathcal{X}$, then \proref{fig:eqextcom} is a $\mathcal{Y}$-equivocal bit commitment satisfying $\mathcal{X}$. 
\end{theorem}
\else
\begin{theorem}
\label{thm:equiv-compiler}
For $\mathcal{X} \in \{\text{quantum extractability},\text{statistical binding}\}$ and $\mathcal{Y} \in \{\text{computationally},\text{statistically}\}$, if $\extcommit$ is a $\mathcal{Y}$-hiding quantum bit commitment satisfying $\mathcal{X}$, then \proref{fig:eqextcom} is a $\mathcal{Y}$-equivocal bit commitment satisfying $\mathcal{X}$. 
\end{theorem}
\fi

\ifsubmission
\else
Definitions of statistical binding and computational hiding for quantum commitments can be found in~\cref{def:binding} and~\cref{def:hiding}. Definitions of quantum extractability and quantum equivocality are given in~\cref{def:extcom} and~\cref{def:eqcom}.
\fi

%\begin{proof}
%It is straightforward to see that \proref{fig:eqextcom} satisfies statistical binding assuming that $\extcommit$ is statistically binding. Thus, in what follows we first prove that \proref{fig:eqextcom} is equivocal, that is, it satisfies Definition \ref{def:eqcom}, and next prove that if $\extcommit$ is extractable according to Definition \ref{def:extcom}, then \proref{fig:eqextcom} is extractable, that is, it satisfies Definition \ref{def:extcom}. This suffices to prove both theorems.

These theorems follow from establishing statistical binding, equivocality, and extractability of the commitment in \proref{fig:eqextcom}, as we do next.
%\subsection{Binding}
First, we note that if $\mathsf{Commit}$ is statistically binding, then \proref{fig:eqextcom} is statistically binding. For any adversarial committer strategy, consider the $\secp$ unopened pairs of commitments after the commit phase. Since $\mathsf{Commit}$ is statistically binding, we can assume that each of the $2\secp$ commitments is binding to a particular bit, except with negligible probability. Now, if any single pair contains binding commitments to the same bit $d_{i}$, then the committer will only be able to open its \proref{fig:eqextcom} commitment to the bit $d_i \oplus e_i$. Thus, to violate binding, the adversarial committer will have to have committed to different bits in each of the $\secp$ unopened pairs. However, in this case, the committer will be caught and the receiver will abort except with probability $1/2^\secp$.

\subsection{Equivocality}
\ifsubmission
The equivocal simulator $(\equivsim_{\cR^*,\com}, \equivsim_{\cR^*,\open})$ is obtained via the use of Watrous's quantum rewinding lemma~\cite{STOC:Watrous06}; a full statement of the lemma is available in the supplementary materials. For the purposes of defining the simulation strategy, it will be sufficient (w.l.o.g.) to consider a restricted receiver $\cR^*$ as follows, for the $i^{th}$ sequential step of the protocol.
In our simulation, the state of $\cR^*$ will be initialized to the final state at the end of simulating the $(i-1)^{th}$ step.
\else
The equivocal simulator $(\equivsim_{\cR^*,\com}, \equivsim_{\cR^*,\open})$ is obtained via the use of the quantum rewinding lemma (Lemma \ref{lem:qrl})~\cite{STOC:Watrous06}.
For the purposes of defining the simulation strategy, it will be sufficient (w.l.o.g.) to consider a restricted receiver $\cR^*$ as follows, for the $i^{th}$ sequential step of the protocol.
In our simulation, the state of $\cR^*$ will be initialized to the final state at the end of simulating the $(i-1)^{th}$ step.
\fi
\begin{enumerate}
\item $\cR^*$ takes a quantum register $\mathsf{W}$, representing its auxiliary quantum input. $\cR^*$ will use two additional quantum registers that function as work space: $\mathsf{V}$, which is an arbitrary (polynomial-size) register, and $\mathsf{A}$, which is a single qubit register. The registers $\mathsf{V}$ and $\mathsf{A}$ are initialized to their all-zero states before the protocol begins.

\item Let
$\textsf{M}$ denote the polynomial-size register used by $\cC$ to send messages to $\cR^*$. After carrying out step 2(a) by running on registers $(\mathsf{W},\mathsf{V},\mathsf{A},\mathsf{M})$, $\cR^*$ measures the register $\mathsf{A}$ to obtain a bit $c_i$, for Step 2(b), which it sends back to $\cC$.

\item Next, $\cR^*$ computes the decommitment phases (with messages from $\cC$ placed in register $\mathsf{M}$) according to Step 2(c). $\cR^*$ outputs registers $(\mathsf{W},\mathsf{V},\mathsf{A}, \mathsf{M})$.
\end{enumerate}

Any polynomial-time quantum receiver can be modeled as a receiver of this restricted form followed by some polynomial-time post-processing of the restricted receiver’s output. The same post-processing can be applied to the output of the simulator that will be constructed for the given restricted receiver.


%Due to the principal of deferred measurements, any polynomial-sized quantum verifier can be modeled as a verifier of this restricted form followed by some polynomial-time post-processing of the restricted verifier’s output. 
%The same post-processing can be applied to the output of the simulator that will be constructed for the given restricted verifier. 

Following~\cite{STOC:Watrous06}, we define a simulator that uses two additional registers, $\mathsf{C}$ and $\mathsf{Z}$.
$\mathsf{C}$ is a one qubit register, while $\mathsf{Z}$ is an auxiliary register used to implement the computation that will be described next.
Consider a quantum procedure $\equivsim_{\partial}$ that implements the strategy described in  \proref{fig:eqsimulator} using these registers.

\protocol
{\proref{fig:eqsimulator}}
{Equivocal Simulator.}
{fig:eqsimulator}
{
%\textbf{Equivocal Simulator $\equivsim_{\cR^*}$:} Message $m \in \{0,1\}$

\underline{\textbf{Circuit $\equivsim_{\partial}$.}}
\begin{enumerate}
\item Sample a uniformly random classical bit $\widehat{c}$, and store it in register $\mathsf{C}$.
\item Sample uniformly random bits $(z,d)$.
\item 
If $\widehat{c} = 0$, initialize committer input as follows, corresponding to four sequential sessions:
\begin{itemize}
    \item For the first two sessions, set committer input to $z$.
    \item For the third and fourth sessions, set committer input to $d$ and $1-d$ respectively.
\end{itemize}
\item 
If $\widehat{c} = 1$, initialize committer input as follows, corresponding to four sequential sessions:
\begin{itemize}
    \item For the first and second sessions, set committer input to $d$ and $1-d$ respectively.
    \item For the last two sessions, set committer input to $z$.
\end{itemize}
\item Run the commitment phase interaction between the honest committer and $\cR^*$'s sequence of unitaries on registers initialized as above.
\item Measure the qubit register $A$ to obtain a bit $c$. If $c=\widehat{c}$, output 0, otherwise output $1$.
%For every $i \in [\lambda]$, $\cC$ and $R$ sequentially perform the following steps.
%\begin{enumerate}
%\item 
%apply unitary $R'$ on the following four sequential sessions:
\end{enumerate}
}

Next, we would like to apply Watrous's quantum rewinding lemma to the $\equivsim_{\partial}$ circuit.
In order to do this, we will argue that the probability $p(\psi)$ that this circuit outputs $0$ is such that $|p(\psi)-\frac{1}{2}| = \mathsf{negl}(\lambda)$, regardless of the auxiliary input $\ket{\psi}$ to $\cR^*$. 
This follows from the fact that the commitments are (statistically/computationally) hiding.
In more detail, by definition, Step 5 produces a distribution on the $\cR^*$'s side that is identical to the distribution generated by $\cR^*$ in its interaction with the committer. 
If $|p(\psi)-\frac{1}{2}|$ were non-negligible, then the sequence of unitaries applied by $\cR^*$ could be used to distinguish commitments generated according to the case $\widehat{c} = 0$ from commitments generated according to the case $\widehat{c} = 1$, leading to a contradiction.

Now consider the state of the residual qubits of $\equivsim_{\partial}$ conditioned on a measurement of its output qubit being $0$. The output state of the general quantum circuit $\widehat{\equivsim}$ resulting from applying Watrous's quantum rewinding lemma will have negligible trace distance from this state. This state is over all of the registers discussed above, so the simulator $\equivsim_{\com,\cR^*}$ must further process this state as follows:
\begin{itemize}
\item Measure the register $\mathsf{C}$, obtaining challenge $c$.
\item Compute decommitment information corresponding to challenge $c$, as in Step 2(c) of the protocol (recall that this information is stored in the message register $\mathsf{M}$). 
\item Output registers $(\mathsf{W}, \mathsf{V}, \mathsf{A}, \mathsf{M})$.  All remaining registers are traced out.
\end{itemize}

%Finally, after simulating $\lambda$ sequential sessions, sample $d_1, \ldots, d_{\lambda} \leftarrow \{0,1\}^{\lambda}$ and run the receiver's unitary on the resulting protocol. 

The simulator $\equivsim_{\cR^*,\com}$ executes all $i$ sequential interactions in this manner, and then
 samples $e_1, \ldots, e_{\lambda} \leftarrow \{0,1\}^{\lambda}$, as the committer messages for Step 3 of \proref{fig:eqextcom}. It runs the receiver's unitary on the resulting protocol, and outputs the resulting registers $(\mathsf{W}, \mathsf{V}, \mathsf{A}, \mathsf{M})$.
It additionally outputs private state $\mathsf{st} = (c_1,d_1,\ldots, c_\lambda,d_\lambda)$ where $c_i,d_i$ were sampled during the $i$th execution of \proref{fig:eqsimulator}. 

%\dakshita{fix this. $\alpha_i = d_i \oplus ..$}
The simulator $\equivsim_{\cR^*,\open}(b,\mathsf{st},\bw, \bv, \ba, \bm)$ 
%samples 
%$%e'_1, \ldots e'_\lambda$ uniformly subject to $\bigoplus_{i \in [\lambda]}e'_i = b$ \andrea{I might be missing something, but I am confused about this last condition, and how $\alpha_i$ is obtained later: shouldn't there be a unique choice of $\alpha_i$ given the committing information sent earlier and the bit $b$?}.
parses $\mathsf{st}$ as $(c_1,d_1,\ldots, c_\lambda,d_\lambda)$.
For every $i \in [\lambda]$ it does the following:\begin{itemize}
\item Let $\widehat{d}_i = b \oplus e_i$.
\item If $c_i = 0$, it executes the decommitment phase corresponding to the $((\widehat{d}_i \oplus d_i)+2)^{th}$ session.
\item If $c_i = 1$, it executes the decommitment phase corresponding to the $(\widehat{d}_i \oplus d_i)^{th}$ session.
\end{itemize}
$\equivsim_{\cR^*,\open}$ then executes the receiver's algorithm on these decommitments and outputs the resulting state. Note that each decommitment will be to the bit $\widehat{d}_i = b \oplus e_i$.

\ifsubmission
To complete the proof of equivocality, we must establish that the view of the receiver interacting with an honest committer the view of the receiver interacting with the equivocator are indistinguishable. This follows from the (statistical/computational) hiding of the commitment scheme, via an identical argument to the one used above. In particular, if the equivocal simulator produces a distribution that is distinguishable from the real distribution, then there exists a session $i \in [\lambda]$ such that the distribution in the real and ideal experiments upto the ${i-1}^{th}$ session are indistinguishable, but upto the $i^{th}$ session are distinguishable. This contradicts the above guarantee given by the quantum rewinding lemma, since for any $i$, the post-processed residual qubits of $\equivsim_{\partial}$ are indistinguishable from the state of $\cR^*$ after the $i^{th}$ sequential session in the real protocol (due to the hiding of the commitment scheme).
\else
To complete the proof of equivocality, we must establish that the distributions $\mathsf{Real}_b$ (the view of the receiver interacting with an honest committer) and $\mathsf{Ideal}_b$ (the view of the receiver interacting with the equivocator) of Definition \ref{def:eqcom}, are indistinguishable. This follows from the (statistical/computational) hiding of the commitment scheme, via an identical argument to the one used above. In particular, if the equivocal simulator produces a distribution that is distinguishable from the real distribution, then there exists a session $i \in [\lambda]$ such that the distribution in the real and ideal experiments upto the ${i-1}^{th}$ session are indistinguishable, but upto the $i^{th}$ session are distinguishable. This contradicts the above guarantee given by the quantum rewinding lemma, since for any $i$, the post-processed residual qubits of $\equivsim_{\partial}$ are indistinguishable from the state of $\cR^*$ after the $i^{th}$ sequential session in the real protocol (due to the hiding of the commitment scheme).
\fi

\subsection{Extractability}

Next, we prove that \proref{fig:eqextcom} satisfies extractability as long as the underlying commitment $(\extcommit,\extdecommit)$ is extractable; in other words, this compiler preserves extractability. Consider the following extractor $\cE_{\cC^*}$.

\begin{itemize}
    \item For $i \in [\secp]$:
    \begin{itemize}
        \item Execute four sequential commitment sessions with $\cC^*$, where the extractor of $\extcommit$ is run on the first and third sessions, and the honest interaction is run for the second and fourth sessions. Obtain  outputs $(\brho_{\cC^*}, \st_{\cR,i,0}, d'_{i,0}, \st_{\cR,i,1}, d'_{i,1})$, where $\brho_{\cC^*}$ is the final state of the committer after engaging in all four sequential sessions, and $\st_{\cR,i,0}$, $\st_{\cR,i,1}$ are receiver states output by the extractor corresponding to the first and third sessions. %Since these receiver states are classical, so they can be collected and stored by the extractor as it proceeds sequentially.
        \item Corresponding to Step 2(b), compute and send $c_i \leftarrow \zo$.
        \item Execute Step 2(c) identically to \proref{fig:eqextcom}.
    \end{itemize}
    \item Executes Step 3 of \proref{fig:eqextcom}, receiving bits $\{e_i\}_{i \in [\secp]}$. Fix $b^*$ to be the most frequently ocurring bit in $\{e_i \oplus d'_{i,1-c_i}\}_{i \in [\secp]}$, and output the final state of $\cC^*$, the receiver states $\{\st_{\cR,i,0},\st_{\cR,i,1}\}_{i \in [\secp]}$, and the extracted bit $b^*$.
\end{itemize}

Indistinguishability between the distributions $\mathsf{Real}$ and $\mathsf{Ideal}$ follows by definition of extractability of the underlying commitment $(\extcommit, \extdecommit)$. 
In more detail, recall that $\mathsf{Real}$ denotes the distribution $(\rho_{\cC^*,\final}, b)$ where $\rho_{\cC^*,\final}$ denotes the final state of $\cC^*$ and $b$ the output of the receiver, and $\mathsf{Ideal}$ denotes the final committer state and opened bit after the opening phase of the scheme is run on the output of the extractor.
Now for every commitment strategy, every $i \in [\lambda]$, the probability that $d'_{i,1-c_i}$ is not equal to the other bit committed in its pair, and yet the receiver does not abort in Step 2(c) in the $i^{th}$ sequential repetition, is $\leq \frac{1}{2} + \negl(\lambda)$. Thus, by the correctness of the extractor, this implies that the probability that an adversarial committer opens to $1-b^*$ is at most $1/2^{\secp/2} + \negl(\secp) = \negl(\secp)$. Finally, by indistinguishability of the extractor's and committer's states, this implies that the distributions $\mathsf{Real}$ and $\mathsf{Ideal}$ are indistinguishable.



==> sec-extractability.tex <==
\newcommand{\eqcommit}{\mathsf{EqCommit}}
\newcommand{\eqdecommit}{\mathsf{EqDecommit}}

\section{Quantum Extractable Commitments}
\label{section: extractable com}
%In what follows, we denote by $\secp$ the security parameter and by $m = m(\secp)$ a statistical security parameter (which can be set to $\secp$).
%, and by $n = n(\secp)$ the length of committer inputs.
We construct extractable commitments by making use of the following building blocks.

\begin{itemize}
\ifsubmission
    \item We let $(\eqcommit,\eqdecommit)$ denote any statistically binding, equivocal quantum commitment scheme. Such a commitment can be obtained by applying the compiler from last section to Naor's commitment scheme~\cite{JC:Naor91}.
\else
    \item We let $(\eqcommit,\eqdecommit)$ denote any quantum statistically binding and equivocal commitment scheme, satisfying \cref{def:binding} and \cref{def:eqcom}. Such a commitment can be obtained by applying the compiler from last section to Naor's commitment scheme~\cite{JC:Naor91}.
\fi
    %That is, for receiver message $u$, $\eqcommit(u,x;r)$ is a commitment to message $x$ with randomness $r$.
    
    %a post-quantum statistically binding, quantum computationally hiding commitment (see \cref{subsec: com definitions}). For ease of presentation, we assume that the commitment is non-interactive, and that $\commit(x;r)$ denotes the algorithm committing to message $x$ with randomness $r$. In reality, we will use Naor's commitment~\cite{JC:Naor91}, which requires a (uniformly random) first message from the receiver, so $\commit$ will be defined with respect to this message.
%    \item Let $\Pi_{\mathsf{ZK}}$ denote any post-quantum computational zero-knowledge argument for $\mathsf{NP}$ (see \cref{subsec: ZK def}), and for $n \in \bbN, u \in \{0,1\}^*$, let language $\cL_{n,u} = \Big\{\{c_i,\alpha_i,\beta_i\}_{i \in [n]}: \forall i \in [n], \exists r_i \text{ s.t. } c_i= \commit\Big(u,(\alpha_i, \beta_i);r_i\Big) \Big\}$.
    \item For a suitable polynomial $k(\cdot)$, let $h : \{0,1\}^{k(\lambda)} \times \{0,1\}^{\lambda^2} \to \{0,1\}$ be a universal hash function that is evaluated on a random seed $s \in \{0,1\}^{k(\lambda)}$ and input $x \in \{0,1\}^{\lambda^2}$.

\end{itemize}
  
Our extractable commitment scheme is described formally in Figure~\ref{fig:ext-com}. We show how to commit to a single bit, though commitment to any arbitrary length string follows by sequential repetition. Correctness of the protocol follows by inspection. In the remainder of this section, we prove the following theorem.

\ifsubmission
\begin{theorem}
\label{thm:qextcom}
\proref{fig:ext-com} describes a quantum statistically hiding and extractable bit commitment whenever $(\eqcommit,\eqdecommit)$ is instantiated with any quantum statistically binding and equivocal bit commitment scheme.
\end{theorem}
\else
\begin{theorem}
\label{thm:qextcom}
\proref{fig:ext-com} describes a quantum statistically hiding and extractable bit commitment (satisfying \cref{def:binding} and \cref{def:extcom}) whenever $(\eqcommit,\eqdecommit)$ is instantiated with any quantum statistically binding and equivocal bit commitment scheme (satisfying \cref{def:binding} and \cref{def:eqcom}).
\end{theorem}
\fi


Throughout, we will consider non-uniform adversaries, but for ease of exposition we drop the indexing by $\secp$.



%and $\Pi_{BB}$ denotes the OT protocol against benign receivers from~\cite{C:BenBra84}.

\protocol
{\proref{fig:ext-com}}
{Extractable Commitment.}
{fig:ext-com}
{

\textbf{Committer $\cC$ Input:} Bit $b \in \{0,1\}$.\\
%\textbf{Receiver $\cR$ Input:} Bit $b \in \{0,1\}$\\

\underline{\textbf{The Protocol: Commit Phase.}}
\begin{enumerate}
\item \label[step]{step:sample} $\cC$ chooses $x \leftarrow \{0, 1\}^{2\lambda^3}$, $\theta \leftarrow \{+, \times \}^{2\lambda^3}$ and sends $\ket{x}_\theta$ to $\cR$. 

%, and a first message $u$ for Naor's commitment scheme, 

\item \label[step]{step:commit} $\cR$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{2\lambda^3}$
and obtains $\widehat{x} \in \{0, 1\}^{2\lambda^3}$ by measuring $\ket{x}_{\theta}$
in basis $\widehat{\theta}$.

$\cR$ commits to $\widehat{\theta}$ and $\widehat{x}$ position-wise: 
$\cR$ and $\cC$ execute sequentially $2\secp^3$ equivocal commitment sessions with $\cR$ as committer and $\cC$ as receiver.
That is, for each $i \in [2\secp^3]$, they compute $(\bx_{\com,i}, \by_{\com,i}) \leftarrow \eqcommit \langle \cR(\widehat{\theta}_i,\widehat{x}_i), \cC \rangle$.

\item \label[step]{step:challenge} $\cC$ sends a random test subset $T \subset [{2\lambda^3}]$ of size ${\lambda^3}$ to $\cR$. 

\item \label[step]{step:open} For every $i \in T$, $\cR$ and $\cC$ engage in 
$(\widehat{\theta}_i,\widehat{x}_i) \gets \eqdecommit\langle \cR(\bx_{\com,i}), \cC(\by_{\com,i}) \rangle$, and $\cC$ aborts if any commitment fails to open.
%sends $\widehat{\theta}_i$, $\widehat{x}_i$, to $\cC$. 


\item \label[step]{step:verify} $\cC$ checks that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $\cC$ proceeds with the protocol,
otherwise, $\cC$ aborts. 

\item The tested positions are discarded by both parties: $\cC$ and $\cR$ restrict $x$ and $\theta$, respectively $\widehat{x}$ and $\widehat{\theta}$,
to the $\lambda^3$ indices $i \in \overline{T}$.
$\cC$ sends $\theta$ to $\cR$.

\item $\cC$ partitions the remaining $\lambda^3$ bits of $x$ into $\lambda$ different $\lambda^2$-bit strings $x^{(1)},\dots,x^{(\lambda)}$. For each $\ell \in [\lambda]$, sample a seed $s_\ell \gets \{0,1\}^{k(\lambda)}$ and compute $d_\ell \coloneqq h(s_\ell,x^{(\ell)})$. Then output $(s_\ell,b \oplus d_\ell)_{\ell \in [\lambda]}$.

\end{enumerate}

\underline{\textbf{The Protocol: Decommit Phase.}}
\begin{enumerate}
    \item $\cC$ sends $b$ and $(x^{(1)},\dots,x^{(\lambda)})$ to $\cR$.
    \item If either of the following fails, $\cR$ rejects and outputs $\bot$. Otherwise, $\cR$ accepts and outputs $b$.
    \begin{itemize}
        \item Let $\{s_\ell,v_\ell\}_{\ell \in [\lambda]}$ be the message received by $\cR$ in step 7. Check that for all $\ell \in [\lambda]$, $v_\ell = b \oplus h(s_\ell,x^{(\ell)})$.
        \item For each $j \in [\lambda^3]$ such that $\widehat{\theta}_j = \theta_j$, check that $\widehat{x}_j = x_j$.
        %\item For $j \in [\lambda], \bu_j = (x_{\mathsf{ind}_{\lambda(j-1)+1}}, x_{\mathsf{ind}_{\lambda(j-1)+2}}, \ldots, x_{\mathsf{ind}_{\lambda(j-1)+\lambda}}), \bc_j = \bu_j \oplus \mathsf{offset}_j$ is a valid codeword.
        %\item $m = h(\bc_1, \bc_2, \ldots, \bc_\lambda) \oplus y$, and
        %\item For every index $\mathsf{ind} \in \overline{T}$ such that $\widehat{\theta}_{\mathsf{ind}} = \theta_{\mathsf{ind}}$, it is the case that $\widehat{x}_{\mathsf{ind}} = x'_{\mathsf{ind}}$.
    \end{itemize}
\end{enumerate}

}



%\begin{theorem}
%The protocol in Figure \ref{fig:ext-com} is a statistically hiding, extractable commitment scheme, satisfying Definitions \ref{def: hiding} and \ref{def:extcom}.
%\end{theorem}


\iffalse{
\subsection{Extractability}

\begin{lemma}
The protocol in Figure \ref{fig:ext-com} is an extractable commitment scheme, satisfying Definition \ref{def:extcom}.
\end{lemma}
}\fi

\subsection{Extractability}
Consider any adversarial committer $\cC^*$ with advice $\brho$. The extractor $\cE_{\cC^*}(\brho)$ is constructed as follows. 
%It computes the output of $\eqcommit$'s equivocal simulator for receiver $R^*(\brho)$, where $R^*(\brho)$ is defined as follows.

%$\simu_{\mathsf{ZK}}(V^*,\brho)$ where the verifier $V^*$ depends on $\cC^*$. $V^*$ is constructed as follows. %\andrea{I was a little confused about how $V^*$ is defined? If I understand correctly the following steps are defining $\cE(S^*)$. I would have expected $\simu_{\mathsf{ZK}}$ to be invoked at step 4?}
%\paragraph{$R^*(\brho)$:}
    \begin{enumerate}
        \item Run the first message algorithm of $\cC^*$ on input $\brho$, obtaining message $\bpsi$.
        \item For $i \in [2\lambda^3]$, 
        sequentially execute equivocal commitment sessions with the equivocal simulator $\cQ_{R^*,\com}$, where $R^*$ is the part of $\cC^*$ that participates as receiver in the $i^{th}$ session. Session $i$ results in output $(\mathbf{z}_i, \by_{\com,i})$, where $\mathbf{z}_i$ is stored by the extractor, and $\by_{\com,i}$ is the current state of $\cC^*$, which is fed as input into the next session.
        %compute $c_i = \eqcommit(u,(0,0);r_i)$ for uniform $r_i$.
        \item Obtain $T$ from $\cC^*$, and sample $\widehat{\theta} \gets \{+,\times\}^{2\secp^3}$. Let $\bpsi_i$ denote the $i^{th}$ qubit of $\bpsi$, and measure the qubits $\bpsi_i$ for $i \in T$, each in basis $\widehat{\theta}_i$. Let $\{\widehat{x}_i\}_{i \in [T]}$ be the results of the measurements.
        \item Let $\bx_\com$ be the current state of $\cC^*$. For each $i \in [T]$, execute $\cQ_{R^*,\open}((\widehat{\theta}_i,\widehat{x}_i),\mathbf{z}_i, \bx_\com)$, where $R^*$ is the part of $\cC^*$ that participates in the $i^{th}$ opening, and $\bx_\com$ is updated to be the current state of $\cC^*$ after each sequential session.
        %Output the instance $\{c_i,\widehat{\theta}_i,\widehat{x}_i\}_{i \in [T]}$ and expect as input external prover messages for $\Pi_{\mathsf{ZK}}$.
        %Forward prover messages to $\cC^*$ and forward $\cC^*$'s responses to the external prover.
        \item If $\cC^*$ aborts at any point, abort and output $\bot$, otherwise continue.
        \item Discard tested positions and restrict $\widehat{\theta}$ to the indices in $\overline{T}$. Obtain $\theta \in \{+,\times\}^{\lambda^3}$ from $\cC^*$.
        Measure the qubits $\bpsi_i$ in basis $\theta_i$ to obtain $\widehat{x}_i$ for $i \in \overline{T}$, and then partition $\widehat{x}$ into $\lambda$ different $\lambda^2$-bit strings $\widehat{y}_1, \ldots, \widehat{y}_\lambda$.
        %$\widehat{\bu}_j = (\widehat{x}_{\mathsf{ind}_{\lambda(j-1)+1}}, \widehat{x}_{\mathsf{ind}_{\lambda(j-1)+2}}, \ldots, \widehat{x}_{\mathsf{ind}_{\lambda(j-1)+\lambda}})$.
        \item Obtain $\{s_\ell, v_\ell\}_{\ell \in [\secp]}$ from $\cC^*$. %\{\mathsf{offset}_j\}_{j \in [\lambda^2]}$ from $\cC$.
        %compute $\widehat{b}_i = h(s_\ell, \widehat{u}_i)$.
        %For $j \in [\lambda]$, compute $\widehat{\bc}_j$ as the nearest codeword to $\widehat{\bu}_j \oplus \mathsf{offset}_j$ and $\widehat{m} = h(\widehat{\bc}_1, \ldots, \widehat{\bc}_\lambda) \oplus y$.
        Let $b^*$ be the most frequently occurring bit in $\{ h(s_\ell, \widehat{x}^{(\ell)}) \oplus v_\ell\}_{\ell \in [\secp]}$. Output $(\bx_\com,\by_\com,b^*)$, where $\bx_\com$ is the resulting state of $\cC^*$ and $\by_\com = (\theta, \widehat{\theta},\widehat{x})$.
        %Finally, sample $\overline{S} \subseteq \overline{T}$ by picking each element in $\overline{T}$ independently with probability $\frac{1}{2}$.
        %Output $\by_\final = \{ \widehat{x}_i\}_{i \in \overline{S}}$.
    \end{enumerate}
    \ifsubmission
    We now prove that $\cE_{\cC^*}$ is a secure extractor; for space reasons, a full definition of extractability in the quantum setting is in the supplementary materials (Definition 3.3). 
    \else
    We now prove that $\cE_{\cC^*}$ is a secure extractor in the sense of~\cref{def:extcom}. We do so via a sequence of hybrids.
    \fi
    \\

        
        \noindent {\textbf{$\mathsf{Hyb}_1$.}} Define distribution $\mathsf{Hyb}_1$ identically to $\mathsf{Real}$ (the honest interaction), except that in Step 2, for $i \in [2\lambda^3]$, sequentially execute equivocal commitment sessions using the equivocal simulator $\cQ_{R^*,\com}$, as described in the extractor. In Step 4, for every $i \in T$, open the $i$'th commitment to $(\widehat{\theta}_i,\widehat{x}_i)$ using $\cQ_{R^*,\open}$, as described in the extractor.
        
        %$\cQ_{R^*,\open}((\widehat{\theta}_i||\widehat{x}_i),\mathbf{z}_i, \by_{\com,i})$, where $R^*$ is the part of $\cC^*$ that participates in the $i^{th}$ opening.
        %$c_i$ for $i \in [m]$ are generated as $c_i = \commit(u,(0,0); r_i)$ instead of as $\commit(u,(\widehat{\theta}_i, \widehat{x}_i); r_i)$.
    
        By the equivocal property of $\Commit$, for any QPT distinguisher $(\cD^*,\bsigma)$, there exists a negligible function $\nu(\cdot)$ such that
        $$\Big|\Pr[\cD^*(\bsigma,\mathsf{Hyb}_1) = 1] - \Pr[\cD^*(\bsigma,\mathsf{Hyb}_0) = 1] \Big|  = \nu(\secp).$$


        \noindent {\textbf{$\mathsf{Hyb}_2$.}} This is identical to $\mathsf{Hyb}_1$,  except that the verifier measures qubits of $\ket{x}_{\theta}$ {\em only after} obtaining a description of the set $T$, and \emph{only measures} the qubits $i \in [T]$.
        The output of this experiment is identical to $\mathsf{Hyb}_1$, therefore for any QPT distinguisher $(\cD^*,\bsigma)$, $$\Pr[\cD^*(\bsigma,\mathsf{Hyb}_3) = 1] = \Pr[\cD^*(\bsigma,\mathsf{Hyb}_2) = 1].$$
        
        Moreover, the only difference between $\mathsf{Hyb}_2$ and $\mathsf{Ideal}$ is that $\mathsf{Ideal}$ outputs $\mathsf{FAIL}$ when the 
        message $b$ opened by $\cC^*$ is not $\bot$ and differs from the one extracted by $\cE_{\cC^*}$ .
        Therefore, to derive a contradiction it will suffice to prove that there exists a negligible function $\nu(\cdot)$ such that
        $$\Pr[\mathsf{FAIL}|\mathsf{Ideal}] = \nu(\lambda).$$
        
        Consider any sender $\cC^*$ that produces a committer state $\bx_\com$ and then decommits to message $b'$ using strings $(y_1,\dots,y_\secp)$ during the decommit phase.
        Let $T' \subseteq [\lambda]$ denote the set of all indices $\ell \in [\lambda]$ such that the corresponding $x^{(\ell)} \neq v_\ell$, where $\widehat{x}^{(\ell)}$ denotes the values obtained by the extractor in Step 6. Then we have the following claim.
        \begin{claim}
        There exists a negligible function $\nu(\cdot)$ such that $$\Pr[|T'| > \lambda/2 ] = \nu(\lambda)$$
        where the probability is over the randomness of the extractor.
        \end{claim}
        \begin{proof}
        For every $\ell \in [\lambda]$, we have that (over the randomness of the extractor):
        $$\Pr \Big[\cR_{\mathsf{open}}(\by_{\mathsf{com}}) \text{ outputs }\bot\text{ in }\langle \cC^*_{\mathsf{open}} (\bx_{\mathsf{com}}), \cR_{\mathsf{open}} (\by_{\mathsf{com}}) \rangle \ \Big| \ x^{(\ell)} \neq \widehat{x}^{(\ell)} \Big] \geq \frac{1}{2}.$$ Indeed, the receiver will reject if for some position $i$ for which $x^{(\ell)} \neq \widehat{x}^{(\ell)}$, it holds that $\theta_i = \widehat{\theta}_i$. Since $\widehat{\theta}$ was sampled uniformly at random, this will occur for a single $i$ with independent probability 1/2. This implies that $\Pr[|T'| > \lambda/2] \leq \frac{1}{2^{\lambda/2}}$, and the claim follows.
        %\dakshita{TODO: w.h.p., any sufficient deviation will be caught by an honest verifier that checks a random subset of the positions for random $\widehat{\theta}$, where $\widehat{\theta}_i = \theta_i$.}
        \end{proof}
        By construction of $\cE_{\cC^*}$, $\Pr[\mathsf{FAIL}|\mathsf{Ideal}] < \Pr[|T'| > \lambda/2]$, and therefore it follows that there exists a negligble function $\nu(\cdot)$ such that $$\Pr[\mathsf{FAIL}|\mathsf{Ideal}] = \nu(\lambda).$$

\ifsubmission
The proof of that the extractable commitment scheme described in~\cref{fig:ext-com} is statistically hiding follows readily from quantum sampling techniques developed by~\cite{C:BouFeh10}, and is deferred to the supplementary materials.
\else

\subsection{Statistical Hiding}
\label{subsec:stat-hiding}

In this subsection, we prove that our extractable commitment scheme described in~\cref{fig:ext-com} is statistically hiding, assuming that $\eqcommit$ is a statistically binding (equivocal) commitment scheme.

Our proof closely follows techniques of~\cite{C:BouFeh10}, who developed techniques for analyzing~\cite{FOCS:CreKil88}-style oblivious transfer protocols based on quantum sampling techniques. We import a lemma from~\cite{C:BouFeh10}.

\paragraph{\cite{C:BouFeh10} Quantum Sampling.} Let $\ket{\psi}_{\gray{X}\gray{Y}}$ be a quantum pure state on $2n$-qubit registers $\gray{X}$ and arbitrary size registers $\gray{Y}$. Let $\hat{x} \in \{0,1\}^{2n}$ and $\hat{\theta} \in \{+,\times\}^{2n}$ be arbitrary. Consider the following ``quantum sampling'' experiment:
\begin{enumerate}
\item Sample a random $2n$-length binary string $\theta \leftarrow \{+,\times\}^{2n}$.
\item Sample a random choice of $n$ indices $T \subset [2n]$.
\item For each index $i \in T$, measure the $i$th qubit of $\ket{\psi}_{\gray{X}\gray{Y}}$ in basis $\hat{\theta}_i$.
\item The experiment is successful if for each $i \in T$ where $\theta_i = \hat{\theta}_i$, the measurement outcome is $\hat{x}_i$.
\end{enumerate}

\begin{lemma}[\cite{C:BouFeh10} Quantum Sampling Lemma]
\label{lemma:sampling}
Let $\overline{T} \coloneqq [2n] \setminus T$ and let $S$ be a subset of $\overline{T}$ of size $s$. Suppose we run the quantum sampling experiment on $\ket{\psi}_{\gray{X}\gray{Y}}$ for some fixed choice of $\hat{x} \in \{0,1\}^{2n}$ and $\hat{\theta} \in \{+,\times\}^{2n}$. Let $X_S$ be the length $s$ bitstring that results from measuring the $i$th qubit of the leftover state in basis $\theta_i$ for each $i \in S$. Then the probability the sampling experiment succeeds and
\[ \mathbf{H}_{\infty}(X_S \mid \gray{Y}) < s/3 \]
is at most $\negl(s^2/n)$.
\end{lemma}

\begin{proof}
This lemma follows readily from the techniques of~\cite{C:BouFeh10}, which we will not reproduce here. In particular,~\cite[Theorem 3]{C:BouFeh10} and~\cite[Corollary 1]{C:BouFeh10} applied to the sampling strategy in~\cite[Example 4]{C:BouFeh10} directly imply the statement above holds with the min-entropy upper bound of $\mathbf{H}_{\infty}(X_S \mid \gray{Y}) < s'- \varepsilon \cdot s$ for any constant $\varepsilon > 0$, where $s'$ is the number of indices $i \in S$ where $\theta_i \neq \hat{\theta}_i$. Since $\theta$ is uniformly random, a Chernoff bound implies $s'$ is at least $s/2 - s/12$ except with probability $\negl(s)$, and we can set $\varepsilon = 1/12$ to obtain a clean fixed bound of $s/3$.
\end{proof}

% Before we apply this lemma to prove statistical hiding of our extractable commitments, we provide some brief intuition behind the~\cite{C:BouFeh10} techniques used to prove this lemma. At a very high level, the main result of~\cite{C:BouFeh10} is that up to polynomial factors, ``quantum sampling'' behaves like classical sampling.

\paragraph{Proof of Statistical Hiding.} We now prove statistical hiding of our extractable commitment scheme in~\cref{fig:ext-com}. The core proof idea is due to~\cite{C:BouFeh10}.

Consider a \emph{purification} of the committer's strategy from~\cref{fig:ext-com}, where instead of sampling random $x \gets \{0,1\}^{2\secp^3}, \theta \gets \{+,\times\}^{2\secp^3}$ and sending $\ket{x}_\theta$ to $\mathcal{R}$ in~\cref{step:sample}, the committer $\mathcal{C}$ generates $2\secp^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$, and sends $\mathcal{R}$ one half of each pair. This change has no effect on the receiver's view. In this modification of~\cref{step:sample}, the committer will still sample random $\theta \gets \{+,\times\}^{2\secp^3}$ but does not use it to perform any measurements (and hence $x$ is not yet determined). We now recast~\cref{step:sample,step:open,step:commit,step:challenge,step:verify} of~\cref{fig:ext-com}, i.e., the ``measurement-check subprotocol'' to correspond with this undetectable modification of the committer's behavior:

% \begin{enumerate}
% \item The committer (inefficiently) opens the commitments to recover the receiver's choice of $(\hat{\theta},\hat{x})$.
% \item Rather than checking that 
% \end{enumerate}

\begin{enumerate}
\item $\cC$ chooses $2\lambda^3$ EPR pairs $(\ket{00} + \ket{11})/\sqrt{2}$ and sends $\mathcal{R}$ one half of each pair. The committer samples random $\theta \gets \{+,\times\}^{2\lambda^3}$ but does not perform any measurements (and hence $x$ is not yet determined).
\item $\cR$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{2\lambda^3}$
and obtains $\widehat{x} \in \{0, 1\}^{2\lambda^3}$ by measuring its $2\lambda^3$ EPR pair halves in bases specified by $\widehat{\theta}$.

$\cR$ commits to $\widehat{\theta}$ and $\widehat{x}$ using \emph{statistically binding commitments}.

\item $\cC$ sends a random test subset $T \subset [{2\lambda^3}]$ of size ${\lambda^3}$ to $\cR$. 

\item For every $i \in T$, $\cR$ decommits to $(\widehat{\theta}_i,\widehat{x}_i)$, and $\cC$ aborts if any decommitment is invalid.

\item $\cC$ checks that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $\cC$ proceeds with the protocol,
otherwise, $\cC$ aborts. 
\end{enumerate}

Notice that $\cC$'s messages are completely independent of its bit $b$ up to this point. If $\cR$ passes the check above, then $\cC$ will obtain a $\secp^3$-bit string $x$ by measuring its qubits (i.e., EPR pair halves) in positions $\overline{T} \coloneqq [2\secp] \setminus T$ in the bases specified in $\theta$. $\cC$ then partitions $x$ into $\secp$ different $\secp^2$-bit strings strings $x^{(1)},\dots,x^{(\secp)}$ and sends the receiver
\[ (s_1,b \oplus h(s_1,x^{(1)})),\dots,(s_\secp,b \oplus h(s_\secp,x^{(\secp)})), \]
where each $s_1,\dots,s_\secp$ is a random seed for the universal hash function $h$. By the leftover hash lemma~\cref{thm:privacy-amplification}, $b$ will be statistically hidden if each $x^{(\ell)}$ has sufficient independent min-entropy.

To that end, observe (following~\cite[Section 5]{C:BouFeh10}) that the committer decides to accept the receiver's commitment openings $(\hat{\theta}_i,\hat{x}_i)_{i \in [T]}$ \emph{only if} a certain quantum sampling strategy succeeds. Since the commitments are statistically binding, the values of $\hat{x},\hat{\theta}$ that $\mathcal{C}$ would accept are statistically determined after $\mathcal{R}$ commits. Let $\ket{\psi}_{\gray{X}\gray{Y}}$ be the joint state of the committer and receiver where $\gray{X}$ corresponds to the committer's $2\secp^3$ registers, and $\gray{Y}$ corresponds to the receiver's state. Then the committer's check can only pass if the sampling strategy of~\cref{lemma:sampling} succeeds for the committed values of $\hat{x},\hat{\theta}$. We remark that while no efficient $\mathcal{C}$ can actually \emph{perform} this sampling strategy (as it involves breaking the computational hiding of the underlying equivocal commitments), its behavior is statistically indistinguishable from $\mathcal{C}$ that does perform this sampling. 

By setting the subset $S$ in~\cref{lemma:sampling} to be an arbitrary $\secp^2$-size subset of $\overline{T}$, we conclude that each $x^{(\ell)}$ must have min-entropy at least $\secp^2/3$. Applying~\cref{thm:privacy-amplification}, this implies that $s_\ell,h(s_\ell,x^{(\ell)})$ is statistically indistinguishable from uniform, and thus $b$ is statistically hidden.

\fi

==> sec-intro.tex <==
\section{Introduction}
\label{sec:intro}

The complexity of cryptographic primitives is central to the study of cryptography. Much of the work in the field focuses on establishing \emph{reductions} between different primitives, typically building more sophisticated primitives from simpler ones. Reductions imply relative measures of complexity among different functionalities, and over the years have resulted in an expansive hierarchy of assumptions and primitives, as well as separations between them.

One-way functions (OWFs) lie at the center of cryptographic complexity: their existence is the minimal assumption necessary for nearly all classical cryptography~\cite{STOC:LubRac86,FOCS:ImpLub89,STOC:ImpLevLub89}. One-way functions are equivalent to so-called ``minicrypt'' primitives like pseudorandom generators, pseudorandom functions and symmetric encryption; 
%but are believed to not imply public-key encryption\footnote{In particular,~\cite{C:ImpRud88,C:BarMah09} proved that  public-key encryption, }
but provably cannot imply key exchange when used in a black-box way~\cite{C:ImpRud88,C:BarMah09}\footnote{In particular,~\cite{C:ImpRud88,C:BarMah09} showed that there cannot exist a key exchange protocol that only has oracle access to the input/output behavior of a one-way function, and makes no additional assumptions. Then~\cite{TCC:Dachman-Soled16} ruled out the possibility of certain types of key exchange protocols that also make use of the {\em code} of a one-way function.  Constructions of key exchange from one-way functions have eluded researchers for decades. This, combined with the aforementioned negative results, is considered to be evidence that key exchange is a qualitatively stronger primitive than one-way functions in the classical regime. In fact, Impagliazzo~\cite{Impagliazzo} stipulates that we live in one of five possible worlds, of which {\em Minicrypt} is one where classical one-way functions exist but classical public-key cryptography does not.}.
%\fermi{todo: one-sentence explanation (can be a footnote) of what black-box means}
Thus, the existence of key exchange is believed to be a stronger assumption than the existence of one-way functions. Oblivious transfer (OT) %--- equivalently, secure computation ---
is believed to be \emph{even stronger}: it implies key exchange, but cannot be obtained from black-box use of a key exchange protocol~\cite{TCC:MahMajPra14}.

The importance of OT stems from the fact that it can be used to achieve secure computation, which is a central cryptographic primitive with widespread applications.
In a nutshell, secure computation allows mutually distrusting participants to compute any public function over their joint private inputs while revealing no private information beyond the output of the computation.

% \fermi{can we add a sentence here to the effect of ``indeed, many classical cryptographic primitives such as public-key encryption, oblivious transfer, private information retrieval, etc can be cast as specific instances of secure computation,'' (for less crypto-experienced readers to appreciate the significance of secure computation)}
% \dakshita{I'm not sure the real estate is worth it :) as in, I don't think this sentence will substantially affect anyone that is not already convinced by the previous sentences. Plus all the primitives you wrote are actually even special cases of OT.}\fermi{okay, fair enough!}

%In this work, we focus on a central primitive, namely secure computation.
%, and we study

%When participants have quantum computation and communication capabilities, 
\paragraph{The Quantum Landscape.}
The landscape of cryptographic possibilities changes significantly when participants have quantum computation and communication capabilities. 
%When participants have access to quantum capabilities and quantum communication channels, 
%In the quantum world, the landscape is very different.
For one, {\em unconditionally} secure key distribution --- commonly known as \emph{quantum key distribution} (QKD) --- becomes possible \cite{BenBra84}. 
Moreover, %techniques have been developed to 
%obtain 
\emph{quantum} oblivious transfer (QOT) is known to be achievable from special types of commitments, as we discuss next.

Crépeau and Kilian~\cite{FOCS:CreKil88} first proposed a protocol for QOT using quantum bit commitments.
%\footnote{While~\cite{C:BBCS91} is often cited as having introduced a template for building QOT from quantum one-way functions, the core template appeared earlier in~\cite{FOCS:CreKil88}. The work of~\cite{C:BBCS91} presents a transmission-error resistant version of the~\cite{FOCS:CreKil88} protocol, but our focus is on a model without transmission errors (or where transmission errors are handled separately).} 
The central idea in these QKD and QOT protocols is the use of (what are now known as) ``BB84 states''. These are single qubit states encoding either $0$ or $1$ in either the computational or Hadamard basis. Crucially, measuring (or essentially attempting to copy the encoded bit) in the wrong basis completely destroys information about the encoded bit. Then~\cite{C:BBCS91} presented a transmission-error resistant version of the~\cite{FOCS:CreKil88} protocol. These protocols did not come with a proof of security, but subsequently 
%The original~\cite{FOCS:CreKil88} proposal did not come with a proof of security. 
%The work of~\cite{C:BBCS91} presents a transmission-error resistant version of the~\cite{FOCS:CreKil88} protocol
Mayers and Salvail~\cite{MayersSalvail94} proved that the~\cite{FOCS:CreKil88} protocol is secure against a restricted class of attackers that only perform single-qubit measurements. This was later improved by Yao~\cite{STOC:Yao95}, who extended the~\cite{MayersSalvail94} result to handle general quantum adversaries.

By an unfortunate historical accident, the aforementioned security proofs claimed the \cite{FOCS:CreKil88} QOT could be \emph{information-theoretically secure}, since at the time it was believed that information-theoretic quantum bit commitment was possible~\cite{FOCS:BCJL93}. Several years later, Mayers~\cite{Mayers97} and Lo and Chau~\cite{LoChau97} independently proved the impossibility of information-theoretic quantum bit commitment, and as a consequence, the precise security of~\cite{FOCS:CreKil88} QOT was once again unclear. This state of affairs remained largely unchanged until 2009, when Damgard, Fehr, Lunemann, Salvail, and Schaffner \cite{C:DFLSS09} proved that bit commitment schemes satisfying certain additional properties, namely \emph{extraction and equivocation}, suffice to instantiate~\cite{FOCS:CreKil88} QOT.~\cite{C:DFLSS09} called their commitments {\em dual-mode} commitments, and provided a construction based on the quantum hardness of the learning with errors (QLWE) assumption. We remark that assumptions about the hardness of specific problems like QLWE are qualitatively even worse than general assumptions like QOWFs and QOT. Thus, the following basic question remains:
%\footnote{Simulation security (as opposed to indistinguishability-based security) is the standard notion of security for oblivious transfer, and more generally for secure computation. More discussion on this can be found in \cref{subsec:related work}.}
%Nevertheless, the following basic question remained:
\begin{center}
        {\em Do quantum-hard one-way functions suffice for quantum oblivious transfer?}
\end{center}
 \vspace{15pt}
% footnote that used to occur at the end of the previous question, commented out below:
% \footnote{Specifically, this question refers to the standard notion of oblivious transfer in the cryptographic literature, which is defined using a \emph{simulation-based} security definition. A previous work of~\cite{C:BouFeh10} answered this  question in the affirmative for a weaker definition of oblivious transfer, which is not known to suffice for secure computation. We refer the reader to~\cref{subsec:related work} for further discussion.}

% \vspace{5mm}
% an error stemming from   assumed that the ``measurement-check'' subprotocol in \cite{FOCS:CreKil88} could be implemented with \emph{information-theoretically secure} quantum commitments described by~\cite{FOCS:BCJL93}. However, Mayers~\cite{Mayers97} and Lo and Chau~\cite{LoChau97} later proved that the~\cite{FOCS:BCJL93} commitment scheme was flawed, and moreover that information-theoretically secure quantum bit commitments are \emph{impossible}. Thus, the protocol from \cite{FOCS:CreKil88} remained without a security proof until 2009, 
%certain 
%statistically binding and quantum computationally hiding 
% bit commitment schemes satisfying certain additional properties, namely extraction and equivocation, suffice.


%While quantum bit commitments satisfying the basic properties of statistical binding and quantum computational hiding can be obtained from post-quantum one-way functions, we note that the commitments required by \cite{C:DFLSS09} require particular extraction and equivocation properties. It has thus remained unclear whether such commitments can be built assuming only (quantum-hard) one-way functions.

\paragraph{Quantum OT: The Basis of Secure Quantum Computation.}
%The primary reason why OT is so well-studied in the classical literature is that it can be used to build 
%In the setting of \emph{malicious} attackers, the security guarantee is that participants that arbitrarily deviate from protocol specifications (1) can only recover information that is efficiently computable given their input and output at any point during the protocol execution, and (2) cannot cause honest players to obtain an incorrect output without being detected. 
%a very general primitive with widespread applications. This allows mutually distrustful parties holding inputs $x_A$ and $y_B$ respectively. They would like to evaluate a function $f$ on their joint input $(x_A, y_B)$. The output is of the form $f(x_A, y_B) = (y_A, y_B)$, so at the end of the protocol Alice and Bob wish to output $y_A$ and $y_B$ respectively. In the setting of \emph{malicious} attackers, the security guarantee is that a malicious Alice (resp. Bob) who may arbitrarily deviate from the protocol specifications (1) can only hold information that is efficiently computable from either her input or output at any point during the protocol execution, and (2) cannot cause Bob (resp. Alice) to obtain an incorrect outcome of the protocol without being detected. 
%These guarantees are formalized via a simulation-based security notion, which requires that no adversary can recover any information in the real world that it cannot recover in an ideal world where it simply hands its input to a trusted party who then returns the output.
There is a natural extension of secure computation to the quantum world, where Alice and Bob wish to compute a \emph{quantum} circuit on (possibly entangled) \emph{quantum} input states.
This setting,
usually referred to as secure \emph{quantum} computation, has been previously studied and in fact has a strong tradition in the quantum cryptography literature. 
%This setting is 

%\dakshita{Add difference between UC and stand alone security. Emphasize that stand alone is great.}

\cite{STOC:CreGotSmi02,FOCS:BCGHS06} constructed unconditional maliciously-secure \emph{multi-party} quantum computation with honest majority. The setting where half (or more) of the players are malicious requires computational assumptions due to the impossibility of unconditionally secure quantum bit commitment~\cite{Mayers97,LoChau97}. 

In this computational setting,~\cite{C:DupNieSal10,DNS12} showed the feasibility of two-party quantum computation (2PQC) assuming post-quantum OT.
%the quantum analogue of semi-honest adversaries (specious adversaries); and this was later extended to the malicious setting by~\cite{DNS12}. 
%\dakshita{assumptions?}
More recently,~\cite{EC:DGJMS20} constructed maliciously-secure general multi-party quantum computation (MPQC) secure against a \emph{dishonest} majority from any maliciously-secure post-quantum multi-party computation (MPC) protocol for classical functionalities, which can itself be obtained from post-quantum OT~\cite{ABGKM20}. 

Nevertheless, the following natural question has remained unanswered:
\begin{center}
%{\em What are the minimal (classical) assumptions from which multiparty (quantum) computation can be built?}
{\em Can secure (quantum) computation be obtained from quantum-hard one-way functions?}
\end{center}
%
%In this paper, we study the following question:
%\begin{center}
%{\em What are the minimal (classical) assumptions from which multiparty (quantum) computation can be built?}
%\end{center}

\subsection{Our Results}
\label{subsec: our results}
Our main result is the following:
\begin{center}
{\em %In the standard model, 
%quantum-hard one-way functions imply the existence of quantum oblivious transfer.} 
Quantum oblivious transfer can be based on the %minimal (classical) 
assumption that quantum-hard one-way functions exist. }
\end{center}

In fact, we prove a stronger result: 
we show that quantum oblivious transfer can be based on the {\em black-box use of any statistically binding, quantum computationally hiding commitment}. Such commitments can be based on the black-box use of quantum-hard one-way functions.
This in turn implies secure two-party computation of classical functionalities, in the presence of quantum computation and communication capabilities, from (black-box use of) quantum-hard one-way functions~\cite{STOC:Kilian88}. The latter can then be used to obtain secure two-party \emph{quantum} computation, by relying on the work of~\cite{DNS12}.
Quantum OT can also be used to obtain {\em multi-party} secure computation of all classical functionalities, in the presence of quantum computation and communication capabilities, and additionally assuming the existence of authenticated channels. This follows from the techniques in~\cite{STOC:Kilian88,C:CreVanTap95,C:DamIsh05,C:IshPraSah08} which obtain classical MPC based on black-box use of any OT protocol.
By relying on~\cite{EC:DGJMS20}, this also implies multi-party secure {\em quantum} computation. 

In summary, our main result implies that: (1) 2PQC can be obtained from (black-box use of) quantum-hard OWFs and  (2) assuming the existence of authenticated channels, MPQC can be obtained from (black-box use of) quantum-hard OWFs.

This gives a potential separation between the complexity of cryptographic primitives in the classical and quantum worlds. In the former, (two-party) secure computation provably cannot be based on black-box use of quantum-hard one-way functions. It is only known from special types of enhanced public-key encryption schemes or from the hardness of specific problems, both of which are believed to be much stronger assumptions than one-way functions. But in the quantum world, prior to our work, (two-party) secure computation was only known from the special commitments required in the protocol of \cite{C:DFLSS09}, which can be based on QLWE following~\cite{C:DFLSS09}, or post-quantum OT  (implicit in~\cite{C:HalSmiSon11,STOC:BS20,ABGKM20}) --- but were not known to be achievable from quantum-hard one-way functions.

%In fact, we make black-box use of any statistically binding, computationally hiding commitment, which can itself be based on the black-box use of any one-way function.

%\dakshita{added paragraph below.}
\paragraph{On the Significance of the Black-Box use of Cryptography in the Quantum Setting.}
Making black-box use of a cryptographic primitive refers to only having oracle access to its input/output behavior, without having the ability to examine the actual code (i.e., representation as a sequence of symbols) of the primitive. For instance, proving in zero-knowledge that a committed value satisfies some given predicate often requires explicit knowledge of the commitment algorithm; classifying the resulting proof as making ``non-black-box'' use of the one-way function. 
In the literature, constructions that make black-box use of cryptographic primitives are often  preferred over those that make non-black-box use of cryptography. Besides their conceptual simplicity and elegance, black-box constructions are also of practical interest since they avoid expensive NP reductions involving circuits of primitives.
Perhaps most importantly, in the case of black-box constructions, one can instantiate the underlying primitive with an arbitrary implementation, including physical implementations via secure hardware or those involving quantum communication.


In many quantum protocols, which involve quantum states being transferred between two or more players, black-box constructions are not only significantly preferable but often become {\em a necessity}. Let us illustrate this with the help of an example. The GMW protocol~\cite{C:GolMicWig86} first showed that secure multi-party computation can be based on any oblivious transfer protocol; however the protocol involved zero-knowledge proofs involving the description of the (classical) oblivious transfer protocol. Due to the GMW~\cite{C:GolMicWig86} protocol being non-black-box in the underlying OT, our OT protocols cannot be used with GMW to obtain multi-party computation of classical functionalities. We instead need to rely on compilers like~\cite{STOC:Kilian88,C:CreVanTap95,C:DamIsh05,C:IshPraSah08} that only make {\em black-box use} of the underlying OT protocol. As discussed above, the black-box nature of these compilers makes them applicable irrespective of whether they are instantiated with classical or quantum OT.

In a similar vein, we believe that our {\em black-box} use of any statistically binding, quantum computationally hiding commitment in our QOT protocol is of particular significance. 
For instance, one can substitute our statistically binding, quantum computationally hiding commitment with an unconditionally secure one in the quantum random oracle model~\cite{C:Unruh14}, resulting in {\em unconditional quantum OT in the quantum random oracle model}.
%This makes it possible to instantiate our compiler even with a suitable commitment that involves quantum communication. 
Moreover if in the future, new constructions of statistically binding, quantum computationally hiding commitments involving quantum communication are discovered based on assumptions weaker than quantum-hard one-way functions, it would be possible to plug those right into our protocol compilers to obtain QOT. 
These applications would not have been possible had we required non-black-box use of the underlying commitment.
%In what follows, we argue that black-box constructions are not only  in the quantum setting. 

\paragraph{Primary Tool: Stand-alone Extractable and Equivocal Commitments.}
As discussed earlier, \cite{C:DFLSS09} show that simulation-secure QOT can be obtained from commitments satisfying certain properties, namely \emph{extraction} and \emph{equivocation}. 
\begin{itemize}
    \item At a high level, extraction requires that there exist an efficient quantum ``extractor'' that is able to extract a committed message from any quantum committer.  
    \item Equivocality requires that there exist an efficient quantum ``equivocator'' capable of simulating an interaction with any quantum receiver such that it can later open the commitment to any message of its choice.
\end{itemize}

These two properties are crucial for proving simulation security of the \cite{FOCS:CreKil88} OT protocol: extraction implies receiver security and equivocality implies sender security\footnote{It is important to note that extraction and equivocation are only made possible in an ideal world where a simulator has access to the adversary's state. Participants in the real protocol cannot access each others' state, which prevents them from extracting or equivocating.}. Our key technical contribution is the following:
\begin{center}
    {\em Extractable and equivocal commitments can be based on the black-box use of\\ quantum-hard one-way functions.}
\end{center}
%a construction of {\em extractable and equivocal commitments} in the plain model, based on via the following two technical steps.
We obtain this result via the following transformations, each of which only makes \emph{black-box} use of the underlying primitives.
\begin{itemize}
    \item {\em Step 1: Quantum Equivocal Commitments from Quantum-Hard One-Way Functions.} We describe a generic unconditional compiler to turn any commitment into an equivocal commitment in the plain model. 
    % This compiler makes black-box use of the underlying commitment.
    %, which will be crucial for a subsequent step, when we apply it to a commitment that involves quantum communication. For this step, we need only 
    By applying our compiler to Naor's statistically binding commitment~\cite{JC:Naor91} --- which can be based on quantum-hard one-way functions --- we obtain a statistically binding, equivocal commitment.

    \item {\em Step 2: Quantum Extractable Commitments from Quantum Equivocal Commitments.}
    We show that  the~\cite{FOCS:CreKil88,C:DFLSS09,C:BouFeh10} framework can be used to obtain an extractable commitment that leverages quantum communication, and can be based on the existence of any quantum equivocal commitment.
    This combined with the previous step implies the existence of quantum extractable commitments based on the existence of quantum-hard one-way functions. 
    
    This is in contrast to existing approaches (eg.,~\cite{C:HalSmiSon11}) that require classical communication but rely on qualitatively stronger assumptions like classical OT with post-quantum security.
    \item {\em Step 3: From Extractable Commitments to Extractable and Equivocal Commitments.} We apply the black-box equivocality compiler from the first step to the quantum extractable commitment obtained above, to produce an extractable and equivocal commitment. 
    
    We point out that it is generally straightforward to make a classical commitment equivocal using zero-knowledge proofs, but this approach does not apply to quantum commitment protocols. We therefore devise our own equivocality compiler capable of handling quantum commitments and use it in both Step 1 and Step 3.
    
    % Moreover, our compiler only makes black-box use of the underlying commitment, which
    
    % this approach does not work our equivocality compiler must be able to compile a quantum commitment. Therefore, generic techniques from the classical setting do not apply.
    
    % Since this step requires us to make a quantum commitment protocol equivocal, we could not directly rely on simple equivocality compilers in the classical cryptography literature. Indeed, generic compilers in the classical setting, in addition to not necessarily being quantum-capable, break down in the setting of quantum communication due to the need to make non-black-box use of the underlying commitment. 
    
    %For example, one way to obtain the equivocality property is as follows. In the opening phase, to open to a bit $b$, the committer does not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$. Equivocation is achieved by simulating the ZK proof. Unfortunately, this technique fails when the commitment involves \emph{quantum} communication, since the statement to be proven is no longer an \textsf{NP} statement (nor a \textsf{QMA} statement).
    %Therefore, we construct a compiler that only makes black-box use of the underlying commitment, and leverages Watrous's rewinding lemma in the proof of equivocality~\cite{STOC:Watrous06}.
    
    
    %Our second technical contribution is a generic unconditional compiler from quantum extractable commitments to quantum extractable and \emph{equivocal} commitments. 
    %Such compilers are known in the classical setting, but break down 
    %in the setting of quantum communication
    %, natural candidate protocols from the classical literature break down 
    %due to the need to make non-black-box use of the underlying commitment. For example, one way to obtain the equivocality property is as follows. In the opening phase, to open to a bit $b$, the committer does not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$.

   %Unfortunately, this technique fails when the commitment involves \emph{quantum} communication, since the statement to be proven is no longer an \textsf{NP} statement (nor a \textsf{QMA} statement).
    %Therefore, we build a new protocol that only makes black-box use of the underlying commitment, and leverages Watrous's rewinding lemma in the proof of equivocality~\cite{STOC:Watrous06}.
    %In the classical setting, such a bootstrapping can be achieved using known techniques. Typically one would obtain the equivocality property as follows. In the opening phase, to open to a bit $b$, the committer does not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$.
    %Existing approaches to constructing extractable commitments against quantum adversaries (implicit in~\cite{C:HalSmiSon11,STOC:BS20,TCC:ALP20}) do not 
    %specific assumptions like Learning with Errors (LWE) and Fully Homomorphic Encryption (FHE).
\end{itemize}

Plugging our quantum extractable and equivocal commitments into the~\cite{FOCS:CreKil88} framework yields a final QOT protocol with an interaction pattern that readers familiar with~\cite{BenBra84,FOCS:CreKil88} may find interesting: the sender sends the receiver several BB84 states, after which the receiver proves to the sender that it has honestly measured the sender's BB84 states by  \emph{generating more BB84 states of their own and asking the sender to prove that they have measured the receiver's BB84 states.}
% To the best of the authors' knowledge, all previously known cryptographic protocols derived from~\cite{BenBra84} start with a single transmission of random BB84 states, followed by exclusively classical messages.
An intriguing open question is whether obtaining QOT from one-way functions \emph{requires} this type of two-way quantum communication or, alternatively, quantum memory.\footnote{Naive approaches to removing one direction of quantum communication appear to require the honest parties to be entangled and subsequently perform quantum teleportation.}


% Interestingly, our final QOT protocol that results from instantiating the \cite{FOCS:CreKil88} framework with the quantum commitments described above requires either \emph{two-way} quantum communication or quantum memory,\footnote{Removing one direction of quantum communication would require the honest parties to be entangled and subsequently perform quantum teleportation.} since the extractable commitment that we build crucially relies on quantum communication from the committer to the receiver. An intriguing question is whether this extra quantum communication (beyond that required by the \cite{FOCS:CreKil88} framework) is necessary to obtain simulation-based oblivious transfer from one-way functions.

\iffalse{
\paragraph{On The Minimality of Quantum One-Way Functions.}
All classical cryptographic primitives imply one-way functions, therefore these are considered the `minimal' cryptographic assumption in the classical world. But the same may not be true when participants have access to quantum resources and quantum communication channels. In this setting, it is not known whether primitives like quantum bit commitments and quantum OT can plausibly be realized from assumptions that are qualitatively even weaker than the existence of (quantum-hard) one-way functions. 
\dakshita{what else can we say here?}
}\fi
%Yet, the result by Mayers does not preclude the possibility of constructing quantum commitment protocols (and thus secure multi-party computation protocols) under assumptions that are much weaker than the assumptions needed for commitment protocols that do not use quantum communication.
%\paragraph{Extractable commitments from one-way functions} Previous works have only considered possible classical constructions of extractable commitments. Our main insight is that extractable commitments can be constructed \emph{quantumly} using the same BB84 idea, in conjunction with post-quantum ZK proofs, which can be obtained from one-way functions (see footnote 1 in Section \ref{sec: tech ovw ext com from owf}). 

%\paragraph{Extractable and \emph{equivocal} commitments from extractable commitments} Our second technical contribution is a generic construction of post-quantum secure extractable and \emph{equivocal} commitments from post-quantum secure equivocal commitments. In the classical setting, such a bootstrapping can be achieved using known techniques. Typically one would obtain the equivocality property as follows. In the opening phase, to open to a bit $b$, the committer does not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$.

%Unfortunately, this technique fails when the commitment involves \emph{quantum} communication, since the statement to be proven is no longer an \textsf{NP} statement (nor a \textsf{QMA} statement).

%To overcome this, we build a novel protocol, and we leverage Watrous' rewinding lemma in the proof of equivocality.


%Our result demonstrates that quantum-hard one-way functions suffice.



\subsection{Related Work}
\label{subsec:related work}

%\paragraph{Indistinguishability-Based vs. Simulation-Based Security.} 
For some readers, it may appear that the central claim of this work --- that quantum-hard one-way functions suffice for oblivious transfer --- has already been established~\cite{C:DFLSS09,C:BouFeh10}. Indeed, prior work~\cite{C:DFLSS09,C:BouFeh10} showed that statistically binding and computational hiding commitments (which are weaker than extractable and equivocal commitments), known to exist from one-way functions, can be plugged into the~\cite{FOCS:CreKil88} template to achieve an oblivious transfer protocol satisfying \emph{indistinguishability-based} security. 

However, the indistinguishability-based security definition for oblivious transfer is \emph{not} standard in the cryptographic literature. When cryptographers refer to ``oblivious transfer'', they almost always mean the standard \emph{simulation-based} security notion. Indeed, the fundamental importance of oblivious transfer in modern cryptography is due to the fact that it is necessary and sufficient for secure computation, but this is only true for the simulation-based notion.

\ifsubmission
\else
Therefore, the goal of this work is to build simulation-secure oblivious transfer, and thereby establish that quantum-hard one-way functions suffice for secure quantum computation. We elaborate further on the details of simulation security in~\cref{sec:techniques}.


We also note that in the setting of Universal Composability (UC), Unruh~\cite{C:Unruh07} obtained quantum oblivious transfer from quantum UC-secure commitments in the common reference string (CRS) model. By contrast, in this work, we focus on the standalone setting in the plain/standard model, and we do not assume the existence of trusted setup or a common reference string. In this setting, we obtain quantum oblivious transfer from quantum-hard one-way functions. 
\fi


\subsection{Concurrent and Independent Work}
In a concurrent and independent work, Grilo, Lin, Song, and Vaikuntanathan~\cite{GLSV} also construct simulation-secure quantum oblivious transfer from quantum-hard one way functions via the intermediate primitive of extractable and equivocal commitments. However, the two works take entirely different approaches to constructing these commitments. We briefly summarize these strategies below.\\

\noindent\underline{This work:}
\begin{enumerate}
\item Construct equivocal commitments from statistically binding commitments via a new ``equivocality compiler'' based on Watrous~\cite{STOC:Watrous06} rewinding.
\item Construct extractable commitments from equivocal commitments via a new “extractability compiler” based on the~\cite{FOCS:CreKil88} template.
\item Construct extractable and equivocal commitments from extractable commitments via the same compiler from Step 1.
\end{enumerate}

\noindent\underline{\cite{GLSV}}:
\begin{enumerate}
\item Construct selective opening secure commitments with inefficient simulation against malicious committers from statistically binding commitments and zero-knowledge proofs.
\item Construct QOT with inefficient simulation against malicious receivers from selective opening secure commitments with inefficient simulation against malicious committers, following the~\cite{FOCS:CreKil88} QOT template.\footnote{\cite{GLSV} point out that the conclusions of Steps 1 and 2 together had also been established in prior works of~\cite{C:Unruh07,C:DFLSS09,C:BouFeh10}.}
\item Construct parallel QOT with inefficient simulation against malicious receivers from (stand-alone) QOT with inefficient simulation against malicious receivers via a new lemma for parallel repetition of protocols.
\item Construct verifiable conditional disclosure of secrets, a new primitive introduced in~\cite{GLSV}, from parallel QOT with inefficient simulation against malicious receivers, statistically binding commitments, Yao’s garbled circuits, and zero-knowledge proofs.
\item Construct extractable commitments from verifiable conditional disclosure of secrets, statistically binding commitments, and zero-knowledge proofs.
\item Construct extractable and equivocal commitments from extractable commitments and zero-knowledge proofs.
\end{enumerate}



We believe that our result is easier to understand and conceptually simpler, as we do not need to define additional primitives beyond extractable and/or equivocal commitments. Aside from differences in approach, there are several other places where the results differ:
\begin{itemize}
\item \textbf{This Work: Black-Box Use of One-Way Functions.} A significant advantage of our work over~\cite{GLSV} is that we construct quantum OT from {\em black-box use} of statistically binding commitments or one-way functions. The OT in~\cite{GLSV} makes non-black-box use of the underlying one-way function.
As discussed above, making black-box use of underlying cryptographic primitives is particularly useful in the quantum setting. Due to the extensive use of zero-knowledge proofs and garbled circuits in~\cite{GLSV}, it appears difficult to modify their approach to be black-box in the underlying one-way function.
\item \textbf{This Work: One-Sided Statistical Security.} Additionally, our oblivious transfer protocol offers {\em one-sided statistical security}. As written, our quantum OT protocol satisfies statistical security against malicious senders (and computational security against malicious receivers). Moreover, this OT can be reversed following the techniques in eg.,~\cite{EC:WolWul06} to obtain a quantum OT protocol that satisfies statistical security against malicious receivers (and computational security against malicious senders). 
On the other hand, the quantum OT protocol in~\cite{GLSV} appears to achieve computational security against both malicious senders and malicious receivers.
\item \textbf{\cite{GLSV}: Verifiable Conditional Disclosure of Secrets.} Towards achieving their main result, \cite{GLSV} introduce and construct verifiable conditional disclosure of secrets (vCDS). This primitive may be of independent interest.
%, and there is no analogue of it in this work.
\item \textbf{\cite{GLSV}: Constant Rounds in the CRS Model.} While both works construct $\poly(\secp)$-round protocols in the plain model, \cite{GLSV} additionally construct a constant round OT protocol in the CRS model based on (non-black-box use of) quantum-hard one-way functions. 

\ifsubmission
\emph{In an earlier version of this work, we did not consider the CRS model. After both works were posted to the Cryptology ePrint Archive (ours on November 26, 2020 and \cite{GLSV} on November 30, 2020), we realized that our techniques could be straightforwardly adapted to achieve constant round complexity in the CRS model, while still making black-box use of one-way functions. For the interested reader, we sketch how this can be achieved in the supplementary materials. We re-emphasize that this brief discussion of CRS model technique, limited to page 8 of our supplementary materials, is the only component of this work that was not concurrently developed independently of~\cite{GLSV}.}
\else
\emph{In an earlier version of this work, we did not consider the CRS model. After both works were posted to the Cryptology ePrint Archive (ours on November 26, 2020 and \cite{GLSV} on November 30, 2020), we realized that our techniques could be adapted straightforwardly to achieve constant round complexity in the CRS model, while still making black-box use of one-way functions. We elaborate further on this below.}
\fi
\end{itemize}

\ifsubmission
\else
\paragraph{Constant Rounds in the CRS Model via Our Techniques.} We now briefly sketch how the protocols in this work can be modified to achieve constant rounds in the CRS model. The following two paragraphs are the only component of this work that was not developed concurrently and independently of \cite{GLSV}.

%, from black-box use of quantum-hard one-way functions. 
In a nutshell, the reason why our protocols require super-constant rounds in the plain model is because they perform sequential repetitions of specific $\Sigma$-protocols to enable rewinding.
%is that we apply Watrous' rewinding lemma to a specific quantum $\Sigma$-protocol (we refer the reader to the equivocality compiler described in Section \ref{sec: equivocal commitment}) that must be sequentially repeated $\lambda$ times.
In the presence of a CRS, it is possible to repeat our protocols in parallel and simulate by means of a trapdoor embedded in the CRS. This avoids the need for rewinding (and therefore sequential repetition), and would bring down the number of rounds from $O(\lambda)$ to $O(1)$ in the CRS model.

In fact, constant round QOT can also be based on the {\em black-box use} of quantum-hard one-way functions in the presence of a CRS by slightly modifying our template, as follows.
Recall that the first step towards getting a constant round protocol is to replace (all of) our sequential repetitions with parallel repetitions.
The challenge for the parallel repetitions can be determined as the outcome of a (one-sided simulatable) coin toss. This coin toss can be carefully designed so that a simulator that programs the CRS can program the output of the coin toss, which would allow the simulator to program the challenge message for the parallel repetition. 
%The ability to program the output of the coin toss also helps simulate the parallel repetition of our $\Sigma$ protocol. 
In the CRS model, such a coin toss can be obtained by having one player commit to a random set of coins via Naor's commitment~\cite{JC:Naor91} (where the first message of the commitment is the CRS). Next, the second player sends their random coins, in the clear, to the first player. Finally, the first player decommits their initial commitment string, and the players set the output of the coin toss to be the XOR of the random coins chosen by each player. A simulator can program the output of the coin toss by programming the CRS to equivocate Naor's commitment. This programming would allow one to simulate the parallel repeated versions of our protocols. 
We note that this protocol has the drawback of the CRS not being reusable, unlike the CRS-based protocol in~\cite{GLSV}.
We stress that our focus is on the plain model, and we leave formal explorations/optimizations of this and related  approaches to building black-box OT in the CRS model to future work.

\fi

% In this work, our focus is on feasibility results, and therefore we restrict ourselves to the plain model where parties do not require access to any trusted setup or common string. In this model, we obtain quantum oblivious transfer from black-box use of quantum-hard one-way functions with a number of rounds that grow linearly with the security parameter.
% We re-emphasize that all results in this paper were developed concurrently and independently of~\cite{GLSV}.



%We do not formally develop this approach in this work because the observation about constant round protocols from black-box use of one-way functions in the CRS model, was made subsequent to the initial posting of this work and the concurrent work of~\cite{GLSV}. 



%Finally, we note that the length of the CRS bounds the number of sessions that can be simulated at any given time. Removing this limitation is an interesting question for future work.

%one can start with Naor's commitment, which is equivocal in the CRS model and can be based on black-box use of one-way functions. Such a commitment can be used to build a coin-tossing protocol where the coin toss is fully simulatable by one player. Now, 
%\dakshita{Talk about UC security - emphasize that standalone is great}

%Our result directly extends to \emph{multi-party} quantum computations, by additionally assuming authenticated channels.

\iffalse{
\subsection{Techniques}
As discussed earlier in the introduction, \cite{C:DFLSS09} show that simulation-secure OT can be obtained from commitments satisfying certain \emph{extraction} and \emph{equivocality} properties. 
\begin{itemize}
    \item Extraction informally requires that there exist an efficient ``extractor'', with access to the committer, that is able to extract its committed value.  
    \item Equivocality informally requires that there exist an efficient simulator, with access to the receiver, that is able to open a commitment to any value of its choice.
\end{itemize}

The two properties are crucial for proving simulation security of the \cite{FOCS:CreKil88} OT protocol: extraction for receiver security, and equivocality for sender security. Our key technical contribution is a construction of {\em extractable and equivocal commitments} in the plain model, based on via the following two technical steps.

\paragraph{Extractable commitments from one-way functions} Previous works have only considered possible classical constructions of extractable commitments. Our main insight is that extractable commitments can be constructed \emph{quantumly} using the same BB84 idea, in conjunction with post-quantum ZK proofs, which can be obtained from one-way functions (see footnote 1 in Section \ref{sec: tech ovw ext com from owf}). 

\paragraph{Extractable and \emph{equivocal} commitments from extractable commitments} Our second technical contribution is a generic construction of post-quantum secure extractable and \emph{equivocal} commitments from post-quantum secure equivocal commitments. In the classical setting, such a bootstrapping can be achieved using known techniques. Typically one would obtain the equivocality property as follows. In the opening phase, to open to a bit $b$, the committer does not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$.

Unfortunately, this technique fails when the commitment involves \emph{quantum} communication, since the statement to be proven is no longer an \textsf{NP} statement (nor a \textsf{QMA} statement).

To overcome this, we build a novel protocol, and we leverage Watrous' rewinding lemma in the proof of equivocality.
}\fi





==> sec-prelim.tex <==
\section{Preliminaries}

\paragraph{Notation.} We will write density matrices/quantum random variables (henceforth, QRVs) in lowercase bold font, e.g. $\bx$. A quantum register $\gray{X}$ will be written in uppercase (grey) serif font. A collection of (possibly entangled) QRVs will be written as $(\bx,\by,\bz)$.

Throughout this paper, $\lambda$ will denote a cryptographic security parameter. We say that a function $\mu(\lambda)$ is \emph{negligible} if $\mu(\lambda) = 1/\lambda^{\omega(1)}$.

The trace distance between two QRVs $\bx$ and $\by$ will be written as $\|\bx - \by\|_1$. Recall that the trace distance captures the maximum probability that two QRVs can be distinguished by any (potentially inefficient) procedure. We therefore say that two infinite collections of QRVs $\{\bx_\secp\}_{\secp \in \bbN}$ and $\{\by_\secp\}_{\secp \in \bbN}$ are \emph{statistically indistinguishable} if there exists a negligible function $\mu(\lambda)$ such that $||\bx_\secp - \by_\secp||_1 \leq \mu(\secp)$, and we will frequently denote this with the shorthand $\{\bx_\lambda\}_{\lambda \in \mathbb{N}} \approx_s \{\by_\lambda\}_{\lambda \in \mathbb{N}}$.

% This corresponds to the fact that there does not exist a quantum procedure that  we write $$\{\bx_\secp\}_{\secp \in \bbN} \approx_s \{\by_\secp\}_{\secp \in \bbN}$$ to mean that there exists a negligible function $\mu(\cdot)$ such that 

% We will write QRVs in lowercase bold font and quantum registers with uppercase gray font. A collection of QRVs $(\bx,\by,\bz)$ on registers $\gray{X},\gray{Y},\gray{Z}$ is also a QRV, and $\bx,\by,\bz$ may or may not be entangled with each other.

\paragraph{Non-Uniform Quantum Advice.} 
We will consider non-uniform quantum polynomial-time (QPT) algorithms \emph{with quantum advice}, denoted by $\cA = \{\cA_\secp,\brho_\secp\}_{\secp \in \bbN}$, where each $\cA_\secp$ is the classical description of a $\poly(\secp)$-size quantum circuit, and each $\brho_\secp$ is some (not necessarily efficiently computable) non-uniform $\poly(\secp)$-qubit quantum advice. We remark that ``non-uniform quantum polynomial-time algorithms'' often means non-uniform \emph{classical advice}, but the cryptographic applications in this work will require us to explicitly consider quantum advice.

\ifsubmission
\else

Therefore, \emph{computational indistinguishability} will be defined with respect to non-uniform QPT distinguishers with quantum advice. That is, two infinite collections of QRVs $\{\bx_\secp\}_{\secp \in \bbN}$ and $\{\by_\secp\}_{\secp \in \bbN}$ are computationally indistinguishable if there exists a negligible function $\mu(\cdot)$ such that for all QPT distinguishers $\cD = \{\cD_\secp,\bsigma_\secp\}_{\secp \in \bbN}$, \[\left|\Pr[\cD_\secp(\bsigma_\secp,\bx_\secp) = 1] - \Pr[\cD_\secp(\bsigma_\secp,\by_\secp) = 1] \right| \leq \mu(\secp).\]
We will frequently denote this with the shorthand $\{\bx_\secp\}_{\secp \in \bbN} \approx_c \{\by_\secp\}_{\secp \in \bbN}$.

\fi

% In addition, we write $$\{\bx_\secp\}_{\secp \in \bbN} \approx_c \{\by_\secp\}_{\secp \in \bbN}$$ to indicate that there exists a negligible function $\mu(\cdot)$ such that for all QPT distinguishers $\cD = \{\cD_\secp,\bsigma_\secp\}_{\secp \in \bbN}$, $$\left|\Pr[\cD_\secp(\bsigma_\secp,\bx_\secp) = 1] - \Pr[\cD_\secp(\bsigma_\secp,\by_\secp) = 1] \right| \leq \mu(\secp).$$ Here, the $c$ refers to ``computational'' indistinguishability.

\ifsubmission

\paragraph{Definitions for Cryptographic Commitments.} Full definitions of cryptographic commitments can be found in the supplementary materials.

\else

\subsection{Commitments}

\subsubsection{Bit Commitments}
\label{subsec: com definitions}
We define bit commitments with quantum players and quantum communication. First, we fix some notation.

A bit commitment scheme is a two-phase interactive protocol between a quantum interactive committer $\cC = (\cC_{\com},\cC_{\open})$ and a quantum interactive receiver $\cR = (\cR_{\com},\cR_{\open})$. In the commit phase, $\cC_{\com}(1^\secp,b)$ for bit $b \in \zo$ interacts with $\cR_{\com}(1^\secp)$, after which $\cC_{\com}$ outputs a state $\bx_{\com}$ and $\cR_{\com}$ outputs a state $\by_{\com}$. We denote this interaction by $(\bx_\com,\by_\com) \gets \langle \cC(1^\secp,b),\cR(1^\secp)\rangle$. 

In the open phase, $\cC_\open(\bx_{\com})$ interacts with $\cR_\open(\by_{\com})$, after which $\cR_\open$ either outputs a bit $b'$ or $\bot$. We will denote this receiver's output by $\mathsf{OUT}_\cR\langle \cC_\open(\bx_\com),\cR_\open(\by_\com)\rangle.$

%We will let $\bx_{\final}$ denote the final state of $\cC_\open$ at the end of the open phase, and $\by_{\final}$ denote the final state of $\cR_\open$ at the end of the open phase.

First, we give the standard notions of hiding and binding. 
\begin{definition}[Hiding Commitment]
\label{def:hiding}
A bit commitment scheme is computationally (resp. statistically) \emph{hiding} if the following holds. For any polynomial-size (resp. unbounded-size) receiver $\cR_\com^* = \{\cR_{\com,\lambda}^*,\brho_\lambda\}$ interacting in the commit phase of the protocol, let $\mathsf{OUT}_\cR\langle \cC_\com(1^\lambda,b),\cR_{\com,\lambda}^*(\brho_\lambda)\rangle$ denote a bit output by $\cR_{\com,\lambda}^*$ after interaction with an honest $\cC_\com$ committing to message $b$. Then for every polynomial-size (resp. unbounded-size) receiver $\cR_\com^* = \{\cR_{\com,\lambda}^*,\brho_\lambda\}$, there exists a negligible function $\nu(\cdot)$ such that $$\left|\Pr[\mathsf{OUT}_\cR\langle\cC_\com(1^\lambda,0),\cR_{\com,\lambda}^*(\brho_\lambda)\rangle = 1] - \Pr[\mathsf{OUT}_\cR\langle\cC_\com(1^\lambda,1),\cR_{\com,\lambda}^*(\brho_\lambda)\rangle = 1]\right| = \nu(\lambda).$$
\end{definition}

% \begin{definition}[Binding Commitment]
% \label{def:binding}
% A bit commitment scheme is computationally (resp. statistically) \emph{binding} if for every polynomial-size (resp. unbounded-size) committer $\cC^* = \{\cC^*_{\com,\lambda},\cC^*_{\open,\lambda},\brho_\lambda\}$, there exists a negligible function $\nu(\cdot)$ such that with probability $\geq 1-\nu(\secp)$ over $(\bx_\com,\by_\com) \gets \langle \cC^*_\com(\brho),\cR(1^\secp)\rangle$ (where the indexing by $\lambda$ is omitted for convenience), there exists a bit $b \in \{0,1\}$ such that $$\Pr[\mathsf{OUT}_\cR\langle \cC^*_\open(\bx_\com),\cR_\open(\by_\com)\rangle = b] \leq \nu(\lambda).$$
% \end{definition}

\begin{definition}[Statistically Binding Commitment]
\label{def:binding}
A bit commitment scheme is statistically binding if for every unbounded-size committer $\cC^*_{\com}$, there exists a negligible function $\nu(\cdot)$ such that with probability at least $1-\nu(\secp)$ over $(\bx_\com,\by_\com) \gets \langle \cC^*_{\com},\cR(1^\lambda) \rangle$, there exists a bit $b \in \{0,1\}$ such that $$\Pr[\mathsf{OUT}_\cR\langle \cC^*_{\open}(1^\lambda, \bx_{\com}),\cR_\open(1^\lambda,\by_\com)\rangle = b] \leq \nu(\lambda).$$
\end{definition}

We will not consider (plain) computationally binding commitments in this work. We remark that there are subtleties to consider when defining computationally binding commitment secure against quantum attackers, and that the ``right'' definition appears to be Unruh's notion of collapse-binding~\cite{EC:Unruh16}. However, for this work, computational notions of binding will only arise in the context of \emph{extractable commitments}, which can be seen as a strong form of computationally binding commitments.

Post-quantum bit commitments satisfying computational hiding and statistical binding can be constructed from any post-quantum pseudorandom generator (PRG)~\cite{JC:Naor91}.\footnote{In Naor's protocol, the receiver first sends a uniformly random $u \gets \{0,1\}^{\lambda^3}$, and the committer commits to bit $b$ by sending $(b \cdot u) \oplus G(s)$, where $s \gets \{0,1\}^\secp$ and $G$ is a length-tripling PRG.} Watrous~\cite{STOC:Watrous06} considers PRGs built from (post-quantum) one-way \emph{permutations} via a ``quantum Goldreich-Levin Theorem'' of~\cite{AdcockCleve02}. However, Aaronson~\cite{Aaronson09} and Zhandry~\cite{FOCS:Zhandry12} later pointed out that the original~\cite{HILL99} construction of PRGs from one-way \emph{functions}  extends to non-uniform quantum adversaries with \emph{classical} advice. This can be extended to handle non-uniform {quantum} advice by giving the one-way function attacker constructed in the~\cite{HILL99} reduction many copies of the PRG attacker's non-uniform quantum advice (which only requires some polynomial upper bound on the number of times the reduction invokes the PRG attacker). Thus, post-quantum computationally hiding and statistically binding  commitments are known from post-quantum one-way functions.


Next, we notions of extractability and equivocation for commitments. 


\subsubsection{Extractable Commitments}
Informally, a commitment is extractable if for every QPT adversarial committer $\cC^*$, there exists a QPT {\em extractor} $\cE_{\cC^*}$ that in an ideal world extracts the message committed by $\cC^*$ while also simulating $\cC^*$'s view. 
Looking ahead, extractable commitments will enable a challenger that runs an experiment against an adversary to extract messages committed by the adversary without having to execute the opening phase.
We formally define this notion below.
%\dakshita{add informal explanation}
% Extractability is a strengthening of (computational) binding, and equivocation is a strengthening of (computational) hiding.

\begin{definition}[Extractable Commitment]\label{def:extcom}
A bit commitment scheme is \emph{extractable} if for every polynomial-size quantum adversarial committer $\cC^* = \{\cC^*_{\com,\lambda},\cC^*_{\open,\lambda}, \brho_{\lambda}\}$, there exists a QPT extractor $\cE_{\cC^*}$ such that for every polynomial-size quantum distinguisher $\cD^* = \{\cD^*_{\lambda}, \bsigma_{\lambda}\}$, there exists a negligible function $\nu(\cdot)$ such that:
$$\big| \Pr[\cD^*_\lambda(\bsigma_\lambda,\mathsf{Real})=1] - \Pr[\cD^*_\lambda(\bsigma_\lambda,\mathsf{Ideal}) = 1] \big| = \nu(\lambda)$$ 
for $\mathsf{Real}$ and $\mathsf{Ideal}$ distributions defined below (where we omit indexing by $\lambda$ for the sake of presentation).
\begin{itemize}
    \item Denote by $\mathsf{Real}$ the distribution consisting of $(\bx_{\final},b)$ where $\bx_{\final}$ denotes the final state of $\cC^*_\open$ and $b \in \{0,1,\bot\}$ denotes the output by $\cR_\open$ after the open phase.
    \item To define the distribution $\mathsf{Ideal}$, first run the extractor $\cE_{\cC^*}$ on input $\rho$ to obtain outputs $(\bx_{\com},\by_{\com},b^*)$, where $\bx_{\com}$ and $\by_{\com}$ are the final states of committer and receiver respectively after the commit phase. Then run $\cC^*(\bx_{\com})$ and $\cR(\by_{\com})$ to produce $(\bx_{\final},b)$, where $\bx_{\final}$ is the final state of the committer. If $b \notin \{\bot,b^*\}$, output $\mathsf{FAIL}$ and otherwise output $(\bx_{\final},b)$.
\end{itemize}
%It must hold that no non-uniform QPT distinguisher can distinguish between the outputs of the real and simulated distributions.
\end{definition}

\subsubsection{Equivocal Commitments}
%Next, we define equivocality. 
Informally, a commitment is equivocal if for every QPT adversarial receiver $\cR^*$, there exists a QPT {\em equivocator} $\cQ_{\cR^*}$ that generates a view for $\cR^*$ in the commit phase {\em without any input}, and then receives an input bit $b$ once the commit phase ends. The equivocator is then able to open the commitment generated in the commit phase to bit $b$ such that: $\cR^*$ cannot distinguish between its interaction with $\cQ_{\cR^*}$ and its interaction with an honest committer that committed to $b$ all along, and opened its commitment honestly in the opening phase.
Looking ahead, equivocal commitments will enable a challenger that runs an experiment against an adversary to generate commitments that can later be opened arbitrarily. We will now formally describe this primitive.

\begin{definition}[Equivocal Commitments]
\label{def:eqcom}
A bit commitment scheme is {\em equivocal} if for every polynomial-size quantum receiver 
$\cR^* = \{\cR^*_{\com,\lambda},\cR^*_{\open,\lambda},\brho_\lambda\}$
there exists a QPT equivocator $\equivsim_{\cR^*} = (\equivsim_{\cR^*,\com}, \equivsim_{\cR^*,\open})$ such that 
%for any polynomial-sized adversarial receiver $R^*$
for every polynomial-size quantum distinguisher $\cD^* = \{\cD^*_{\lambda}, \bsigma_{\lambda}\}$ there exists a negligible function $\nu(\cdot)$ such that for every bit $b \in \zo$,
$$\big| \Pr[\cD^*(\bsigma_\lambda,\mathsf{Real}_b)=1] - \Pr[\cD^*(\bsigma_\lambda,\mathsf{Ideal}_b) = 1] \big| = \nu(\lambda)$$ 
for $\mathsf{Real}_b$ and $\mathsf{Ideal}_b$ distributions as defined below (where we omit indexing by $\lambda$ for the sake of presentation).
%that at the end of the commitment phase outputs view denoted by $\view_{R^*}$, 
\begin{itemize}
    \item $\mathsf{Real}_b$: 
    Let $\cR^*$ interact with $\cC_{\com}(1^\lambda,b)$ in the commit phase, after which $\cC_{\com}$ obtains state $\bx_\com$ and $\cR^*$ obtains state $\by_\com$.
    Next, obtain output signal bit $s \in \zo$ from $\cR^*$, specifying whether or not the commit phase aborts. If $s = 0$, output $\by_\com$. Otherwise, 
    output the final state $\by_{\final}$ of $\cR^*$ after it interacts with $\cC_{\open}(\bx_\com)$ in the open phase.
    %Denote by $\mathsf{Real}_b$ the distribution $\rho_{\cR^*,\final}$, which denotes the final state of $\cR^*_\open$ after the open phase, 
    \item $\mathsf{Ideal}_b$:
    To define $\mathsf{Ideal}_b$, first run the equivocator
    %Let $\cR^*$ interact with 
    $\equivsim_{\cR^*,\com}(\brho)$ to obtain state $(\bz$, $\by_\com)$ and signal bit $s \in \{0,1\}$. 
    If $s = 0$, output $\by_\com$. 
    Otherwise, obtain and output $\by_{\final} \leftarrow \equivsim_{\cR^*, \open}(b,\bz,\by_\com)$.
    %output the final state of $\cR^*$ after it interacts with $\cC_{\open}(\rho_\cC)$ in the open phase.
    %in the commit phase, after with $\cC_{\com}$ obtains state $\rho_\cC$ and $\cR^*$ obtains state $\rho_{\cR^*}$.
    %Next, $\cR^*$ sends a signal $s \in \{0,1\}$. If $s = 0$, set $\mathsf{Real}_b = \rho_{\cR^*}$. Otherwise, set $\mathsf{Real}_b$ to be the final state of $\cR^*$ after it interacts with $\cC_{\open}(\rho_\cC)$ in the open phase.
\end{itemize}




%$\equivsim_{\cR^*,\com} \rightarrow \rho_\cR$ and
%(\rho_\cR, \mathsf{st})$, and
\iffalse{
$\equivsim_{\cR^*,\open}
(b, \mathsf{st}, R^*) \rightarrow (\simu\text{-}\mathsf{Decommit}\text{-}{\view}_{R^*})$
such that: \andrea{How is access to $R^*$ given to $\equivsim$?}
\dakshita{I didnt say because we will use Watrous' rewinding lemma and I'm not sure if it is referred to as black box or non black box access to the adversary?}
$$\view_{R^*} \left( \mathsf{Commit} \langle S(b), R^* \rangle, \mathsf{Decommit} \langle S(b), R^* \rangle \right) \approx_c \left( \simu\text{-}\mathsf{Commit}\text{-}{\view}_{R^*}, \simu\text{-}\mathsf{Decommit}\text{-}{\view}_{R^*} \right).$$
}\fi
\end{definition}

\fi

% \begin{definition}[Equivocal and Extractable Commitments]
% \label{def:eecom}
% We say that a commitment scheme is equivocal and extractable if it satisfies Definitions \ref{def:hiding}, \ref{def:extcom}, and \ref{def:eqcom}.
% \end{definition}

\iffalse
\subsection{Post-Quantum Zero-Knowledge Arguments}
\label{subsec: ZK def}

In the following definition, $R$ is an NP relation and $\mathcal{L}(R)$ is the associated language $\{x \mid \exists w \text{ s.t. } (x,w) \in R\}$. We denote by $\langle P(w), V \rangle(x)$ an interactive protocol between a prover $P$ given witness $w$ and verifier $V$ on shared input $x$. The output of the verifier at the end of the interaction will be denoted as $\mathsf{OUT}_V\langle P(w),V \rangle(x)$. For an honest verifier, $\mathsf{OUT}_V\langle P(w),V \rangle(x)$ will be a single bit indicating accept/reject, but we make no restrictions on the output of a malicious verifier. We stress that the honest prover and verifier are both classical polynomial-time algorithms, but malicious provers and verifiers are allowed to be quantum polynomial-time algorithms (though communication is always classical).



\begin{definition}[Classical Zero-Knowledge Arguments with Post-Quantum Security]
\label{def:zk}
A zero-knowledge (ZK) argument system $\langle P, V\rangle$ for an NP relation $R$ is an interaction between a prover $P(w)$ and verifier $V$ satisfying the following:
\begin{itemize}
\item \textbf{Completeness.} For every $\lambda \in \mathbb{N}$ and $(x,w) \in R$ where $|x| = \lambda$,
\[ \Pr[\mathsf{OUT}_V \langle P(w), V \rangle(x)] = 1.\]
\item \textbf{Post-Quantum Soundness.} For any polynomial-size quantum cheating prover $P^* = \{P^*_\lambda\}_\lambda$, there exists a negligible function $\nu(\lambda)$ such that for every $\lambda$ and $x \in \{0,1\}^\lambda \setminus \mathcal{L}(R)$
\[ \Pr[\mathsf{OUT}_V \langle P^*_{\lambda}, V\rangle(x) = 1] \leq \nu(\lambda).\]
\item \textbf{Post-Quantum Zero-Knowledge.} For every polynomial-size quantum cheating verifier $V^* = \{V^*_\lambda\}_\lambda$ with quantum auxiliary input $z = \{z_\lambda\}_\lambda$, there exists a quantum polynomial-time simulator $S = \{S_\lambda\}_\lambda$ such that for every $\lambda$ and $(x,w) \in R$ where $|x| = \lambda$,
\[ \mathsf{OUT}_{V^*_\lambda} \langle P_{\lambda}, V^*_\lambda(z_\lambda) \rangle(x) \approx_C S_\lambda(x,z_\lambda).\]
\end{itemize}
\end{definition}

\paragraph{Instantiations.} Any of the classic ``commit-challenge-response'' argument systems such as Blum's Hamiltonicity protocol~\cite{Blum86} or Goldreich, Micali, and Wigderson's 3-coloring protocol~\cite{C:GolMicWig86}, instantiated with an unconditionally binding and (quantum) computationally-hiding bit commitment, will satisfy~\cref{def:zk} using the quantum zero-knowledge simulator of Watrous~\cite{STOC:Watrous06}. Such bit commitments are known from any (post-quantum) one-way function, as discussed in \cref{subsec: com definitions}.
\fi



%It is well-known~\cite{STOC:Kilian88} that general purpose two-party secure computation can be obtained based only on black-box use of OT.
%We also review here the implications of simulation-secure oblivious transfer to secure multi-party computation. The work of \cite{C:IshPraSah08} shows that (assuming one-way functions) any multi-party classical functionality can be computed with malicious security against dishonest majority in a model where parties have black-box access to an ideal OT functionality. 
%Thus, any stand-alone secure OT protocol gives a stand-alone secure MPC protocol in the plain model.
%The \cite{C:IshPraSah08} theorem also immediately implies that any \emph{stand-alone} secure OT (which is the definition given above) implies a stand-alone secure MPC, as long as the calls to the OT functionality are executed \emph{sequentially}. 
%Moreover, the reductions and simulator in their security proof only access the OT functionality in a black-box manner, and do not rewind. Thus, implicit in \cite{C:IshPraSah08} is the following theorem.

%\begin{theorem}[Implicit in \cite{C:IshPraSah08}]
%Assuming that parties have access to authenticated channels and assuming the existence of one-way functions, any post-quantum maliciously-secure oblivious transfer protocol in the plain model (potentially involving quantum communication) implies a post-quantum maliciously-secure multi-party computation protocol (secure against dishonest majority) for general classical functionalities in the plain model.
%\end{theorem}

%Next, we have the following theorem from \cite{EC:DGJMS20}.

%\begin{theorem}[Implicit in \cite{EC:DGJMS20}]
%Any post-quantum maliciously-secure MPC for classical functionalities (potentially involving quantum communication) implies a maliciously-secure MPC for \emph{quantum} functionalities (MPQC). If the MPC protocol is in the plain model and secure against dishonest majority, then so is the MPQC protocol. 
%\end{theorem}

%As a result of these two theorems, we see that it suffices to construct the above notion of oblivious transfer in order to construct general-purpose multi-party classical or quantum computation that is maliciously-secure against a dishonest majority in the plain model  (assuming parties have access to authenticated channels).

\ifsubmission
\else
\subsection{Quantum Rewinding Lemma}

We will make use of the following lemma from~\cite{STOC:Watrous06}.

\begin{lemma}\label{lem:qrl} Let $\cQ$ be a general quantum circuit with $n$ input qubits that outputs a classical bit $b$ and $m$ qubits. For an $n$-qubit state $\ket{\psi}$, let $p(\ket{\psi})$ denote the probability that $b =0$ when executing $\cQ$ on input $\ket{\psi}$. Let $p_0, q \in (0,1)$ and $\epsilon \in (0,1/2)$ be such that:

\begin{itemize}
    \item For every $n$-qubit state $\ket{\psi},p_0 \leq p(\psi)$,
    \item For every $n$-qubit state $\ket{\psi}$, $|p(\psi)-q| < \epsilon$,
    \item $p_0(1-p_0) \leq q(1-q)$,
\end{itemize}

Then, there is a general quantum circuit $\widehat{\cQ}$ of size $O\left(\frac{\log(1/\epsilon)}{4 \cdot p_0(1-p_0)} |\cQ|\right)$, taking as input $n$ qubits, and returning as output $m$ qubits, with the following guarantee. For an $n$ qubit state $\ket{\psi}$, let $\cQ_0(\ket{\psi})$ denote the output of $\cQ$ on input $\ket{\psi}$ conditioned on $b=0$, and let $\widehat{\cQ}(\ket{\psi})$ denote the output of $\widehat{\cQ}$ on input $\ket{\psi}$. Then, for any $n$-qubit state $\ket{\psi}$,

$$\mathsf{TD}\left(\cQ_0(\ket{\psi}),\widehat{\cQ}(\ket{\psi})\right) \leq 4\sqrt{\epsilon}\frac{\log(1/\epsilon)}{p_0(1-p_0)}.$$

\end{lemma}
\fi


\ifsubmission
\else
\subsection{Quantum Entropy and Leftover Hashing}
\label{subsec: quantum min entropy}

\paragraph{Classical Min-Entropy.}For a classical random variable $X$, its min-entropy $\mathbf{H}_\infty(X)$ is defined as
\[ \mathbf{H}_\infty(X) \coloneqq -\log(\max_{x} \Pr[X = x]).\]

In cryptographic settings, we are often interested in the min-entropy of a random variable $X$ sampled from a joint distribution $(X,Y)$, where $Y$ is side information available to an adversary/distinguisher. Following~\cite{AC:RenWol05}, we define the conditional min-entropy of $X$ given $Y$ as
\[ \mathbf{H}_\infty(X \mid Y) \coloneqq -\log(\max_{x,y}\Pr[X = x \mid Y = y]).\]

That is, $\mathbf{H}_\infty(X \mid Y)$ is (the negative log of) the maximum probability of guessing the outcome of $X$, maximized over the possible outcomes of $Y$.

\fi

% \paragraph{(Version 1) Min-Entropy with Quantum Side Information .} We will consider joint distributions $(X,\mathbf{y})$ where $X$ is a classical random variable and $\mathbf{y}$ is a quantum random variable. Such distributions may naturally arise, for instance, if one has joint (possibly entangled) quantum random variables $(\mathbf{x},\mathbf{y})$, and obtains $X$ by applying an arbitrary quantum measurement to $\mathbf{x}$.

% Following the~\cite{KonRenSch09} characterization of quantum conditional min-entropy, we can define the conditional min-entropy of $\mathbf{H}_\infty(X \mid \mathbf{y})$ in terms of the maximum probability of guessing $X$ given $\mathbf{y}$.

% Let $\gray{Y}$ denote the register of $\mathbf{y}$. Write the joint state $(X,\mathbf{y})$ as
% \[ \sum_x \Pr[X = x] \ket{x}\bra{x} \otimes \mathbf{y}_x. \]
% Define
% \[ p_{\text{guess}}(X \mid \mathbf{y}) \coloneqq \sup_{\{E_x\}_x}\left(\sum_x \Pr[X = x]\text{tr}(E_x \mathbf{y}_x)\right),\]
% where the supremum is taken over all POVMs $\{E_x\}_x$ on $\gray{Y}$. 

% Finally, we can define
% \[\mathbf{H}_\infty(X \mid \mathbf{y}) \coloneqq - \log (p_{\text{guess}}(X \mid \mathbf{y})).\]

\ifsubmission
\else

\paragraph{Quantum Conditional Min-Entropy.} 

Let $\boldsymbol{\rho}_{\gray{X}\gray{Y}}$ denote a bipartite quantum state over registers $\gray{X}\gray{Y}$. Following~\cite{Renner08,KonRenSch09}, the conditional min-entropy of $\boldsymbol{\rho}_{\gray{X}\gray{Y}}$ given $\gray{Y}$ is then defined to be 
\[\mathbf{H}_\infty(\boldsymbol{\rho}_{\gray{X}\gray{Y}} \mid \gray{Y}) \coloneqq \sup_\mathbf{y} \max \{h \in \mathbb{R} : 2^{-h} \cdot I_{\gray{X}} \otimes \mathbf{y}_{\gray{Y}} - \boldsymbol{\rho}_{\gray{X}\gray{Y}} \geq 0\}.\]

In this work, we will exclusively consider the case where the $\boldsymbol{\rho}_{\gray{X}\gray{Y}}$ is a joint distribution of the form $(X,\mathbf{y})$ where $X$ is a classical random variable. In other words, $\boldsymbol{\rho}_{\gray{X}\gray{Y}}$  can be written as 
\[ \sum_x \Pr[X = x] \ket{x}\bra{x} \otimes \mathbf{y}_x. \]

In this case, we will write $\mathbf{H}_\infty(\boldsymbol{\rho}_{\gray{X}\gray{Y}} \mid \gray{Y})$ as $\mathbf{H}_\infty(X \mid \mathbf{y})$. We remark that in this particular setting, $\mathbf{H}_\infty(X \mid \mathbf{y})$ can be interpreted as the (negative log of) the maximum probability of guessing $X$ given quantum state $\mathbf{y}$~\cite{KonRenSch09}.

\paragraph{Leftover Hash Lemma with Quantum Side Information.} We now state a generalization of the leftover hash lemma to the setting of quantum side information. 
\begin{lemma}[\cite{TCC:RenKon05}]\label{thm:privacy-amplification}
Let $\mathcal{H}$ be a family of universal hash functions from $\mathcal{X}$ to $\{0,1\}^\ell$, i.e. for any $x \neq x'$, $\Pr_{h \leftarrow \mathcal{H}}[h(x) = h(x')] = 2^{-\ell}$. Then for joint random variables $(X,\mathbf{y})$ where $X$ is a classical random variable over $\mathcal{X}$ and $\mathbf{y}$ is a quantum random variable,
\[\left\|(h,h(X),\mathbf{y}) - (h,u,\mathbf{y})\right\|_1 \leq \frac{1}{2^{1+\frac{1}{2}(\mathbf{H}_\infty(X|\mathbf{y})-\ell)}},\]
where $h \leftarrow \mathcal{H}$ and $u \leftarrow \{0,1\}^\ell$.

\end{lemma}

\fi

==> sec-qot.tex <==
\section{Quantum Oblivious Transfer from Extractable and Equivocal Commitments}
\label{sec: OT from eecom}
\renewcommand{\commit}{\mathsf{EECom}}

\subsection{Definitions for Oblivious Transfer with Quantum Communication}
\label{sec:otdef}
An oblivious transfer with quantum communication is a protocol between a quantum interactive sender $\cS$ and a quantum interactive receiver $\cR$, where the sender $\cS$ has input $m_0,m_1 \in \{0,1\}^\secp$ and the receiver $\cR$ has input $b \in \{0,1\}$. After interaction the sender outputs $(m_0,m_1)$ and the receiver outputs $(b,m_b)$. 

Let $\cF(\cdot,\cdot)$ be the following functionality. $\cF(b,\cdot)$ takes as input either $(m_0,m_1)$ or $\abort$ from the sender, returns $\mathsf{end}$ to the sender, and outputs $m_b$ to the receiver in the non-$\abort$ case and $\bot$ in the $\abort$ case. $\cF(\cdot,(m_0,m_1))$ takes as input either $b$ or $\abort$ from the receiver,
returns $m_b$ to the receiver, and
returns $\mathsf{end}$ to the sender  %and outputs $(m_0,m_1)$ 
in the non-$\abort$ case, and returns $\bot$ to the sender  in the $\abort$ case. 

\begin{definition}
\label{def:ot}
We let $\langle S(m_0, m_1), R(b) \rangle$ denote an execution of the OT protocol with sender input $(m_0, m_1)$ and receiver input bit $b$. 
We denote by $\brho_{\out,S^*}\langle S^*(\brho), R (b) \rangle$ and $\mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle$ the final state of a non-uniform malicious sender $S^*(\brho)$ and the output of the receiver $R(b)$ at the end of an interaction (leaving the indexing by $\secp$ implicit). We denote by $\brho_{\out,R^*}\langle S(m_0, m_1), R^*(\brho) \rangle$ and $\mathsf{OUT}_{S}\langle  S(m_0, m_1), R^*(\brho) \rangle$ the final state of a non-uniform malicious receiver $R^*(\brho)$ and the output of the sender $S(m_0,m_1)$ at the end of an interaction.
We require OT to satisfy the following security properties:
\begin{itemize}
\item \noindent {\bf Receiver Security.} 
For every receiver bit $b \in \zo$, every QPT non-uniform malicious sender $S^*(\brho)$, and QPT non-uniform distinguisher $D^*(\bsigma,\cdot)$, where $\brho$ and $\bsigma$ may be entangled, there exists a simulator $\simu_{S^*}$ such that the following holds.
$\simu_{S^*}(\brho)$ sends inputs $(m_0, m_1)$ or $\mathsf{abort}$ to the ideal functionality ${\fot(b,\cdot)}$, whose output to the receiver is denoted by $\mathsf{OUT}_R$. $\simu_{S^*}(\brho)$ also outputs a final state $\brho_{\mathsf{Sim},\out,S^*}$ such that 

\begin{align*}
\bigg|&\Pr\left[D^*\left(\bsigma,\left(\brho_{\mathsf{Sim},\out,S^*}, \mathsf{OUT}_{R} \right)\right) = 1\right]\\
&-\Pr\left[D^*\left(\bsigma,\left(\brho_{\out,S^*}\langle S^*(\brho), R(b) \rangle, \mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle\right) \right) = 1\right]\bigg| = \negl(\secp).
\end{align*}

%$$\big(\brho_{\mathsf{Sim},\out,S^*}, \mathsf{OUT}_{R} \big) \approx_c \big(\brho_{\out,S^*}\langle S^*(\brho), R(b) \rangle, \mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle \big).$$

%We say that the OT scheme is $T$-secure if $T.\poly(\secpar)$-size malicious senders have distinguishing advantage less than $\frac{1}{T}$.
\item \noindent {\bf Sender Security.} For every pair of sender inputs $(m_0, m_1)$, every QPT non-uniform malicious receiver $R^*(\brho)$, and QPT non-uniform distinguisher $D^*(\bsigma,\cdot)$, where $\brho$ and $\bsigma$ may be entangled, there exists a  simulator $\simu_{R^*}$ such that the following holds. $\simu_{R^*}(\brho)$ sends bit $b$ or $\mathsf{abort}$ to the ideal functionality ${\fot(m_0,m_1,\cdot)}$, whose output to the sender is denoted by $\mathsf{OUT}_S$. $\simu_{R^*}(\brho)$ also outputs a final state $\brho_{\mathsf{Sim},\out,R^*}$ such that

\begin{align*}
\bigg|&\Pr\left[D^*\left(\bsigma,\left(\brho_{\mathsf{Sim},\out,R^*}, \mathsf{OUT}_S \right)\right) = 1\right]\\
&-\Pr\left[D^*\left(\bsigma,\left(\brho_{\out,R^*}\langle S(m_0,m_1), R^*(\brho) \rangle, \mathsf{OUT}_S\langle S(m_0,m_1), R^*(\brho) \rangle\right) \right) = 1\right]\bigg| = \negl(\secp).
\end{align*}

%$$
%\big(\brho_{\mathsf{Sim},\out,R^*}, \mathsf{OUT}_S \big) \approx_c \big(\brho_{\out,R^*}\langle S(m_0, m_1), R^*(\brho) \rangle, \mathsf{OUT}_{S} \langle S(m_0, m_1), R^*(\brho) \rangle \big).$$
%%where $\fot(m_0,m_1,\cdot)$ is an oracle that on input $b$ outputs $m_b$ and then self destructs.
%We say that the OT protocol satisfies $(1 - \delta)$ statistical sender security if the statistical distance between the real and ideal distributions is at most $\delta$.
\end{itemize}
\end{definition}

\subsection{Our Construction}

We construct simulation-secure quantum oblivious transfer by making use of the following building blocks.

\begin{itemize}
\ifsubmission
    \item Let $(\eecommit,\eedecommit)$ denote any quantum bit commitment scheme satisfying extractability and equivocality. Such a commitment scheme may be obtained by applying the compiler from~\cref{sec: equivocal commitment} to the extractable commitment constructed in~\cref{section: extractable com}. 
\else
    \item Let $(\eecommit,\eedecommit)$ denote any quantum bit commitment scheme satisfying extractability (\cref{def:extcom}) and equivocality (\cref{def:eqcom}). Such a commitment scheme may be obtained by applying the compiler from~\cref{sec: equivocal commitment} to the extractable commitment constructed in~\cref{section: extractable com}. 
\fi
    \item Let $h: \{0,1\}^{k(\secp)} \times \mathcal{X} \rightarrow \{0,1\}^\secp$ be a universal hash function with seed length $k(\secp) = \poly(\secp)$ and domain $\mathcal{X}$ defined to be the set of all binary strings of length \emph{at most} $8 \secp$. 
    % Let $\{h_p\}_{p \in [\secp,7\secp]}$ be a family of universal hash functions, where for suitable polynomial $k(\cdot)$, $h_p : \{0,1\}^{k(\secp)} \times \{0,1\}^{p} \to \{0,1\}^\secp$.\fermi{the $[\secp,7\secp]$ thing looks quite strange... we should fix it}
\end{itemize}


Our QOT protocol is described in Protocol \ref{fig:ot}, which is essentially the~\cite{FOCS:CreKil88} protocol instantiated with our extractable and equivocal commitment scheme. 


%It makes use of a suitable universal hash function family $h$, that on input a seed $s \leftarrow \{0,1\}^\lambda$ and input $x \in \{0,1\}^{p(\lambda)}$ for arbitrary $p(\lambda) \in [\lambda,15\lambda]$, generates an output in $\{0,1\}^{\lambda}$.
%, and $\Pi_{BB}$ denote the OT protocol against benign receivers from~\cite{C:BenBra84}.

\protocol
{\proref{fig:ot}}
{Quantum Oblivious Transfer.}
{fig:ot}
{
\textbf{Sender $S$ Input:} Messages $m_0, m_1 \in \{0,1\}^{\lambda} \times \{0,1\}^{\lambda}$\\
\textbf{Receiver $R$ Input:} Bit $b \in \{0,1\}$\\

\underline{\textbf{The Protocol:}}
\begin{enumerate}
\item $S$ chooses $x \leftarrow \{0, 1\}^{16\lambda}$ and $\theta \leftarrow \{+, \times \}^{16\lambda}$ 
and sends $\ket{x}_\theta$ to $R$. 

\item $R$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^{16\lambda}$
and obtains $\widehat{x} \in \{0, 1\}^{16\lambda}$ by measuring $\ket{x}_{\theta}$
in basis $\widehat{\theta}$. Then, $S$ and $R$ execute $16\lambda$ sessions of $\eecommit$ sequentially with $R$ acting as committer and $S$ as receiver. In session $i$, $R$ commits to the bits $\widehat{\theta}_i,\widehat{x}_i$.

%$R$ commits to $\widehat{\theta}$ and $\widehat{x}$ position-wise: for %$i \in [2\lambda^3]$, $R$ sends $c_i$ to $S$, where
%$c_i : = \commit((\widehat{\theta}_i, \widehat{x}_i); r_i)$
%for uniform randomness $r_i$. 

\item $S$ sends a random test subset $T \subset [16\lambda]$ of size $8\lambda$ to $R$. 

\item For each $i \in T$, $R$ and $S$ sequentially execute the $i$'th $\eedecommit$, after which $S$ receives the opened bits $\widehat{\theta}_i,\widehat{x}_i$.

%\item For $i \in T$, $R$ and $S$ take the roles of prover and verifier in $\Pi_{\mathsf{ZK}} (X_i,w_i,L)$ where: \\ $X_i = (c_i,\widehat{x}_i,\widehat{\theta}_i), w_i = \big(r_i\big)$ 
%and $L = \Big\{(c,\alpha,\beta): \exists r \text{ s.t. } X= \commit\Big((\alpha, \beta);r\Big) \Big\}$.
%%$(c_i,r_i;r_{A,i})$ for all $i \in T$. 

\item $S$ checks that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $S$ accepts,
otherwise, $S$ rejects and aborts.

\item The tested positions are discarded by both parties: $S$ and $R$ restrict $x$ and $\theta$, respectively $\widehat{x}$ and $\widehat{\theta}$, to the $8\secp$ indices $i \in \overline{T}$.
$S$ sends $\theta$ to $R$.

\item $R$ partitions the positions of $\overline{T}$ into two parts: the ``good'' subset $I_b = \{i : \theta_i = \widehat{\theta}_i\}$ and the ``bad'' subset $I_{1-b} = \{i : \theta_i \neq \widehat{\theta}_i\}$. $R$ sends $(I_0,I_1)$ to $S$.

\item $S$ samples seeds $s_0,s_1 \leftarrow \{0,1\}^{k(\lambda)}$ and sends $\left(s_0,h(s_0,x_0) \oplus m_0,s_1,h(s_1,x_1) \oplus m_1\right)$, where $x_0$ is $x$ restricted to the set of indices $I_0$ and $x_1$ is $x$ restricted to the set of indices $I_1$.

\item $R$ decrypts $s_b$ using $\widehat{x}_b$, the string $\widehat{x}$ restricted to the set of indices $I_b$.
\end{enumerate}
}

\ifsubmission
\begin{theorem}
\label{theorem:QOT}
The protocol in Figure \ref{fig:ot} is a simulation-secure QOT protocol whenever $(\eecommit,\eedecommit)$ is instantiated with a quantum bit commitment satisfying extractability and equivocality.
\end{theorem}
\else
\begin{theorem}
\label{theorem:QOT}
The protocol in Figure \ref{fig:ot} is a QOT protocol satisfying Definition \ref{def:ot} whenever $(\eecommit,\eedecommit)$ is instantiated with a quantum bit commitment satisfying extractability (\cref{def:extcom}) and equivocality (\cref{def:eqcom}).
\end{theorem}
\fi

We prove that the resulting QOT protocol satisfies standard simulation-based notions of receiver and sender security. 

\ifsubmission
The proof of sender security follows readily from quantum sampling techniques developed by~\cite{C:BouFeh10}, and is deferred to the supplementary materials.
\else
\fi

\subsection{Receiver Security}
%    This follows by the equivocal property of the commitment scheme $\commit$ and the zero-knowledge property of $\Pi_{ZK}$.
    Consider any adversarial sender $S^*$ with advice $\brho$. The simulator $\mathsf{Sim}_{S^*}(\brho)$ is constructed as follows.
    %We will demonstrate the existence of a simulator $\mathsf{Sim}_{S^*}$ that simulates the state of any malicious sender $S^*$.
    %It computes the output of the equivocal simulator for the protocol $\mathsf{EECom}$ corresponding to $\cV^*(\brho)$, which has the code of $S^*$ hardwired, and is defined as follows.
    %\noindent $\cV^*(\brho)$:
    \begin{enumerate}
        \item Run the first message algorithm of $S^*$ on input $\brho$ to obtain message $\bpsi$. %$\ket{x}_{\theta}$ from $S^*$.
        \item Execute $16\lambda$ sequential sessions of $\eecommit$. In each session, run the equivocator $\cQ_{\cR^*,\com}$, where $\cR^*$ denotes the portion of $S^*$ that participates as receiver in the $i^{th}$ sequential $\eecommit$ session.
        \item Obtain test subset $T$ of size $8\lambda$ from $S^*$.
        \item For each $i \in T$, sample $\widehat{\theta}_i \leftarrow \{+, \times\}$. 
        Obtain $\widehat{x}_i$ by measuring the $i^{th}$ qubit of $\bpsi$ in basis $\widehat{\theta}_i$.
        For each $i \in T$, sequentially execute the equivocal simulator $\cQ_{\cR^*, \open}$ on input $(\widehat{\theta}_i,\widehat{x}_i)$ and the state obtained from $\cQ_{\cR^*, \com}$.
        \item If $S^*$ continues, discard positions indexed by $T$. Obtain $\theta_i$ for $i \in \overline{T}$ from $S^*$, and compute $x_i$ for $i \in \overline{T}$ by measuring the $i^{th}$ qubit of $\bpsi$ in basis $\theta_i$.
        \item For every $i \in \overline{T}$, sample bit $d_i \leftarrow \{0,1\}$. Partition the set $\overline{T}$ into two subsets $(I_0, I_1)$, where for every $i \in \overline{T}$, place $i \in I_0$ if $d= 0$ and otherwise place $i \in I_1$. Send $(I_0, I_1)$ to $S$.
        \item Obtain $(y_0, y_1)$ from $S$. Set $x_0$ to be $x$ restricted to the set of indices $I_0$ and $x_1$ to be $x$ restricted to the set of indices $I_1$.
        For $b \in \{0,1\}$, parse $y_b = (s_b, t_b)$ and compute $m_b = t_b \oplus h(s_b, x_b)$. %Send $(m_0, m_1)$ to the OT ideal functionality.
        \item If $S^*$ aborts anywhere in the process, send $\mathsf{abort}$ to the ideal functionality. Otherwise, send $(m_0, m_1)$ to the ideal functionality. Output the final state of $S^*$.
    \end{enumerate}
    %\dakshita{TODO: Add simulator}
%    
   
    
    %by proving that for each $b \in \{0,1\},$
    %$$\big(\brho_{\mathsf{Sim},\out,S^*}, \mathsf{OUT}_{R} \big) \approx_c \big(\brho_{\out,S^*}\langle S^*(\brho), R(b) \rangle, \mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle \big).$$
    %where $\brho_{\simu_{S^*}}$ is the final state output by the simulator, and $\mathsf{OUT}_{R}$ refers to the output of the ideal functionality in the simulated world. 
    
     Next, we establish receiver security according to \cref{def:ot}. Towards a contradiction, suppose there exists a 
    bit $b \in \zo$,
    a non-uniform QPT sender $(S^*,\brho)$, a non-uniform QPT distinguisher $(D^*,\bsigma)$, and polynomial $\mathsf{poly}(\cdot)$ such that 
    \begin{align*}\Big|&\Pr\left[D^*\left(\bsigma,\left(\brho_{\mathsf{Sim},\out,S^*}, \mathsf{OUT}_{R}\right)\right) = 1\right] \\ &- \Pr\left[D^*\left(\bsigma,\left(\brho_{\out,S^*}\langle S^*(\brho), R(b) \rangle, \mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle\right)\right) = 1\right] \Big| \geq \frac{1}{\mathsf{poly}(\secp)}.\end{align*}
    %
    Fix any such $b$, sender $(S^*,\brho)$ and distinguisher $(D^*,\bsigma)$. We derive a contradiction via an intermediate hybrid experiment, defined as follows with respect to bit $b$ and sender $(S^*,\brho)$.\\
    
    \noindent {\textbf{$\mathsf{Hyb}$.}} In this hybrid, we generate the QOT receiver commitments via the equivocal simulator $\cQ_{\cR^*}$ (where $\cR^*$ is derived from the malicious QOT sender $S^*$), and otherwise follow the honest QOT receiver's algorithm. %The string $m_b$ will be recovered as in the honest protocol, and $m_{1-b}$ will be fixed to 0. Finally, the ideal functionality is queried as in the simulation.
    
    %Consider any adversarial sender $S^*$ with advice $\brho$. The output of $\mathsf{Hyb}$ depends on $R$'s input bit $b$ and is generated as follows.
    \begin{enumerate}
        \item Run the first message algorithm of $S^*$ on input $\brho$ to obtain message $\bpsi$. %$\ket{x}_{\theta}$ from $S^*$.
        \item Choose $\widehat{\theta} \leftarrow \{+, \times\}^{16\lambda}$ and obtain $\widehat{x} \in \{0,1\}^{16\lambda}$ by measuring $\bpsi$ in basis $\widehat{\theta}$.
        Execute $16\lambda$ sequential sessions of $\eecommit$. In each session, run the equivocator $\cQ_{\cR^*,\com}$, where $\cR^*$ denotes the portion of $S^*$ that participates as receiver in the $i^{th}$ sequential $\eecommit$ session.
        \item Obtain test subset $T$ of size $8\lambda$ from $S^*$.
        \item For each $i \in T$, sequentially execute the equivocal simulator $\cQ_{\cR^*, \open}$ on input $\widehat{\theta}_i,\widehat{x}_i$ and the state obtained from $\cQ_{\cR^*, \com}$.
        \item If $S^*$ continues, discard positions indexed by $T$. Obtain $\theta_i$ for $i \in \overline{T}$ from $S^*$.
        %, and compute $x_i$ for $i \in \overline{T}$ by measuring the $i^{th}$ qubit of $\bpsi$ in basis $\theta_i$.
        \item Partition the set $\overline{T}$ into two subsets: the ``good'' subset $I_b = \{i:\theta_i = \widehat{\theta}_i\}$ and the ``bad'' subset $I_{1-b} = \{i: \theta_i \neq \widehat{\theta}_i\}$. Send $(I_0, I_1)$ to $S$.
        \item Obtain $(y_0, y_1)$ from $S$. Set $x_b$ to be $\widehat{x}$ restricted to the set of indices $I_b$, and compute and set $m_b = t_b \oplus h(s_b, x_b)$. If $S^*$ aborts anywhere in the process, let $\bot$ be the output of the receiver, otherwise let $m_b$ be the output of the receiver. 
        %Set $m_{1-b}$ to $0^{n(\secp)}$.
       % \item Obtain $(y_0, y_1)$ from $S$. Set $x_b$ to be $\widehat{x}$ restricted to the set of indices $I_b$ and $x_1$ to be $x$ restricted to the set of indices $I_1$.
        %Parse $y_b = (s_b, t_b)$ and compute $m_b = t_b \oplus h(s_b, x_b)$. Set $m_{1-b}$ to $0^{n(\secp)}$.
       % \item If $S^*$ aborts anywhere in the process, send $\mathsf{abort}$ to the ideal functionality. Otherwise, send $(m_0, m_1)$.
    \end{enumerate}
    The output of $\mathsf{Hyb}$ is the joint distribution of the final state of $S^*$ and the output of the receiver.

Receiver security then follows from the following two claims.

\begin{claim}
%There exists a negligible function $\mu(\cdot)$ such that
    $$\Pr\left[D^*\left(\bsigma,\left(\brho_{\mathsf{Sim},\out,S^*}, \mathsf{OUT}_{R}\right)\right) = 1\right] \equiv \Pr\left[D^*(\bsigma,\mathsf{Hyb}) = 1\right].$$
\end{claim}
\begin{proof} The only differences in the simulated distribution are (1) that measurements of $S^*$'s initial message $\bpsi$ are delayed (which cannot be noticed by $S^*$), and (2) a syntactic difference in that the ideal functionality is queried to produce the receiver's output. %The only difference is the interaction with the ideal functionality in the simulation.
\end{proof}
    
\begin{claim}
    There exists a negligible function $\nu(\cdot)$ such that
    $$\Big|\Pr[D^*(\bsigma,\mathsf{Hyb}) = 1] - \Pr\left[D^*\left(\bsigma,\left(\brho_{\out,S^*}\langle S^*(\brho), R(b) \rangle, \mathsf{OUT}_{R}\langle S^*(\brho), R(b) \rangle\right)\right) = 1\right] \Big| = \nu(\secp).$$
\end{claim}

\begin{proof}
    The only difference between the two distributions is that in the first, the receiver generates commitments according to the honest commit algorithms of $\eecommit$ while in the second, commitments in step 2 are generated via the equivocal simulator $\cQ_{\cR^*}$ of $\eecommit$. Therefore, this claim follows by the equivocality of 
    $(\eecommit,\eedecommit)$ .
\end{proof}
    
\ifsubmission
\else
\subsection{Sender Security} 
    Consider any adversarial receiver $R^*$ with quantum auxiliary state $\brho$. The simulator $\simu_{R^*}(\brho)$ is constructed as follows:
    \begin{enumerate}
        \item Choose $x \leftarrow \{0,1\}^{16\lambda}$ and $\theta \leftarrow \{+,\times\}^{16\lambda}$. Send $\ket{x}_{\theta}$ to $R^*$. 
        \item Execute $16\lambda$ sequential sessions of $\eecommit$. 
        In the $i^{th}$  session for $i \in [16\lambda]$, run the extractor $\cE_{\cC^*_i, \com}$ where $\cC^*_i$ denotes the portion of $R^*$ that participates as committer in the $i^{th}$ sequential $\eecommit$ session.
        Obtain from $\cE_{\cC^*_i, \com}$ the extracted values $(\widehat{\theta}_i, \widehat{x}_i)$.
        \item Sample and send a random test subset $T \subset [16\lambda]$ of size $8\lambda$ to $R^*$.
        \item For each index in $T$ execute the opening phases $\eedecommit$ with $R^*$, and abort if any fail. Discard the opened values, and relabel the remaining indices from $1$ to $8 \secp$.
        
        %Execute the $i^{th}$ open phase of $\mathsf{EECom}$, and obtain the openings $\widehat{\theta}_i, \widehat{x}_i$ from $R^*$. 
        \item Check that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$, and if not abort.
        %\item Partition $\overline{T}$ into two subsets $I_0$ and $I_1$ such that: for $i \in S$, $\theta_i = \beta_i$ and for $i \in \overline{S}$,
        %$\theta_i \neq \beta_i$.
        \item Send $\theta$ to $R^*$.
        \item Obtain $R^*$'s message, which specifies sets $I_0$ and $I_1 = [8\secp] \setminus I_0$. Let $S$ be the set of indices in $I_0$ such that $\theta_i \neq \widehat{\theta}_i$. If $|S| \geq 3\secp/2$ then set $b = 1$ and otherwise set $b=0$; intuitively, if $|S| \geq 3\secp/2$, we treat $I_0$ as the ``bad'' subset $I_{1-b}$ where $\theta_i \neq \hat{\theta}_i$ for many indices $i$.
        \item Obtain the output $m_b$ of $\fot$ on input bit $b$. Set $m_{1-b} = 0^{\lambda}$.
        \item Let $x_0,x_1$ denote $x$ restricted to indices $I_0,I_1$ respectively. Sample seeds $s_0,s_1 \leftarrow \{0,1\}^{k(\lambda)}$ and send $s_0,h(s_0,x_0) \oplus m_0,s_1,h(s_1,x_1) \oplus m_1$. Output the final state of $R^*$.
    \end{enumerate}
    
    %$$
%\big(\brho_{\mathsf{Sim},\out,R^*}, \mathsf{OUT}_S \big) \approx_c \big(\brho_{\out,R^*}\langle S(m_0, m_1), R^*(\brho) \rangle, \mathsf{OUT}_{S} \langle S(m_0, m_1), R^*(\brho) \rangle \big).$$

We will now establish sender security according to \cref{def:ot}. Towards a contradiction, suppose there exists a  pair of messages $(m_0, m_1) \in \{0,1\}^{\secp}$, a non-uniform QPT receiver $(R^*,\brho)$, a non-uniform QPT distinguisher $(D^*,\bsigma)$, and a polynomial $\mathsf{poly}(\cdot)$ such that 
    \begin{align*}\Big|&\Pr\left[D^*\left(\bsigma,\left(\brho_{\mathsf{Sim},\out,R^*}, \mathsf{OUT}_S\right)\right) = 1\right] \\&- \Pr\left[D^*\left(\bsigma,\left(\brho_{\out,R^*}\langle S(m_0, m_1), R^*(\brho) \rangle, \mathsf{OUT}_{S} \langle S(m_0, m_1), R^*(\brho) \rangle\right)\right) = 1\right] \Big| \geq \frac{1}{\mathsf{poly}(\secp)}.
    \end{align*}
    %
    Fix any such $(m_0, m_1)$, receiver $(R^*,\brho)$ and distinguisher $(D^*,\bsigma)$. We derive a contradiction via an intermediate hybrid experiment, defined as follows. Like the simulator, this hybrid simulates and extracts from the receiver's commitments, but does not yet replace the sender string $m_{1-b}$ with $0^\lambda$. \\
    
    %Note that the extracted values $\theta^*,x^*$ are not actually used in this hybrid - they are only used in the simulator whne determining the value of $b$.\\

%\Delta \big(\mathsf{View}_{\simu^{\fot(m_0,m_1,\cdot)}_{R^*}}, \mathsf{View}_{R^*}\langle S(m_0, m_1), R^* \rangle \big) = \negl(\secp)$$

%\dakshita{TODO from here. Added an intermediate hybrid but not sure if this is the right way to complete the proof. Also @James, I didn't quite follow why you needed $16\lambda$ but left it as is.}


\noindent $\mathsf{Hyb}$. Consider any adversarial receiver $R^*$ with advice $\brho$. The output of $\mathsf{Hyb}$ depends on $(m_0, m_1)$ and is generated as follows.
\begin{enumerate}
        \item Choose $x \leftarrow \{0,1\}^{16\lambda}$ and $\theta \leftarrow \{+,\times\}^{16\lambda}$. Send $\ket{x}_{\theta}$ to $R^*$. 
        \item Execute $16\lambda$ sequential sessions of $\eecommit$. 
        In the $i^{th}$  session for $i \in [16\lambda]$, run the extractor $\cE_{\cC^*_i, \com}$ where $\cC^*_i$ denotes the portion of $R^*$ that participates as committer in the $i^{th}$ sequential $\eecommit$ session.
        Obtain from $\cE_{\cC^*_i, \com}$ the extracted values $\widehat{\theta}_i, \widehat{x}_i$.
        \item Sample and send a random test subset $T \subset [16\lambda]$ of size $8\lambda$ to $R^*$.
        \item For each index in $T$ execute the opening phases $\eedecommit$ with $R^*$, and abort if any fail. Discard the opened values, and relabel the remaining indices from $1$ to $8 \secp$.
        \item Check that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$, and if not abort.
        %\item Partition $\overline{T}$ into two subsets $I_0$ and $I_1$ such that: for $i \in S$, $\theta_i = \beta_i$ and for $i \in \overline{S}$,
        %$\theta_i \neq \beta_i$.
        \item Obtain $R^*$'s message, which specifies sets $I_0$ and $I_1$. 
        \item Let $x_0,x_1$ denote $x$ restricted to indices $I_0,I_1$ respectively. Sample seeds $s_0,s_1 \leftarrow \{0,1\}^{k(\lambda)}$ and send $s_0,h(s_0,x_0) \oplus m_0,s_1,h(s_1,x_1) \oplus m_1$. Output the final state of $R^*$.
    \end{enumerate}

This hybrid distribution is indistinguishable from the real distribution due to the extractability (Definition \ref{def:extcom}). Indeed, the values extracted from the simulator are used in place of the values opened by $R^*$. Conditioned on the opening phases succeeding, these values will be equal with all but negligible probability.


%The only difference between this hybrid experiment and the real game is that intermediate states of $R^*$ are computed via the $\mathsf{EECom}$ simulator. Thus, indistinguishability follows immediately from Definition \ref{def:extcom}. 

Now, the only difference between this hybrid experiment and the simulation is the value of the string $m_{1-b}$, where $b$ is the bit extracted in the simulated game. Thus, to complete the proof, it suffices to argue that in the simulation, the string $h(s_{1-b},x_{1-b})$, which is used to mask $m_{1-b}$, is statistically close to a uniformly random string. 

The remaining argument is essentially identical in structure to the argument of statistical hiding of the extractable commitment in~\cref{subsec:stat-hiding}, which in turn is a direct application of quantum sampling techniques developed by~\cite{C:BouFeh10}. We therefore sketch the following statistical steps, highlighting where the argument differs from~\cref{subsec:stat-hiding}.

The idea, as in~\cref{subsec:stat-hiding}, is to consider a purification of the strategy for the challenger implementing $\mathsf{Hyb}$. In particular, suppose instead of the challenger generating $\ket{x}_{\theta}$ by sampling $x,\theta$ at random, it generates $16\secp$ EPR pairs and sends $R^*$ half of each pair, keeping the other half of each pair for itself. The challenger still samples $\theta \gets \{+,\times\}^{16\secp}$, but does not yet measure to determine $x$. When the challenger implementing $\mathsf{Hyb}$ needs to check $x_i = \hat{x}_i$, it obtains $x_i$ by measuring its $i$th EPR pair half in basis $\hat{\theta}_i$. Instead of invoking statistical binding to extract the committed values of $\hat{x},\hat{\theta}$ as done in~\cref{subsec:stat-hiding}, we can simply run the $\mathsf{EECommit}$ extractor to extract $\hat{x},\hat{\theta}$. Now, if $R^*$ can successfully opens its commitments and the challenger implementing $\mathsf{Hyb}$ does not abort, this corresponds to a successful execution of the quantum sampling experiment in~\cref{lemma:sampling} for $n = 16\secp$ and the extracted values of $\hat{x},\hat{\theta}$.

Now, consider the two subsets $I_0,I_1 \subset [8\secp]$ sent by $R^*$. For $c \in \{0,1\}$, let $\mathsf{wt}(I_c)$ be the number of indices in $I_c$ such that $\theta_i \neq \widehat{\theta}_i$. If $\mathsf{wt}(I_0) > 3\secp/2$, then $b$ will be set to 1, and by~\cref{lemma:sampling} for $S = I_0$ followed by an application of the leftover hash lemma (\cref{thm:privacy-amplification}), $(s_0,h(s_0,x_0))$ will be statistically close to a uniformly random string. Otherwise, we have $\mathsf{wt}(I_0) \leq 3\secp/2$. By a Chernoff bound, with probability $1 - \negl(\secp)$, the strings $\theta$ and $\widehat{\theta}$ must differ in more than $3\lambda$ positions, which means in this case we have $\mathsf{wt}(I_1) > 3\secp/2$. As a result, we have $b = 0$, and by the same argument as above, $(s_1,h(s_1,x_1))$ is statistically close to a uniformly random string.

\fi

Finally, the following corollary follows from Theorem \ref{thm:equiv-compiler}, Theorem \ref{thm:qextcom}, and Theorem \ref{theorem:QOT}.
\begin{corollary}
\label{cor:two}
Quantum oblivious transfer (QOT) satisfying Definition \ref{def:ot} can be based on black-box use of statistically binding bit commitments, or on black-box use of quantum-hard one-way functions.
\end{corollary}

==> sec-quantum-sampling.tex <==
\section{Proof of~\cref{lemma:quantum-sampling}}
\label{appendix:sampling}

We give a proof of~\cref{lemma:quantum-sampling}, which we restate here for convenience.

Consider the following interaction between a challenger and an unbounded quantum receiver $\cR$ (initialized with an arbitrary quantum ``advice'' state):
\begin{enumerate}
\item The challenger generates $k$ EPR pairs and sends one half of each to a receiver.
\item The receiver $\cR$ replies with $k$-bit strings $\hat{\theta}, \hat{x}$ purported to be the results of measuring these EPR pairs in bases specified by $\hat{\theta}$.
\item The challenger picks a random subset $T$ (of size $t$) of $[k]$ and measures its halves of the corresponding EPR pairs in the bases dictated by $\hat{\theta}_T$. The interaction is deemed \emph{successful} if the measurement outcomes correspond with $\hat{x}_T$.
\item Define $\overline{T} \coloneqq [k] \setminus T$ and let $n \coloneqq |\overline{T}|$. If the interaction has been successful, the challenger samples a random $n$-bit string $\theta$ and measures its $n$ remaining EPR states in the bases specified by $\theta$, obtaining measurement outcomes $x_T$.
\end{enumerate}

\begin{lemma}[Quantum Sampling]
Let $\brho$ be the quantum state of any successful receiver $\cR$ in the above interaction. Then for any $\epsilon > 0$, we have
\[ \mathbf{H}_{\infty}(x_T \mid \brho) \geq \frac{(1-\epsilon)t}{2}\]
with probability $1-\negl$ \fermi{fill in the negligible} (over the randomness of $\theta$).
\end{lemma}



\subsection{The~\cite{C:BouFeh10} EPR Protocol}

We describe a protocol we call the ``EPR Protocol,'' which is essentially equivalent to the ``QOT*'' protocol described by~\cite{C:BouFeh10}. This protocol is exclusively stated as a tool for arguing about the security of BB84-style protocols, and should not be viewed as a functional protocol.

In the EPR protocol, party $A$ deviates from the standard BB84-style template, instead generating EPR pairs and sending one half of each pair. From the other party's point of view, this message is distributed identically to random BB84 states, since in both cases each qubit is maximally mixed. Note that in a standard BB84-style protocol, $A$ samples a random bit string $x$ and encodes it in a random bases before interacting with $B$. But in the EPR protocol, $A$ obtains $x$ as the result of measuring her halves of the EPR pairs; this has the advantage of significantly simplifying arguments about the entropy of $x$ from $B$'s point of view~\cite{C:BouFeh10}. 

This is captured in~\cref{lemma:min-entropy}, which relies heavily on quantum sampling techniques of~\cite{C:BouFeh10}.

\protocol
{\proref{fig:epr-protocol}}
{EPR Protocol.}
{fig:epr-protocol}
{

\textbf{Parameters:} $m = n+k$. 

\begin{enumerate}
\item $A$ prepares $m$ EPR pairs and sends one of each pair to $B$. $A$ also samples $\theta \gets \{+,\times\}^m$.

\item $B$ responds with $\widehat{\theta} \in \{+,\times\}^m,\widehat{x} \in \{0,1\}^m$.

\item $A$ sends a random test subset $T \subset [m]$ of size $k$.

\item $B$ responds with either continue or abort.

\item $A$ measures each of her qubits in $T$ in the corresponding basis of $\widehat{\theta}$. For any index $i$ such that $\widehat{\theta}_i = \theta_i$, $A$ checks that the measured $x_i$ matches $\widehat{x}_i$. If not, $A$ aborts. If all checks pass, $A$ restricts her qubits and $\theta$ to subset $\overline{T}$ of size $n$. Then she measures her qubits in basis $\theta$ to produce a string $x$, and sends $\theta$ to $B$.

\item \textit{Post-processing}: $A$ and $B$ engage in some protocol using the strings $x$ and $\theta$, and $\widehat{x},\widehat{\theta}$ restricted to positions in $\overline{T}$.







\end{enumerate}



}

\begin{lemma}\label{lemma:min-entropy}
Consider the protocol in~\cref{fig:epr-protocol}. Let $n \geq m/2$. For any subset of $I \subset [n]$ of size $t$, let $\mathsf{wt}(I)$ be the number of positions in $I$ that $\theta$ and $\widehat{\theta}$ differ, and let $x_I$ be the string $x$ restricted to positions in $I$. Then for any $\epsilon > 0$, $x_I$ has quantum min-entropy (see definition in \cref{subsec: quantum min entropy}) at least $\mathsf{wt}(I) - \epsilon t$ conditioned on $B$'s view and on $x_{\overline{I}}$, except with probability $\negl(kt^2/n^2)$.
\end{lemma}

\begin{proof} (Sketch) We argue for the case where the strings $\widehat{\theta},\widehat{x}$ returned by $B$ are both the all-zeros strings; all other possibilities can be handled by applying the same arguments after an appropriate change of bases. Now consider the (purified) joint state $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ of $A$ and $B$ in the middle of step 5, after $A$ has restricted her state to $n$ qubits. The check at the beginning of step 5 is essentially establishing that $A$'s part of $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ is close to the all zeros state $\ket{0}^{\otimes n}$. Indeed, applying \cite[Theorem 3]{C:BouFeh10} (plus analysis in \cite[Appendix B.4]{C:BouFeh10} bounding the error probability of the corresponding classical sampling strategy) with some $\delta > 0$ shows that, conditioned on $A$ not aborting after this check, $A$'s part of the state is within trace distance $\negl(k \delta^2)$ of a superposition of states with Hamming weight at most $\delta n$. That is, we can assume that the state $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ is a superposition of vectors that only contain at most $\delta n$ 1s among the $n$ positions in $\mathsf{A}$. Now, letting $\delta = \epsilon' t/n$ for a small enough constant $\epsilon' > 0$ and applying \cite[Corollary 1]{C:BouFeh10} shows that the conditional min-entropy (conditioned on $R$'s portion of the state) of $x_I$ is at least $\mathsf{wt}(I) - \epsilon t$.



\end{proof}


==> sec-tech-overview.tex <==
\section{Technical Overview}
\label{sec:techniques}

This work establishes that (1) black-box use of post-quantum one-way functions suffices for post-quantum \emph{extractable and equivocal} commitment schemes and moreover, that (2)~\cite{FOCS:CreKil88} quantum oblivious transfer instantiated with such commitments is a standard \emph{simulation-secure} oblivious transfer. Crucially, the standard notion of simulation-secure (quantum) oblivious transfer that we achieve is sequentially composable and suffices to achieve general-purpose secure quantum computation.

Before explaining our technical approach, we provide a complete review of the original~\cite{FOCS:CreKil88} protocol.

\subsection{Recap: Quantum Oblivious Transfer from Commitments}
\label{subsec:bbcs}

In quantum oblivious transfer (QOT), a quantum sender holding two classical messages $m_0,m_1$ engages in an interactive protocol over a quantum channel with a quantum receiver holding a classical choice bit $b$. Correctness requires the receiver to learn $m_b$ by the end of the protocol.
Informally, security demands that a malicious receiver only learn information about one of $m_0,m_1$, and that a malicious sender learn nothing about $b$.
Somewhat more formally, as discussed earlier, our focus is on the standard simulation-based notion of security. This stipulates the existence of an efficient quantum simulator that generates the view of an adversary (sender/receiver) when given access to an ideal OT functionality. In particular, when simulating the view of a malicious sender, this simulator must extract the sender's inputs $(m_0, m_1)$ without knowledge of the receiver's input $b$. And when simulating the view of a malicious receiver, the simulator must extract the receiver's input $b$, and then simulate the receiver's view given just $m_b$.

We recall the construction of quantum oblivious transfer due to~\cite{FOCS:CreKil88} (henceforth CK88), which combines the information theoretic quantum key distribution protocol of~\cite{BenBra84} (henceforth BB84) with cryptographic bit commitments.
%We clarify that this protocol {\em does not satisfy} simulation-based security.

\paragraph{CK88 First Message.} The first message of the CK88 protocol exactly follows the beginning of the BB84 protocol. For classical bits $y,z$, let $\ket{y}_z$ denote $\ket{y}$ if $z = 0$, and $(\ket{0} + (-1)^y\ket{1})/\sqrt{2}$ if $z = 1$, i.e. the choice of $z$ specifies whether to interpret $y$ as a computational or Hadamard basis vector. Let $\lambda$ denote the security parameter. The sender samples two random $2\lambda$-bit strings $x$ and $\theta$, and constructs ``BB84 states'' $\ket{x_i}_{\theta_i}$ for $i \in [2\lambda]$. The sender forwards these $2\lambda$ BB84 states $(\ket{x_i}_{\theta_i})_{i \in [2\lambda]}$ to the receiver. Next, the receiver samples a $2\lambda$-bit string $\hat{\theta}$, measures each $\ket{x_i}_{\theta_i}$ in the basis specified by $\hat{\theta}_i$, and obtains a $2\lambda$-bit measurement result string $\hat{x}$.

\paragraph{CK88 Measurement-Check Subprotocol.} At this point, the CK88 and BB84 protocols diverge. Since the BB84 protocol is an interaction between two \emph{honest} parties, it assumes the parties comply with the protocol instructions. However, in the CK88 protocol, a malicious receiver who does not measure these BB84 states will be able to compromise sender privacy later in the protocol. Therefore, the next phase of CK88 is a measurement-check subprotocol designed to catch a malicious receiver who skips the specified measurements. This subprotocol requires the use of a quantum-secure classical commitment scheme; for the purposes of this recap, one should imagine a commitment with idealized hiding and binding properties. The subprotocol proceeds as follows:
\begin{itemize}
\item For each $i \in [2\lambda]$, the receiver commits to $(\hat{\theta}_i,\hat{x}_i)$.
\item Next, the sender picks a random set $T$ of $\lambda$ indices from $[2\lambda]$, and challenges the receiver to open the corresponding commitments.
\item The receiver sends $(\hat{\theta}_i,\hat{x}_i)$ along with the corresponding opening for each $i \in T$. 
\item The sender verifies each commitment opening, and furthermore checks that $\hat{x}_i = x_i$ for each $i \in T$ where $\hat{\theta}_i = \theta_i$. If any of these checks fail, the sender aborts.
\end{itemize}

The rough intuition for the subprotocol is simple: from the receiver's point of view, the BB84 states are maximally mixed and therefore completely hide $x_i$ and $\theta_i$. For any index $i$ that the receiver does not measure, it must guess $\hat{x}_i$. From the receiver's perspective, the sender checks $\hat{x}_i$ against $x_i$ if two $1/2$-probability events occur: (1) $i$ is included in $T$, and (2) $\hat{\theta}_i = \theta_i$. This means a malicious receiver who skips a significant number of measurements will be caught with overwhelming probability.

\paragraph{CK88 Privacy Amplification.} If all the subprotocol checks pass, the sender continues to the final stage of the CK88 protocol. For convenience, relabel the $\lambda$ indices in $[2\lambda] \setminus T$ from $1$ to $\lambda$; all indices corresponding to opened commitments are discarded for the remainder of the protocol.

For each $i \in [\lambda]$, the sender reveals the correct measurement basis $\theta_i$. The receiver then constructs the index set $I_b$ --- where $b$ is its choice bit for the oblivious transfer --- as the set of all $i \in [\lambda]$ where $\theta_i = \hat{\theta}_i$. It sets $I_{1-b}$ to be the remaining indices, and sends $(I_0, I_1)$ to the sender. Note that by the hiding property of the commitments, the sender should not be able to deduce $b$ from $(I_0,I_1)$; furthermore, $I_0$ and $I_1$ will both be close to size $\lambda/2$, since for each $i \in [\lambda]$, the receiver committed to $\hat{\theta}_i$ before obtaining $\theta_i$.

On receiving $I_0,I_1$, the sender sets $x_0 \coloneqq (x_i)_{i \in I_0}$ and $x_1 \coloneqq (x_i)_{i \in I_1}$. The intuition is that if a receiver honestly constructs $(I_0, I_1)$, it will only have information about $x_b$ corresponding to its choice bit $b$. However, it turns out that even if the receiver maliciously constructs $(I_0,I_1)$, at least one of $x_0$ and $x_1$ will have high min-entropy from its point of view. Thus, by standard privacy amplification techniques, the sender can complete the oblivious transfer as follows. It samples two universal hash functions $h_0$ and $h_1$, both with $\ell$-bit outputs, and uses $h_0(x_0)$ to mask the $\ell$-bit message $m_0$, and uses $h_1(x_1)$ to mask $m_1$. That is, the sender sends $(h_0,h_1,h_0(x_0) \oplus m_0, h_1(x_1) \oplus m_1)$ to the receiver, who can then use $x_b$ to recover $m_b$. Since $x_{1-b}$ will have high entropy, the leftover hash lemma implies that $h_{1-b}(x_{1-b})$ is statistically close to uniform, which hides $m_{1-b}$ from the receiver.

\dakshita{Added the section below}
\paragraph{Simulation-Based Security.}
Turning this intuition into a proof of simulation-based security of the resulting QOT requires some additional insights~\cite{C:DFLSS09}, and requires the commitments used in the measurement-check subprotocol to satisfy two additional properties: extractability and equivocality. In what follows, we briefly summarize why these properties help achieve simulation-based security. 


To argue that the resulting QOT protocol satisfies security against a malicious sender, one must demonstrate the existence of a simulator that simulates the sender's view by generating messages on behalf of an honest receiver, and extracts both QOT inputs of the sender\footnote{We refer the reader to Section~\ref{sec:otdef} for a formal definition of simulation-based QOT.}. Now, the measurement-check subprotocol described above is designed to ensure that at least one of the sender's inputs is hidden from a receiver. To nevertheless enable the simulator to extract both sender inputs, the idea in~\cite{C:DFLSS09} is to modify the commitments used in the measurement-check subprotocol with {\em equivocal commitments} that allow the simulator to later open these commitments to any value of its choice. This enables the simulator to defer any measurements until after it obtains the set $T$ from the sender, and then selectively measure {\em only} the states that correspond to indices in $T$. All other states are left untouched until the sender reveals its measurement bases in the final stage of the CK88 protocol.
Upon obtaining the sender's ``correct'' measurement bases, the simulator measures all the remaining states in the correct bases, allowing it to learn both the inputs of the sender.
%In summary, the key tool that enables simulation against a malicious sender is an {\em equivocal} commitment, that allows the simulator to generate commitments that can be opened to any value. 


To demonstrate that the resulting QOT protocol satisfies security against a malicious receiver, one must demonstrate the existence of a simulator that simulates the receiver's view by generating messages on behalf of an honest sender, and extracts the receiver's choice bit. 
Again by design, the measurement-check subprotocol ensures that the receiver's choice bit hidden is hidden from the sender. To nevertheless enable the simulator to extract this choice bit,~\cite{C:DFLSS09} modify the commitments in the measurement-check subprotocol so that the simulator is able to extract all of the $\{(\widehat{\theta}_i, \widehat{x}_i)\}_{i \in [2\lambda]}$ from the receiver's commitments. This enables the simulator to compute which one of the sets $I_0, I_1$ contain more indices $i$ for which $\theta_i = \widehat{\theta}_i$; clearly the set with more indices corresponds to the receiver's choice bit.
In summary, the key tool that enables simulation against a malicious receiver is an {\em extractable} commitment, that forces the receiver to use commitments for which the simulator can extract the committed value, without ever running the opening phase. 



%and requires the bit commitments used in the protocol to satisfy some additional properties.
To conclude, following~\cite{C:DFLSS09} the CK88 protocol can be shown to satisfy simulation-based security as long as the commitments used in the measurement-check subprotocol satisfy both the {\em extractability} and {\em equivocality} properties that were informally described above.
%Specifically, it is known that such a proof can be obtained as long as the underlying commitments are simultaneously \emph{extractable and equivocal}~\cite{C:DFLSS09}. 
%that the CK88 QOT protocol satisfies simulation-based security when instantiated with an \emph{extractable and equivocal} commitment.

%Roughly speaking, a commitment scheme is said to be \emph{extractable} if for any adversarial quantum committer that successfully completes the commitment phase, there exists an efficient quantum algorithm (called the extractor) which outputs the committed bit.
%Informally, a quantum commitment protocol is \emph{equivocal} if there exists an efficient quantum algorithm called the \emph{equivocator}, that with access to the receiver, can generate commitments that can be opened to any value. 





With this in mind, we now describe our primary technical contribution: a construction of the required extractable and equivocal commitments based on black-box use of quantum-hard one-way functions. 
%that will suffice to instantiate the measurement-check subprotocol.

\subsection{Our Construction: A High-Level Overview}
\label{subsec:overview}

The rest of this technical overview describes our \emph{black-box} construction of simultaneously \emph{extractable and equivocal} quantum bit commitments from any quantum-hard one-way function. 

The ingredients for our construction are the following:
\begin{itemize}
\item A general-purpose ``equivocality compiler'' that turns any bit commitment scheme --- classical or quantum --- into an \emph{equivocal} quantum commitment scheme. Moreover, if the original commitment scheme is \emph{extractable}, this compiler outputs an \emph{extractable and equivocal} commitment scheme. 
\item A general-purpose ``extractability compiler'' that turns any \emph{equivocal} bit commitment scheme --- classical or quantum --- into an \emph{extractable but not equivocal} commitment scheme.
\end{itemize}
Both of these compilers require no additional computational assumptions beyond those of the original commitment schemes. Given these compilers, we build extractable and equivocal commitments via the following steps:
\begin{itemize}
\item \textbf{Instantiation:} Begin with Naor's statistically-binding, computationally hiding commitments~\cite{JC:Naor91}. Naor's construction makes black-box use of one-way functions and achieves post-quantum computational hiding assuming post-quantum security of the one-way function.\footnote{In slightly more detail, Naor's commitment scheme makes black-box use of any pseudo-random generator (PRG). It is straightforward to verify that if the PRG is post-quantum secure, the commitment satisfies computational hiding against quantum attackers. A black-box construction of pseudo-random generators from one-way functions is due to~\cite{HILL99}; Aaronson~\cite{Aaronson09} and Zhandry~\cite{FOCS:Zhandry12} observed that~\cite{HILL99} applies to non-uniform quantum attackers with \emph{classical} advice. This can be extended to handle non-uniform {quantum} advice by giving the one-way function attacker constructed in the~\cite{HILL99} reduction many copies of the PRG attacker's non-uniform quantum advice (which only requires some polynomial upper bound on the number of times the reduction invokes the PRG attacker).}
\item \textbf{Step 1:} Plug Naor's commitments into our equivocality compiler to obtain an \emph{equivocal} quantum bit commitment scheme.
\item \textbf{Step 2:} Feed the resulting equivocal quantum bit commitments into our extractability compiler to obtain an \emph{extractable but not equivocal} quantum bit commitment.
\item \textbf{Step 3:} Run the equivocality compiler \emph{a second time}, but now starting with the extractable commitments produced by the previous step. This gives the desired \emph{extractable and equivocal} quantum bit commitments.
\end{itemize}

\ifsubmission
\else
We briefly remark that if one did not care about obtaining a construction that only makes \emph{black-box} use of one-way functions, it would only be necessary to invoke the equivocality compiler once. In slightly more detail, we could design an alternative extractability compiler that works with any (not necessarily equivocal) bit commitment scheme by additionally relying on post-quantum zero-knowledge proofs~\cite{STOC:Watrous06}; this approach would still give a construction of quantum oblivious transfer from post-quantum one-way functions, but the zero-knowledge proofs would be used to prove statements involving the \emph{description} of some one-way function, which is a non-black-box use of the primitive. 
We believe that constructing QOT from quantum-hard one-way functions is interesting regardless of whether or not the construction is black-box. 
However, as discussed in Section \ref{subsec: our results}, black-box constructions are significantly preferred over non-black-box ones, especially in the quantum setting. Therefore our focus in the rest of this overview will be on presenting a black-box construction.
\fi

\ifsubmission
\else
\paragraph{Organization.} We describe our equivocality compiler in~\cref{subsec:equiv-compiler} and our extractability compiler in~\cref{subsec:ext-compiler}. In~\cref{subsec:putting-it-together}, we briefly discuss implications for secure computation in a quantum world.
\fi

\subsection{Making Any Quantum (or Classical) Commitment Equivocal}
\label{subsec:equiv-compiler}
%\dakshita{add more general comment about classical compilers and NBB use somewhere.}

Recall that a quantum commitment protocol is \emph{equivocal} if an efficient quantum algorithm called the \emph{equivocator}, with access to the receiver, can generate commitments that can be opened to any value. More precisely, for any receiver (modeled as an efficient malicious quantum algorithm), there must exist an equivocator who can generate a computationally indistinguishable commitment that the equivocator can later open arbitrarily. 

In this subsection, we describe a \emph{black-box} compiler for a fairly general task (which may be of independent interest): making any \emph{classical or quantum} commitment equivocal. Recall from~\cref{subsec:overview} that we will need to invoke our equivocality compiler \emph{twice}, once on a classical bit commitment scheme, and once on an extractable quantum bit commitment scheme; in the latter case, our compiler will need to preserve the extractability of the original commitment. Since classical commitments are a subclass of quantum commitments, our exposition will focus on challenges unique to the quantum setting.  

\ifsubmission
\else

\paragraph{Why Existing Classical Solutions Are Insufficient.} Let us briefly relax our goal of using one-way functions in an exclusively black-box way. Then there is a simple equivocality compiler that applies to any (statistically-binding and computationally-hiding) classical commitment. Recall that quantum-hard one-way functions imply post-quantum zero-knowledge proofs for $\mathsf{NP}$~\cite{STOC:Watrous06}. Now, in the opening phase of the commitment, to open to a bit $b$, the committer will not send the randomness used to commit to $b$ in the clear. Instead, the committer sends a zero-knowledge proof for the \textsf{NP} statement that there exist randomness consistent with the commitment, and opening to $b$. Equivocation is achieved by simulating the zero-knowledge proof. Unfortunately, this technique fails when the commitment involves \emph{quantum} communication, since the statement to be proven is no longer an \textsf{NP} statement (nor a \textsf{QMA} statement). Therefore, we construct a compiler that only makes black-box use of the underlying commitment, and leverages Watrous's rewinding lemma in the proof of equivocality~\cite{STOC:Watrous06}.

\fi



%A classical bit commitment can be made equivocal by having the committer (1) run the original commitment twice, sequentially, and then (2) prove in zero-knowledge that both commitments are to the same bit (note that this step is non-black-box in the underlying commitment scheme). To decommit, the committer randomly decommits to one of the two commitments. To equivocate, commit to a random bit $b$ in the first commitment, $1-b$ in the second commitment, and then use the zero-knowledge simulator to simulate a proof that the commitments are to the same bit. This commitment can later be opened arbitrarily.

%This equivocality compiler immediately runs into issues if the base commitment scheme (i.e. the commitment scheme we begin with) involves quantum communication. When the commitment transcripts --- say $c_1$ and $c_2$ --- are classical, the committer gives a zero-knowledge proof of the $\mathsf{NP}$ statement ``$c_1$ and $c_2$ are commitments to the same bit $b$.'' However, if the commitments are quantum, then the committer would need to prove a statement that explicitly contains/references quantum states. Such proof systems are currently beyond the reach of known techniques. We stress that even interactive arguments for QMA do not suffice here, since QMA only permits quantum \emph{witnesses}, not statements.

%We overcome this barrier by replacing the zero-knowledge proof with a quantum-compatible consistency check (while also removing the non-black-box use of one-way functions).

\paragraph{Our Equivocality Compiler.} In our construction, to commit to a bit $b$, the committer and receiver will perform $\lambda$ sequential repetitions of the following subprotocol:
\begin{itemize}
\item The (honest) committer samples 2 uniformly random bits $u_0,u_1$, and commits to each one \emph{twice} using the base commitment scheme. Let the resulting commitments be $\mathbf{c}_{0}^{(0)},\mathbf{c}_{0}^{(1)},\mathbf{c}_{1}^{(0)},\mathbf{c}_{1}^{(1)}$, where the first two are to $u_0$ and the second two are to $u_1$. Note that since the base commitment scheme can be an arbitrary quantum interactive commitment, each commitment $\mathbf{c}_{b_1}^{(b_2)}$ corresponds to the receiver’s quantum state after the commitment phase of the base commitment.
\item The receiver sends the committer a random challenge bit $\beta$.
\item The committer opens the two base commitments $\mathbf{c}_{\beta}^{(0)},\mathbf{c}_{\beta}^{(1)}$. If the openings are invalid or the revealed messages are different, the receiver aborts the entire protocol.
\end{itemize}
If these $\lambda$ executions pass, the receiver is convinced that a majority of the committer's remaining $2\lambda$ unopened commitments are honestly generated, i.e. most pairs of commitments are to the same bit. 

Rewriting the (honest) committer’s unopened bits as $u_1,\dots,u_\lambda$, the final step of the commitment phase is for the committer to send $h_i \coloneqq u_i \oplus b$ for each $i \in [\lambda]$ (recall that $b$ is the committed bit).

To decommit, the committer reveals each $u_i$ by picking one of the two corresponding base commitments at random, and opening it. The receiver accepts if each one of the base commitment openings is valid, and the opened $u_i$ satisfies $h_i \oplus u_i = b$ for every $i$.

The (statistical) binding property of the resulting commitment can be seen to follow from the (statistical) binding of the underlying commitment. For any commitment, define the unique committed value as the majority of $(h_i \oplus u_i)$ values in the unopened commitments, setting $u_i$ to $\bot$ if both committed bits in the $i^{th}$ session differ.
Due to the randomized checks by the receiver, any committer that tries to open to a value that differs from the unique committed value will already have been caught in the commit phase, and the commitment will have been rejected with overwhelming probability. A similar argument also allows us to establish that this transformation preserves extractability of the underlying commitment. We now discuss why the resulting commitment is {\em equivocal}.
%It is straightforward to verify that this commitment scheme satisfies the standard properties.

\paragraph{Quantum Equivocation.} The natural equivocation strategy should have the equivocator (somehow) end up with $\lambda$ pairs of base commitments where for each $i \in [\lambda]$, the pair of commitments is to $u_i$ and $1-u_i$ for some random bit $u_i$. This way, it can send an appropriately distributed string $h_1,\cdots,h_\lambda$, and later open to any $b$ by opening the commitment to $b \oplus h_i$ for each $i$. 

We construct our equivocator using Watrous’s quantum rewinding lemma~\cite{STOC:Watrous06} (readers familiar with Watrous’s technique may have already noticed our construction is tailored to enable its use).

We give a brief, intuition-level recap of the rewinding technique as it pertains to our equivocator. Without loss of generality, the malicious quantum receiver derives its challenge bit $\beta$ by performing some binary outcome measurement on the four quantum commitments it has just received (and on any auxiliary states). Our equivocator succeeds (in one iteration) if it can prepare four quantum commitments $\mathbf{c}_{0}^{(0)},\mathbf{c}_{0}^{(1)},\mathbf{c}_{1}^{(0)},\mathbf{c}_{1}^{(1)}$ where:
\begin{enumerate}
\item $\mathbf{c}_{\alpha}^{(0)},\mathbf{c}_{\alpha}^{(0)}$ are commitments to the same random bit,
\item $\mathbf{c}_{1-\alpha}^{(0)},\mathbf{c}_{1-\alpha}^{(0)}$ are commitments to a random bit and its complement,
\item on input $\mathbf{c}_{0}^{(0)},\mathbf{c}_{0}^{(1)},\mathbf{c}_{1}^{(0)},\mathbf{c}_{1}^{(1)}$, the receiver produces challenge bit $\beta = \alpha$.
\end{enumerate}
That is, the equivocator is successful if the receiver’s challenge bit $\beta$ corresponds to the bit $\alpha$ that it can open honestly. Watrous's~\cite{STOC:Watrous06} rewinding lemma applies if the distribution of $\beta$ is \emph{independent} of the receiver’s choice of $\alpha$, which is guaranteed here by the hiding of the base commitments. Thus, the rewinding lemma yields a procedure for obtaining an honest-looking interaction where all three properties above are met. Given the output of the rewinding process, the equivocator has successfully ``fooled’’ the committer on this interaction and proceeds to perform this for all $\lambda$ iterations. As described above, fooling the committer on all $\lambda$ iterations enables the equivocator to later open the commitment arbitrarily.

%\paragraph{Extractable and Equivocal Quantum Bit Commitments.} It is straightforward to verify that our compiler preserves extractability of the base commitment scheme. 

\subsection{An Extractability Compiler for Equivocal Commitments}
\label{subsec:ext-compiler}

In this subsection, we compile any classical or quantum \emph{equivocal} bit commitment into a quantum \emph{extractable} bit commitment. We stress that even though this compiler is applied to equivocal bit commitments, the resulting commitment is \emph{not} guaranteed to be simultaneously \emph{extractable and equivocal}; we refer the reader to~\cref{subsec:overview} for details on how this compiler fits into our final construction.

% Our first technical step is to construct an extractable (but not yet equivocal) quantum commitment from any quantum-hard one-way function. Unlike prior work on post-quantum OT that required public-key assumptions, we leverage quantum communication to improve assumptions to quantum one-way functions.
% Our extractable quantum bit commitment builds on the BB84/BBCS template.

Recall that a commitment scheme is \emph{extractable} if for any adversarial quantum committer that successfully completes the commitment phase, there exists an efficient quantum algorithm (called the extractor) which outputs the committed bit.

% \footnote{The precise definition requires slightly more care to state correctly (\cref{def:extcom}, but this intuitive extraction definition is sufficient for the technical overview.}

% originally was going to recall a more technical definition of extractability, but it seemed too complicated for the tech overview / unnecessary for understanding the key ideas. 
% 
% A quantum bit commitment is \emph{extractable} if for any efficient adversarial committer, there exists an efficient quantum algorithm called the extractor such that the following two distributions are \emph{computationally} indistinguishable:
% \begin{itemize}
% \item The ``real'' view $(\boldsymbol{\rho},b)$ obtained after an interaction between the adversarial committer and the honest receiver, where $\boldsymbol{\rho}$ is the leftover state of the committer after opening the commitment, and $b$ is the output of the receiver (i.e. if the receiver accepts the opening, then $b$ is the committed bit, and otherwise $b = \bot$).
% \item The ``simulated'' view $(\boldsymbol{\rho}_{\mathsf{sim}},b)$, where $b$ is output by the 
% \end{itemize}


% \paragraph{Ingredients.} We will use the following cryptographic tools:
% \begin{itemize}
% \item A classical bit commitment scheme that satisfies computational hiding against quantum attackers and statistical binding. 
% \item A classical zero-knowledge interactive argument system for $\mathsf{NP}$ where zero-knowledge holds against malicious quantum verifiers.
% \end{itemize}
% Both of these ingredients can be realized from any post-quantum one-way function.\footnote{In particular, post-quantum one-way functions imply post-quantum pseudorandom generators via~\cite{HILL99} (that this holds for quantum adversaries was observed independently by Aaronson~\cite{Aaronson09} and Zhandry~\cite{FOCS:Zhandry12}) It is straightforward to verify that Naor's construction~\cite{JC:Naor91} of bit commitments with statistical binding and computational hiding from any pseudorandom generator is post-quantum if the pseudo-random generator is post-quantum. Finally, these commitments can be plugged into any of the classic ``commit-challenge-response'' argument systems for $\mathsf{NP}$ such as Blum's Hamiltonicity protocol~\cite{Blum86} or Goldreich, Micali, and Wigderson's 3-coloring protocol~\cite{C:GolMicWig86} to yield a zero-knowledge argument system; post-quantum zero-knowledge is argued with Watrous's simulation technique~\cite{STOC:Watrous06}.}. Looking ahead, we will use extractable and equivocal commitments to instantiate the commitments in the QOT protocol of Section \ref{subsec:bbcs}. When we do this, the receiver of the QOT protocol will take the role of the \emph{committer} in the following construction, and the sender of the QOT protocol will take the role of the \emph{receiver} of an extractable and equivocal commitment. Thus, interestingly, in the fully compiled QOT protocol, both the sender and the receiver have to prepare BB84 states in different parts of the protocol.

\paragraph{Construction.} The committer, who intends to commit to a classical bit $b$, begins by sampling $2\lambda$-bit strings $x$ and $\theta$. It generates the corresponding $2\lambda$ BB84 states $\ket{x_i}_{\theta_i}$ and sends this to the receiver. The receiver picks $2\lambda$ random measurement bases $\hat{\theta}_i$, and measures each $\ket{x_i}_{\theta_i}$ in the corresponding basis, obtaining outcomes $\hat{x}_i$. 

Next, the receiver and committer engage in a CK88-style measurement-check subprotocol. That is, they temporarily switch roles (for the duration of the subprotocol), and perform the following steps:
\begin{enumerate}
\item The receiver (acting as a committer in the subprotocol), commits to each $\hat{\theta}_i$ and $\hat{x}_i$ (for each $i \in [2\lambda]$) with an \emph{equivocal} commitment.
\item The committer (acting as a receiver in the subprotocol), asks the receiver to open the equivocal commitments for all $i \in T$, where $T \subset [2\lambda]$ is a random set of size $\lambda$.
\item The receiver (acting as a committer in the subprotocol) opens the $\lambda$ commitments specified by $T$.
\end{enumerate}


% That is, the receiver commits to each $\hat{\theta}_i$ and $\hat{x}_i$, the   difference in our setting  receiver commits to each $\hat{\theta}_i$ and $\hat{x}_i$ using a (possibly quantum) \emph{equivocal} commitment. 

% However, the measurement-check subprotocol used here will differ from the one described in~\cref{subsec:bbcs} in several ways:
% \begin{itemize}
% \item In~\cref{subsec:bbcs}, the precise instantiation of the commitment scheme is unspecified. Here, we have the receiver commit to each $\hat{\theta}_i$ and $\hat{x}_i$ by generating statistically-binding and computationally-hiding commitments. Concretely, for each $i$, the receiver samples randomness $r_i$ and $s_i$, computes $c_i = \mathsf{Com}(\hat{\theta}_i,r_i)$ and $d_i = \mathsf{Com}(\hat{x}_i,s_i)$, and sends $c_i,d_i$. 
% \item The sender will still challenge the receiver to open the commitments to $\hat{\theta}_i$ and $\hat{x}_i$ on a random selection $T \subset [2\lambda]$ of size $\lambda$. For each $i \in [T]$, the receiver will send the committed messages $\hat{\theta}_i$ and $\hat{x}_i$, but crucially does not send the openings $r_i,s_i$. Instead, the receiver \emph{proves in zero-knowledge} the $\mathsf{NP}$ statement: ``for $c_i,d_i,\hat{\theta}_i,\hat{x}_i$, there exist $r_i,s_i$ such that $c_i = \mathsf{Com}(\hat{\theta}_i,r_i)$ and $d_i = \mathsf{Com}(\hat{\theta}_i,r_i)$.'' The committer will only proceed if it accepts all of the zero-knowledge arguments, and for all $i \in [T]$ where $\theta_i = \hat{\theta}_i$, the measurement outcomes $x_i$ and $\hat{x}_i$ agree.
% \end{itemize}
% By the statistical binding of $\mathsf{Com}$ and the soundness of the zero-knowledge argument system, an efficient receiver will only be able to convince the verifier there exist openings if the claimed values of $\hat{\theta}_i,\hat{x}_i$ match the initially committed values. Note that known zero-knowledge argument systems from one-way functions are interactive, so this modification will increase the number of rounds for the measurement-check subprotocol.

Provided the receiver passes the measurement-check subprotocol, the committer generates the final message of the commitment phase as follows:
\begin{itemize}
\item Discard the indices in $T$ and relabel the remaining $\lambda$ indices from $1$ to $\lambda$. 
\item Partition $\{x_1,\dots,x_\lambda\}$ into $\sqrt{\lambda}$ strings $\vec{x}_1,\dots,\vec{x}_{\sqrt{\lambda}}$ each of length $\sqrt{\lambda}$. 
\item Sample $\sqrt{\lambda}$ universal hash functions $h_1,\dots,h_{\sqrt{\lambda}}$ each with 1-bit output.
\item Finally, send
\[ (\theta_i)_{i \in [\lambda]}, (h_j,h_j(\vec{x}_j) \oplus b)_{j \in [\sqrt{\lambda}]}.\]
\end{itemize}

This concludes the commitment phase.

To decommit, the committer reveals $b$ and $(\vec{x}_1,\dots,\vec{x}_{\sqrt{\lambda}})$. The receiver accepts if (1) for each $j$, the bit $b$ and the value $\vec{x}_j$ are consistent with the claimed value of $h_j(\vec{x}_j) \oplus b$ from the commit phase, and (2) for each index $i \in [\lambda]$ where $\theta_i = \hat{\theta}_i$, the $x_i$ from the opening is consistent with $\hat{x}_i$.

\paragraph{Extraction.} The use of equivocal commitments in the measurement-check subprotocol makes extraction simple. Given any malicious committer, we construct an extractor as follows. 

The extractor plays the role of the receiver and begins an interaction with the malicious committer. But once the committer sends its $2\lambda$ BB84 states, the extractor skips the specified measurements, instead leaving these states unmeasured. Next, instead of performing honest commitments to each $\hat{\theta}_i,\hat{x}_i$, the extractor invokes (for each commitment) the equivocator algorithm of the underlying equivocal commitment scheme. Since the equivocator is guaranteed to produce an indistinguishable commitment from the point of view of any malicious receiver for the equivocal commitment, this dishonest behavior by the extractor will go undetected. 

% (recall that our malicious committer is playing the role of a malicious receiver for the equivocal commitment in the measurement-check subprotocol)

When the malicious committer responds with a challenge set $T \subset [2\lambda]$, the extractor samples uniformly random bases $\hat{\theta}_i$ for each $i \in T$, measures the corresponding BB84 states to obtain $\hat{x}_i$ values, and sends $(\hat{\theta}_i,\hat{x}_i)_{i \in T}$. Moreover, the equivocator (for each commitment) will enable the extractor to generate valid-looking openings for all of these claimed values. 

Thus, the malicious committer proceeds with the commitment protocol, and sends 
\[(\theta_i)_{i \in [\lambda]}, (h_j,h_j(\vec{x}_j)\oplus b)_{j \in [\sqrt{\lambda}]}\]
to the extractor. These correspond to the $\lambda$ BB84 states that the extractor has not yet measured, so it can simply read off the bases $\theta_i$, perform the specified measurements, and extract the committer's choice of $b$.

% In summary, the key technical trick is the following: by replacing the commitment opening step with post-quantum zero-knowledge arguments, we enable an extractor to bypass the committer's measurement checks and extract the committed value.

\ifsubmission
\paragraph{Statistical Hiding.}
Intuitively, statistical hiding of the above commitment protocol follows because the measurement-check subprotocol forces the receiver to measure states in arbitrary bases, which destroys information about the corresponding $x_i$ values whenever $\widehat{\theta}_i \neq \theta_i$. The formal argument is a straightforward application of a quantum sampling lemma of~\cite{C:BouFeh10}, devised in part to simplify analysis of~\cite{FOCS:CreKil88}-style protocols, and we defer further details to the supplementary materials.
\else
\paragraph{Statistical Hiding.}
Intuitively, statistical hiding of the above commitment protocol follows because the measurement-check subprotocol forces the receiver to measure states in arbitrary bases, which destroys information about the corresponding $x_i$ values whenever $\widehat{\theta}_i \neq \theta_i$. The formal argument is a straightforward application of a quantum sampling lemma of~\cite{C:BouFeh10}, devised in part to simplify analysis of~\cite{FOCS:CreKil88}-style protocols, and we defer further details to the body of the paper.
\fi

\subsection{Putting it Together: From Commitments to Secure Computation.}
\label{subsec:putting-it-together}

\ifsubmission
Plugging the compilers of~\cref{subsec:equiv-compiler,subsec:ext-compiler} into the steps described in~\cref{subsec:overview} yields a black-box construction of simultaneously extractable and equivocal quantum bit commitments from quantum-hard one-way functions. Following~\cite{C:DFLSS09}, these commitments can be plugged into CK88 to obtain maliciously simulation-secure QOT (see~\cref{sec: OT from eecom} for further details). Finally, going from QOT to arbitrary secure computation (in a black-box way) follows from prior works of~\cite{STOC:Kilian88,C:IshPraSah08,DNS12,EC:DGJMS20}; a more thorough discussion is available in the supplementary materials.
\else
Plugging the compilers of~\cref{subsec:equiv-compiler,subsec:ext-compiler} into the steps described in~\cref{subsec:overview} yields a black-box construction of simultaneously extractable and equivocal quantum bit commitments from quantum-hard one-way functions. Following~\cite{C:DFLSS09}, these commitments can be plugged into CK88 to obtain maliciously simulation-secure QOT (see~\cref{sec: OT from eecom} for further details). Finally, going from QOT to arbitrary secure computation (in a black-box way) follows from a number of prior works, which we briefly survey here for the sake of completeness (see also the discussion in~\cref{subsec: our results}).
\begin{itemize}
\item \textbf{Secure Computation of Classical Functionalities.} It is well known that maliciously simulation-secure (classical) oblivious transfer can be used in a black-box way to build two-party (classical) computation~\cite{STOC:Kilian88}. This also extends to the multi-party setting tolerating upto all-but-one corruptions~\cite{C:IshPraSah08}. Since the constructions of \cite{STOC:Kilian88} and \cite{C:IshPraSah08} only make black-box use of the underlying oblivious transfer and the simulators are straight-line, their correctness/security guarantees continue to hold if parties are quantum and the oblivious transfer uses quantum communication. Therefore, if all parties are quantum and all pairs of parties are connected via authenticated quantum channels, they can securely compute any classical functionality assuming quantum-hard one way functions (and authenticated channels in the multi-party setting).
\item \textbf{Secure Computation of Quantum Functionalities.} \cite{DNS12} constructed a secure two-party quantum computation protocol assuming black-box access to any secure two-party classical computation protocol. \cite{EC:DGJMS20} proved the analogous statement in the multi-party setting: secure multi-party classical computation implies (in a black-box way) secure multi-party quantum computation. Therefore, by invoking the results in the previous bullet, quantum-hard one-way functions also suffice for arbitrary secure quantum computation (additionally assuming authenticated channels in the multi-party setting).
\end{itemize}
While the results in the second bullet technically subsume the first, stating them separately enables direct comparison with the classical setting. In particular, one takeaway is that while oblivious transfer is necessary and sufficient for secure computation in the classical world, quantum-hard one-way functions suffice for \emph{exactly the same task} when  parties (and their communication channels) are quantum. 
\fi

% Finally, as discussed in \cref{subsec: our results}, the previous works of \cite{EC:KatOstSmi03} and \cite{C:IshPraSah08} show how to construct two-party, respectively multi-party (assuming access to authenticated channels), secure computation with \emph{black-box} access to OT. In particular, these constructions are agnostic to how the underlying OT is implemented and thus work even if the OT involves quantum communication. Thus, our quantum OT immediately implies secure computation of classical functionalities. Moreover, the previous works of \cite{C:DupNieSal12} and \cite{EC:DGJMS20} show that black-box access to classical two-party, respectively multi-party, secure computation implies secure \emph{quantum} computation. 

%\fermi{to do: cite DFLSS, cite Dulek et al. say something about how Dulek makes black-box use of the classical secure computation protocol, etc}


% remark that this is fully generic, and is potentially of independent interest since it applies to any quantum commitment scheme


% Next, we give a generic transformation to make any quantum commitment equivocal. This transformation preserves extractability.

% \begin{itemize}
% \item \textbf{Key Idea 2:} By sending four commitments to two random bits and having the receiver randomly open one pair, we can assure the receiver (with constant error) that our other pair of commitments is in fact equal. But to equivocate, we can appeal to Watrous's Lemma and say that no matter how the receiver picks the pair of commitments to open to, we can set the other pair of commitments to be to two different bits commitment to be to two

% The zero-knowledge proof can be simulated, convincing the committer that the receiver actually performed the measurements. Finally when the committer sends the last message of the commit phase, the extractor can simply perform the measurements, learn the message, and output it.

% For reference, a full description is given in~\cref{fig:bbcs91}.

% \begin{figure}[ht!]
% \begin{pcvstack}[center]
% \centering
% \procedure[mode=text]{}{
%     $\mathsf{Sender} (m_0,m_1)$ \> \> $\mathsf{Receiver}(b)$
%     \\
%     \begin{subprocedure}{\pseudocode[width=5cm]{Define $\psi_{0,0} \coloneqq \ket{0}; \psi_{1,0} \coloneqq \ket{1};$\\ $\psi_{0,1} \coloneqq \ket{+}; \psi_{1,1} \coloneqq \ket{-}$.\\For $i \in [2n]$: $(x_i,\theta_i) \leftarrow \{0,1\}^2$.}}
%     \end{subprocedure}
% 	\>
% 	\sendmessageright*[2.5cm]{(\psi_{x_i,\theta_i})_{i \in [2n]}}
% 	\>
% 	\begin{subprocedure}\pseudocode[width=5cm]{For $i \in [2n]$: $\hat{\theta}_i \leftarrow \{0,1\}$.\\
% 	Let $\hat{x}_i$ be result of measuring $\psi_{x_i,\theta_i}$\\
% 	in $0/1$ basis if $\hat{\theta}_i =0$, $\pm$ basis if $\hat{\theta}_i = 1$.}
% 	\end{subprocedure}
% }

% \dbox{
% \procedure[mode=text]{\centering \footnotesize \textbf{Subprotocol:} Sender checks if receiver has performed measurements}{
% 	\>
% 	\sendmessageleft*[2.5cm]{(\com_i)_{i \in [2n]}}
% 	\>
% 	\begin{subprocedure}\pseudocode[width=5cm]{For $i \in [2n]$: $r_i \leftarrow \{0,1\}^\lambda$.\\
% 		$\com_i \coloneqq \Commit((\hat{\theta}_i,\hat{x}_i);r_i)$.}
% 	\end{subprocedure}
% 	\\
% 	\begin{subprocedure}\pseudocode[width=5cm]{Sample $T \subset [2n]$ of size $n$.}
% 	\end{subprocedure}
% 	\> 
% 	\sendmessageright*[2.5cm]{T}
% 	\>
% 	\\
% 	\begin{subprocedure}\pseudocode[width=5cm]{Check openings and $\hat{x}_i = x_i$ if $\hat{\theta}_i = \theta_i$.}
% 	\end{subprocedure} 
% 	\>
% 	\sendmessageleft*[2.5cm]{(\hat{\theta}_i,\hat{x}_i,r_i)_{i \in T}}
% 	\>
% }
% }

% \procedure[mode=text]{}{
%     \begin{subprocedure}\pseudocode[width=5cm]{$\overline{T} \coloneqq [2n]\setminus T$.}
%     \end{subprocedure}
% 	\>
% 	\sendmessageright*[2.5cm]{(\theta_i)_{i \in \overline{T}}}
% 	\>
% 	\\
% 	\>
% 	\sendmessageleft*[2.5cm]{I_0,I_1}
% 	\>
% 	\begin{subprocedure}\pseudocode[width=5cm]{$I_b \coloneqq \{i \in \overline{T} \mid \theta_i = \hat{\theta}_i\}; I_{1-b} \coloneqq \overline{T} \setminus I_b$.}
% 	\end{subprocedure}
% 	\\
% 	\begin{subprocedure}\pseudocode[width=5cm]{$x_0 \coloneqq (x_i)_{i \in I_0}$; $x_1 \coloneqq (x_i)_{i \in I_1}$;\\$s_0 \gets \{0,1\}^{|x_0|}; s_1 \gets \{0,1\}^{|x_1|}$;\\ $y_0 \coloneqq \langle s_0,x_0 \rangle \oplus m_0$; $y_1 \coloneqq \langle s_1,x_1 \rangle \oplus m_1$. }
% 	\end{subprocedure}
% 	\>
% 	\sendmessageright*[2.5cm]{s_0,s_1,y_0,y_1}
% 	\>
% 	\begin{subprocedure}\pseudocode[width=5cm]{Use $x_b$ to decrypt $m_b$.}
% 	\end{subprocedure}
% }
% \end{pcvstack}
% \caption{BBCS91 Oblivious Transfer from Commitments.}
% \label{fig:bbcs91}
% \end{figure}

% First, we show how to construct extractable quantum commitments from any post-quantum one-way function.

% \fermi{the following is just a temporary sketch}
% Key Points
% \begin{itemize}
% \item We consider commitments which are interactive quantum protocols. Such a commitment is extractable if there is a simulator such that for any adversarial committer, its view and the successfully decommitted message can be simulated.
% \item We show how to construct such a commitment assuming one-way functions. The sender sends the receiver a bunch of BB84 states. The receiver picks random measurement bases and commits to these bases using a statistically binding commitment scheme. The sender challenges the receiver to open half of these commitments on some set $T$. The receiver sends the messages (the bases and the resulting measurements) and engages in a ZK proof that there exists an opening (since we're only proving existence an opening, we'll need a statistically binding commitment). The sender checks that the measurements are correct where the bases match, and that the zero-knowledge proofs accept. If these accept, then the sender sends all the measurement bases for all the indices outside of $T$. Then for all the remaining indices, they are partitioned into $\lambda$-many $\lambda$-bit strings. We take the dot product of each one of these $x_i$ strings with a fresh random string $s_i$, and send over each $s_i$ along with $\langle s_i,x_i \rangle \oplus m$ where $m$ is the committed bit.
% \item The intuition is that because the sender does not know the receiver's measurement bases, the sender cannot equivocate on a superlog number of positions. 
% \item This is equivocal because the extractor can simply commit to all 0's, then perform honest measurements in random bases for all indices in $T$. Crucially, it doesn't measure anything outside of $T$. The zero-knowledge proof can be simulated, convincing the committer that the receiver actually performed the measurements. Finally when the committer sends the last message of the commit phase, the extractor can simply perform the measurements, learn the message, and output it.
% \item \textbf{Key Idea 1:} By having the receiver engage in ZK proofs that it can open the statistically binding commitments instead of actually opening them, we allow an extractor to simulate the ZK proofs, bypass the forced measurements on the BB84 states, and ``decrypt'' the commitments.
% \end{itemize}

% \subsection{Making Any Commitment Equivocal}

% Next, we give a generic transformation to make any quantum commitment equivocal. This transformation preserves extractability.

% \begin{itemize}
% \item \textbf{Key Idea 2:} By sending four commitments to two random bits and having the receiver randomly open one pair, we can assure the receiver (with constant error) that our other pair of commitments is in fact equal. But to equivocate, we can appeal to Watrous's Lemma and say that no matter how the receiver picks the pair of commitments to open to, we can set the other pair of commitments to be to two different bits commitment to be to two
% \end{itemize}

% \fermi{in progress}
% \begin{center}
% \begin{tikzpicture}
% \draw (0,0) -- (0,2);
% \draw (3,0) -- (3,2);
% \draw (6,0) -- (6,2);
% \draw (7,0) -- (7,2);
% \draw (10,0) -- (10,2);
% \draw (0,0) -- (10,0);
% \draw (0,1) -- (10,1);
% \draw (0,2) -- (10,2);
% \draw (1.5,1.7) node[font=\footnotesize] {$\Com(b_{1,0};r_{1,0})$};
% \draw (1.5,1.3) node[font=\footnotesize] {$\Com(b_{1,0};r'_{1,0})$};
% \draw (1.5,0.7) node[font=\footnotesize] {$\Com(b_{1,1};r_{1,1})$};
% \draw (1.5,0.3) node[font=\footnotesize] {$\Com(b_{1,1};r'_{1,1})$};
% \draw (4.5,1.7) node[font=\footnotesize] {$\Com(b_{2,0};r_{2,0})$};
% \draw (4.5,1.3) node[font=\footnotesize] {$\Com(b_{2,0};r'_{2,0})$};
% \draw (4.5,0.7) node[font=\footnotesize] {$\Com(b_{2,1};r_{2,1})$};
% \draw (4.5,0.3) node[font=\footnotesize] {$\Com(b_{2,1};r'_{2,1})$};
% \draw (6.5,1.5) node[font=\footnotesize] {$\cdots$};
% \draw (6.5,0.5) node[font=\footnotesize] {$\cdots$};
% \draw (8.5,1.7) node[font=\footnotesize] {$\Com(b_{n,0};r_{n,0})$};
% \draw (8.5,1.3) node[font=\footnotesize] {$\Com(b_{n,0};r'_{n,0})$};
% \draw (8.5,0.7) node[font=\footnotesize] {$\Com(b_{n,1};r_{n,1})$};
% \draw (8.5,0.3) node[font=\footnotesize] {$\Com(b_{n,1};r'_{n,1})$};
% \end{tikzpicture}
% \end{center}

==> specious.tex <==
\section{Specious adversaries in the QROM}

In this section, we recall the notion of privacy against specious adversaries, first defined in \cite{C:DupNieSal10}, and adapt this notion to setting of protocols for classical functionalities in the quantum random oracle model.

\paragraph{Two-party protocols in the QROM.} In order to define the notion of a specious adversary, we first give a more explicit description of an $n$-message two-party protocol $\Pi_\RO$ in the QROM. $\Pi_\RO$ describes an interaction between two oracle algorithms $A^H$ and $B^H$ that have access to a random oracle $H \gets \cH_{\cX,\cY}$. Assuming the party $A$ speaks first and last, the protocol consists of the following.

\begin{enumerate}
    \item Memory registers $\gray{A_1},\gray{B_2},\dots,\gray{A_{n-1}},\gray{B_n}$ and communication registers $\gray{C_1},\dots,\gray{C_n}$. We assume that $\gray{A_1}$ holds $A$'s input and $\gray{B_2}$ holds $B$'s input.
    \item Oracle quantum algorithms 
\end{enumerate}

\paragraph{Specious adversaries.}

\paragraph{Privacy against specious adversaries.}

==> spsot-from-owf.tex <==
\section{Weak OT from Extractable and Equivocal Commitments}
\renewcommand{\commit}{\mathsf{EECom}}

In what follows, we denote by $\secp$ the security parameter, by $m = m(\secp)$ a statistical security parameter (which can be set to $\secp$), and by $n = n(\secp)$ the length of sender inputs.
We let $\commit$ denote any statistically binding, quantum computationally hiding commitment, $\Pi_{\mathsf{ZK}}$ denote any quantum computational zero-knowledge proof for $\mathsf{NP}$, and $\Pi_{BB}$ denotes the OT protocol against benign receivers from~\cite{C:BenBra84}.

\protocol
{\proref{fig:weakot}}
{Weak OT Protocol.}
{fig:weakot}
{
\textbf{Sender $S$ Input:} Messages $m_0, m_1 \in \{0,1\}^{n} \times \{0,1\}^{n}$\\
\textbf{Receiver $R$ Input:} Bit $b \in \{0,1\}$\\

\underline{\textbf{The Protocol:}}
\begin{enumerate}
\item $S$ chooses $x \leftarrow \{0, 1\}^m$ and $\theta \leftarrow \{+, \times \}^m$ 
and sends $\ket{x}_\theta$ to $R$. 

\item $R$ chooses $\widehat{\theta} \leftarrow \{+, \times\}^m$
and obtains $\widehat{x} \in \{0, 1\}^m$ by measuring $\ket{x}_{\theta}$
in basis $\widehat{\theta}$.

$R$ commits to $\widehat{\theta}$ and $\widehat{x}$ position-wise: for $i \in [m]$, $R$ sends $c_i$ to $S$, where
$c_i : = \commit((\widehat{\theta}_i, \widehat{x}_i); r_i)$
for uniform randomness $r_i$. 

\item $S$ sends a random test subset $T \subset [m]$ of size $(m/2)$ to $R$. For every $i \in T$, $R$ sends $\widehat{x}_i$, $\widehat{\theta}_i$ to $S$. 

\item For $i \in T$, 
$R$ and $S$ take the roles of prover and verifier in $\Pi_{\mathsf{ZK}} (X_i,w_i,L)$ where: \\
$X_i = (c_i,\widehat{x}_i,\widehat{\theta}_i), w_i = \big(r_i\big)$ 
and $L = \Big\{(c,\alpha,\beta): \exists r \text{ s.t. } X= \commit\Big((\alpha, \beta);r\Big) \Big\}$.
%$(c_i,r_i;r_{A,i})$ for all $i \in T$. 

\item $S$ checks that the ZK proofs were accepted and that $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$. If all tests pass, $S$ accepts,
otherwise, $S$ rejects and aborts.

\item The tested positions are discarded by both parties: $S$ and $R$ restrict $x$ and $\theta$, respectively $\widehat{\theta}$ and $\widehat{x}$,
to $i \in \overline{T}$.

\item $S$ and $R$ execute $\Pi_{BB}$ (with $x, \theta, \widehat{x}$ and $\widehat{\theta}$ restricted to the positions $i \in \overline{T}$).
\end{enumerate}
}


\begin{lemma}
The protocol in Figure \ref{fig:weakot} is a weak OT protocol satisfying Definition \ref{def:ot} whenever $\commit$ is instantiated with any statistically binding quantum computationally hiding commitment and $\Pi_{ZK}$ is any post-quantum computational zero-knowledge proof.
\end{lemma}

\begin{proof}
Correctness of the protocol in Figure \ref{fig:weakot} follows by inspection. We now prove that the resulting weak OT protocol satisfies the following properties.
\begin{enumerate}
    \item {\bf Indistinguishability of Receiver Inputs.}
    This follows by the computational hiding of the commitment scheme $\mathsf{Commit}$, the zero-knowledge property of $\Pi_{ZK}$ and the (unconditional) receiver security of $\Pi_{BB}$.
    
    Specifically, suppose there exist
    bits $(b, b') \in \zo$, 
    a quantum polynomial-size sender $S^*$ and distinguisher $D^*$, and polynomial $\mathsf{poly}(\cdot)$ such that 
    $$\Big|\Pr[D^*(\view_{S^*}\langle S^*, R(b) \rangle) = 1] - \Pr[D^*(\view_{S^*}\langle S^*, R(b') \rangle) = 1] \Big| \geq \frac{1}{\mathsf{poly}(\secp)}$$
    
    Fix any such $(b,b')$, sender $S^*$ and distinguisher $D^*$.
    
    \noindent {\textbf{$\mathsf{Hyb}_1$.}} Define distribution $\mathsf{Hyb}_1$ as the output of $\simu_{\mathsf{ZK}}(V^*)$, where verifier $V^*$, which has the code of $S^*$ hardwired, is constructed as follows:
    \begin{enumerate}
        \item Emulate an interaction of $S^*$ with receiver $R(b)$ until the end of Step 3, in Figure~\ref{fig:weakot}.
        \item Output $(X_i, w_i)_{i \in T}, L$ and expect as input external prover messages for $\Pi_{\mathsf{ZK}}(X_i, w_i, L)$.
        \item Forward prover messages for $\Pi_{\mathsf{ZK}}(X_i, w_i, L)$ to $S^*$ and forward $S^*$'s responses to the external prover.
        \item Resume emulating an interaction of $S^*$ with $R(b)$ from Step 5 until the end of Step 7 in Figure~\ref{fig:weakot}.
        \item Output the view of $S^*$.
    \end{enumerate}
    
    By the zero-knowledge property of $\Pi_{\mathsf{ZK}}$, there exists a negligible function $\mu(\cdot)$ such that:
    $$\Big|\Pr[D^*(\view_{S^*}\langle S^*, R(b) \rangle) = 1] - \Pr[D^*(\mathsf{Hyb}_1) = 1] \Big|  = \mu(\secp)$$
    
        
    \noindent {\textbf{$\mathsf{Hyb}_2$.}} Define distribution $\mathsf{Hyb}_2$ identically to $\mathsf{Hyb}_1$, 
    except that the commitments $c_i$ for $i \in [m]$ are generated as $c_i =
    \commit(00; r_i)$ instead of as $\commit((\widehat{\theta}_i, \widehat{x}_i); r_i)$.
    
    By the quantum computational hiding of $\Commit$, since $S^*$ and $D^*$ are quantum polynomial-size adversaries, there exists a negligible function $\nu(\cdot)$ such that:
    $$\Big|\Pr[D^*(\mathsf{Hyb}_2) = 1] - \Pr[D^*(\mathsf{Hyb}_1) = 1] \Big|  = \nu(\secp)$$


    \noindent {\textbf{$\mathsf{Hyb}_3$.}}
    This is identical to $\mathsf{Hyb}_2$, 
    except that no measurements are performed inn Step 2. Instead, $R$ only measures $\ket{x}_{\theta}$ restricted to $T$ at the beginning of Step 4. Moreover, $\ket{x}_{\theta}$ restricted to $\overline{T}$ is never explicitly measured unless required within Step 7.
    The output of this experiment is identical to $\mathsf{Hyb}_2$, therefore 
    $$\Pr[D^*(\mathsf{Hyb}_3) = 1] = \Pr[D^*(\mathsf{Hyb}_4) = 1].$$

    
    \noindent {\textbf{$\mathsf{Hyb}_4$.}} This is identical to $\mathsf{Hyb}_3$, 
    except that $\Pi_{BB}$ is executed with receiver input $b'$.
    Note that since $\ket{x}_{\theta}$ restricted to $\overline{T}$ is not measured in Steps 1-6, there is a direct reduction that forwards messages to an external receiver and obtains responses during the execution of $\Pi_BB$ in Step 7.
    
    Thus by the hiding of $\Pi_{BB}$, there exists a negligible function $v(\cdot)$ such that:
    $$\Big|\Pr[D^*(\mathsf{Hyb}_4) = 1] - \Pr[D^*(\mathsf{Hyb}_3) = 1] \Big|  = v(\secp)$$

    By the same arguments as above, there exists a negligible function $v'(\cdot)$ such that 
    $$\Big|\Pr[D^*(\mathsf{Hyb}_4) = 1] - \Pr[D^*(\view_{S^*}\langle S^*, R(b') \rangle) = 1] \Big|  = v'(\secp)$$
    %
    This implies that 
    $$\Big|\Pr[D^*(\view_{S^*}\langle S^*, R(b) \rangle) = 1] - \Pr[D^*(\view_{S^*}\langle S^*, R(b') \rangle) = 1] \Big|  = \negl(\secp)$$
    which yields a contradiction, as desired.

    \item {\bf Statistical Sender Security.} This follows by the statistical binding of the commitment scheme $\commit$, statistical soundness of $\Pi_{\mathsf{ZK}}$ and the statistical sender security of $\Pi_{BB}$.
    
    The definition of statistical sender security requires the existence of a simulator $\simu_{R^*}$. This is constructed as follows:
    \begin{enumerate}
        \item Choose $x \leftarrow \{0,1\}^m$ and $\theta \leftarrow \{+,\times\}^m$. Send $\ket{x}_{\theta}$ to $R^*$. 
        \item Obtain $\{c_i\}_{i \in [n]}$ from $R^*$.
        \item
        For every $i \in [m]$, find (in time $2^{|r_i|+2}$) values $(\alpha_i, \beta_i, r_i)$ such that $c_i = \commit((\alpha_i, \beta_i);r_i)$.
         Alternately, if $\mathsf{Commit}$ is an extractable commitment, execute the extractor to efficiently extract $\alpha_i, \beta_i$ for every $i \in [n]$.
        \item Sample a random test subset $T \subset [m]$ of size $m/2$ and send it to $R^*$.
        \item Take the role of verifier $\Pi_{\mathsf{ZK}}$ according to Step 4 in Figure \ref{fig:weakot}.
        \item If the ZK proofs are accepted, and $x_i = \widehat{x}_i$ whenever $\theta_i = \widehat{\theta}_i$, continue, otherwise reject.
        \item Partition $\overline{T}$ into two subsets $S$ and $\overline{S}$ such that: for $i \in S$, $\theta_i = \widehat{\theta}_i$ and for $i \in \overline{S}$,
        $\theta_i \neq \widehat{\theta}_i$.
        \item Obtain $R^*$'s message for $\Pi_BB$ and parse this message as consisting of sets $S_0$ and $S_1$.
        \item Obtain the output $m_b$ of $\fot$ on input bit $b$, where $b = 0$ iff $S_0 \subseteq S$.
        \item Execute sender strategy for $\Pi_{BB}$ with sender input $(m_b, m_b)$.
\end{enumerate}
    
We will now prove that
$$
\Delta \big(\mathsf{View}_{\simu^{\fot(m_0,m_1,\cdot)}_{R^*}}, \mathsf{View}_{R^*}\langle S(m_0, m_1), R^* \rangle \big) = \negl(\secp)$$

\dakshita{TODO.}

\end{enumerate}
\end{proof}

==> todo.tex <==
- replace BBCS with CK.

- add a section on equivalence between collapse binding quantum computationally hiding commitments and qOT

- comparison section
1. black-box use of one-way functions/statistically binding commitments.
2. which also implies unconditional result in QROM.
3. possibly weaker assumptions.

-finish updating statistical hiding proof in section 5.2, and anywhere else the "EPR protocol" is used (fermi)

-define collapse-binding (fermi)

==> uc-composition.tex <==
\section{Quantum Universal Composability in the QROM}

In this section, we present the quantum universal composability framework in the quantum random oracle model (QROM). We take inspiration from existing work on the Quantum UC model~\cite{unruh2010universally} and adapt the definition to fit the QROM.

%There are two major differences in our setting. First, we strengthen the notion of quantum stand-alone (QSA) emulation from \cite{C:HalSmiSon11} to quantum \emph{oracle} stand-alone emulation (QOSA), where emulation must hold with respect to any external oracle $O$ that may be accessed by the honest party, adversary, and environment \nishant{i think it would be nice to define what the environment is informally as well? found this para hard to follow without knowing what environment was referring to?}. This enables us to use the security of an ``inner'' protocol even when the inner protocol adversary can access the random oracle used in an ``outer'' protocol. \amit{The following statement is unclear. Specifically, what exactly does ``simulator interacting in the actual protocol'' mean ?}Next, we weaken the notion of simulation to allow for simulators that can answer random oracle queries made by the environment (and share state with the simulator interacting in the actual protocol). We also further weaken this notion to consider simulators that only work for environments that make some bounded number of $q$ queries to the random oracle.


\paragraph{Quantum interactive machines.} A quantum interactive machine (QIM) is a family of machines $\{M_\secp\}_{\secp \in \bbN}$, where each $M_{\secp}$ consists of a sequence of quantum operations $M_{\secp,1},\dots,M_{\secp,\ell(\secp)}$, where $\ell(\secp)$ is the number of rounds in which $M_\secp$ operates. Usually, we drop the indexing by $\secp$ and refer to $M = M_1,\dots,M_\ell$. 

%$M$ operates on an input register $\gray{M_0}$, memory registers $\gray{M_1},\dots,\gray{M_\ell}$, and communication registers $\gray{C_1},\dots,\gray{C_\ell}$.

When two QIMs $A$ and $B$ interact in a $(2\ell-1)$-round protocol, they share communication registers $\gray{C_1},\dots,\gray{C_{2\ell}}$. $A$ additionally operates on an input register $\gray{A_\inp}$, memory registers $\gray{A_1,\dots,\gray{A_{\ell}}}$, and output register $\gray{A_\out}$, where 

\begin{itemize}
    \item $A_1: \gray{A_\inp} \otimes \gray{A_1} \to \gray{A_2} \otimes \gray{C_1}$,
    \item for each $i \in [\ell-1]$, $A_i : \gray{A_i} \otimes \gray{C_{2i-2}} \to \gray{A_{i+1}} \otimes \gray{C_{2i-1}}$,
    \item and $A_\ell: \gray{A_\ell} \otimes \gray{C_{2\ell-2}} \to \gray{A_\out} \otimes \gray{C_{2\ell-1}}$.
\end{itemize}

$B$ additionally operates on an input register $\gray{B_\inp}$, memory registers $\gray{B_1},\dots,\gray{B_{\ell-1}}$, and output register $\gray{B_\out}$, where 

\begin{itemize}
    \item $B_1: \gray{B_\inp} \otimes \gray{B_1} \otimes \gray{C_1} \to \gray{B_2} \otimes \gray{C_2}$,
    \item for each $i \in [\ell-1]$, $B_i: \gray{B_i} \otimes \gray{C_{2i-1}} \to \gray{B_{i+1}} \otimes \gray{C_{2i}}$,
    \item and $B_\ell : \gray{B_\ell} \otimes \gray{C_{2\ell-1}} \to \gray{B_\out}$.
\end{itemize}

We can also consider more than two QIMs interacting, and set up communication registers between each pair of machines.
 

\paragraph{Functionalities, protocols, and emulation.} Let $\cF$ denote a \emph{functionality}, which is a classical interactive machine specifying the instructions to realize a cryptographic task. A two-party protocol\footnote{One can also consider multi-party protocols, but we restrict to the two-party setting in this work.} $\Pi$ for $\cF$ consists of two QIMs $(A,B)$.\footnote{Technically, each of $A$ and $B$ is an infinite family of interactive machines, parameterized by the security parameter $\secp$.} An adversary $\cA$ is another quantum interactive machine that intends to attack the protocol. In this work, we only consider \emph{static} adversaries, that operate in the presence of an \emph{environment} $\cZ = (\cZ_0,\cZ_1)$ that consists of two quantum operations. The execution of the protocol $\Pi$ in the presence of environment $\cZ$ and adversary $\cA$ defines a quantum operation that outputs a single bit, which we denote by $M[\Pi,\cZ,\cA](1^\secp)$. This quantum operation is defined as follows. \nishant{following is incorrect right now, working on changing it .. the network execution model needs to be written up so that env can execute with adv}

\begin{itemize}
    \item $\cA$ is defined to either corrupt party $A$ or $B$, $P \in \{A,B\}$ is defined to be the uncorrupted party, and $\secp \in \bbN^+$ is the security parameter. 
    \item $\cZ_0(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$,
    where $\brho_\secp$ is $\cA$'s input, $x$ is $P$'s (classical) input, and $\bsigma_\secp$ is an auxiliary quantum state.
    \item $\cA(\brho_\secp)$ interacts with $P(x)$ during the execution of $\Pi$, and outputs a quantum state $\btau_\secp$.
    \item $\cZ_1(\btau_\secp,\bsigma_\secp)$ outputs a bit $b$.
\end{itemize}

Let $\Pi$ and $\Gamma$ be two protocols. We say that $\Pi$ statistically \emph{quantum UC emulates}\footnote{One can also consider the notion of \emph{computational} UC emulation, in which $\Pi,\Gamma,\cA,\cS,$ and $\cZ_1$ are all restricted to be polynomial-time (though $\cZ_0$ may be unbounded).} (QUC emulates) $\Gamma$ if for all $\cA$ there exists a $\cS$ (sometimes called a \emph{simulator}) such that for all $\cZ$, \[\left|\Pr[M[\Pi,\cZ,\cA](1^\secp)] - \Pr[M[\Gamma,\cZ,\cS](1^\secp)]\right| = \negl(\secp).\]  

An \emph{ideal-world} protocol $\widetilde{\Pi}_\cF$ for functionality $\cF$ consists of two ``dummy'' parties $\widetilde{A},\widetilde{B}$ that have access to an additional ``trusted'' party that implements $\cF$. That is, $\widetilde{A},\widetilde{B}$ each interact with $\cF$, such that at the end of the interaction $\widetilde{A},\widetilde{B}$ hold their respective outputs (possibly by sending their inputs to $\cF$ and $\cF$ returning the computed output to both the parties). An execution of $\widetilde{\Pi}_\cF$ in the presence of an adversary $\cS$ and environment $\cZ$ is defined as before except that $\cS$ may not corrupt $\cF$. We say that a protocol $\Pi$ (statistically) \emph{quantum UC realizes} (QUC realizes) $\cF$ if $\Pi$ statistically QUC emulates $\widetilde{\Pi}_\cF$.

% \paragraph{\cite{C:HalSmiSon11} composition.} Let $\Pi$ be a protocol that uses another protocol $\Gamma$ as a subroutine, and let $\Gamma'$ be a protocol that QSA emulates $\Gamma$. Define the \emph{composed} protocol $\Pi^{\Gamma/\Gamma'}$ to be the protocol $\Pi$ with every execution of $\Gamma$ replaced by $\Gamma'$. In this work, we consider protocols $\Pi$ that can invoke $\Gamma$ (and potentially other subprotocols) multiple times, but where only a \emph{single invocation} of any subprotocol is invoked at any given time. In a \emph{hybrid} model, parties can make calls to an ideal-world protocol $\widetilde{\Pi}_\cG$ for some functionality $\cG$. We call such a protocol a $\cG$-hybrid protocol and denote it $\Pi^\cG$.

% \begin{theorem}[\cite{C:HalSmiSon11}]
% Let $\cF$ and $\cG$ be functionalities, let $\Pi_\cG$ be a $\cG$-hybrid protocol that statistically (resp. computationally) QSA realizes $\cF$ and let $\Gamma$ be a protocol that statistically (resp. computationally) QSA realizes $\cG$. Then $\Pi^{\cG/\Gamma}$ statistically (resp. computationally) QSA realizes $\cF$.
% \end{theorem}

\paragraph{Quantum oracle algorithms.} \nishant{Need to change this to allow for parallel queries - a bounded query depth and total bound} Let $\cX,\cY$ be finite sets and let $O : \cX \to \cY$ be an arbitrary function. We say that $A^{O}$ is a $q$-query \emph{quantum oracle algorithm} if it can be written as $A_{q+1}U_OA_{q}U_O\dots U_OA_2U_OA_1$, where $A_1,\dots,A_{q+1}$ are arbitrary quantum operations, and $U_O$ is the unitary defined by \[U_O: \ket{x}\ket{y} \to \ket{x}\ket{y \oplus O(x)},\] operating on the appropriate registers of $A$'s state. Sometimes, it will be convenient to consider algorithms $A^{O_1,O_2}$ with access to \emph{multiple} oracles $O_1: \cX_1 \to \cY_1, O_2: \cX_2 \to \cY_2$, written as $A_{q+1}U_{O_2}A_{q}U_{O_1}\dots U_{O_2}A_2U_{O_1}A_1$. Defining $O(b,x) = O_b(x)$ for $(b,x) \in (1,\cX_1) \union (2,\cX_2)$, it is easy to see that any $A^{O_1,O_2}$ can be written as an oracle algorithm ${A'}^O$ and that any $A^O$ can be written as an oracle algorithm ${A'}^{O_1,O_2}$, with an appropriate increase in number of queries.

We say that $A$ is a \emph{quantum interactive oracle machine} if $A = A_1^O,\dots,A_\ell^O$ is such that each $A_i^O$ is a quantum oracle algorithm.

\paragraph{The quantum random oracle model.} We will consider protocols $\Pi_\RO$ that operate in the \emph{quantum random-oracle model} (QROM). In such a protocol, a random function $H \gets \cH_{\cX,\cY}$ is first sampled, where $\cH_{\cX,\cY}$ is the uniform distribution over functions $H: \cX \to \cY$. Then, oracle algorithms $A^H$ and $B^H$ interact in the protocol. Note that this model also captures protocols that are defined with respect to \emph{multiple} random oracles $H_1 \gets \cH_{\cX_1,\cY_1}, H_2 \gets \cH_{\cX_2,\cY_2}$, where honest parties are oracle algorithms $A^{H_1,H_2}$ and $B^{H_1,H_2}$. This follows by letting $\cX \coloneqq (1,\cX_1) \cup (2,\cX_2)$, letting $\cY$ be such that $|\cY| \geq \max\{|\cY_1|,|\cY_2|\}$, and defining appropriate embedding operations from $\cY$ to $\cY_1$ and to $\cY_2$.

\paragraph{QUC emulation in the QROM.} 
Quantum UC security of a protocol $\Pi_\RO$ in the quantum random oracle model is formalized by splitting the random oracle into an ``internal'' random oracle $H_\internal$ and an external random oralce $H_\ext$, where $H_\internal$ is the oracle used in $\Pi_\RO$, and $H_\ext$ is an oracle that may be accessed in the case that $\Pi_\RO$ is run within a larger context. Our ideal-world adversary $\cS$ may answer random oracle queries to $H_\internal$ made by the environtment. That is, when $\cZ$ issues a query to $H_\internal$, the unitary $U_{H_\internal}$ is replaced with a quantum operation specified by $\cS$, that itself may make calls to $H_\internal$.


%We now formally define what it means for a protocol $\Pi_\RO$ to statistically quantum oracle stand-alone (QOSA) realize a functionality $\cF$ in the QROM.




%In this work, we will consider protocol execution in the presence of adversaries and environments that have access to some external oracle $O$. That is, adversaries $\cA^O$ and environments $\cZ^O = (\cZ_0^O,\cZ_1^O)$ may be \emph{quantum oracle algorithms} that query $O$ throughout their execution. The following definition can be seen as a strict generalization of the notions of QSA emulation / realization.

%\begin{definition}

%\amit{Why are we quantifying over \textbf{all} oracles in the security definition ? Seems that it would be too strong of a definition ? (e.g. consider an oracle for halting problem, no protocol would be secure in the presence of this oracle) }


%Let $\Pi$ and $\Gamma$ be two protocols. We say that $\Pi$ statistically \emph{quantum oracle stand-alone emulates} (QOSA emulates) $\Gamma$ if for all quantum oracle adversaries $\cA$, there exists a quantum oracle algorithm $\cS$ such that for all finite sets $\cX,\cY$, oracles $O: \cX \to \cY$, and environments $\cZ^O = (\cZ_0^O,\cZ_1^O)$,

%\[\left|\Pr[M[\Pi,\cZ^O,\cA^O](1^\secp) = 1] - \Pr[M[\Gamma,\cZ^O,\cS^O](1^\secp) = 1]\right| = \negl(\secp).\]

%Let $\cF$ be a functionality. We say that a protocol statistically \emph{quantum oracle stand-alone realizes} (QOSA realizes) $\cF$ if $\Pi$ statistically QOSA emulates $\widetilde{\Pi}_\cF$.

%\end{definition}






%\footnote{It is also meaningful to consider protocols $\Pi_\RO$ that just QSA realize a functionality $\cF$ in the QROM, but here we explicitly describe the more general notion of QOSA realization.} 

%\amit{Again, I think quantifying over all oracles $O$ is quite strong. Also, shouldn't $H$ be simulated at some point i.e. in one of the experiments, $H$ shouldn't appear as an oracle at all ?}

\begin{definition}\label{def:QSA-in-QROM}
Let $\Pi_\RO$ be a protocol in the QROM and let $\cF$ be a functionality. We say that $\Pi_\RO$, which operates with respect to a random oracle sampled from $\cH_{\cX_\internal,\cY_\internal}$, statistically quantum oracle UC realizes (QOUC realizes) $\cF$ in the QROM if for any quantum oracle adversary $\cA$, there exists a quantum oracle algorithm $\cS$ such that for all finite sets $\cX_\ext,\cY_\ext$ and environments $\cZ = \left(\cZ_0,\cZ_1\right)$, \nishant{I think this probability below should not be over the probability of sampling $H_\ext$ and that $H_\ext$ should be something fixed?}

\begin{align*}
&\bigg|\Pr_{\substack{H_\internal \gets \cH_{\cX_\internal,\cY_\internal},\\ H_\ext \gets \cH_{\cX_\ext,\cY_\ext}}}\left[M\left[\Pi_\RO,\cZ^{H_\internal,H_\ext},\cA^{H_\internal,H_\ext}\right](1^\secp) = 1\right]\\ &- \Pr_{\substack{H_\internal \gets \cH_{\cX_\internal,\cY_\internal},\\ H_\ext \gets \cH_{\cX_\ext,\cY_\ext}}}\left[M\left[\widetilde{\Pi}_\cF,\cZ^{\cS^{H_\internal},H_\ext},\cS^{H_\internal,H_\ext}\right](1^\secp) = 1\right]\bigg| = \negl(\secp).
\end{align*}


%where $M\left[\widetilde{\Pi}_\cF,\cZ^{\cS^{H_\internal},H_\ext},\cS^{H_\internal,H_\ext}\right](1^\secp)$ consists of the following steps:

%\begin{itemize}
    %\item $\cZ_0^{O,\cS_0^H}(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$. $\cZ_0$'s queries to $H$ are answered by the (stateful) oracle machine $\cS_0^H$.  \nishant{$\cS_0^H$ state also passed to $\cS_1^{O,H}$ right? if so, we should state it explicitly otherwise it is not clear if that is happening}
    %\item $\cS_1^{O,H}(\brho_\secp)$ interacts with the honest party $P(x)$ and the trusted party implementing $\cF$, and outputs a quantum state $\btau_\secp$, along with an additional quantum state that is passed back to $\cS_0$. \amit{Should we be more explcit about this state transfer from $\cS_1 \rightarrow \cS_0$ ? i.e. what exactly is the consequence of allowing such transfer versus not allowing ?}
    %\item $\cZ_1^{O,\cS_0^H}(\btau_\secp,\bsigma_\secp)$ outputs a bit $b$. $\cZ_1$'s queries to $H$ are answered by the (stateful) oracle machine $\cS_0^H$. 
%\end{itemize}

%\amit{Should we also be defining $M\left[\Pi_\RO,\cZ^{O,H},\cA^{O,H}\right](1^\secp)$ ?}

\end{definition}

\iffalse{
    Next, we define a weakening of QSA realization of functionalities in the QROM that allows the simulator $\cS$ to have some dependence on the environment $\cZ$. In particular, we will consider simulators that may depend on the number of queries that $\cZ$ makes to the random oracle $H$, and we call this \emph{$q$-dependent simulation}.
    
    \begin{definition}
    Let $\Pi_\RO$ be a protocol in the QROM and let $\cF$ be a functionality. We say that $\Pi_\RO$ statistically quantum stand-alone realizes $\cF$ in the QROM with \emph{query-dependent simulation} if for any $q \in \bbN$, \cref{def:QSA-in-QROM} holds with respect to any environment $\cZ$ that makes at most $q$ total queries to $H_\internal$. We refer to the simulator guaranteed by the definition as $(\cS[\cA,q])$.
    \end{definition}
    
    
    \paragraph{Oracle composition theorem.} Finally, we give a quantum stand-alone composition theorem that may be utilized for the composition of protocols operating in the QROM.
    
    \begin{theorem}
    \label{thm:malc-qrom-composition}
    Let $\cF$ and $\cG$ be functionalities, let $\Pi_\RO^\cG$ be a $\cG$-hybrid protocol in the QROM that QSA realizes $\cF$ with query-dependent simulation (resp. without query-dependent simulation) and let $\Gamma_\RO$ be a protocol in the QROM that QSA realizes $\cG$ with query-dependent simulation (resp. without query-dependent simulation). Then $\Pi_\RO^{\cG/\Gamma_\RO}$ is a protocol in the QROM that QSA realizes $\cF$ with query-dependent simulation (resp. without query-dependent simulation).
    \end{theorem}
    
    \begin{proof}
    We prove the theorem for the case of query-dependent simulation, since it is the harder case to prove. We also assume without loss of generality that $\Pi$ calls $\Gamma$ exactly once, since we anyway only allow at most one session of $\Gamma$ to be called at a time. Let $H_\Pi$ be the random oracle used in $\Pi_\RO^\cG$ and let $H_\Gamma$ be the random oracle used in $\Gamma_\RO$. Then the random oracle used in $\Pi_\RO^{\cG/\Gamma_\RO}$ consists of the pair of oracles $(H_\Pi,H_\Gamma)$. Now, we want to show that for any $q \in \bbN$ and any adversary $\cA$ interacting in $\Pi_\RO^{\cG/\Gamma_\RO}$, there exists a simulator $\cS[\cA,q]$ such that for any finite sets $\cX_\ext,\cY_\ext$, and any environment $\cZ$ that makes at most a total of $q$ combined queries to $H_\Pi$ and $H_\Gamma$, it holds that 
    
    \begin{align*}
    &\bigg|\Pr_{H_\Pi,H_\Gamma,H_\ext}\left[M\left[\Pi_\RO,\cZ^{H_\Pi,H_\Gamma,H_\ext},\cA^{H_\Pi,H_\Gamma,H_\ext}\right](1^\secp) = 1\right]\\ &- \Pr_{H_\Pi,H_\Gamma,H_\ext}\left[M\left[\widetilde{\Pi}_\cF,\cZ^{\cS[\cA,q]^{H_\Pi,H_\Gamma},H_\ext},\cS[\cA,q]^{H_\Pi,H_\Gamma,H_\ext}\right](1^\secp) = 1\right]\bigg| = \negl(\secp).
    \end{align*}
    
    We will show this in the two steps.
    
    \begin{enumerate}
        \item First, we split $\cA$ into three parts $(\cA_0,\cA_\Gamma,\cA_1)$, \nishant{since $\Gamma$ can be an interactive machine, $\cA_0,\cA_1$ are not necessarily the part before/after $\Gamma$ right? i think $\cA_0$ is part of $\cA$ before any call to $\Gamma$, in the remaining adversary $\cA_\Gamma$ is the part which interacts with $\Gamma$ and $\cA_1$ is the remaining adversary. Is this how you are also thinking about it?}\james{good point, I think we will actually have to use a more UC-style definition. Our setting differs from that considered by HSS, since we want to combine the invocation of the inner protocol with messages exchanged for the outer protocol, and we could have interleaved inner and outer protocol messages.} where $\cA_\Gamma$ is the part of $\cA$ that interacts in $\Gamma_\RO$. Let $q_\Gamma$ be the total number of queries that $(\cA_0,\cA_1)$ make to $H_\Gamma$. Let $O_\Gamma = (O,H_\Pi)$ \nishant{this is not used in this step right?}. Then since $\Gamma_\RO$ QOSA realizes $\cG$ with $q$-dependent simulation, there exist algorithms $(\cS[\cA_\Gamma,q+q_\Gamma]_0,\cS[\cA_\Gamma,q+q_\Gamma]_1)$ such that, for any $\cZ$ that makes at most $q$ total queries to $H_\Pi$ or $H_\Gamma$, the output of $M
        \left[\Pi_\RO,\cZ^{O,H_\Pi,H_\Gamma},\cA^{O,H_\Pi,H_\Gamma}\right](1^\secp)$ is negligibly close to the output of the following experiment.
        \begin{itemize}
            \item $\cZ_0^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(1^\secp)$ outputs $(\brho_\secp,x,\bsigma_\secp)$.
            \item $\cA_0^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\brho_\secp)$ interacts with the honest party $P(x)$ and outputs a quantum state $\brho'_\secp$.
            \item $\cS[\cA_\Gamma,q+q_\Gamma]_1^{O,H_\Pi,H_\Gamma}(\brho'_\secp)$ interacts with the honest party $P(x)$ and the trusted party implementing $\cG$, and outputs a quantum state $\brho''_\secp$.
            \item $\cA_1^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\brho''_\secp)$ interacts with the honest party $P(x)$ and outputs a quantum state $\btau_\secp$.
            \item $\cZ_1^{O,H_\Pi,\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}}(\btau_\secp,\bsigma_\secp)$ outputs a bit b.
        \end{itemize}
        \item Next, define \nishant{should the $q_\Gamma$ be $q+q_\Gamma$ all over below?}
        \begin{align*}
        &\cZ_{0,\Pi}^{O,H_\Pi,H_\Gamma} \coloneqq \cZ_0^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}\\
        &\cA_\Pi^{O,H_\Pi,H_\Gamma} \coloneqq \left(\cA_0^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}},\cS[\cA_\Gamma,q_\Gamma]_1^{O,H_\Pi,H_\Gamma},\cA_1^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}\right)\\
        &\cZ_{1,\Pi}^{O,H_\Pi,H_\Gamma} \coloneqq \cZ_1^{O,H_\Pi,\cS[\cA_\Gamma,q_\Gamma]_0^{H_\Gamma}}.
        \end{align*}
        Define $O_\Pi = (O,H_\Gamma)$ and note that $\cA_\Pi^{O,H_\Pi,H_\Gamma}$ is an adversary for $\Pi_\RO$ in the $\cG$-hybrid model, with access to external oracle $O_\Pi$. Since $\Pi_\RO^\cG$ QOSA realizes $\cF$ with $q$-dependent simulation, there exist algorithms $(\cS[\cA_\Pi,q]_0,\cS[\cA_\Pi,q]_1)$  such that the output of the above experiment is negligibly close to the output of $M\left[\widetilde{\Pi}_\cF,\cZ^{O,\cS[\cA_\Pi,q]_0^{H_\Pi},\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}},\cS[\cA_\Pi,q]_1^{O,H_\Pi,H_\Gamma}\right](1^\secp)$,
        since the environment $(\cZ_{0,\Pi},\cZ_{1,\Pi})$ makes at most $q$ queries the random oracle $H_\Pi$. Thus, define $\cS[\cA,q]_0$ to run $\cS[\cA_\Pi,q]_0^{H_\Pi}$ on $H_\Pi$ queries and $\cS[\cA_\Gamma,q+q_\Gamma]_0^{H_\Gamma}$ on $H_\Gamma$ queries, and define $\cS[\cA,q]_1 \coloneqq \cS[\cA_\Pi,q]_1$. This completes the proof. 
        
      
        
    \end{enumerate}
    
    
    %Let $\cX_\Pi,\cY_\Pi$ be the domain and range for the random oracle used in $\Pi_\RO^\cG$, and let $\cX_\Gamma,\cY_\Gamma$ be the domain and range for the random oracle used in $\Gamma_\RO$. Then define $\cX_{\Pi/\Gamma} \coloneqq (0,\cX_\Pi) \union (1,\cX_\Gamma)$ and $\cY_{\Pi/\Gamma}$ of appropriate size. We consider $\Pi_\RO^{\cG/\Gamma_\RO}$ to be a protocol in the QROM  
    \end{proof}
}\fi
